AeroBelief: Budgeted First-Action Verification for Evidence-Guided Aerial Sensing

Aerial sensing must combine uncertain overhead context with current observations while budgeting prediction, movement and image processing. AeroBelief uses the next executable action as the unit of verification against reference scores. It groups candidate views by first action, scans them with an inexpensive proposer, and selectively queries a structured world model (WM). Calibrated group bounds support strict commitment; a six-query controller connects selective prediction with belief updates, acceptance checks and scheduled sensing. Across four layout families, 40 worlds and 960 closed-loop executions, the AeroBelief controller completes 75.42% of tasks, compared with 73.33% for exhaustive WM scoring and 65.83% for line-of-sight geometry, using 91.81% fewer reference-candidate evaluations than exhaustive scoring. In fixed-reference replay with a six-query cap, proposer-scaled anchored bounds raised first-action certificate availability from 36.25% to 54.69% and reduced mean queries per state by 13.54% relative to unit-scale anchored bounds. A complete ground-hosted pipeline processes 2,685 self-collected 20-megapixel unmanned aerial vehicle (UAV) images from seven DJI Mavic 3M routes. Context-guided admission and feedback retain all eight independently supported target confirmations with 76.05% fewer processed images and 70.02% less accumulated active processing service than uncapped all-frame processing; feedback saves another 5.17% of images relative to static context. The studies connect budgeted action selection with evidence-driven processing of recorded flight imagery.

==> LKey.tex <==
\DeclareRobustCommand*\LKey[1]{%
\ifx#10\biolinumKeyGlyph{zero}%  % spurious space removed 2016/06/24
\else\ifx#11\biolinumKeyGlyph{one}%
\else\ifx#12\biolinumKeyGlyph{two}%
\else\ifx#13\biolinumKeyGlyph{three}%
\else\ifx#14\biolinumKeyGlyph{four}%
\else\ifx#15\biolinumKeyGlyph{five}%
\else\ifx#16\biolinumKeyGlyph{six}%
\else\ifx#17\biolinumKeyGlyph{seven}%
\else\ifx#18\biolinumKeyGlyph{eight}%
\else\ifx#19\biolinumKeyGlyph{nine}%
\else\biolinumKeyGlyph{#1}%
\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}
\DeclareRobustCommand*\LKeyTux{\biolinumKeyGlyph{T_u_x}}
\DeclareRobustCommand*\LKeyWin{\biolinumKeyGlyph{uniE168}}
\DeclareRobustCommand*\LKeyMenu{\biolinumKeyGlyph{uniE104}}
\DeclareRobustCommand*\LKeyStrg{\biolinumKeyGlyph{S_t_r_g}}
\DeclareRobustCommand*{\LKeyCtrl}{\biolinumKeyGlyph{uniE173}}
\DeclareRobustCommand*\LKeyAlt{\biolinumKeyGlyph{A_l_t}}
\DeclareRobustCommand*\LKeyAltGr{\biolinumKeyGlyph{A_l_t_G_r}}
\DeclareRobustCommand*\LKeyShift{\biolinumKeyGlyph{S_h_i_f_t}}
\DeclareRobustCommand*\LKeyTab{\biolinumKeyGlyph{T_a_b}}
\DeclareRobustCommand*\LKeyEnter{\biolinumKeyGlyph{E_n_t_e_r}}
\DeclareRobustCommand*\LKeyCapsLock{\biolinumKeyGlyph{C_a_p_s_l_o_c_k}}
\DeclareRobustCommand*\LKeyPos{\biolinumKeyGlyph{P_o_s_1}}
\DeclareRobustCommand*\LKeyEntf{\biolinumKeyGlyph{E_n_t_f}}
\DeclareRobustCommand*\LKeyEinf{\biolinumKeyGlyph{E_i_n_f}}
\DeclareRobustCommand*\LKeyLeer{\biolinumKeyGlyph{L_e_e_r}}
\DeclareRobustCommand*\LKeyEsc{\biolinumKeyGlyph{E_s_c}}
\DeclareRobustCommand*\LKeyEnde{\biolinumKeyGlyph{E_n_d_e}}
\DeclareRobustCommand*\LKeyCommand{\biolinumKeyGlyph{uni2318}}
\DeclareRobustCommand*\LKeyOptionKey{\biolinumKeyGlyph{uni2325}}
%
\DeclareRobustCommand*\LKeyBack{\biolinumKeyGlyph{B_a_c_k}}
\DeclareRobustCommand*\LKeyUp{\biolinumKeyGlyph{arrowup}}
\DeclareRobustCommand*\LKeyDown{\biolinumKeyGlyph{arrowdown}}
\DeclareRobustCommand*\LKeyLeft{\biolinumKeyGlyph{arrowleft}}
\DeclareRobustCommand*\LKeyRight{\biolinumKeyGlyph{arrowright}}
\DeclareRobustCommand*\LKeyPgUp{\biolinumKeyGlyph{uniE198}}
\DeclareRobustCommand*\LKeyPgDown{\biolinumKeyGlyph{uniE199}}
\DeclareRobustCommand*\LKeyAt{\biolinumKeyGlyph{at}}
\DeclareRobustCommand*\LKeyFn{\biolinumKeyGlyph{uniE188}}
\DeclareRobustCommand*\LKeyHome{\biolinumKeyGlyph{H_o_m_e}}
\DeclareRobustCommand*\LKeyDel{\biolinumKeyGlyph{D_e_l}}
\DeclareRobustCommand*{\LKeySpace}{\biolinumKeyGlyph{uniE18C}}
\DeclareRobustCommand*{\LKeyScreenUp}{\biolinumKeyGlyph{uni21A5}}
\DeclareRobustCommand*{\LKeyScreenDown}{\biolinumKeyGlyph{uni21A7}}
\DeclareRobustCommand*\LKeyIns{\biolinumKeyGlyph{I_n_s}}
\DeclareRobustCommand*\LKeyEnd{\biolinumKeyGlyph{E_n_d}}
\DeclareRobustCommand*\LKeyGNU{\biolinumKeyGlyph{G_N_U}}
\DeclareRobustCommand*\LKeyPageUp{\biolinumKeyGlyph{uniE19A}}
\DeclareRobustCommand*\LKeyPageDown{\biolinumKeyGlyph{uniE19B}}
%
\@namedef{libertine@key@F@1}{\biolinumKeyGlyph{F_1}}
\@namedef{libertine@key@F@2}{\biolinumKeyGlyph{F_2}}
\@namedef{libertine@key@F@3}{\biolinumKeyGlyph{F_3}}
\@namedef{libertine@key@F@4}{\biolinumKeyGlyph{F_4}}
\@namedef{libertine@key@F@5}{\biolinumKeyGlyph{F_5}}
\@namedef{libertine@key@F@6}{\biolinumKeyGlyph{F_6}}
\@namedef{libertine@key@F@7}{\biolinumKeyGlyph{F_7}}
\@namedef{libertine@key@F@8}{\biolinumKeyGlyph{F_8}}
\@namedef{libertine@key@F@9}{\biolinumKeyGlyph{F_9}}
\@namedef{libertine@key@F@10}{\biolinumKeyGlyph{F_1_0}}
\@namedef{libertine@key@F@11}{\biolinumKeyGlyph{F_1_1}}
\@namedef{libertine@key@F@12}{\biolinumKeyGlyph{F_1_2}}
\@namedef{libertine@key@F@13}{\biolinumKeyGlyph{F_1_3}}
\@namedef{libertine@key@F@14}{\biolinumKeyGlyph{F_1_4}}
\@namedef{libertine@key@F@15}{\biolinumKeyGlyph{F_1_5}}
\@namedef{libertine@key@F@16}{\biolinumKeyGlyph{F_1_6}}
\DeclareRobustCommand*\LKeyF[1]{\@nameuse{libertine@key@F@#1}}
\DeclareRobustCommand*\LKeyAltF[1]{\LKeyAlt+\@nameuse{libertine@key@F@#1}}
\DeclareRobustCommand*\LKeyStrgAltF[1]{\LKeyStrg+\LKeyAlt+\@nameuse{libertine@key@F@#1}}
\DeclareRobustCommand*\LKeyCtrlAltF[1]{\LKeyCtrl+\LKeyAlt+\@nameuse{libertine@key@F@#1}}
\DeclareRobustCommand*\LKeyStrgX[1]{\LKeyStrg+\LKey{#1}}
\DeclareRobustCommand*\LKeyCtrlX[1]{\LKeyCtrl+\LKey{#1}}
\DeclareRobustCommand*\LKeyShiftX[1]{\LKeyShift+\LKey{#1}}
\DeclareRobustCommand*\LKeyAltX[1]{\LKeyAlt+\LKey{#1}}
\DeclareRobustCommand*\LKeyAltGrX[1]{\LKeyAltGr+\LKey{#1}}
\DeclareRobustCommand*\LKeyShiftStrgX[1]{\LKeyShift+\LKeyStrg+\LKey{#1}}
\DeclareRobustCommand*\LKeyShiftCtrlX[1]{\LKeyShift+\LKeyCtrl+\LKey{#1}}
\DeclareRobustCommand*\LKeyShiftAltX[1]{\LKeyShift+\LKeyAlt+\LKey{#1}}
\DeclareRobustCommand*\LKeyShiftAltGrX[1]{\LKeyShift+\LKeyAltGr+\LKey{#1}}
\DeclareRobustCommand*\LKeyStrgAltX[1]{\LKeyStrg+\LKeyAlt+\LKey{#1}}
\DeclareRobustCommand*\LKeyCtrlAltX[1]{\LKeyCtrl+\LKeyAlt+\LKey{#1}}
\DeclareRobustCommand*\LKeyStrgAltEnt{\LKeyStrg+\LKeyAlt+\LKeyEntf}
\DeclareRobustCommand*\LKeyCtrlAltEnt{\LKeyCtrl+\LKeyAlt+\LKeyEntf}
\let\LKeyReset\LKeyStrgAltEnt
%
\@namedef{libertine@key@Pad@0}{\biolinumKeyGlyph{uniE1A0}}
\@namedef{libertine@key@Pad@1}{\biolinumKeyGlyph{uniE1A1}}
\@namedef{libertine@key@Pad@2}{\biolinumKeyGlyph{uniE1A2}}
\@namedef{libertine@key@Pad@3}{\biolinumKeyGlyph{uniE1A3}}
\@namedef{libertine@key@Pad@4}{\biolinumKeyGlyph{uniE1A4}}
\@namedef{libertine@key@Pad@5}{\biolinumKeyGlyph{uniE1A5}}
\@namedef{libertine@key@Pad@6}{\biolinumKeyGlyph{uniE1A6}}
\@namedef{libertine@key@Pad@7}{\biolinumKeyGlyph{uniE1A7}}
\@namedef{libertine@key@Pad@8}{\biolinumKeyGlyph{uniE1A8}}
\@namedef{libertine@key@Pad@9}{\biolinumKeyGlyph{uniE1A9}}
\@namedef{libertine@key@Pad@10}{\biolinumKeyGlyph{uniE1AA}}
\@namedef{libertine@key@Pad@11}{\biolinumKeyGlyph{uniE1AB}}
\@namedef{libertine@key@Pad@12}{\biolinumKeyGlyph{uniE1AC}}
\@namedef{libertine@key@Pad@13}{\biolinumKeyGlyph{uniE1AD}}
\@namedef{libertine@key@Pad@14}{\biolinumKeyGlyph{uniE1AE}}
\DeclareRobustCommand*\LKeyPad[1]{\@nameuse{libertine@key@Pad@#1}}
%
% Maus
%
\DeclareRobustCommand*\LMouseEmpty{\biolinumKeyGlyph{uniE130}}
\DeclareRobustCommand*\LMouseN{\biolinumKeyGlyph{uniE131}}
\DeclareRobustCommand*\LMouseL{\biolinumKeyGlyph{uniE132}}
\DeclareRobustCommand*\LMouseM{\biolinumKeyGlyph{uniE133}}
\DeclareRobustCommand*\LMouseR{\biolinumKeyGlyph{uniE134}}
\DeclareRobustCommand*\LMouseLR{\biolinumKeyGlyph{uniE135}}
\DeclareRobustCommand*\LMouseIIEmpty{\biolinumKeyGlyph{uniE138}}
\DeclareRobustCommand*\LMouseIIN{\biolinumKeyGlyph{uniE139}}
\DeclareRobustCommand*\LMouseIIL{\biolinumKeyGlyph{uniE13A}}
\DeclareRobustCommand*\LMouseIIR{\biolinumKeyGlyph{uniE13C}}
\DeclareRobustCommand*\LMouseIILR{\biolinumKeyGlyph{uniE13D}}
%


==> LinBiolinum_K.tex <==
\DeclareTextGlyphY{LinBiolinum_K}{space}{32}
\DeclareTextGlyphY{LinBiolinum_K}{uni0020}{32}
\DeclareTextGlyphY{LinBiolinum_K}{exclam}{33}
\DeclareTextGlyphY{LinBiolinum_K}{uni0021}{33}
\DeclareTextGlyphY{LinBiolinum_K}{quotedbl}{34}
\DeclareTextGlyphY{LinBiolinum_K}{uni0022}{34}
\DeclareTextGlyphY{LinBiolinum_K}{numbersign}{35}
\DeclareTextGlyphY{LinBiolinum_K}{uni0023}{35}
\DeclareTextGlyphY{LinBiolinum_K}{dollar}{36}
\DeclareTextGlyphY{LinBiolinum_K}{uni0024}{36}
\DeclareTextGlyphY{LinBiolinum_K}{percent}{37}
\DeclareTextGlyphY{LinBiolinum_K}{uni0025}{37}
\DeclareTextGlyphY{LinBiolinum_K}{ampersand}{38}
\DeclareTextGlyphY{LinBiolinum_K}{uni0026}{38}
\DeclareTextGlyphY{LinBiolinum_K}{quotesingle}{39}
\DeclareTextGlyphY{LinBiolinum_K}{uni0027}{39}
\DeclareTextGlyphY{LinBiolinum_K}{parenleft}{40}
\DeclareTextGlyphY{LinBiolinum_K}{uni0028}{40}
\DeclareTextGlyphY{LinBiolinum_K}{parenright}{41}
\DeclareTextGlyphY{LinBiolinum_K}{uni0029}{41}
\DeclareTextGlyphY{LinBiolinum_K}{asterisk}{42}
\DeclareTextGlyphY{LinBiolinum_K}{uni002A}{42}
\DeclareTextGlyphY{LinBiolinum_K}{plus}{43}
\DeclareTextGlyphY{LinBiolinum_K}{uni002B}{43}
\DeclareTextGlyphY{LinBiolinum_K}{comma}{44}
\DeclareTextGlyphY{LinBiolinum_K}{uni002C}{44}
\DeclareTextGlyphY{LinBiolinum_K}{hyphen}{45}
\DeclareTextGlyphY{LinBiolinum_K}{uni002D}{45}
\DeclareTextGlyphY{LinBiolinum_K}{period}{46}
\DeclareTextGlyphY{LinBiolinum_K}{uni002E}{46}
\DeclareTextGlyphY{LinBiolinum_K}{slash}{47}
\DeclareTextGlyphY{LinBiolinum_K}{uni002F}{47}
\DeclareTextGlyphY{LinBiolinum_K}{zero}{48}
\DeclareTextGlyphY{LinBiolinum_K}{uni0030}{48}
\DeclareTextGlyphY{LinBiolinum_K}{one}{49}
\DeclareTextGlyphY{LinBiolinum_K}{uni0031}{49}
\DeclareTextGlyphY{LinBiolinum_K}{two}{50}
\DeclareTextGlyphY{LinBiolinum_K}{uni0032}{50}
\DeclareTextGlyphY{LinBiolinum_K}{three}{51}
\DeclareTextGlyphY{LinBiolinum_K}{uni0033}{51}
\DeclareTextGlyphY{LinBiolinum_K}{four}{52}
\DeclareTextGlyphY{LinBiolinum_K}{uni0034}{52}
\DeclareTextGlyphY{LinBiolinum_K}{five}{53}
\DeclareTextGlyphY{LinBiolinum_K}{uni0035}{53}
\DeclareTextGlyphY{LinBiolinum_K}{six}{54}
\DeclareTextGlyphY{LinBiolinum_K}{uni0036}{54}
\DeclareTextGlyphY{LinBiolinum_K}{seven}{55}
\DeclareTextGlyphY{LinBiolinum_K}{uni0037}{55}
\DeclareTextGlyphY{LinBiolinum_K}{eight}{56}
\DeclareTextGlyphY{LinBiolinum_K}{uni0038}{56}
\DeclareTextGlyphY{LinBiolinum_K}{nine}{57}
\DeclareTextGlyphY{LinBiolinum_K}{uni0039}{57}
\DeclareTextGlyphY{LinBiolinum_K}{colon}{58}
\DeclareTextGlyphY{LinBiolinum_K}{uni003A}{58}
\DeclareTextGlyphY{LinBiolinum_K}{semicolon}{59}
\DeclareTextGlyphY{LinBiolinum_K}{uni003B}{59}
\DeclareTextGlyphY{LinBiolinum_K}{less}{60}
\DeclareTextGlyphY{LinBiolinum_K}{uni003C}{60}
\DeclareTextGlyphY{LinBiolinum_K}{equal}{61}
\DeclareTextGlyphY{LinBiolinum_K}{uni003D}{61}
\DeclareTextGlyphY{LinBiolinum_K}{greater}{62}
\DeclareTextGlyphY{LinBiolinum_K}{uni003E}{62}
\DeclareTextGlyphY{LinBiolinum_K}{question}{63}
\DeclareTextGlyphY{LinBiolinum_K}{uni003F}{63}
\DeclareTextGlyphY{LinBiolinum_K}{at}{64}
\DeclareTextGlyphY{LinBiolinum_K}{uni0040}{64}
\DeclareTextGlyphY{LinBiolinum_K}{A}{65}
\DeclareTextGlyphY{LinBiolinum_K}{uni0041}{65}
\DeclareTextGlyphY{LinBiolinum_K}{B}{66}
\DeclareTextGlyphY{LinBiolinum_K}{uni0042}{66}
\DeclareTextGlyphY{LinBiolinum_K}{C}{67}
\DeclareTextGlyphY{LinBiolinum_K}{uni0043}{67}
\DeclareTextGlyphY{LinBiolinum_K}{D}{68}
\DeclareTextGlyphY{LinBiolinum_K}{uni0044}{68}
\DeclareTextGlyphY{LinBiolinum_K}{E}{69}
\DeclareTextGlyphY{LinBiolinum_K}{uni0045}{69}
\DeclareTextGlyphY{LinBiolinum_K}{F}{70}
\DeclareTextGlyphY{LinBiolinum_K}{uni0046}{70}
\DeclareTextGlyphY{LinBiolinum_K}{G}{71}
\DeclareTextGlyphY{LinBiolinum_K}{uni0047}{71}
\DeclareTextGlyphY{LinBiolinum_K}{H}{72}
\DeclareTextGlyphY{LinBiolinum_K}{uni0048}{72}
\DeclareTextGlyphY{LinBiolinum_K}{I}{73}
\DeclareTextGlyphY{LinBiolinum_K}{uni0049}{73}
\DeclareTextGlyphY{LinBiolinum_K}{J}{74}
\DeclareTextGlyphY{LinBiolinum_K}{uni004A}{74}
\DeclareTextGlyphY{LinBiolinum_K}{K}{75}
\DeclareTextGlyphY{LinBiolinum_K}{uni004B}{75}
\DeclareTextGlyphY{LinBiolinum_K}{L}{76}
\DeclareTextGlyphY{LinBiolinum_K}{uni004C}{76}
\DeclareTextGlyphY{LinBiolinum_K}{M}{77}
\DeclareTextGlyphY{LinBiolinum_K}{uni004D}{77}
\DeclareTextGlyphY{LinBiolinum_K}{N}{78}
\DeclareTextGlyphY{LinBiolinum_K}{uni004E}{78}
\DeclareTextGlyphY{LinBiolinum_K}{O}{79}
\DeclareTextGlyphY{LinBiolinum_K}{uni004F}{79}
\DeclareTextGlyphY{LinBiolinum_K}{P}{80}
\DeclareTextGlyphY{LinBiolinum_K}{uni0050}{80}
\DeclareTextGlyphY{LinBiolinum_K}{Q}{81}
\DeclareTextGlyphY{LinBiolinum_K}{uni0051}{81}
\DeclareTextGlyphY{LinBiolinum_K}{R}{82}
\DeclareTextGlyphY{LinBiolinum_K}{uni0052}{82}
\DeclareTextGlyphY{LinBiolinum_K}{S}{83}
\DeclareTextGlyphY{LinBiolinum_K}{uni0053}{83}
\DeclareTextGlyphY{LinBiolinum_K}{T}{84}
\DeclareTextGlyphY{LinBiolinum_K}{uni0054}{84}
\DeclareTextGlyphY{LinBiolinum_K}{U}{85}
\DeclareTextGlyphY{LinBiolinum_K}{uni0055}{85}
\DeclareTextGlyphY{LinBiolinum_K}{V}{86}
\DeclareTextGlyphY{LinBiolinum_K}{uni0056}{86}
\DeclareTextGlyphY{LinBiolinum_K}{W}{87}
\DeclareTextGlyphY{LinBiolinum_K}{uni0057}{87}
\DeclareTextGlyphY{LinBiolinum_K}{X}{88}
\DeclareTextGlyphY{LinBiolinum_K}{uni0058}{88}
\DeclareTextGlyphY{LinBiolinum_K}{Y}{89}
\DeclareTextGlyphY{LinBiolinum_K}{uni0059}{89}
\DeclareTextGlyphY{LinBiolinum_K}{Z}{90}
\DeclareTextGlyphY{LinBiolinum_K}{uni005A}{90}
\DeclareTextGlyphY{LinBiolinum_K}{bracketleft}{91}
\DeclareTextGlyphY{LinBiolinum_K}{uni005B}{91}
\DeclareTextGlyphY{LinBiolinum_K}{backslash}{92}
\DeclareTextGlyphY{LinBiolinum_K}{uni005C}{92}
\DeclareTextGlyphY{LinBiolinum_K}{bracketright}{93}
\DeclareTextGlyphY{LinBiolinum_K}{uni005D}{93}
\DeclareTextGlyphY{LinBiolinum_K}{asciicircum}{94}
\DeclareTextGlyphY{LinBiolinum_K}{uni005E}{94}
\DeclareTextGlyphY{LinBiolinum_K}{underscore}{95}
\DeclareTextGlyphY{LinBiolinum_K}{uni005F}{95}
\DeclareTextGlyphY{LinBiolinum_K}{grave}{96}
\DeclareTextGlyphY{LinBiolinum_K}{uni0060}{96}
\DeclareTextGlyphY{LinBiolinum_K}{a}{97}
\DeclareTextGlyphY{LinBiolinum_K}{uni0061}{97}
\DeclareTextGlyphY{LinBiolinum_K}{b}{98}
\DeclareTextGlyphY{LinBiolinum_K}{uni0062}{98}
\DeclareTextGlyphY{LinBiolinum_K}{c}{99}
\DeclareTextGlyphY{LinBiolinum_K}{uni0063}{99}
\DeclareTextGlyphY{LinBiolinum_K}{d}{100}
\DeclareTextGlyphY{LinBiolinum_K}{uni0064}{100}
\DeclareTextGlyphY{LinBiolinum_K}{e}{101}
\DeclareTextGlyphY{LinBiolinum_K}{uni0065}{101}
\DeclareTextGlyphY{LinBiolinum_K}{f}{102}
\DeclareTextGlyphY{LinBiolinum_K}{uni0066}{102}
\DeclareTextGlyphY{LinBiolinum_K}{g}{103}
\DeclareTextGlyphY{LinBiolinum_K}{uni0067}{103}
\DeclareTextGlyphY{LinBiolinum_K}{h}{104}
\DeclareTextGlyphY{LinBiolinum_K}{uni0068}{104}
\DeclareTextGlyphY{LinBiolinum_K}{i}{105}
\DeclareTextGlyphY{LinBiolinum_K}{uni0069}{105}
\DeclareTextGlyphY{LinBiolinum_K}{j}{106}
\DeclareTextGlyphY{LinBiolinum_K}{uni006A}{106}
\DeclareTextGlyphY{LinBiolinum_K}{k}{107}
\DeclareTextGlyphY{LinBiolinum_K}{uni006B}{107}
\DeclareTextGlyphY{LinBiolinum_K}{l}{108}
\DeclareTextGlyphY{LinBiolinum_K}{uni006C}{108}
\DeclareTextGlyphY{LinBiolinum_K}{m}{109}
\DeclareTextGlyphY{LinBiolinum_K}{uni006D}{109}
\DeclareTextGlyphY{LinBiolinum_K}{n}{110}
\DeclareTextGlyphY{LinBiolinum_K}{uni006E}{110}
\DeclareTextGlyphY{LinBiolinum_K}{o}{111}
\DeclareTextGlyphY{LinBiolinum_K}{uni006F}{111}
\DeclareTextGlyphY{LinBiolinum_K}{p}{112}
\DeclareTextGlyphY{LinBiolinum_K}{uni0070}{112}
\DeclareTextGlyphY{LinBiolinum_K}{q}{113}
\DeclareTextGlyphY{LinBiolinum_K}{uni0071}{113}
\DeclareTextGlyphY{LinBiolinum_K}{r}{114}
\DeclareTextGlyphY{LinBiolinum_K}{uni0072}{114}
\DeclareTextGlyphY{LinBiolinum_K}{s}{115}
\DeclareTextGlyphY{LinBiolinum_K}{uni0073}{115}
\DeclareTextGlyphY{LinBiolinum_K}{t}{116}
\DeclareTextGlyphY{LinBiolinum_K}{uni0074}{116}
\DeclareTextGlyphY{LinBiolinum_K}{u}{117}
\DeclareTextGlyphY{LinBiolinum_K}{uni0075}{117}
\DeclareTextGlyphY{LinBiolinum_K}{v}{118}
\DeclareTextGlyphY{LinBiolinum_K}{uni0076}{118}
\DeclareTextGlyphY{LinBiolinum_K}{w}{119}
\DeclareTextGlyphY{LinBiolinum_K}{uni0077}{119}
\DeclareTextGlyphY{LinBiolinum_K}{x}{120}
\DeclareTextGlyphY{LinBiolinum_K}{uni0078}{120}
\DeclareTextGlyphY{LinBiolinum_K}{y}{121}
\DeclareTextGlyphY{LinBiolinum_K}{uni0079}{121}
\DeclareTextGlyphY{LinBiolinum_K}{z}{122}
\DeclareTextGlyphY{LinBiolinum_K}{uni007A}{122}
\DeclareTextGlyphY{LinBiolinum_K}{braceleft}{123}
\DeclareTextGlyphY{LinBiolinum_K}{uni007B}{123}
\DeclareTextGlyphY{LinBiolinum_K}{bar}{124}
\DeclareTextGlyphY{LinBiolinum_K}{uni007C}{124}
\DeclareTextGlyphY{LinBiolinum_K}{braceright}{125}
\DeclareTextGlyphY{LinBiolinum_K}{uni007D}{125}
\DeclareTextGlyphY{LinBiolinum_K}{asciitilde}{126}
\DeclareTextGlyphY{LinBiolinum_K}{uni007E}{126}
\DeclareTextGlyphY{LinBiolinum_K}{exclamdown}{161}
\DeclareTextGlyphY{LinBiolinum_K}{uni00A1}{161}
\DeclareTextGlyphY{LinBiolinum_K}{cent}{162}
\DeclareTextGlyphY{LinBiolinum_K}{uni00A2}{162}
\DeclareTextGlyphY{LinBiolinum_K}{sterling}{163}
\DeclareTextGlyphY{LinBiolinum_K}{uni00A3}{163}
\DeclareTextGlyphY{LinBiolinum_K}{currency}{164}
\DeclareTextGlyphY{LinBiolinum_K}{uni00A4}{164}
\DeclareTextGlyphY{LinBiolinum_K}{yen}{165}
\DeclareTextGlyphY{LinBiolinum_K}{uni00A5}{165}
\DeclareTextGlyphY{LinBiolinum_K}{brokenbar}{166}
\DeclareTextGlyphY{LinBiolinum_K}{uni00A6}{166}
\DeclareTextGlyphY{LinBiolinum_K}{section}{167}
\DeclareTextGlyphY{LinBiolinum_K}{uni00A7}{167}
\DeclareTextGlyphY{LinBiolinum_K}{dieresis}{168}
\DeclareTextGlyphY{LinBiolinum_K}{uni00A8}{168}
\DeclareTextGlyphY{LinBiolinum_K}{guillemotleft}{171}
\DeclareTextGlyphY{LinBiolinum_K}{uni00AB}{171}
\DeclareTextGlyphY{LinBiolinum_K}{uni00AD}{173}
\DeclareTextGlyphY{LinBiolinum_K}{degree}{176}
\DeclareTextGlyphY{LinBiolinum_K}{uni00B0}{176}
\DeclareTextGlyphY{LinBiolinum_K}{plusminus}{177}
\DeclareTextGlyphY{LinBiolinum_K}{uni00B1}{177}
\DeclareTextGlyphY{LinBiolinum_K}{acute}{180}
\DeclareTextGlyphY{LinBiolinum_K}{uni00B4}{180}
\DeclareTextGlyphY{LinBiolinum_K}{uni00B5}{181}
\DeclareTextGlyphY{LinBiolinum_K}{periodcentered}{183}
\DeclareTextGlyphY{LinBiolinum_K}{uni00B7}{183}
\DeclareTextGlyphY{LinBiolinum_K}{cedilla}{184}
\DeclareTextGlyphY{LinBiolinum_K}{uni00B8}{184}
\DeclareTextGlyphY{LinBiolinum_K}{guillemotright}{187}
\DeclareTextGlyphY{LinBiolinum_K}{uni00BB}{187}
\DeclareTextGlyphY{LinBiolinum_K}{Agrave}{192}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C0}{192}
\DeclareTextGlyphY{LinBiolinum_K}{Aacute}{193}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C1}{193}
\DeclareTextGlyphY{LinBiolinum_K}{Acircumflex}{194}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C2}{194}
\DeclareTextGlyphY{LinBiolinum_K}{Atilde}{195}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C3}{195}
\DeclareTextGlyphY{LinBiolinum_K}{Adieresis}{196}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C4}{196}
\DeclareTextGlyphY{LinBiolinum_K}{Aring}{197}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C5}{197}
\DeclareTextGlyphY{LinBiolinum_K}{Ccedilla}{199}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C7}{199}
\DeclareTextGlyphY{LinBiolinum_K}{Egrave}{200}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C8}{200}
\DeclareTextGlyphY{LinBiolinum_K}{Eacute}{201}
\DeclareTextGlyphY{LinBiolinum_K}{uni00C9}{201}
\DeclareTextGlyphY{LinBiolinum_K}{Ecircumflex}{202}
\DeclareTextGlyphY{LinBiolinum_K}{uni00CA}{202}
\DeclareTextGlyphY{LinBiolinum_K}{Edieresis}{203}
\DeclareTextGlyphY{LinBiolinum_K}{uni00CB}{203}
\DeclareTextGlyphY{LinBiolinum_K}{Igrave}{204}
\DeclareTextGlyphY{LinBiolinum_K}{uni00CC}{204}
\DeclareTextGlyphY{LinBiolinum_K}{Iacute}{205}
\DeclareTextGlyphY{LinBiolinum_K}{uni00CD}{205}
\DeclareTextGlyphY{LinBiolinum_K}{Icircumflex}{206}
\DeclareTextGlyphY{LinBiolinum_K}{uni00CE}{206}
\DeclareTextGlyphY{LinBiolinum_K}{Idieresis}{207}
\DeclareTextGlyphY{LinBiolinum_K}{uni00CF}{207}
\DeclareTextGlyphY{LinBiolinum_K}{Eth}{208}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D0}{208}
\DeclareTextGlyphY{LinBiolinum_K}{Ntilde}{209}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D1}{209}
\DeclareTextGlyphY{LinBiolinum_K}{Ograve}{210}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D2}{210}
\DeclareTextGlyphY{LinBiolinum_K}{Oacute}{211}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D3}{211}
\DeclareTextGlyphY{LinBiolinum_K}{Ocircumflex}{212}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D4}{212}
\DeclareTextGlyphY{LinBiolinum_K}{Otilde}{213}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D5}{213}
\DeclareTextGlyphY{LinBiolinum_K}{Odieresis}{214}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D6}{214}
\DeclareTextGlyphY{LinBiolinum_K}{multiply}{215}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D7}{215}
\DeclareTextGlyphY{LinBiolinum_K}{Oslash}{216}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D8}{216}
\DeclareTextGlyphY{LinBiolinum_K}{Ugrave}{217}
\DeclareTextGlyphY{LinBiolinum_K}{uni00D9}{217}
\DeclareTextGlyphY{LinBiolinum_K}{Uacute}{218}
\DeclareTextGlyphY{LinBiolinum_K}{uni00DA}{218}
\DeclareTextGlyphY{LinBiolinum_K}{Ucircumflex}{219}
\DeclareTextGlyphY{LinBiolinum_K}{uni00DB}{219}
\DeclareTextGlyphY{LinBiolinum_K}{Udieresis}{220}
\DeclareTextGlyphY{LinBiolinum_K}{uni00DC}{220}
\DeclareTextGlyphY{LinBiolinum_K}{Yacute}{221}
\DeclareTextGlyphY{LinBiolinum_K}{uni00DD}{221}
\DeclareTextGlyphY{LinBiolinum_K}{Thorn}{222}
\DeclareTextGlyphY{LinBiolinum_K}{uni00DE}{222}
\DeclareTextGlyphY{LinBiolinum_K}{germandbls}{223}
\DeclareTextGlyphY{LinBiolinum_K}{uni00DF}{223}
\DeclareTextGlyphY{LinBiolinum_K}{agrave}{224}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E0}{224}
\DeclareTextGlyphY{LinBiolinum_K}{aacute}{225}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E1}{225}
\DeclareTextGlyphY{LinBiolinum_K}{acircumflex}{226}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E2}{226}
\DeclareTextGlyphY{LinBiolinum_K}{atilde}{227}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E3}{227}
\DeclareTextGlyphY{LinBiolinum_K}{adieresis}{228}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E4}{228}
\DeclareTextGlyphY{LinBiolinum_K}{aring}{229}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E5}{229}
\DeclareTextGlyphY{LinBiolinum_K}{ae}{230}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E6}{230}
\DeclareTextGlyphY{LinBiolinum_K}{ccedilla}{231}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E7}{231}
\DeclareTextGlyphY{LinBiolinum_K}{egrave}{232}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E8}{232}
\DeclareTextGlyphY{LinBiolinum_K}{eacute}{233}
\DeclareTextGlyphY{LinBiolinum_K}{uni00E9}{233}
\DeclareTextGlyphY{LinBiolinum_K}{ecircumflex}{234}
\DeclareTextGlyphY{LinBiolinum_K}{uni00EA}{234}
\DeclareTextGlyphY{LinBiolinum_K}{edieresis}{235}
\DeclareTextGlyphY{LinBiolinum_K}{uni00EB}{235}
\DeclareTextGlyphY{LinBiolinum_K}{igrave}{236}
\DeclareTextGlyphY{LinBiolinum_K}{uni00EC}{236}
\DeclareTextGlyphY{LinBiolinum_K}{iacute}{237}
\DeclareTextGlyphY{LinBiolinum_K}{uni00ED}{237}
\DeclareTextGlyphY{LinBiolinum_K}{icircumflex}{238}
\DeclareTextGlyphY{LinBiolinum_K}{uni00EE}{238}
\DeclareTextGlyphY{LinBiolinum_K}{idieresis}{239}
\DeclareTextGlyphY{LinBiolinum_K}{uni00EF}{239}
\DeclareTextGlyphY{LinBiolinum_K}{eth}{240}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F0}{240}
\DeclareTextGlyphY{LinBiolinum_K}{ntilde}{241}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F1}{241}
\DeclareTextGlyphY{LinBiolinum_K}{ograve}{242}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F2}{242}
\DeclareTextGlyphY{LinBiolinum_K}{oacute}{243}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F3}{243}
\DeclareTextGlyphY{LinBiolinum_K}{ocircumflex}{244}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F4}{244}
\DeclareTextGlyphY{LinBiolinum_K}{otilde}{245}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F5}{245}
\DeclareTextGlyphY{LinBiolinum_K}{odieresis}{246}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F6}{246}
\DeclareTextGlyphY{LinBiolinum_K}{divide}{247}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F7}{247}
\DeclareTextGlyphY{LinBiolinum_K}{oslash}{248}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F8}{248}
\DeclareTextGlyphY{LinBiolinum_K}{ugrave}{249}
\DeclareTextGlyphY{LinBiolinum_K}{uni00F9}{249}
\DeclareTextGlyphY{LinBiolinum_K}{uacute}{250}
\DeclareTextGlyphY{LinBiolinum_K}{uni00FA}{250}
\DeclareTextGlyphY{LinBiolinum_K}{ucircumflex}{251}
\DeclareTextGlyphY{LinBiolinum_K}{uni00FB}{251}
\DeclareTextGlyphY{LinBiolinum_K}{udieresis}{252}
\DeclareTextGlyphY{LinBiolinum_K}{uni00FC}{252}
\DeclareTextGlyphY{LinBiolinum_K}{yacute}{253}
\DeclareTextGlyphY{LinBiolinum_K}{uni00FD}{253}
\DeclareTextGlyphY{LinBiolinum_K}{thorn}{254}
\DeclareTextGlyphY{LinBiolinum_K}{uni00FE}{254}
\DeclareTextGlyphY{LinBiolinum_K}{ydieresis}{255}
\DeclareTextGlyphY{LinBiolinum_K}{uni00FF}{255}
\DeclareTextGlyphY{LinBiolinum_K}{Amacron}{256}
\DeclareTextGlyphY{LinBiolinum_K}{uni0100}{256}
\DeclareTextGlyphY{LinBiolinum_K}{amacron}{257}
\DeclareTextGlyphY{LinBiolinum_K}{uni0101}{257}
\DeclareTextGlyphY{LinBiolinum_K}{Abreve}{258}
\DeclareTextGlyphY{LinBiolinum_K}{uni0102}{258}
\DeclareTextGlyphY{LinBiolinum_K}{abreve}{259}
\DeclareTextGlyphY{LinBiolinum_K}{uni0103}{259}
\DeclareTextGlyphY{LinBiolinum_K}{Aogonek}{260}
\DeclareTextGlyphY{LinBiolinum_K}{uni0104}{260}
\DeclareTextGlyphY{LinBiolinum_K}{aogonek}{261}
\DeclareTextGlyphY{LinBiolinum_K}{uni0105}{261}
\DeclareTextGlyphY{LinBiolinum_K}{Cacute}{262}
\DeclareTextGlyphY{LinBiolinum_K}{uni0106}{262}
\DeclareTextGlyphY{LinBiolinum_K}{cacute}{263}
\DeclareTextGlyphY{LinBiolinum_K}{uni0107}{263}
\DeclareTextGlyphY{LinBiolinum_K}{Ccircumflex}{264}
\DeclareTextGlyphY{LinBiolinum_K}{uni0108}{264}
\DeclareTextGlyphY{LinBiolinum_K}{ccircumflex}{265}
\DeclareTextGlyphY{LinBiolinum_K}{uni0109}{265}
\DeclareTextGlyphY{LinBiolinum_K}{Cdotaccent}{266}
\DeclareTextGlyphY{LinBiolinum_K}{uni010A}{266}
\DeclareTextGlyphY{LinBiolinum_K}{cdotaccent}{267}
\DeclareTextGlyphY{LinBiolinum_K}{uni010B}{267}
\DeclareTextGlyphY{LinBiolinum_K}{Ccaron}{268}
\DeclareTextGlyphY{LinBiolinum_K}{uni010C}{268}
\DeclareTextGlyphY{LinBiolinum_K}{ccaron}{269}
\DeclareTextGlyphY{LinBiolinum_K}{uni010D}{269}
\DeclareTextGlyphY{LinBiolinum_K}{Dcaron}{270}
\DeclareTextGlyphY{LinBiolinum_K}{uni010E}{270}
\DeclareTextGlyphY{LinBiolinum_K}{dcaron}{271}
\DeclareTextGlyphY{LinBiolinum_K}{uni010F}{271}
\DeclareTextGlyphY{LinBiolinum_K}{Dcroat}{272}
\DeclareTextGlyphY{LinBiolinum_K}{uni0110}{272}
\DeclareTextGlyphY{LinBiolinum_K}{dcroat}{273}
\DeclareTextGlyphY{LinBiolinum_K}{uni0111}{273}
\DeclareTextGlyphY{LinBiolinum_K}{Emacron}{274}
\DeclareTextGlyphY{LinBiolinum_K}{uni0112}{274}
\DeclareTextGlyphY{LinBiolinum_K}{emacron}{275}
\DeclareTextGlyphY{LinBiolinum_K}{uni0113}{275}
\DeclareTextGlyphY{LinBiolinum_K}{Ebreve}{276}
\DeclareTextGlyphY{LinBiolinum_K}{uni0114}{276}
\DeclareTextGlyphY{LinBiolinum_K}{ebreve}{277}
\DeclareTextGlyphY{LinBiolinum_K}{uni0115}{277}
\DeclareTextGlyphY{LinBiolinum_K}{Edotaccent}{278}
\DeclareTextGlyphY{LinBiolinum_K}{uni0116}{278}
\DeclareTextGlyphY{LinBiolinum_K}{edotaccent}{279}
\DeclareTextGlyphY{LinBiolinum_K}{uni0117}{279}
\DeclareTextGlyphY{LinBiolinum_K}{Eogonek}{280}
\DeclareTextGlyphY{LinBiolinum_K}{uni0118}{280}
\DeclareTextGlyphY{LinBiolinum_K}{eogonek}{281}
\DeclareTextGlyphY{LinBiolinum_K}{uni0119}{281}
\DeclareTextGlyphY{LinBiolinum_K}{Ecaron}{282}
\DeclareTextGlyphY{LinBiolinum_K}{uni011A}{282}
\DeclareTextGlyphY{LinBiolinum_K}{ecaron}{283}
\DeclareTextGlyphY{LinBiolinum_K}{uni011B}{283}
\DeclareTextGlyphY{LinBiolinum_K}{Gcircumflex}{284}
\DeclareTextGlyphY{LinBiolinum_K}{uni011C}{284}
\DeclareTextGlyphY{LinBiolinum_K}{gcircumflex}{285}
\DeclareTextGlyphY{LinBiolinum_K}{uni011D}{285}
\DeclareTextGlyphY{LinBiolinum_K}{Gbreve}{286}
\DeclareTextGlyphY{LinBiolinum_K}{uni011E}{286}
\DeclareTextGlyphY{LinBiolinum_K}{gbreve}{287}
\DeclareTextGlyphY{LinBiolinum_K}{uni011F}{287}
\DeclareTextGlyphY{LinBiolinum_K}{Gdotaccent}{288}
\DeclareTextGlyphY{LinBiolinum_K}{uni0120}{288}
\DeclareTextGlyphY{LinBiolinum_K}{gdotaccent}{289}
\DeclareTextGlyphY{LinBiolinum_K}{uni0121}{289}
\DeclareTextGlyphY{LinBiolinum_K}{Gcommaaccent}{290}
\DeclareTextGlyphY{LinBiolinum_K}{uni0122}{290}
\DeclareTextGlyphY{LinBiolinum_K}{gcommaaccent}{291}
\DeclareTextGlyphY{LinBiolinum_K}{uni0123}{291}
\DeclareTextGlyphY{LinBiolinum_K}{Hcircumflex}{292}
\DeclareTextGlyphY{LinBiolinum_K}{uni0124}{292}
\DeclareTextGlyphY{LinBiolinum_K}{hcircumflex}{293}
\DeclareTextGlyphY{LinBiolinum_K}{uni0125}{293}
\DeclareTextGlyphY{LinBiolinum_K}{Hbar}{294}
\DeclareTextGlyphY{LinBiolinum_K}{uni0126}{294}
\DeclareTextGlyphY{LinBiolinum_K}{hbar}{295}
\DeclareTextGlyphY{LinBiolinum_K}{uni0127}{295}
\DeclareTextGlyphY{LinBiolinum_K}{Itilde}{296}
\DeclareTextGlyphY{LinBiolinum_K}{uni0128}{296}
\DeclareTextGlyphY{LinBiolinum_K}{itilde}{297}
\DeclareTextGlyphY{LinBiolinum_K}{uni0129}{297}
\DeclareTextGlyphY{LinBiolinum_K}{Imacron}{298}
\DeclareTextGlyphY{LinBiolinum_K}{uni012A}{298}
\DeclareTextGlyphY{LinBiolinum_K}{imacron}{299}
\DeclareTextGlyphY{LinBiolinum_K}{uni012B}{299}
\DeclareTextGlyphY{LinBiolinum_K}{Ibreve}{300}
\DeclareTextGlyphY{LinBiolinum_K}{uni012C}{300}
\DeclareTextGlyphY{LinBiolinum_K}{ibreve}{301}
\DeclareTextGlyphY{LinBiolinum_K}{uni012D}{301}
\DeclareTextGlyphY{LinBiolinum_K}{Iogonek}{302}
\DeclareTextGlyphY{LinBiolinum_K}{uni012E}{302}
\DeclareTextGlyphY{LinBiolinum_K}{iogonek}{303}
\DeclareTextGlyphY{LinBiolinum_K}{uni012F}{303}
\DeclareTextGlyphY{LinBiolinum_K}{Idotaccent}{304}
\DeclareTextGlyphY{LinBiolinum_K}{uni0130}{304}
\DeclareTextGlyphY{LinBiolinum_K}{dotlessi}{305}
\DeclareTextGlyphY{LinBiolinum_K}{uni0131}{305}
\DeclareTextGlyphY{LinBiolinum_K}{IJ}{306}
\DeclareTextGlyphY{LinBiolinum_K}{uni0132}{306}
\DeclareTextGlyphY{LinBiolinum_K}{ij}{307}
\DeclareTextGlyphY{LinBiolinum_K}{uni0133}{307}
\DeclareTextGlyphY{LinBiolinum_K}{Jcircumflex}{308}
\DeclareTextGlyphY{LinBiolinum_K}{uni0134}{308}
\DeclareTextGlyphY{LinBiolinum_K}{jcircumflex}{309}
\DeclareTextGlyphY{LinBiolinum_K}{uni0135}{309}
\DeclareTextGlyphY{LinBiolinum_K}{Kcommaaccent}{310}
\DeclareTextGlyphY{LinBiolinum_K}{uni0136}{310}
\DeclareTextGlyphY{LinBiolinum_K}{kcommaaccent}{311}
\DeclareTextGlyphY{LinBiolinum_K}{uni0137}{311}
\DeclareTextGlyphY{LinBiolinum_K}{kgreenlandic}{312}
\DeclareTextGlyphY{LinBiolinum_K}{uni0138}{312}
\DeclareTextGlyphY{LinBiolinum_K}{Lacute}{313}
\DeclareTextGlyphY{LinBiolinum_K}{uni0139}{313}
\DeclareTextGlyphY{LinBiolinum_K}{lacute}{314}
\DeclareTextGlyphY{LinBiolinum_K}{uni013A}{314}
\DeclareTextGlyphY{LinBiolinum_K}{Lcommaaccent}{315}
\DeclareTextGlyphY{LinBiolinum_K}{uni013B}{315}
\DeclareTextGlyphY{LinBiolinum_K}{lcommaaccent}{316}
\DeclareTextGlyphY{LinBiolinum_K}{uni013C}{316}
\DeclareTextGlyphY{LinBiolinum_K}{Lcaron}{317}
\DeclareTextGlyphY{LinBiolinum_K}{uni013D}{317}
\DeclareTextGlyphY{LinBiolinum_K}{lcaron}{318}
\DeclareTextGlyphY{LinBiolinum_K}{uni013E}{318}
\DeclareTextGlyphY{LinBiolinum_K}{Ldot}{319}
\DeclareTextGlyphY{LinBiolinum_K}{uni013F}{319}
\DeclareTextGlyphY{LinBiolinum_K}{ldot}{320}
\DeclareTextGlyphY{LinBiolinum_K}{uni0140}{320}
\DeclareTextGlyphY{LinBiolinum_K}{Lslash}{321}
\DeclareTextGlyphY{LinBiolinum_K}{uni0141}{321}
\DeclareTextGlyphY{LinBiolinum_K}{lslash}{322}
\DeclareTextGlyphY{LinBiolinum_K}{uni0142}{322}
\DeclareTextGlyphY{LinBiolinum_K}{Nacute}{323}
\DeclareTextGlyphY{LinBiolinum_K}{uni0143}{323}
\DeclareTextGlyphY{LinBiolinum_K}{nacute}{324}
\DeclareTextGlyphY{LinBiolinum_K}{uni0144}{324}
\DeclareTextGlyphY{LinBiolinum_K}{Ncommaaccent}{325}
\DeclareTextGlyphY{LinBiolinum_K}{uni0145}{325}
\DeclareTextGlyphY{LinBiolinum_K}{ncommaaccent}{326}
\DeclareTextGlyphY{LinBiolinum_K}{uni0146}{326}
\DeclareTextGlyphY{LinBiolinum_K}{Ncaron}{327}
\DeclareTextGlyphY{LinBiolinum_K}{uni0147}{327}
\DeclareTextGlyphY{LinBiolinum_K}{ncaron}{328}
\DeclareTextGlyphY{LinBiolinum_K}{uni0148}{328}
\DeclareTextGlyphY{LinBiolinum_K}{napostrophe}{329}
\DeclareTextGlyphY{LinBiolinum_K}{uni0149}{329}
\DeclareTextGlyphY{LinBiolinum_K}{Omacron}{332}
\DeclareTextGlyphY{LinBiolinum_K}{uni014C}{332}
\DeclareTextGlyphY{LinBiolinum_K}{omacron}{333}
\DeclareTextGlyphY{LinBiolinum_K}{uni014D}{333}
\DeclareTextGlyphY{LinBiolinum_K}{Obreve}{334}
\DeclareTextGlyphY{LinBiolinum_K}{uni014E}{334}
\DeclareTextGlyphY{LinBiolinum_K}{obreve}{335}
\DeclareTextGlyphY{LinBiolinum_K}{uni014F}{335}
\DeclareTextGlyphY{LinBiolinum_K}{Ohungarumlaut}{336}
\DeclareTextGlyphY{LinBiolinum_K}{uni0150}{336}
\DeclareTextGlyphY{LinBiolinum_K}{ohungarumlaut}{337}
\DeclareTextGlyphY{LinBiolinum_K}{uni0151}{337}
\DeclareTextGlyphY{LinBiolinum_K}{Racute}{340}
\DeclareTextGlyphY{LinBiolinum_K}{uni0154}{340}
\DeclareTextGlyphY{LinBiolinum_K}{racute}{341}
\DeclareTextGlyphY{LinBiolinum_K}{uni0155}{341}
\DeclareTextGlyphY{LinBiolinum_K}{Rcommaaccent}{342}
\DeclareTextGlyphY{LinBiolinum_K}{uni0156}{342}
\DeclareTextGlyphY{LinBiolinum_K}{rcommaaccent}{343}
\DeclareTextGlyphY{LinBiolinum_K}{uni0157}{343}
\DeclareTextGlyphY{LinBiolinum_K}{Rcaron}{344}
\DeclareTextGlyphY{LinBiolinum_K}{uni0158}{344}
\DeclareTextGlyphY{LinBiolinum_K}{rcaron}{345}
\DeclareTextGlyphY{LinBiolinum_K}{uni0159}{345}
\DeclareTextGlyphY{LinBiolinum_K}{Sacute}{346}
\DeclareTextGlyphY{LinBiolinum_K}{uni015A}{346}
\DeclareTextGlyphY{LinBiolinum_K}{sacute}{347}
\DeclareTextGlyphY{LinBiolinum_K}{uni015B}{347}
\DeclareTextGlyphY{LinBiolinum_K}{Scircumflex}{348}
\DeclareTextGlyphY{LinBiolinum_K}{uni015C}{348}
\DeclareTextGlyphY{LinBiolinum_K}{scircumflex}{349}
\DeclareTextGlyphY{LinBiolinum_K}{uni015D}{349}
\DeclareTextGlyphY{LinBiolinum_K}{Scedilla}{350}
\DeclareTextGlyphY{LinBiolinum_K}{uni015E}{350}
\DeclareTextGlyphY{LinBiolinum_K}{scedilla}{351}
\DeclareTextGlyphY{LinBiolinum_K}{uni015F}{351}
\DeclareTextGlyphY{LinBiolinum_K}{Scaron}{352}
\DeclareTextGlyphY{LinBiolinum_K}{uni0160}{352}
\DeclareTextGlyphY{LinBiolinum_K}{scaron}{353}
\DeclareTextGlyphY{LinBiolinum_K}{uni0161}{353}
\DeclareTextGlyphY{LinBiolinum_K}{Tcedilla}{354}
\DeclareTextGlyphY{LinBiolinum_K}{uni0162}{354}
\DeclareTextGlyphY{LinBiolinum_K}{tcedilla}{355}
\DeclareTextGlyphY{LinBiolinum_K}{uni0163}{355}
\DeclareTextGlyphY{LinBiolinum_K}{Tcaron}{356}
\DeclareTextGlyphY{LinBiolinum_K}{uni0164}{356}
\DeclareTextGlyphY{LinBiolinum_K}{tcaron}{357}
\DeclareTextGlyphY{LinBiolinum_K}{uni0165}{357}
\DeclareTextGlyphY{LinBiolinum_K}{Tbar}{358}
\DeclareTextGlyphY{LinBiolinum_K}{uni0166}{358}
\DeclareTextGlyphY{LinBiolinum_K}{tbar}{359}
\DeclareTextGlyphY{LinBiolinum_K}{uni0167}{359}
\DeclareTextGlyphY{LinBiolinum_K}{Utilde}{360}
\DeclareTextGlyphY{LinBiolinum_K}{uni0168}{360}
\DeclareTextGlyphY{LinBiolinum_K}{utilde}{361}
\DeclareTextGlyphY{LinBiolinum_K}{uni0169}{361}
\DeclareTextGlyphY{LinBiolinum_K}{Umacron}{362}
\DeclareTextGlyphY{LinBiolinum_K}{uni016A}{362}
\DeclareTextGlyphY{LinBiolinum_K}{umacron}{363}
\DeclareTextGlyphY{LinBiolinum_K}{uni016B}{363}
\DeclareTextGlyphY{LinBiolinum_K}{Ubreve}{364}
\DeclareTextGlyphY{LinBiolinum_K}{uni016C}{364}
\DeclareTextGlyphY{LinBiolinum_K}{ubreve}{365}
\DeclareTextGlyphY{LinBiolinum_K}{uni016D}{365}
\DeclareTextGlyphY{LinBiolinum_K}{Uring}{366}
\DeclareTextGlyphY{LinBiolinum_K}{uni016E}{366}
\DeclareTextGlyphY{LinBiolinum_K}{uring}{367}
\DeclareTextGlyphY{LinBiolinum_K}{uni016F}{367}
\DeclareTextGlyphY{LinBiolinum_K}{Uhungarumlaut}{368}
\DeclareTextGlyphY{LinBiolinum_K}{uni0170}{368}
\DeclareTextGlyphY{LinBiolinum_K}{uhungarumlaut}{369}
\DeclareTextGlyphY{LinBiolinum_K}{uni0171}{369}
\DeclareTextGlyphY{LinBiolinum_K}{Uogonek}{370}
\DeclareTextGlyphY{LinBiolinum_K}{uni0172}{370}
\DeclareTextGlyphY{LinBiolinum_K}{uogonek}{371}
\DeclareTextGlyphY{LinBiolinum_K}{uni0173}{371}
\DeclareTextGlyphY{LinBiolinum_K}{Wcircumflex}{372}
\DeclareTextGlyphY{LinBiolinum_K}{uni0174}{372}
\DeclareTextGlyphY{LinBiolinum_K}{wcircumflex}{373}
\DeclareTextGlyphY{LinBiolinum_K}{uni0175}{373}
\DeclareTextGlyphY{LinBiolinum_K}{Ycircumflex}{374}
\DeclareTextGlyphY{LinBiolinum_K}{uni0176}{374}
\DeclareTextGlyphY{LinBiolinum_K}{ycircumflex}{375}
\DeclareTextGlyphY{LinBiolinum_K}{uni0177}{375}
\DeclareTextGlyphY{LinBiolinum_K}{Ydieresis}{376}
\DeclareTextGlyphY{LinBiolinum_K}{uni0178}{376}
\DeclareTextGlyphY{LinBiolinum_K}{Zacute}{377}
\DeclareTextGlyphY{LinBiolinum_K}{uni0179}{377}
\DeclareTextGlyphY{LinBiolinum_K}{zacute}{378}
\DeclareTextGlyphY{LinBiolinum_K}{uni017A}{378}
\DeclareTextGlyphY{LinBiolinum_K}{Zdotaccent}{379}
\DeclareTextGlyphY{LinBiolinum_K}{uni017B}{379}
\DeclareTextGlyphY{LinBiolinum_K}{zdotaccent}{380}
\DeclareTextGlyphY{LinBiolinum_K}{uni017C}{380}
\DeclareTextGlyphY{LinBiolinum_K}{Zcaron}{381}
\DeclareTextGlyphY{LinBiolinum_K}{uni017D}{381}
\DeclareTextGlyphY{LinBiolinum_K}{zcaron}{382}
\DeclareTextGlyphY{LinBiolinum_K}{uni017E}{382}
\DeclareTextGlyphY{LinBiolinum_K}{h.superior}{688}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B0}{688}
\DeclareTextGlyphY{LinBiolinum_K}{hhook.superior}{689}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B1}{689}
\DeclareTextGlyphY{LinBiolinum_K}{j.superior}{690}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B2}{690}
\DeclareTextGlyphY{LinBiolinum_K}{r.superior}{691}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B3}{691}
\DeclareTextGlyphY{LinBiolinum_K}{rturned.superior}{692}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B4}{692}
\DeclareTextGlyphY{LinBiolinum_K}{rhookturned.superior}{693}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B5}{693}
\DeclareTextGlyphY{LinBiolinum_K}{Rsmallinverted.superior}{694}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B6}{694}
\DeclareTextGlyphY{LinBiolinum_K}{w.superior}{695}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B7}{695}
\DeclareTextGlyphY{LinBiolinum_K}{y.superior}{696}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B8}{696}
\DeclareTextGlyphY{LinBiolinum_K}{uni02B9}{697}
\DeclareTextGlyphY{LinBiolinum_K}{uni02BA}{698}
\DeclareTextGlyphY{LinBiolinum_K}{uni02BB}{699}
\DeclareTextGlyphY{LinBiolinum_K}{afii57929}{700}
\DeclareTextGlyphY{LinBiolinum_K}{uni02BC}{700}
\DeclareTextGlyphY{LinBiolinum_K}{afii64937}{701}
\DeclareTextGlyphY{LinBiolinum_K}{uni02BD}{701}
\DeclareTextGlyphY{LinBiolinum_K}{uni02BE}{702}
\DeclareTextGlyphY{LinBiolinum_K}{uni02BF}{703}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C0}{704}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C1}{705}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C2}{706}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C3}{707}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C4}{708}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C5}{709}
\DeclareTextGlyphY{LinBiolinum_K}{circumflex}{710}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C6}{710}
\DeclareTextGlyphY{LinBiolinum_K}{caron}{711}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C7}{711}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C8}{712}
\DeclareTextGlyphY{LinBiolinum_K}{uni02C9}{713}
\DeclareTextGlyphY{LinBiolinum_K}{uni02CA}{714}
\DeclareTextGlyphY{LinBiolinum_K}{uni02CB}{715}
\DeclareTextGlyphY{LinBiolinum_K}{uni02CC}{716}
\DeclareTextGlyphY{LinBiolinum_K}{uni02CD}{717}
\DeclareTextGlyphY{LinBiolinum_K}{uni02CE}{718}
\DeclareTextGlyphY{LinBiolinum_K}{uni02CF}{719}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D0}{720}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D1}{721}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D2}{722}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D3}{723}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D4}{724}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D5}{725}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D6}{726}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D7}{727}
\DeclareTextGlyphY{LinBiolinum_K}{breve}{728}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D8}{728}
\DeclareTextGlyphY{LinBiolinum_K}{dotaccent}{729}
\DeclareTextGlyphY{LinBiolinum_K}{uni02D9}{729}
\DeclareTextGlyphY{LinBiolinum_K}{ring}{730}
\DeclareTextGlyphY{LinBiolinum_K}{uni02DA}{730}
\DeclareTextGlyphY{LinBiolinum_K}{ogonek}{731}
\DeclareTextGlyphY{LinBiolinum_K}{uni02DB}{731}
\DeclareTextGlyphY{LinBiolinum_K}{tilde}{732}
\DeclareTextGlyphY{LinBiolinum_K}{uni02DC}{732}
\DeclareTextGlyphY{LinBiolinum_K}{hungarumlaut}{733}
\DeclareTextGlyphY{LinBiolinum_K}{uni02DD}{733}
\DeclareTextGlyphY{LinBiolinum_K}{uni02DE}{734}
\DeclareTextGlyphY{LinBiolinum_K}{uni02DF}{735}
\DeclareTextGlyphY{LinBiolinum_K}{gammalatin.superior}{736}
\DeclareTextGlyphY{LinBiolinum_K}{uni02E0}{736}
\DeclareTextGlyphY{LinBiolinum_K}{l.superior}{737}
\DeclareTextGlyphY{LinBiolinum_K}{uni02E1}{737}
\DeclareTextGlyphY{LinBiolinum_K}{s.superior}{738}
\DeclareTextGlyphY{LinBiolinum_K}{uni02E2}{738}
\DeclareTextGlyphY{LinBiolinum_K}{x.superior}{739}
\DeclareTextGlyphY{LinBiolinum_K}{uni02E3}{739}
\DeclareTextGlyphY{LinBiolinum_K}{glottalstopreversed.superior}{740}
\DeclareTextGlyphY{LinBiolinum_K}{uni02E4}{740}
\DeclareTextGlyphY{LinBiolinum_K}{uni02EC}{748}
\DeclareTextGlyphY{LinBiolinum_K}{uni02ED}{749}
\DeclareTextGlyphY{LinBiolinum_K}{uni02EE}{750}
\DeclareTextGlyphY{LinBiolinum_K}{gravecomb}{768}
\DeclareTextGlyphY{LinBiolinum_K}{uni0300}{768}
\DeclareTextGlyphY{LinBiolinum_K}{acutecomb}{769}
\DeclareTextGlyphY{LinBiolinum_K}{uni0301}{769}
\DeclareTextGlyphY{LinBiolinum_K}{uni0302}{770}
\DeclareTextGlyphY{LinBiolinum_K}{tildecomb}{771}
\DeclareTextGlyphY{LinBiolinum_K}{uni0303}{771}
\DeclareTextGlyphY{LinBiolinum_K}{uni0304}{772}
\DeclareTextGlyphY{LinBiolinum_K}{uni0305}{773}
\DeclareTextGlyphY{LinBiolinum_K}{uni0306}{774}
\DeclareTextGlyphY{LinBiolinum_K}{uni0307}{775}
\DeclareTextGlyphY{LinBiolinum_K}{uni0308}{776}
\DeclareTextGlyphY{LinBiolinum_K}{hookabovecomb}{777}
\DeclareTextGlyphY{LinBiolinum_K}{uni0309}{777}
\DeclareTextGlyphY{LinBiolinum_K}{uni030A}{778}
\DeclareTextGlyphY{LinBiolinum_K}{uni030B}{779}
\DeclareTextGlyphY{LinBiolinum_K}{uni030C}{780}
\DeclareTextGlyphY{LinBiolinum_K}{uni030D}{781}
\DeclareTextGlyphY{LinBiolinum_K}{uni030E}{782}
\DeclareTextGlyphY{LinBiolinum_K}{uni030F}{783}
\DeclareTextGlyphY{LinBiolinum_K}{uni0310}{784}
\DeclareTextGlyphY{LinBiolinum_K}{uni0311}{785}
\DeclareTextGlyphY{LinBiolinum_K}{uni0312}{786}
\DeclareTextGlyphY{LinBiolinum_K}{uni0313}{787}
\DeclareTextGlyphY{LinBiolinum_K}{uni0314}{788}
\DeclareTextGlyphY{LinBiolinum_K}{uni0315}{789}
\DeclareTextGlyphY{LinBiolinum_K}{uni0316}{790}
\DeclareTextGlyphY{LinBiolinum_K}{uni0317}{791}
\DeclareTextGlyphY{LinBiolinum_K}{uni0318}{792}
\DeclareTextGlyphY{LinBiolinum_K}{uni0319}{793}
\DeclareTextGlyphY{LinBiolinum_K}{uni031A}{794}
\DeclareTextGlyphY{LinBiolinum_K}{uni031B}{795}
\DeclareTextGlyphY{LinBiolinum_K}{uni031C}{796}
\DeclareTextGlyphY{LinBiolinum_K}{uni031D}{797}
\DeclareTextGlyphY{LinBiolinum_K}{uni031E}{798}
\DeclareTextGlyphY{LinBiolinum_K}{uni031F}{799}
\DeclareTextGlyphY{LinBiolinum_K}{uni0320}{800}
\DeclareTextGlyphY{LinBiolinum_K}{uni0321}{801}
\DeclareTextGlyphY{LinBiolinum_K}{uni0322}{802}
\DeclareTextGlyphY{LinBiolinum_K}{dotbelowcomb}{803}
\DeclareTextGlyphY{LinBiolinum_K}{uni0323}{803}
\DeclareTextGlyphY{LinBiolinum_K}{uni0324}{804}
\DeclareTextGlyphY{LinBiolinum_K}{uni0325}{805}
\DeclareTextGlyphY{LinBiolinum_K}{uni0326}{806}
\DeclareTextGlyphY{LinBiolinum_K}{uni0327}{807}
\DeclareTextGlyphY{LinBiolinum_K}{uni0328}{808}
\DeclareTextGlyphY{LinBiolinum_K}{uni0329}{809}
\DeclareTextGlyphY{LinBiolinum_K}{uni032A}{810}
\DeclareTextGlyphY{LinBiolinum_K}{uni032B}{811}
\DeclareTextGlyphY{LinBiolinum_K}{uni032C}{812}
\DeclareTextGlyphY{LinBiolinum_K}{uni032D}{813}
\DeclareTextGlyphY{LinBiolinum_K}{uni032E}{814}
\DeclareTextGlyphY{LinBiolinum_K}{uni032F}{815}
\DeclareTextGlyphY{LinBiolinum_K}{uni0330}{816}
\DeclareTextGlyphY{LinBiolinum_K}{uni0331}{817}
\DeclareTextGlyphY{LinBiolinum_K}{uni0338}{824}
\DeclareTextGlyphY{LinBiolinum_K}{uni0342}{834}
\DeclareTextGlyphY{LinBiolinum_K}{uni0343}{835}
\DeclareTextGlyphY{LinBiolinum_K}{uni0351}{849}
\DeclareTextGlyphY{LinBiolinum_K}{uni0357}{855}
\DeclareTextGlyphY{LinBiolinum_K}{uni0358}{856}
\DeclareTextGlyphY{LinBiolinum_K}{uni0359}{857}
\DeclareTextGlyphY{LinBiolinum_K}{uni035A}{858}
\DeclareTextGlyphY{LinBiolinum_K}{uni035B}{859}
\DeclareTextGlyphY{LinBiolinum_K}{uni035C}{860}
\DeclareTextGlyphY{LinBiolinum_K}{uni035D}{861}
\DeclareTextGlyphY{LinBiolinum_K}{uni035E}{862}
\DeclareTextGlyphY{LinBiolinum_K}{uni035F}{863}
\DeclareTextGlyphY{LinBiolinum_K}{uni0360}{864}
\DeclareTextGlyphY{LinBiolinum_K}{uni0361}{865}
\DeclareTextGlyphY{LinBiolinum_K}{uni0362}{866}
\DeclareTextGlyphY{LinBiolinum_K}{uni0363}{867}
\DeclareTextGlyphY{LinBiolinum_K}{uni0374}{884}
\DeclareTextGlyphY{LinBiolinum_K}{uni0375}{885}
\DeclareTextGlyphY{LinBiolinum_K}{afii57799}{1456}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B0}{1456}
\DeclareTextGlyphY{LinBiolinum_K}{afii57801}{1457}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B1}{1457}
\DeclareTextGlyphY{LinBiolinum_K}{afii57800}{1458}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B2}{1458}
\DeclareTextGlyphY{LinBiolinum_K}{afii57802}{1459}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B3}{1459}
\DeclareTextGlyphY{LinBiolinum_K}{afii57793}{1460}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B4}{1460}
\DeclareTextGlyphY{LinBiolinum_K}{afii57794}{1461}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B5}{1461}
\DeclareTextGlyphY{LinBiolinum_K}{afii57795}{1462}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B6}{1462}
\DeclareTextGlyphY{LinBiolinum_K}{afii57798}{1463}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B7}{1463}
\DeclareTextGlyphY{LinBiolinum_K}{afii57797}{1464}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B8}{1464}
\DeclareTextGlyphY{LinBiolinum_K}{afii57806}{1465}
\DeclareTextGlyphY{LinBiolinum_K}{uni05B9}{1465}
\DeclareTextGlyphY{LinBiolinum_K}{uni05BA}{1466}
\DeclareTextGlyphY{LinBiolinum_K}{afii57796}{1467}
\DeclareTextGlyphY{LinBiolinum_K}{uni05BB}{1467}
\DeclareTextGlyphY{LinBiolinum_K}{afii57807}{1468}
\DeclareTextGlyphY{LinBiolinum_K}{uni05BC}{1468}
\DeclareTextGlyphY{LinBiolinum_K}{afii57839}{1469}
\DeclareTextGlyphY{LinBiolinum_K}{uni05BD}{1469}
\DeclareTextGlyphY{LinBiolinum_K}{afii57645}{1470}
\DeclareTextGlyphY{LinBiolinum_K}{uni05BE}{1470}
\DeclareTextGlyphY{LinBiolinum_K}{afii57841}{1471}
\DeclareTextGlyphY{LinBiolinum_K}{uni05BF}{1471}
\DeclareTextGlyphY{LinBiolinum_K}{afii57842}{1472}
\DeclareTextGlyphY{LinBiolinum_K}{uni05C0}{1472}
\DeclareTextGlyphY{LinBiolinum_K}{afii57804}{1473}
\DeclareTextGlyphY{LinBiolinum_K}{uni05C1}{1473}
\DeclareTextGlyphY{LinBiolinum_K}{afii57803}{1474}
\DeclareTextGlyphY{LinBiolinum_K}{uni05C2}{1474}
\DeclareTextGlyphY{LinBiolinum_K}{afii57658}{1475}
\DeclareTextGlyphY{LinBiolinum_K}{uni05C3}{1475}
\DeclareTextGlyphY{LinBiolinum_K}{uni05C6}{1478}
\DeclareTextGlyphY{LinBiolinum_K}{afii57664}{1488}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D0}{1488}
\DeclareTextGlyphY{LinBiolinum_K}{afii57665}{1489}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D1}{1489}
\DeclareTextGlyphY{LinBiolinum_K}{afii57666}{1490}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D2}{1490}
\DeclareTextGlyphY{LinBiolinum_K}{afii57667}{1491}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D3}{1491}
\DeclareTextGlyphY{LinBiolinum_K}{afii57668}{1492}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D4}{1492}
\DeclareTextGlyphY{LinBiolinum_K}{afii57669}{1493}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D5}{1493}
\DeclareTextGlyphY{LinBiolinum_K}{afii57670}{1494}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D6}{1494}
\DeclareTextGlyphY{LinBiolinum_K}{afii57671}{1495}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D7}{1495}
\DeclareTextGlyphY{LinBiolinum_K}{afii57672}{1496}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D8}{1496}
\DeclareTextGlyphY{LinBiolinum_K}{afii57673}{1497}
\DeclareTextGlyphY{LinBiolinum_K}{uni05D9}{1497}
\DeclareTextGlyphY{LinBiolinum_K}{afii57674}{1498}
\DeclareTextGlyphY{LinBiolinum_K}{uni05DA}{1498}
\DeclareTextGlyphY{LinBiolinum_K}{afii57675}{1499}
\DeclareTextGlyphY{LinBiolinum_K}{uni05DB}{1499}
\DeclareTextGlyphY{LinBiolinum_K}{afii57676}{1500}
\DeclareTextGlyphY{LinBiolinum_K}{uni05DC}{1500}
\DeclareTextGlyphY{LinBiolinum_K}{afii57677}{1501}
\DeclareTextGlyphY{LinBiolinum_K}{uni05DD}{1501}
\DeclareTextGlyphY{LinBiolinum_K}{afii57678}{1502}
\DeclareTextGlyphY{LinBiolinum_K}{uni05DE}{1502}
\DeclareTextGlyphY{LinBiolinum_K}{afii57679}{1503}
\DeclareTextGlyphY{LinBiolinum_K}{uni05DF}{1503}
\DeclareTextGlyphY{LinBiolinum_K}{afii57680}{1504}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E0}{1504}
\DeclareTextGlyphY{LinBiolinum_K}{afii57681}{1505}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E1}{1505}
\DeclareTextGlyphY{LinBiolinum_K}{afii57682}{1506}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E2}{1506}
\DeclareTextGlyphY{LinBiolinum_K}{afii57683}{1507}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E3}{1507}
\DeclareTextGlyphY{LinBiolinum_K}{afii57684}{1508}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E4}{1508}
\DeclareTextGlyphY{LinBiolinum_K}{afii57685}{1509}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E5}{1509}
\DeclareTextGlyphY{LinBiolinum_K}{afii57686}{1510}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E6}{1510}
\DeclareTextGlyphY{LinBiolinum_K}{afii57687}{1511}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E7}{1511}
\DeclareTextGlyphY{LinBiolinum_K}{afii57688}{1512}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E8}{1512}
\DeclareTextGlyphY{LinBiolinum_K}{afii57689}{1513}
\DeclareTextGlyphY{LinBiolinum_K}{uni05E9}{1513}
\DeclareTextGlyphY{LinBiolinum_K}{afii57690}{1514}
\DeclareTextGlyphY{LinBiolinum_K}{uni05EA}{1514}
\DeclareTextGlyphY{LinBiolinum_K}{afii57716}{1520}
\DeclareTextGlyphY{LinBiolinum_K}{uni05F0}{1520}
\DeclareTextGlyphY{LinBiolinum_K}{afii57717}{1521}
\DeclareTextGlyphY{LinBiolinum_K}{uni05F1}{1521}
\DeclareTextGlyphY{LinBiolinum_K}{afii57718}{1522}
\DeclareTextGlyphY{LinBiolinum_K}{uni05F2}{1522}
\DeclareTextGlyphY{LinBiolinum_K}{arrowleft}{8592}
\DeclareTextGlyphY{LinBiolinum_K}{uni2190}{8592}
\DeclareTextGlyphY{LinBiolinum_K}{arrowup}{8593}
\DeclareTextGlyphY{LinBiolinum_K}{uni2191}{8593}
\DeclareTextGlyphY{LinBiolinum_K}{arrowright}{8594}
\DeclareTextGlyphY{LinBiolinum_K}{uni2192}{8594}
\DeclareTextGlyphY{LinBiolinum_K}{arrowdown}{8595}
\DeclareTextGlyphY{LinBiolinum_K}{uni2193}{8595}
\DeclareTextGlyphY{LinBiolinum_K}{arrowboth}{8596}
\DeclareTextGlyphY{LinBiolinum_K}{uni2194}{8596}
\DeclareTextGlyphY{LinBiolinum_K}{arrowupdn}{8597}
\DeclareTextGlyphY{LinBiolinum_K}{uni2195}{8597}
\DeclareTextGlyphY{LinBiolinum_K}{uni2196}{8598}
\DeclareTextGlyphY{LinBiolinum_K}{uni2197}{8599}
\DeclareTextGlyphY{LinBiolinum_K}{uni2198}{8600}
\DeclareTextGlyphY{LinBiolinum_K}{uni2199}{8601}
\DeclareTextGlyphY{LinBiolinum_K}{uni219A}{8602}
\DeclareTextGlyphY{LinBiolinum_K}{uni219B}{8603}
\DeclareTextGlyphY{LinBiolinum_K}{uni21A5}{8613}
\DeclareTextGlyphY{LinBiolinum_K}{uni21A7}{8615}
\DeclareTextGlyphY{LinBiolinum_K}{uni21BC}{8636}
\DeclareTextGlyphY{LinBiolinum_K}{uni21BD}{8637}
\DeclareTextGlyphY{LinBiolinum_K}{uni21C0}{8640}
\DeclareTextGlyphY{LinBiolinum_K}{uni21C1}{8641}
\DeclareTextGlyphY{LinBiolinum_K}{arrowdblleft}{8656}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D0}{8656}
\DeclareTextGlyphY{LinBiolinum_K}{arrowdblup}{8657}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D1}{8657}
\DeclareTextGlyphY{LinBiolinum_K}{arrowdblright}{8658}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D2}{8658}
\DeclareTextGlyphY{LinBiolinum_K}{arrowdbldown}{8659}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D3}{8659}
\DeclareTextGlyphY{LinBiolinum_K}{arrowdblboth}{8660}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D4}{8660}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D5}{8661}
\DeclareTextGlyphY{LinBiolinum_K}{Nwarrow}{8662}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D6}{8662}
\DeclareTextGlyphY{LinBiolinum_K}{Nearrow}{8663}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D7}{8663}
\DeclareTextGlyphY{LinBiolinum_K}{Searrow}{8664}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D8}{8664}
\DeclareTextGlyphY{LinBiolinum_K}{Swarrow}{8665}
\DeclareTextGlyphY{LinBiolinum_K}{uni21D9}{8665}
\DeclareTextGlyphY{LinBiolinum_K}{uni2318}{8984}
\DeclareTextGlyphY{LinBiolinum_K}{uni2325}{8997}
\DeclareTextGlyphY{LinBiolinum_K}{uni2326}{8998}
\DeclareTextGlyphY{LinBiolinum_K}{uni2327}{8999}
\DeclareTextGlyphY{LinBiolinum_K}{uni232B}{9003}
\DeclareTextGlyphY{LinBiolinum_K}{uni237D}{9085}
\DeclareTextGlyphY{LinBiolinum_K}{uni2380}{9088}
\DeclareTextGlyphY{LinBiolinum_K}{uni2423}{9251}
\DeclareTextGlyphY{LinBiolinum_K}{filledbox}{9632}
\DeclareTextGlyphY{LinBiolinum_K}{uni25A0}{9632}
\DeclareTextGlyphY{LinBiolinum_K}{H22073}{9633}
\DeclareTextGlyphY{LinBiolinum_K}{uni25A1}{9633}
\DeclareTextGlyphY{LinBiolinum_K}{triagup}{9650}
\DeclareTextGlyphY{LinBiolinum_K}{uni25B2}{9650}
\DeclareTextGlyphY{LinBiolinum_K}{uni25B3}{9651}
\DeclareTextGlyphY{LinBiolinum_K}{uni25B6}{9654}
\DeclareTextGlyphY{LinBiolinum_K}{uni25B7}{9655}
\DeclareTextGlyphY{LinBiolinum_K}{triagdn}{9660}
\DeclareTextGlyphY{LinBiolinum_K}{uni25BC}{9660}
\DeclareTextGlyphY{LinBiolinum_K}{uni25BD}{9661}
\DeclareTextGlyphY{LinBiolinum_K}{uni25C0}{9664}
\DeclareTextGlyphY{LinBiolinum_K}{uni25C1}{9665}
\DeclareTextGlyphY{LinBiolinum_K}{uni25C6}{9670}
\DeclareTextGlyphY{LinBiolinum_K}{uni25C7}{9671}
\DeclareTextGlyphY{LinBiolinum_K}{uni25C9}{9673}
\DeclareTextGlyphY{LinBiolinum_K}{lozenge}{9674}
\DeclareTextGlyphY{LinBiolinum_K}{uni25CA}{9674}
\DeclareTextGlyphY{LinBiolinum_K}{circle}{9675}
\DeclareTextGlyphY{LinBiolinum_K}{uni25CB}{9675}
\DeclareTextGlyphY{LinBiolinum_K}{uni25CE}{9678}
\DeclareTextGlyphY{LinBiolinum_K}{H18533}{9679}
\DeclareTextGlyphY{LinBiolinum_K}{uni25CF}{9679}
\DeclareTextGlyphY{LinBiolinum_K}{uni25D0}{9680}
\DeclareTextGlyphY{LinBiolinum_K}{uni25D1}{9681}
\DeclareTextGlyphY{LinBiolinum_K}{uni25D2}{9682}
\DeclareTextGlyphY{LinBiolinum_K}{uni25D3}{9683}
\DeclareTextGlyphY{LinBiolinum_K}{uni25D4}{9684}
\DeclareTextGlyphY{LinBiolinum_K}{uni25D5}{9685}
\DeclareTextGlyphY{LinBiolinum_K}{uni25D6}{9686}
\DeclareTextGlyphY{LinBiolinum_K}{uni25D7}{9687}
\DeclareTextGlyphY{LinBiolinum_K}{openbullet}{9702}
\DeclareTextGlyphY{LinBiolinum_K}{uni25E6}{9702}
\DeclareTextGlyphY{LinBiolinum_K}{uni2605}{9733}
\DeclareTextGlyphY{LinBiolinum_K}{uni2619}{9753}
\DeclareTextGlyphY{LinBiolinum_K}{uni261B}{9755}
\DeclareTextGlyphY{LinBiolinum_K}{uni261E}{9758}
\DeclareTextGlyphY{LinBiolinum_K}{uni2627}{9767}
\DeclareTextGlyphY{LinBiolinum_K}{uni262F}{9775}
\DeclareTextGlyphY{LinBiolinum_K}{uni2639}{9785}
\DeclareTextGlyphY{LinBiolinum_K}{uni263A}{9786}
\DeclareTextGlyphY{LinBiolinum_K}{uni263B}{9787}
\DeclareTextGlyphY{LinBiolinum_K}{uni263C}{9788}
\DeclareTextGlyphY{LinBiolinum_K}{uni263D}{9789}
\DeclareTextGlyphY{LinBiolinum_K}{uni263E}{9790}
\DeclareTextGlyphY{LinBiolinum_K}{uni263F}{9791}
\DeclareTextGlyphY{LinBiolinum_K}{female}{9792}
\DeclareTextGlyphY{LinBiolinum_K}{uni2640}{9792}
\DeclareTextGlyphY{LinBiolinum_K}{uni2641}{9793}
\DeclareTextGlyphY{LinBiolinum_K}{male}{9794}
\DeclareTextGlyphY{LinBiolinum_K}{uni2642}{9794}
\DeclareTextGlyphY{LinBiolinum_K}{uni2643}{9795}
\DeclareTextGlyphY{LinBiolinum_K}{uni2644}{9796}
\DeclareTextGlyphY{LinBiolinum_K}{uni2645}{9797}
\DeclareTextGlyphY{LinBiolinum_K}{uni2646}{9798}
\DeclareTextGlyphY{LinBiolinum_K}{uni2647}{9799}
\DeclareTextGlyphY{LinBiolinum_K}{uni2648}{9800}
\DeclareTextGlyphY{LinBiolinum_K}{uni2649}{9801}
\DeclareTextGlyphY{LinBiolinum_K}{uni264A}{9802}
\DeclareTextGlyphY{LinBiolinum_K}{uni264B}{9803}
\DeclareTextGlyphY{LinBiolinum_K}{uni264C}{9804}
\DeclareTextGlyphY{LinBiolinum_K}{uni264D}{9805}
\DeclareTextGlyphY{LinBiolinum_K}{uni264E}{9806}
\DeclareTextGlyphY{LinBiolinum_K}{uni264F}{9807}
\DeclareTextGlyphY{LinBiolinum_K}{uni2650}{9808}
\DeclareTextGlyphY{LinBiolinum_K}{uni2651}{9809}
\DeclareTextGlyphY{LinBiolinum_K}{uni2652}{9810}
\DeclareTextGlyphY{LinBiolinum_K}{uni2653}{9811}
\DeclareTextGlyphY{LinBiolinum_K}{uni2660}{9824}
\DeclareTextGlyphY{LinBiolinum_K}{uni2663}{9827}
\DeclareTextGlyphY{LinBiolinum_K}{uni2665}{9829}
\DeclareTextGlyphY{LinBiolinum_K}{uni2666}{9830}
\DeclareTextGlyphY{LinBiolinum_K}{uni2669}{9833}
\DeclareTextGlyphY{LinBiolinum_K}{musicalnote}{9834}
\DeclareTextGlyphY{LinBiolinum_K}{uni266A}{9834}
\DeclareTextGlyphY{LinBiolinum_K}{musicalnotedbl}{9835}
\DeclareTextGlyphY{LinBiolinum_K}{uni266B}{9835}
\DeclareTextGlyphY{LinBiolinum_K}{uni266C}{9836}
\DeclareTextGlyphY{LinBiolinum_K}{uni2695}{9877}
\DeclareTextGlyphY{LinBiolinum_K}{uni2698}{9880}
\DeclareTextGlyphY{LinBiolinum_K}{uni26A2}{9890}
\DeclareTextGlyphY{LinBiolinum_K}{uni26A3}{9891}
\DeclareTextGlyphY{LinBiolinum_K}{uni26A4}{9892}
\DeclareTextGlyphY{LinBiolinum_K}{uni26A5}{9893}
\DeclareTextGlyphY{LinBiolinum_K}{uni26AD}{9901}
\DeclareTextGlyphY{LinBiolinum_K}{uni2767}{10087}
\DeclareTextGlyphY{LinBiolinum_K}{uni2776}{10102}
\DeclareTextGlyphY{LinBiolinum_K}{uni2777}{10103}
\DeclareTextGlyphY{LinBiolinum_K}{uni2778}{10104}
\DeclareTextGlyphY{LinBiolinum_K}{uni2779}{10105}
\DeclareTextGlyphY{LinBiolinum_K}{uni277A}{10106}
\DeclareTextGlyphY{LinBiolinum_K}{uni277B}{10107}
\DeclareTextGlyphY{LinBiolinum_K}{uni277C}{10108}
\DeclareTextGlyphY{LinBiolinum_K}{uni277D}{10109}
\DeclareTextGlyphY{LinBiolinum_K}{uni277E}{10110}
\DeclareTextGlyphY{LinBiolinum_K}{uni277F}{10111}
\DeclareTextGlyphY{LinBiolinum_K}{T_u_x}{57344}
\DeclareTextGlyphY{LinBiolinum_K}{uniE000}{57344}
\DeclareTextGlyphY{LinBiolinum_K}{uniE104}{57604}
\DeclareTextGlyphY{LinBiolinum_K}{uniE128}{57640}
\DeclareTextGlyphY{LinBiolinum_K}{uniE129}{57641}
\DeclareTextGlyphY{LinBiolinum_K}{uniE12A}{57642}
\DeclareTextGlyphY{LinBiolinum_K}{uniE130}{57648}
\DeclareTextGlyphY{LinBiolinum_K}{uniE131}{57649}
\DeclareTextGlyphY{LinBiolinum_K}{uniE132}{57650}
\DeclareTextGlyphY{LinBiolinum_K}{uniE133}{57651}
\DeclareTextGlyphY{LinBiolinum_K}{uniE134}{57652}
\DeclareTextGlyphY{LinBiolinum_K}{uniE135}{57653}
\DeclareTextGlyphY{LinBiolinum_K}{uniE138}{57656}
\DeclareTextGlyphY{LinBiolinum_K}{uniE139}{57657}
\DeclareTextGlyphY{LinBiolinum_K}{uniE13A}{57658}
\DeclareTextGlyphY{LinBiolinum_K}{uniE13C}{57660}
\DeclareTextGlyphY{LinBiolinum_K}{uniE13D}{57661}
\DeclareTextGlyphY{LinBiolinum_K}{uniE168}{57704}
\DeclareTextGlyphY{LinBiolinum_K}{B_a_c_k}{57710}
\DeclareTextGlyphY{LinBiolinum_K}{uniE16E}{57710}
\DeclareTextGlyphY{LinBiolinum_K}{S_t_r_g}{57712}
\DeclareTextGlyphY{LinBiolinum_K}{uniE170}{57712}
\DeclareTextGlyphY{LinBiolinum_K}{A_l_t}{57713}
\DeclareTextGlyphY{LinBiolinum_K}{uniE171}{57713}
\DeclareTextGlyphY{LinBiolinum_K}{A_l_t_G_r}{57714}
\DeclareTextGlyphY{LinBiolinum_K}{uniE172}{57714}
\DeclareTextGlyphY{LinBiolinum_K}{C_t_r_l}{57715}
\DeclareTextGlyphY{LinBiolinum_K}{uniE173}{57715}
\DeclareTextGlyphY{LinBiolinum_K}{S_h_i_f_t}{57716}
\DeclareTextGlyphY{LinBiolinum_K}{uniE174}{57716}
\DeclareTextGlyphY{LinBiolinum_K}{T_a_b}{57717}
\DeclareTextGlyphY{LinBiolinum_K}{uniE175}{57717}
\DeclareTextGlyphY{LinBiolinum_K}{E_n_t_e_r}{57718}
\DeclareTextGlyphY{LinBiolinum_K}{uniE176}{57718}
\DeclareTextGlyphY{LinBiolinum_K}{C_a_p_s_l_o_c_k}{57719}
\DeclareTextGlyphY{LinBiolinum_K}{uniE177}{57719}
\DeclareTextGlyphY{LinBiolinum_K}{F_1}{57720}
\DeclareTextGlyphY{LinBiolinum_K}{uniE178}{57720}
\DeclareTextGlyphY{LinBiolinum_K}{F_2}{57721}
\DeclareTextGlyphY{LinBiolinum_K}{uniE179}{57721}
\DeclareTextGlyphY{LinBiolinum_K}{F_3}{57722}
\DeclareTextGlyphY{LinBiolinum_K}{uniE17A}{57722}
\DeclareTextGlyphY{LinBiolinum_K}{F_4}{57723}
\DeclareTextGlyphY{LinBiolinum_K}{uniE17B}{57723}
\DeclareTextGlyphY{LinBiolinum_K}{F_5}{57724}
\DeclareTextGlyphY{LinBiolinum_K}{uniE17C}{57724}
\DeclareTextGlyphY{LinBiolinum_K}{F_6}{57725}
\DeclareTextGlyphY{LinBiolinum_K}{uniE17D}{57725}
\DeclareTextGlyphY{LinBiolinum_K}{F_7}{57726}
\DeclareTextGlyphY{LinBiolinum_K}{uniE17E}{57726}
\DeclareTextGlyphY{LinBiolinum_K}{F_8}{57727}
\DeclareTextGlyphY{LinBiolinum_K}{uniE17F}{57727}
\DeclareTextGlyphY{LinBiolinum_K}{F_9}{57728}
\DeclareTextGlyphY{LinBiolinum_K}{uniE180}{57728}
\DeclareTextGlyphY{LinBiolinum_K}{F_1_0}{57729}
\DeclareTextGlyphY{LinBiolinum_K}{uniE181}{57729}
\DeclareTextGlyphY{LinBiolinum_K}{F_1_1}{57730}
\DeclareTextGlyphY{LinBiolinum_K}{uniE182}{57730}
\DeclareTextGlyphY{LinBiolinum_K}{F_1_2}{57731}
\DeclareTextGlyphY{LinBiolinum_K}{uniE183}{57731}
\DeclareTextGlyphY{LinBiolinum_K}{F_1_3}{57732}
\DeclareTextGlyphY{LinBiolinum_K}{uniE184}{57732}
\DeclareTextGlyphY{LinBiolinum_K}{F_1_4}{57733}
\DeclareTextGlyphY{LinBiolinum_K}{uniE185}{57733}
\DeclareTextGlyphY{LinBiolinum_K}{F_1_5}{57734}
\DeclareTextGlyphY{LinBiolinum_K}{uniE186}{57734}
\DeclareTextGlyphY{LinBiolinum_K}{F_1_6}{57735}
\DeclareTextGlyphY{LinBiolinum_K}{uniE187}{57735}
\DeclareTextGlyphY{LinBiolinum_K}{uniE188}{57736}
\DeclareTextGlyphY{LinBiolinum_K}{H_o_m_e}{57737}
\DeclareTextGlyphY{LinBiolinum_K}{uniE189}{57737}
\DeclareTextGlyphY{LinBiolinum_K}{D_e_l}{57738}
\DeclareTextGlyphY{LinBiolinum_K}{uniE18A}{57738}
\DeclareTextGlyphY{LinBiolinum_K}{I_n_s}{57739}
\DeclareTextGlyphY{LinBiolinum_K}{uniE18B}{57739}
\DeclareTextGlyphY{LinBiolinum_K}{uniE18C}{57740}
\DeclareTextGlyphY{LinBiolinum_K}{E_n_d}{57742}
\DeclareTextGlyphY{LinBiolinum_K}{uniE18E}{57742}
\DeclareTextGlyphY{LinBiolinum_K}{G_N_U}{57744}
\DeclareTextGlyphY{LinBiolinum_K}{uniE190}{57744}
\DeclareTextGlyphY{LinBiolinum_K}{P_o_s_1}{57745}
\DeclareTextGlyphY{LinBiolinum_K}{uniE191}{57745}
\DeclareTextGlyphY{LinBiolinum_K}{E_n_t_f}{57746}
\DeclareTextGlyphY{LinBiolinum_K}{uniE192}{57746}
\DeclareTextGlyphY{LinBiolinum_K}{E_i_n_f}{57747}
\DeclareTextGlyphY{LinBiolinum_K}{uniE193}{57747}
\DeclareTextGlyphY{LinBiolinum_K}{L_e_e_r}{57748}
\DeclareTextGlyphY{LinBiolinum_K}{uniE194}{57748}
\DeclareTextGlyphY{LinBiolinum_K}{E_s_c}{57749}
\DeclareTextGlyphY{LinBiolinum_K}{uniE195}{57749}
\DeclareTextGlyphY{LinBiolinum_K}{E_n_d_e}{57750}
\DeclareTextGlyphY{LinBiolinum_K}{uniE196}{57750}
\DeclareTextGlyphY{LinBiolinum_K}{uniE198}{57752}
\DeclareTextGlyphY{LinBiolinum_K}{uniE199}{57753}
\DeclareTextGlyphY{LinBiolinum_K}{uniE19A}{57754}
\DeclareTextGlyphY{LinBiolinum_K}{uniE19B}{57755}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A0}{57760}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A1}{57761}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A2}{57762}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A3}{57763}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A4}{57764}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A5}{57765}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A6}{57766}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A7}{57767}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A8}{57768}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1A9}{57769}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1AA}{57770}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1AB}{57771}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1AC}{57772}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1AD}{57773}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1AE}{57774}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1B0}{57776}
\DeclareTextGlyphY{LinBiolinum_K}{uniE1B1}{57777}
\DeclareTextGlyphY{LinBiolinum_K}{grave.cap}{58200}
\DeclareTextGlyphY{LinBiolinum_K}{uniE358}{58200}
\DeclareTextGlyphY{LinBiolinum_K}{acute.cap}{58201}
\DeclareTextGlyphY{LinBiolinum_K}{uniE359}{58201}
\DeclareTextGlyphY{LinBiolinum_K}{circumflex.cap}{58202}
\DeclareTextGlyphY{LinBiolinum_K}{uniE35A}{58202}
\DeclareTextGlyphY{LinBiolinum_K}{caron.cap}{58203}
\DeclareTextGlyphY{LinBiolinum_K}{uniE35B}{58203}
\DeclareTextGlyphY{LinBiolinum_K}{breve.cap}{58204}
\DeclareTextGlyphY{LinBiolinum_K}{uniE35C}{58204}
\DeclareTextGlyphY{LinBiolinum_K}{hungarumlaut.cap}{58205}
\DeclareTextGlyphY{LinBiolinum_K}{uniE35D}{58205}
\DeclareTextGlyphY{LinBiolinum_K}{space_uni030F.cap}{58206}
\DeclareTextGlyphY{LinBiolinum_K}{uniE35E}{58206}
\DeclareTextGlyphY{LinBiolinum_K}{breveinvertedcmb.cap}{58207}
\DeclareTextGlyphY{LinBiolinum_K}{uniE35F}{58207}
\DeclareTextGlyphY{LinBiolinum_K}{breve.cyrcap}{58208}
\DeclareTextGlyphY{LinBiolinum_K}{uniE360}{58208}
\DeclareTextGlyphY{LinBiolinum_K}{breve.cyr}{58209}
\DeclareTextGlyphY{LinBiolinum_K}{uniE361}{58209}
\DeclareTextGlyphY{LinBiolinum_K}{dieresis.cap}{58210}
\DeclareTextGlyphY{LinBiolinum_K}{uniE362}{58210}
\DeclareTextGlyphY{LinBiolinum_K}{hookabovecomb.cap}{58211}
\DeclareTextGlyphY{LinBiolinum_K}{uniE363}{58211}
\DeclareTextGlyphY{LinBiolinum_K}{uniFFFD}{65533}


==> LinBiolinum_R.tex <==
\DeclareTextGlyphY{LinBiolinum_R}{space}{32}
\DeclareTextGlyphY{LinBiolinum_R}{uni0020}{32}
\DeclareTextGlyphY{LinBiolinum_R}{exclam}{33}
\DeclareTextGlyphY{LinBiolinum_R}{uni0021}{33}
\DeclareTextGlyphY{LinBiolinum_R}{quotedbl}{34}
\DeclareTextGlyphY{LinBiolinum_R}{uni0022}{34}
\DeclareTextGlyphY{LinBiolinum_R}{numbersign}{35}
\DeclareTextGlyphY{LinBiolinum_R}{uni0023}{35}
\DeclareTextGlyphY{LinBiolinum_R}{dollar}{36}
\DeclareTextGlyphY{LinBiolinum_R}{uni0024}{36}
\DeclareTextGlyphY{LinBiolinum_R}{percent}{37}
\DeclareTextGlyphY{LinBiolinum_R}{uni0025}{37}
\DeclareTextGlyphY{LinBiolinum_R}{ampersand}{38}
\DeclareTextGlyphY{LinBiolinum_R}{uni0026}{38}
\DeclareTextGlyphY{LinBiolinum_R}{quotesingle}{39}
\DeclareTextGlyphY{LinBiolinum_R}{uni0027}{39}
\DeclareTextGlyphY{LinBiolinum_R}{parenleft}{40}
\DeclareTextGlyphY{LinBiolinum_R}{uni0028}{40}
\DeclareTextGlyphY{LinBiolinum_R}{parenright}{41}
\DeclareTextGlyphY{LinBiolinum_R}{uni0029}{41}
\DeclareTextGlyphY{LinBiolinum_R}{asterisk}{42}
\DeclareTextGlyphY{LinBiolinum_R}{uni002A}{42}
\DeclareTextGlyphY{LinBiolinum_R}{plus}{43}
\DeclareTextGlyphY{LinBiolinum_R}{uni002B}{43}
\DeclareTextGlyphY{LinBiolinum_R}{comma}{44}
\DeclareTextGlyphY{LinBiolinum_R}{uni002C}{44}
\DeclareTextGlyphY{LinBiolinum_R}{hyphen}{45}
\DeclareTextGlyphY{LinBiolinum_R}{uni002D}{45}
\DeclareTextGlyphY{LinBiolinum_R}{period}{46}
\DeclareTextGlyphY{LinBiolinum_R}{uni002E}{46}
\DeclareTextGlyphY{LinBiolinum_R}{slash}{47}
\DeclareTextGlyphY{LinBiolinum_R}{uni002F}{47}
\DeclareTextGlyphY{LinBiolinum_R}{zero}{48}
\DeclareTextGlyphY{LinBiolinum_R}{uni0030}{48}
\DeclareTextGlyphY{LinBiolinum_R}{one}{49}
\DeclareTextGlyphY{LinBiolinum_R}{uni0031}{49}
\DeclareTextGlyphY{LinBiolinum_R}{two}{50}
\DeclareTextGlyphY{LinBiolinum_R}{uni0032}{50}
\DeclareTextGlyphY{LinBiolinum_R}{three}{51}
\DeclareTextGlyphY{LinBiolinum_R}{uni0033}{51}
\DeclareTextGlyphY{LinBiolinum_R}{four}{52}
\DeclareTextGlyphY{LinBiolinum_R}{uni0034}{52}
\DeclareTextGlyphY{LinBiolinum_R}{five}{53}
\DeclareTextGlyphY{LinBiolinum_R}{uni0035}{53}
\DeclareTextGlyphY{LinBiolinum_R}{six}{54}
\DeclareTextGlyphY{LinBiolinum_R}{uni0036}{54}
\DeclareTextGlyphY{LinBiolinum_R}{seven}{55}
\DeclareTextGlyphY{LinBiolinum_R}{uni0037}{55}
\DeclareTextGlyphY{LinBiolinum_R}{eight}{56}
\DeclareTextGlyphY{LinBiolinum_R}{uni0038}{56}
\DeclareTextGlyphY{LinBiolinum_R}{nine}{57}
\DeclareTextGlyphY{LinBiolinum_R}{uni0039}{57}
\DeclareTextGlyphY{LinBiolinum_R}{colon}{58}
\DeclareTextGlyphY{LinBiolinum_R}{uni003A}{58}
\DeclareTextGlyphY{LinBiolinum_R}{semicolon}{59}
\DeclareTextGlyphY{LinBiolinum_R}{uni003B}{59}
\DeclareTextGlyphY{LinBiolinum_R}{less}{60}
\DeclareTextGlyphY{LinBiolinum_R}{uni003C}{60}
\DeclareTextGlyphY{LinBiolinum_R}{equal}{61}
\DeclareTextGlyphY{LinBiolinum_R}{uni003D}{61}
\DeclareTextGlyphY{LinBiolinum_R}{greater}{62}
\DeclareTextGlyphY{LinBiolinum_R}{uni003E}{62}
\DeclareTextGlyphY{LinBiolinum_R}{question}{63}
\DeclareTextGlyphY{LinBiolinum_R}{uni003F}{63}
\DeclareTextGlyphY{LinBiolinum_R}{at}{64}
\DeclareTextGlyphY{LinBiolinum_R}{uni0040}{64}
\DeclareTextGlyphY{LinBiolinum_R}{A}{65}
\DeclareTextGlyphY{LinBiolinum_R}{uni0041}{65}
\DeclareTextGlyphY{LinBiolinum_R}{B}{66}
\DeclareTextGlyphY{LinBiolinum_R}{uni0042}{66}
\DeclareTextGlyphY{LinBiolinum_R}{C}{67}
\DeclareTextGlyphY{LinBiolinum_R}{uni0043}{67}
\DeclareTextGlyphY{LinBiolinum_R}{D}{68}
\DeclareTextGlyphY{LinBiolinum_R}{uni0044}{68}
\DeclareTextGlyphY{LinBiolinum_R}{E}{69}
\DeclareTextGlyphY{LinBiolinum_R}{uni0045}{69}
\DeclareTextGlyphY{LinBiolinum_R}{F}{70}
\DeclareTextGlyphY{LinBiolinum_R}{uni0046}{70}
\DeclareTextGlyphY{LinBiolinum_R}{G}{71}
\DeclareTextGlyphY{LinBiolinum_R}{uni0047}{71}
\DeclareTextGlyphY{LinBiolinum_R}{H}{72}
\DeclareTextGlyphY{LinBiolinum_R}{uni0048}{72}
\DeclareTextGlyphY{LinBiolinum_R}{I}{73}
\DeclareTextGlyphY{LinBiolinum_R}{uni0049}{73}
\DeclareTextGlyphY{LinBiolinum_R}{J}{74}
\DeclareTextGlyphY{LinBiolinum_R}{uni004A}{74}
\DeclareTextGlyphY{LinBiolinum_R}{K}{75}
\DeclareTextGlyphY{LinBiolinum_R}{uni004B}{75}
\DeclareTextGlyphY{LinBiolinum_R}{L}{76}
\DeclareTextGlyphY{LinBiolinum_R}{uni004C}{76}
\DeclareTextGlyphY{LinBiolinum_R}{M}{77}
\DeclareTextGlyphY{LinBiolinum_R}{uni004D}{77}
\DeclareTextGlyphY{LinBiolinum_R}{N}{78}
\DeclareTextGlyphY{LinBiolinum_R}{uni004E}{78}
\DeclareTextGlyphY{LinBiolinum_R}{O}{79}
\DeclareTextGlyphY{LinBiolinum_R}{uni004F}{79}
\DeclareTextGlyphY{LinBiolinum_R}{P}{80}
\DeclareTextGlyphY{LinBiolinum_R}{uni0050}{80}
\DeclareTextGlyphY{LinBiolinum_R}{Q}{81}
\DeclareTextGlyphY{LinBiolinum_R}{uni0051}{81}
\DeclareTextGlyphY{LinBiolinum_R}{R}{82}
\DeclareTextGlyphY{LinBiolinum_R}{uni0052}{82}
\DeclareTextGlyphY{LinBiolinum_R}{S}{83}
\DeclareTextGlyphY{LinBiolinum_R}{uni0053}{83}
\DeclareTextGlyphY{LinBiolinum_R}{T}{84}
\DeclareTextGlyphY{LinBiolinum_R}{uni0054}{84}
\DeclareTextGlyphY{LinBiolinum_R}{U}{85}
\DeclareTextGlyphY{LinBiolinum_R}{uni0055}{85}
\DeclareTextGlyphY{LinBiolinum_R}{V}{86}
\DeclareTextGlyphY{LinBiolinum_R}{uni0056}{86}
\DeclareTextGlyphY{LinBiolinum_R}{W}{87}
\DeclareTextGlyphY{LinBiolinum_R}{uni0057}{87}
\DeclareTextGlyphY{LinBiolinum_R}{X}{88}
\DeclareTextGlyphY{LinBiolinum_R}{uni0058}{88}
\DeclareTextGlyphY{LinBiolinum_R}{Y}{89}
\DeclareTextGlyphY{LinBiolinum_R}{uni0059}{89}
\DeclareTextGlyphY{LinBiolinum_R}{Z}{90}
\DeclareTextGlyphY{LinBiolinum_R}{uni005A}{90}
\DeclareTextGlyphY{LinBiolinum_R}{bracketleft}{91}
\DeclareTextGlyphY{LinBiolinum_R}{uni005B}{91}
\DeclareTextGlyphY{LinBiolinum_R}{backslash}{92}
\DeclareTextGlyphY{LinBiolinum_R}{uni005C}{92}
\DeclareTextGlyphY{LinBiolinum_R}{bracketright}{93}
\DeclareTextGlyphY{LinBiolinum_R}{uni005D}{93}
\DeclareTextGlyphY{LinBiolinum_R}{asciicircum}{94}
\DeclareTextGlyphY{LinBiolinum_R}{uni005E}{94}
\DeclareTextGlyphY{LinBiolinum_R}{underscore}{95}
\DeclareTextGlyphY{LinBiolinum_R}{uni005F}{95}
\DeclareTextGlyphY{LinBiolinum_R}{grave}{96}
\DeclareTextGlyphY{LinBiolinum_R}{uni0060}{96}
\DeclareTextGlyphY{LinBiolinum_R}{a}{97}
\DeclareTextGlyphY{LinBiolinum_R}{uni0061}{97}
\DeclareTextGlyphY{LinBiolinum_R}{b}{98}
\DeclareTextGlyphY{LinBiolinum_R}{uni0062}{98}
\DeclareTextGlyphY{LinBiolinum_R}{c}{99}
\DeclareTextGlyphY{LinBiolinum_R}{uni0063}{99}
\DeclareTextGlyphY{LinBiolinum_R}{d}{100}
\DeclareTextGlyphY{LinBiolinum_R}{uni0064}{100}
\DeclareTextGlyphY{LinBiolinum_R}{e}{101}
\DeclareTextGlyphY{LinBiolinum_R}{uni0065}{101}
\DeclareTextGlyphY{LinBiolinum_R}{f}{102}
\DeclareTextGlyphY{LinBiolinum_R}{uni0066}{102}
\DeclareTextGlyphY{LinBiolinum_R}{g}{103}
\DeclareTextGlyphY{LinBiolinum_R}{uni0067}{103}
\DeclareTextGlyphY{LinBiolinum_R}{h}{104}
\DeclareTextGlyphY{LinBiolinum_R}{uni0068}{104}
\DeclareTextGlyphY{LinBiolinum_R}{i}{105}
\DeclareTextGlyphY{LinBiolinum_R}{uni0069}{105}
\DeclareTextGlyphY{LinBiolinum_R}{j}{106}
\DeclareTextGlyphY{LinBiolinum_R}{uni006A}{106}
\DeclareTextGlyphY{LinBiolinum_R}{k}{107}
\DeclareTextGlyphY{LinBiolinum_R}{uni006B}{107}
\DeclareTextGlyphY{LinBiolinum_R}{l}{108}
\DeclareTextGlyphY{LinBiolinum_R}{uni006C}{108}
\DeclareTextGlyphY{LinBiolinum_R}{m}{109}
\DeclareTextGlyphY{LinBiolinum_R}{uni006D}{109}
\DeclareTextGlyphY{LinBiolinum_R}{n}{110}
\DeclareTextGlyphY{LinBiolinum_R}{uni006E}{110}
\DeclareTextGlyphY{LinBiolinum_R}{o}{111}
\DeclareTextGlyphY{LinBiolinum_R}{uni006F}{111}
\DeclareTextGlyphY{LinBiolinum_R}{p}{112}
\DeclareTextGlyphY{LinBiolinum_R}{uni0070}{112}
\DeclareTextGlyphY{LinBiolinum_R}{q}{113}
\DeclareTextGlyphY{LinBiolinum_R}{uni0071}{113}
\DeclareTextGlyphY{LinBiolinum_R}{r}{114}
\DeclareTextGlyphY{LinBiolinum_R}{uni0072}{114}
\DeclareTextGlyphY{LinBiolinum_R}{s}{115}
\DeclareTextGlyphY{LinBiolinum_R}{uni0073}{115}
\DeclareTextGlyphY{LinBiolinum_R}{t}{116}
\DeclareTextGlyphY{LinBiolinum_R}{uni0074}{116}
\DeclareTextGlyphY{LinBiolinum_R}{u}{117}
\DeclareTextGlyphY{LinBiolinum_R}{uni0075}{117}
\DeclareTextGlyphY{LinBiolinum_R}{v}{118}
\DeclareTextGlyphY{LinBiolinum_R}{uni0076}{118}
\DeclareTextGlyphY{LinBiolinum_R}{w}{119}
\DeclareTextGlyphY{LinBiolinum_R}{uni0077}{119}
\DeclareTextGlyphY{LinBiolinum_R}{x}{120}
\DeclareTextGlyphY{LinBiolinum_R}{uni0078}{120}
\DeclareTextGlyphY{LinBiolinum_R}{y}{121}
\DeclareTextGlyphY{LinBiolinum_R}{uni0079}{121}
\DeclareTextGlyphY{LinBiolinum_R}{z}{122}
\DeclareTextGlyphY{LinBiolinum_R}{uni007A}{122}
\DeclareTextGlyphY{LinBiolinum_R}{braceleft}{123}
\DeclareTextGlyphY{LinBiolinum_R}{uni007B}{123}
\DeclareTextGlyphY{LinBiolinum_R}{bar}{124}
\DeclareTextGlyphY{LinBiolinum_R}{uni007C}{124}
\DeclareTextGlyphY{LinBiolinum_R}{braceright}{125}
\DeclareTextGlyphY{LinBiolinum_R}{uni007D}{125}
\DeclareTextGlyphY{LinBiolinum_R}{asciitilde}{126}
\DeclareTextGlyphY{LinBiolinum_R}{uni007E}{126}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A0}{160}
\DeclareTextGlyphY{LinBiolinum_R}{exclamdown}{161}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A1}{161}
\DeclareTextGlyphY{LinBiolinum_R}{cent}{162}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A2}{162}
\DeclareTextGlyphY{LinBiolinum_R}{sterling}{163}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A3}{163}
\DeclareTextGlyphY{LinBiolinum_R}{currency}{164}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A4}{164}
\DeclareTextGlyphY{LinBiolinum_R}{yen}{165}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A5}{165}
\DeclareTextGlyphY{LinBiolinum_R}{brokenbar}{166}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A6}{166}
\DeclareTextGlyphY{LinBiolinum_R}{section}{167}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A7}{167}
\DeclareTextGlyphY{LinBiolinum_R}{dieresis}{168}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A8}{168}
\DeclareTextGlyphY{LinBiolinum_R}{copyright}{169}
\DeclareTextGlyphY{LinBiolinum_R}{uni00A9}{169}
\DeclareTextGlyphY{LinBiolinum_R}{ordfeminine}{170}
\DeclareTextGlyphY{LinBiolinum_R}{uni00AA}{170}
\DeclareTextGlyphY{LinBiolinum_R}{guillemotleft}{171}
\DeclareTextGlyphY{LinBiolinum_R}{uni00AB}{171}
\DeclareTextGlyphY{LinBiolinum_R}{logicalnot}{172}
\DeclareTextGlyphY{LinBiolinum_R}{uni00AC}{172}
\DeclareTextGlyphY{LinBiolinum_R}{uni00AD}{173}
\DeclareTextGlyphY{LinBiolinum_R}{registered}{174}
\DeclareTextGlyphY{LinBiolinum_R}{uni00AE}{174}
\DeclareTextGlyphY{LinBiolinum_R}{macron}{175}
\DeclareTextGlyphY{LinBiolinum_R}{uni00AF}{175}
\DeclareTextGlyphY{LinBiolinum_R}{degree}{176}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B0}{176}
\DeclareTextGlyphY{LinBiolinum_R}{plusminus}{177}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B1}{177}
\DeclareTextGlyphY{LinBiolinum_R}{two.superior}{178}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B2}{178}
\DeclareTextGlyphY{LinBiolinum_R}{three.superior}{179}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B3}{179}
\DeclareTextGlyphY{LinBiolinum_R}{acute}{180}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B4}{180}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B5}{181}
\DeclareTextGlyphY{LinBiolinum_R}{paragraph}{182}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B6}{182}
\DeclareTextGlyphY{LinBiolinum_R}{periodcentered}{183}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B7}{183}
\DeclareTextGlyphY{LinBiolinum_R}{cedilla}{184}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B8}{184}
\DeclareTextGlyphY{LinBiolinum_R}{one.superior}{185}
\DeclareTextGlyphY{LinBiolinum_R}{uni00B9}{185}
\DeclareTextGlyphY{LinBiolinum_R}{ordmasculine}{186}
\DeclareTextGlyphY{LinBiolinum_R}{uni00BA}{186}
\DeclareTextGlyphY{LinBiolinum_R}{guillemotright}{187}
\DeclareTextGlyphY{LinBiolinum_R}{uni00BB}{187}
\DeclareTextGlyphY{LinBiolinum_R}{onequarter}{188}
\DeclareTextGlyphY{LinBiolinum_R}{uni00BC}{188}
\DeclareTextGlyphY{LinBiolinum_R}{onehalf}{189}
\DeclareTextGlyphY{LinBiolinum_R}{uni00BD}{189}
\DeclareTextGlyphY{LinBiolinum_R}{threequarters}{190}
\DeclareTextGlyphY{LinBiolinum_R}{uni00BE}{190}
\DeclareTextGlyphY{LinBiolinum_R}{questiondown}{191}
\DeclareTextGlyphY{LinBiolinum_R}{uni00BF}{191}
\DeclareTextGlyphY{LinBiolinum_R}{Agrave}{192}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C0}{192}
\DeclareTextGlyphY{LinBiolinum_R}{Aacute}{193}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C1}{193}
\DeclareTextGlyphY{LinBiolinum_R}{Acircumflex}{194}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C2}{194}
\DeclareTextGlyphY{LinBiolinum_R}{Atilde}{195}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C3}{195}
\DeclareTextGlyphY{LinBiolinum_R}{Adieresis}{196}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C4}{196}
\DeclareTextGlyphY{LinBiolinum_R}{Aring}{197}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C5}{197}
\DeclareTextGlyphY{LinBiolinum_R}{AE}{198}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C6}{198}
\DeclareTextGlyphY{LinBiolinum_R}{Ccedilla}{199}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C7}{199}
\DeclareTextGlyphY{LinBiolinum_R}{Egrave}{200}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C8}{200}
\DeclareTextGlyphY{LinBiolinum_R}{Eacute}{201}
\DeclareTextGlyphY{LinBiolinum_R}{uni00C9}{201}
\DeclareTextGlyphY{LinBiolinum_R}{Ecircumflex}{202}
\DeclareTextGlyphY{LinBiolinum_R}{uni00CA}{202}
\DeclareTextGlyphY{LinBiolinum_R}{Edieresis}{203}
\DeclareTextGlyphY{LinBiolinum_R}{uni00CB}{203}
\DeclareTextGlyphY{LinBiolinum_R}{Igrave}{204}
\DeclareTextGlyphY{LinBiolinum_R}{uni00CC}{204}
\DeclareTextGlyphY{LinBiolinum_R}{Iacute}{205}
\DeclareTextGlyphY{LinBiolinum_R}{uni00CD}{205}
\DeclareTextGlyphY{LinBiolinum_R}{Icircumflex}{206}
\DeclareTextGlyphY{LinBiolinum_R}{uni00CE}{206}
\DeclareTextGlyphY{LinBiolinum_R}{Idieresis}{207}
\DeclareTextGlyphY{LinBiolinum_R}{uni00CF}{207}
\DeclareTextGlyphY{LinBiolinum_R}{Eth}{208}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D0}{208}
\DeclareTextGlyphY{LinBiolinum_R}{Ntilde}{209}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D1}{209}
\DeclareTextGlyphY{LinBiolinum_R}{Ograve}{210}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D2}{210}
\DeclareTextGlyphY{LinBiolinum_R}{Oacute}{211}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D3}{211}
\DeclareTextGlyphY{LinBiolinum_R}{Ocircumflex}{212}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D4}{212}
\DeclareTextGlyphY{LinBiolinum_R}{Otilde}{213}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D5}{213}
\DeclareTextGlyphY{LinBiolinum_R}{Odieresis}{214}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D6}{214}
\DeclareTextGlyphY{LinBiolinum_R}{multiply}{215}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D7}{215}
\DeclareTextGlyphY{LinBiolinum_R}{Oslash}{216}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D8}{216}
\DeclareTextGlyphY{LinBiolinum_R}{Ugrave}{217}
\DeclareTextGlyphY{LinBiolinum_R}{uni00D9}{217}
\DeclareTextGlyphY{LinBiolinum_R}{Uacute}{218}
\DeclareTextGlyphY{LinBiolinum_R}{uni00DA}{218}
\DeclareTextGlyphY{LinBiolinum_R}{Ucircumflex}{219}
\DeclareTextGlyphY{LinBiolinum_R}{uni00DB}{219}
\DeclareTextGlyphY{LinBiolinum_R}{Udieresis}{220}
\DeclareTextGlyphY{LinBiolinum_R}{uni00DC}{220}
\DeclareTextGlyphY{LinBiolinum_R}{Yacute}{221}
\DeclareTextGlyphY{LinBiolinum_R}{uni00DD}{221}
\DeclareTextGlyphY{LinBiolinum_R}{Thorn}{222}
\DeclareTextGlyphY{LinBiolinum_R}{uni00DE}{222}
\DeclareTextGlyphY{LinBiolinum_R}{germandbls}{223}
\DeclareTextGlyphY{LinBiolinum_R}{uni00DF}{223}
\DeclareTextGlyphY{LinBiolinum_R}{agrave}{224}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E0}{224}
\DeclareTextGlyphY{LinBiolinum_R}{aacute}{225}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E1}{225}
\DeclareTextGlyphY{LinBiolinum_R}{acircumflex}{226}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E2}{226}
\DeclareTextGlyphY{LinBiolinum_R}{atilde}{227}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E3}{227}
\DeclareTextGlyphY{LinBiolinum_R}{adieresis}{228}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E4}{228}
\DeclareTextGlyphY{LinBiolinum_R}{aring}{229}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E5}{229}
\DeclareTextGlyphY{LinBiolinum_R}{ae}{230}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E6}{230}
\DeclareTextGlyphY{LinBiolinum_R}{ccedilla}{231}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E7}{231}
\DeclareTextGlyphY{LinBiolinum_R}{egrave}{232}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E8}{232}
\DeclareTextGlyphY{LinBiolinum_R}{eacute}{233}
\DeclareTextGlyphY{LinBiolinum_R}{uni00E9}{233}
\DeclareTextGlyphY{LinBiolinum_R}{ecircumflex}{234}
\DeclareTextGlyphY{LinBiolinum_R}{uni00EA}{234}
\DeclareTextGlyphY{LinBiolinum_R}{edieresis}{235}
\DeclareTextGlyphY{LinBiolinum_R}{uni00EB}{235}
\DeclareTextGlyphY{LinBiolinum_R}{igrave}{236}
\DeclareTextGlyphY{LinBiolinum_R}{uni00EC}{236}
\DeclareTextGlyphY{LinBiolinum_R}{iacute}{237}
\DeclareTextGlyphY{LinBiolinum_R}{uni00ED}{237}
\DeclareTextGlyphY{LinBiolinum_R}{icircumflex}{238}
\DeclareTextGlyphY{LinBiolinum_R}{uni00EE}{238}
\DeclareTextGlyphY{LinBiolinum_R}{idieresis}{239}
\DeclareTextGlyphY{LinBiolinum_R}{uni00EF}{239}
\DeclareTextGlyphY{LinBiolinum_R}{eth}{240}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F0}{240}
\DeclareTextGlyphY{LinBiolinum_R}{ntilde}{241}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F1}{241}
\DeclareTextGlyphY{LinBiolinum_R}{ograve}{242}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F2}{242}
\DeclareTextGlyphY{LinBiolinum_R}{oacute}{243}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F3}{243}
\DeclareTextGlyphY{LinBiolinum_R}{ocircumflex}{244}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F4}{244}
\DeclareTextGlyphY{LinBiolinum_R}{otilde}{245}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F5}{245}
\DeclareTextGlyphY{LinBiolinum_R}{odieresis}{246}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F6}{246}
\DeclareTextGlyphY{LinBiolinum_R}{divide}{247}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F7}{247}
\DeclareTextGlyphY{LinBiolinum_R}{oslash}{248}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F8}{248}
\DeclareTextGlyphY{LinBiolinum_R}{ugrave}{249}
\DeclareTextGlyphY{LinBiolinum_R}{uni00F9}{249}
\DeclareTextGlyphY{LinBiolinum_R}{uacute}{250}
\DeclareTextGlyphY{LinBiolinum_R}{uni00FA}{250}
\DeclareTextGlyphY{LinBiolinum_R}{ucircumflex}{251}
\DeclareTextGlyphY{LinBiolinum_R}{uni00FB}{251}
\DeclareTextGlyphY{LinBiolinum_R}{udieresis}{252}
\DeclareTextGlyphY{LinBiolinum_R}{uni00FC}{252}
\DeclareTextGlyphY{LinBiolinum_R}{yacute}{253}
\DeclareTextGlyphY{LinBiolinum_R}{uni00FD}{253}
\DeclareTextGlyphY{LinBiolinum_R}{thorn}{254}
\DeclareTextGlyphY{LinBiolinum_R}{uni00FE}{254}
\DeclareTextGlyphY{LinBiolinum_R}{ydieresis}{255}
\DeclareTextGlyphY{LinBiolinum_R}{uni00FF}{255}
\DeclareTextGlyphY{LinBiolinum_R}{Amacron}{256}
\DeclareTextGlyphY{LinBiolinum_R}{uni0100}{256}
\DeclareTextGlyphY{LinBiolinum_R}{amacron}{257}
\DeclareTextGlyphY{LinBiolinum_R}{uni0101}{257}
\DeclareTextGlyphY{LinBiolinum_R}{Abreve}{258}
\DeclareTextGlyphY{LinBiolinum_R}{uni0102}{258}
\DeclareTextGlyphY{LinBiolinum_R}{abreve}{259}
\DeclareTextGlyphY{LinBiolinum_R}{uni0103}{259}
\DeclareTextGlyphY{LinBiolinum_R}{Aogonek}{260}
\DeclareTextGlyphY{LinBiolinum_R}{uni0104}{260}
\DeclareTextGlyphY{LinBiolinum_R}{aogonek}{261}
\DeclareTextGlyphY{LinBiolinum_R}{uni0105}{261}
\DeclareTextGlyphY{LinBiolinum_R}{Cacute}{262}
\DeclareTextGlyphY{LinBiolinum_R}{uni0106}{262}
\DeclareTextGlyphY{LinBiolinum_R}{cacute}{263}
\DeclareTextGlyphY{LinBiolinum_R}{uni0107}{263}
\DeclareTextGlyphY{LinBiolinum_R}{Ccircumflex}{264}
\DeclareTextGlyphY{LinBiolinum_R}{uni0108}{264}
\DeclareTextGlyphY{LinBiolinum_R}{ccircumflex}{265}
\DeclareTextGlyphY{LinBiolinum_R}{uni0109}{265}
\DeclareTextGlyphY{LinBiolinum_R}{Cdotaccent}{266}
\DeclareTextGlyphY{LinBiolinum_R}{uni010A}{266}
\DeclareTextGlyphY{LinBiolinum_R}{cdotaccent}{267}
\DeclareTextGlyphY{LinBiolinum_R}{uni010B}{267}
\DeclareTextGlyphY{LinBiolinum_R}{Ccaron}{268}
\DeclareTextGlyphY{LinBiolinum_R}{uni010C}{268}
\DeclareTextGlyphY{LinBiolinum_R}{ccaron}{269}
\DeclareTextGlyphY{LinBiolinum_R}{uni010D}{269}
\DeclareTextGlyphY{LinBiolinum_R}{Dcaron}{270}
\DeclareTextGlyphY{LinBiolinum_R}{uni010E}{270}
\DeclareTextGlyphY{LinBiolinum_R}{dcaron}{271}
\DeclareTextGlyphY{LinBiolinum_R}{uni010F}{271}
\DeclareTextGlyphY{LinBiolinum_R}{Dcroat}{272}
\DeclareTextGlyphY{LinBiolinum_R}{uni0110}{272}
\DeclareTextGlyphY{LinBiolinum_R}{dcroat}{273}
\DeclareTextGlyphY{LinBiolinum_R}{uni0111}{273}
\DeclareTextGlyphY{LinBiolinum_R}{Emacron}{274}
\DeclareTextGlyphY{LinBiolinum_R}{uni0112}{274}
\DeclareTextGlyphY{LinBiolinum_R}{emacron}{275}
\DeclareTextGlyphY{LinBiolinum_R}{uni0113}{275}
\DeclareTextGlyphY{LinBiolinum_R}{Ebreve}{276}
\DeclareTextGlyphY{LinBiolinum_R}{uni0114}{276}
\DeclareTextGlyphY{LinBiolinum_R}{ebreve}{277}
\DeclareTextGlyphY{LinBiolinum_R}{uni0115}{277}
\DeclareTextGlyphY{LinBiolinum_R}{Edotaccent}{278}
\DeclareTextGlyphY{LinBiolinum_R}{uni0116}{278}
\DeclareTextGlyphY{LinBiolinum_R}{edotaccent}{279}
\DeclareTextGlyphY{LinBiolinum_R}{uni0117}{279}
\DeclareTextGlyphY{LinBiolinum_R}{Eogonek}{280}
\DeclareTextGlyphY{LinBiolinum_R}{uni0118}{280}
\DeclareTextGlyphY{LinBiolinum_R}{eogonek}{281}
\DeclareTextGlyphY{LinBiolinum_R}{uni0119}{281}
\DeclareTextGlyphY{LinBiolinum_R}{Ecaron}{282}
\DeclareTextGlyphY{LinBiolinum_R}{uni011A}{282}
\DeclareTextGlyphY{LinBiolinum_R}{ecaron}{283}
\DeclareTextGlyphY{LinBiolinum_R}{uni011B}{283}
\DeclareTextGlyphY{LinBiolinum_R}{Gcircumflex}{284}
\DeclareTextGlyphY{LinBiolinum_R}{uni011C}{284}
\DeclareTextGlyphY{LinBiolinum_R}{gcircumflex}{285}
\DeclareTextGlyphY{LinBiolinum_R}{uni011D}{285}
\DeclareTextGlyphY{LinBiolinum_R}{Gbreve}{286}
\DeclareTextGlyphY{LinBiolinum_R}{uni011E}{286}
\DeclareTextGlyphY{LinBiolinum_R}{gbreve}{287}
\DeclareTextGlyphY{LinBiolinum_R}{uni011F}{287}
\DeclareTextGlyphY{LinBiolinum_R}{Gdotaccent}{288}
\DeclareTextGlyphY{LinBiolinum_R}{uni0120}{288}
\DeclareTextGlyphY{LinBiolinum_R}{gdotaccent}{289}
\DeclareTextGlyphY{LinBiolinum_R}{uni0121}{289}
\DeclareTextGlyphY{LinBiolinum_R}{Gcommaaccent}{290}
\DeclareTextGlyphY{LinBiolinum_R}{uni0122}{290}
\DeclareTextGlyphY{LinBiolinum_R}{gcommaaccent}{291}
\DeclareTextGlyphY{LinBiolinum_R}{uni0123}{291}
\DeclareTextGlyphY{LinBiolinum_R}{Hcircumflex}{292}
\DeclareTextGlyphY{LinBiolinum_R}{uni0124}{292}
\DeclareTextGlyphY{LinBiolinum_R}{hcircumflex}{293}
\DeclareTextGlyphY{LinBiolinum_R}{uni0125}{293}
\DeclareTextGlyphY{LinBiolinum_R}{Hbar}{294}
\DeclareTextGlyphY{LinBiolinum_R}{uni0126}{294}
\DeclareTextGlyphY{LinBiolinum_R}{hbar}{295}
\DeclareTextGlyphY{LinBiolinum_R}{uni0127}{295}
\DeclareTextGlyphY{LinBiolinum_R}{Itilde}{296}
\DeclareTextGlyphY{LinBiolinum_R}{uni0128}{296}
\DeclareTextGlyphY{LinBiolinum_R}{itilde}{297}
\DeclareTextGlyphY{LinBiolinum_R}{uni0129}{297}
\DeclareTextGlyphY{LinBiolinum_R}{Imacron}{298}
\DeclareTextGlyphY{LinBiolinum_R}{uni012A}{298}
\DeclareTextGlyphY{LinBiolinum_R}{imacron}{299}
\DeclareTextGlyphY{LinBiolinum_R}{uni012B}{299}
\DeclareTextGlyphY{LinBiolinum_R}{Ibreve}{300}
\DeclareTextGlyphY{LinBiolinum_R}{uni012C}{300}
\DeclareTextGlyphY{LinBiolinum_R}{ibreve}{301}
\DeclareTextGlyphY{LinBiolinum_R}{uni012D}{301}
\DeclareTextGlyphY{LinBiolinum_R}{Iogonek}{302}
\DeclareTextGlyphY{LinBiolinum_R}{uni012E}{302}
\DeclareTextGlyphY{LinBiolinum_R}{iogonek}{303}
\DeclareTextGlyphY{LinBiolinum_R}{uni012F}{303}
\DeclareTextGlyphY{LinBiolinum_R}{Idotaccent}{304}
\DeclareTextGlyphY{LinBiolinum_R}{uni0130}{304}
\DeclareTextGlyphY{LinBiolinum_R}{dotlessi}{305}
\DeclareTextGlyphY{LinBiolinum_R}{uni0131}{305}
\DeclareTextGlyphY{LinBiolinum_R}{IJ}{306}
\DeclareTextGlyphY{LinBiolinum_R}{uni0132}{306}
\DeclareTextGlyphY{LinBiolinum_R}{ij}{307}
\DeclareTextGlyphY{LinBiolinum_R}{uni0133}{307}
\DeclareTextGlyphY{LinBiolinum_R}{Jcircumflex}{308}
\DeclareTextGlyphY{LinBiolinum_R}{uni0134}{308}
\DeclareTextGlyphY{LinBiolinum_R}{jcircumflex}{309}
\DeclareTextGlyphY{LinBiolinum_R}{uni0135}{309}
\DeclareTextGlyphY{LinBiolinum_R}{Kcommaaccent}{310}
\DeclareTextGlyphY{LinBiolinum_R}{uni0136}{310}
\DeclareTextGlyphY{LinBiolinum_R}{kcommaaccent}{311}
\DeclareTextGlyphY{LinBiolinum_R}{uni0137}{311}
\DeclareTextGlyphY{LinBiolinum_R}{kgreenlandic}{312}
\DeclareTextGlyphY{LinBiolinum_R}{uni0138}{312}
\DeclareTextGlyphY{LinBiolinum_R}{Lacute}{313}
\DeclareTextGlyphY{LinBiolinum_R}{uni0139}{313}
\DeclareTextGlyphY{LinBiolinum_R}{lacute}{314}
\DeclareTextGlyphY{LinBiolinum_R}{uni013A}{314}
\DeclareTextGlyphY{LinBiolinum_R}{Lcommaaccent}{315}
\DeclareTextGlyphY{LinBiolinum_R}{uni013B}{315}
\DeclareTextGlyphY{LinBiolinum_R}{lcommaaccent}{316}
\DeclareTextGlyphY{LinBiolinum_R}{uni013C}{316}
\DeclareTextGlyphY{LinBiolinum_R}{Lcaron}{317}
\DeclareTextGlyphY{LinBiolinum_R}{uni013D}{317}
\DeclareTextGlyphY{LinBiolinum_R}{lcaron}{318}
\DeclareTextGlyphY{LinBiolinum_R}{uni013E}{318}
\DeclareTextGlyphY{LinBiolinum_R}{Ldot}{319}
\DeclareTextGlyphY{LinBiolinum_R}{uni013F}{319}
\DeclareTextGlyphY{LinBiolinum_R}{ldot}{320}
\DeclareTextGlyphY{LinBiolinum_R}{uni0140}{320}
\DeclareTextGlyphY{LinBiolinum_R}{Lslash}{321}
\DeclareTextGlyphY{LinBiolinum_R}{uni0141}{321}
\DeclareTextGlyphY{LinBiolinum_R}{lslash}{322}
\DeclareTextGlyphY{LinBiolinum_R}{uni0142}{322}
\DeclareTextGlyphY{LinBiolinum_R}{Nacute}{323}
\DeclareTextGlyphY{LinBiolinum_R}{uni0143}{323}
\DeclareTextGlyphY{LinBiolinum_R}{nacute}{324}
\DeclareTextGlyphY{LinBiolinum_R}{uni0144}{324}
\DeclareTextGlyphY{LinBiolinum_R}{Ncommaaccent}{325}
\DeclareTextGlyphY{LinBiolinum_R}{uni0145}{325}
\DeclareTextGlyphY{LinBiolinum_R}{ncommaaccent}{326}
\DeclareTextGlyphY{LinBiolinum_R}{uni0146}{326}
\DeclareTextGlyphY{LinBiolinum_R}{Ncaron}{327}
\DeclareTextGlyphY{LinBiolinum_R}{uni0147}{327}
\DeclareTextGlyphY{LinBiolinum_R}{ncaron}{328}
\DeclareTextGlyphY{LinBiolinum_R}{uni0148}{328}
\DeclareTextGlyphY{LinBiolinum_R}{napostrophe}{329}
\DeclareTextGlyphY{LinBiolinum_R}{uni0149}{329}
\DeclareTextGlyphY{LinBiolinum_R}{Eng}{330}
\DeclareTextGlyphY{LinBiolinum_R}{uni014A}{330}
\DeclareTextGlyphY{LinBiolinum_R}{eng}{331}
\DeclareTextGlyphY{LinBiolinum_R}{uni014B}{331}
\DeclareTextGlyphY{LinBiolinum_R}{Omacron}{332}
\DeclareTextGlyphY{LinBiolinum_R}{uni014C}{332}
\DeclareTextGlyphY{LinBiolinum_R}{omacron}{333}
\DeclareTextGlyphY{LinBiolinum_R}{uni014D}{333}
\DeclareTextGlyphY{LinBiolinum_R}{Obreve}{334}
\DeclareTextGlyphY{LinBiolinum_R}{uni014E}{334}
\DeclareTextGlyphY{LinBiolinum_R}{obreve}{335}
\DeclareTextGlyphY{LinBiolinum_R}{uni014F}{335}
\DeclareTextGlyphY{LinBiolinum_R}{Ohungarumlaut}{336}
\DeclareTextGlyphY{LinBiolinum_R}{uni0150}{336}
\DeclareTextGlyphY{LinBiolinum_R}{ohungarumlaut}{337}
\DeclareTextGlyphY{LinBiolinum_R}{uni0151}{337}
\DeclareTextGlyphY{LinBiolinum_R}{OE}{338}
\DeclareTextGlyphY{LinBiolinum_R}{uni0152}{338}
\DeclareTextGlyphY{LinBiolinum_R}{oe}{339}
\DeclareTextGlyphY{LinBiolinum_R}{uni0153}{339}
\DeclareTextGlyphY{LinBiolinum_R}{Racute}{340}
\DeclareTextGlyphY{LinBiolinum_R}{uni0154}{340}
\DeclareTextGlyphY{LinBiolinum_R}{racute}{341}
\DeclareTextGlyphY{LinBiolinum_R}{uni0155}{341}
\DeclareTextGlyphY{LinBiolinum_R}{Rcommaaccent}{342}
\DeclareTextGlyphY{LinBiolinum_R}{uni0156}{342}
\DeclareTextGlyphY{LinBiolinum_R}{rcommaaccent}{343}
\DeclareTextGlyphY{LinBiolinum_R}{uni0157}{343}
\DeclareTextGlyphY{LinBiolinum_R}{Rcaron}{344}
\DeclareTextGlyphY{LinBiolinum_R}{uni0158}{344}
\DeclareTextGlyphY{LinBiolinum_R}{rcaron}{345}
\DeclareTextGlyphY{LinBiolinum_R}{uni0159}{345}
\DeclareTextGlyphY{LinBiolinum_R}{Sacute}{346}
\DeclareTextGlyphY{LinBiolinum_R}{uni015A}{346}
\DeclareTextGlyphY{LinBiolinum_R}{sacute}{347}
\DeclareTextGlyphY{LinBiolinum_R}{uni015B}{347}
\DeclareTextGlyphY{LinBiolinum_R}{Scircumflex}{348}
\DeclareTextGlyphY{LinBiolinum_R}{uni015C}{348}
\DeclareTextGlyphY{LinBiolinum_R}{scircumflex}{349}
\DeclareTextGlyphY{LinBiolinum_R}{uni015D}{349}
\DeclareTextGlyphY{LinBiolinum_R}{Scedilla}{350}
\DeclareTextGlyphY{LinBiolinum_R}{uni015E}{350}
\DeclareTextGlyphY{LinBiolinum_R}{scedilla}{351}
\DeclareTextGlyphY{LinBiolinum_R}{uni015F}{351}
\DeclareTextGlyphY{LinBiolinum_R}{Scaron}{352}
\DeclareTextGlyphY{LinBiolinum_R}{uni0160}{352}
\DeclareTextGlyphY{LinBiolinum_R}{scaron}{353}
\DeclareTextGlyphY{LinBiolinum_R}{uni0161}{353}
\DeclareTextGlyphY{LinBiolinum_R}{Tcedilla}{354}
\DeclareTextGlyphY{LinBiolinum_R}{uni0162}{354}
\DeclareTextGlyphY{LinBiolinum_R}{tcedilla}{355}
\DeclareTextGlyphY{LinBiolinum_R}{uni0163}{355}
\DeclareTextGlyphY{LinBiolinum_R}{Tcaron}{356}
\DeclareTextGlyphY{LinBiolinum_R}{uni0164}{356}
\DeclareTextGlyphY{LinBiolinum_R}{tcaron}{357}
\DeclareTextGlyphY{LinBiolinum_R}{uni0165}{357}
\DeclareTextGlyphY{LinBiolinum_R}{Tbar}{358}
\DeclareTextGlyphY{LinBiolinum_R}{uni0166}{358}
\DeclareTextGlyphY{LinBiolinum_R}{tbar}{359}
\DeclareTextGlyphY{LinBiolinum_R}{uni0167}{359}
\DeclareTextGlyphY{LinBiolinum_R}{Utilde}{360}
\DeclareTextGlyphY{LinBiolinum_R}{uni0168}{360}
\DeclareTextGlyphY{LinBiolinum_R}{utilde}{361}
\DeclareTextGlyphY{LinBiolinum_R}{uni0169}{361}
\DeclareTextGlyphY{LinBiolinum_R}{Umacron}{362}
\DeclareTextGlyphY{LinBiolinum_R}{uni016A}{362}
\DeclareTextGlyphY{LinBiolinum_R}{umacron}{363}
\DeclareTextGlyphY{LinBiolinum_R}{uni016B}{363}
\DeclareTextGlyphY{LinBiolinum_R}{Ubreve}{364}
\DeclareTextGlyphY{LinBiolinum_R}{uni016C}{364}
\DeclareTextGlyphY{LinBiolinum_R}{ubreve}{365}
\DeclareTextGlyphY{LinBiolinum_R}{uni016D}{365}
\DeclareTextGlyphY{LinBiolinum_R}{Uring}{366}
\DeclareTextGlyphY{LinBiolinum_R}{uni016E}{366}
\DeclareTextGlyphY{LinBiolinum_R}{uring}{367}
\DeclareTextGlyphY{LinBiolinum_R}{uni016F}{367}
\DeclareTextGlyphY{LinBiolinum_R}{Uhungarumlaut}{368}
\DeclareTextGlyphY{LinBiolinum_R}{uni0170}{368}
\DeclareTextGlyphY{LinBiolinum_R}{uhungarumlaut}{369}
\DeclareTextGlyphY{LinBiolinum_R}{uni0171}{369}
\DeclareTextGlyphY{LinBiolinum_R}{Uogonek}{370}
\DeclareTextGlyphY{LinBiolinum_R}{uni0172}{370}
\DeclareTextGlyphY{LinBiolinum_R}{uogonek}{371}
\DeclareTextGlyphY{LinBiolinum_R}{uni0173}{371}
\DeclareTextGlyphY{LinBiolinum_R}{Wcircumflex}{372}
\DeclareTextGlyphY{LinBiolinum_R}{uni0174}{372}
\DeclareTextGlyphY{LinBiolinum_R}{wcircumflex}{373}
\DeclareTextGlyphY{LinBiolinum_R}{uni0175}{373}
\DeclareTextGlyphY{LinBiolinum_R}{Ycircumflex}{374}
\DeclareTextGlyphY{LinBiolinum_R}{uni0176}{374}
\DeclareTextGlyphY{LinBiolinum_R}{ycircumflex}{375}
\DeclareTextGlyphY{LinBiolinum_R}{uni0177}{375}
\DeclareTextGlyphY{LinBiolinum_R}{Ydieresis}{376}
\DeclareTextGlyphY{LinBiolinum_R}{uni0178}{376}
\DeclareTextGlyphY{LinBiolinum_R}{Zacute}{377}
\DeclareTextGlyphY{LinBiolinum_R}{uni0179}{377}
\DeclareTextGlyphY{LinBiolinum_R}{zacute}{378}
\DeclareTextGlyphY{LinBiolinum_R}{uni017A}{378}
\DeclareTextGlyphY{LinBiolinum_R}{Zdotaccent}{379}
\DeclareTextGlyphY{LinBiolinum_R}{uni017B}{379}
\DeclareTextGlyphY{LinBiolinum_R}{zdotaccent}{380}
\DeclareTextGlyphY{LinBiolinum_R}{uni017C}{380}
\DeclareTextGlyphY{LinBiolinum_R}{Zcaron}{381}
\DeclareTextGlyphY{LinBiolinum_R}{uni017D}{381}
\DeclareTextGlyphY{LinBiolinum_R}{zcaron}{382}
\DeclareTextGlyphY{LinBiolinum_R}{uni017E}{382}
\DeclareTextGlyphY{LinBiolinum_R}{longs}{383}
\DeclareTextGlyphY{LinBiolinum_R}{uni017F}{383}
\DeclareTextGlyphY{LinBiolinum_R}{uni0180}{384}
\DeclareTextGlyphY{LinBiolinum_R}{uni0181}{385}
\DeclareTextGlyphY{LinBiolinum_R}{uni0182}{386}
\DeclareTextGlyphY{LinBiolinum_R}{uni0183}{387}
\DeclareTextGlyphY{LinBiolinum_R}{uni0184}{388}
\DeclareTextGlyphY{LinBiolinum_R}{uni0185}{389}
\DeclareTextGlyphY{LinBiolinum_R}{uni0186}{390}
\DeclareTextGlyphY{LinBiolinum_R}{uni0187}{391}
\DeclareTextGlyphY{LinBiolinum_R}{uni0188}{392}
\DeclareTextGlyphY{LinBiolinum_R}{uni0189}{393}
\DeclareTextGlyphY{LinBiolinum_R}{uni018A}{394}
\DeclareTextGlyphY{LinBiolinum_R}{uni018B}{395}
\DeclareTextGlyphY{LinBiolinum_R}{uni018C}{396}
\DeclareTextGlyphY{LinBiolinum_R}{uni018D}{397}
\DeclareTextGlyphY{LinBiolinum_R}{uni018E}{398}
\DeclareTextGlyphY{LinBiolinum_R}{uni018F}{399}
\DeclareTextGlyphY{LinBiolinum_R}{uni0190}{400}
\DeclareTextGlyphY{LinBiolinum_R}{uni0191}{401}
\DeclareTextGlyphY{LinBiolinum_R}{florin}{402}
\DeclareTextGlyphY{LinBiolinum_R}{uni0192}{402}
\DeclareTextGlyphY{LinBiolinum_R}{uni0193}{403}
\DeclareTextGlyphY{LinBiolinum_R}{uni0194}{404}
\DeclareTextGlyphY{LinBiolinum_R}{uni0195}{405}
\DeclareTextGlyphY{LinBiolinum_R}{uni0196}{406}
\DeclareTextGlyphY{LinBiolinum_R}{uni0197}{407}
\DeclareTextGlyphY{LinBiolinum_R}{uni0198}{408}
\DeclareTextGlyphY{LinBiolinum_R}{uni0199}{409}
\DeclareTextGlyphY{LinBiolinum_R}{uni019A}{410}
\DeclareTextGlyphY{LinBiolinum_R}{uni019B}{411}
\DeclareTextGlyphY{LinBiolinum_R}{uni019C}{412}
\DeclareTextGlyphY{LinBiolinum_R}{uni019D}{413}
\DeclareTextGlyphY{LinBiolinum_R}{uni019E}{414}
\DeclareTextGlyphY{LinBiolinum_R}{uni019F}{415}
\DeclareTextGlyphY{LinBiolinum_R}{Ohorn}{416}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A0}{416}
\DeclareTextGlyphY{LinBiolinum_R}{ohorn}{417}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A1}{417}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A2}{418}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A3}{419}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A4}{420}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A5}{421}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A6}{422}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A7}{423}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A8}{424}
\DeclareTextGlyphY{LinBiolinum_R}{uni01A9}{425}
\DeclareTextGlyphY{LinBiolinum_R}{uni01AA}{426}
\DeclareTextGlyphY{LinBiolinum_R}{uni01AB}{427}
\DeclareTextGlyphY{LinBiolinum_R}{uni01AC}{428}
\DeclareTextGlyphY{LinBiolinum_R}{uni01AD}{429}
\DeclareTextGlyphY{LinBiolinum_R}{uni01AE}{430}
\DeclareTextGlyphY{LinBiolinum_R}{Uhorn}{431}
\DeclareTextGlyphY{LinBiolinum_R}{uni01AF}{431}
\DeclareTextGlyphY{LinBiolinum_R}{uhorn}{432}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B0}{432}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B1}{433}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B2}{434}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B3}{435}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B4}{436}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B5}{437}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B6}{438}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B7}{439}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B8}{440}
\DeclareTextGlyphY{LinBiolinum_R}{uni01B9}{441}
\DeclareTextGlyphY{LinBiolinum_R}{uni01BA}{442}
\DeclareTextGlyphY{LinBiolinum_R}{uni01BB}{443}
\DeclareTextGlyphY{LinBiolinum_R}{uni01BC}{444}
\DeclareTextGlyphY{LinBiolinum_R}{uni01BD}{445}
\DeclareTextGlyphY{LinBiolinum_R}{uni01BE}{446}
\DeclareTextGlyphY{LinBiolinum_R}{uni01BF}{447}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C0}{448}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C1}{449}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C2}{450}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C3}{451}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C4}{452}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C5}{453}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C6}{454}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C7}{455}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C8}{456}
\DeclareTextGlyphY{LinBiolinum_R}{uni01C9}{457}
\DeclareTextGlyphY{LinBiolinum_R}{uni01CA}{458}
\DeclareTextGlyphY{LinBiolinum_R}{uni01CB}{459}
\DeclareTextGlyphY{LinBiolinum_R}{uni01CC}{460}
\DeclareTextGlyphY{LinBiolinum_R}{uni01CD}{461}
\DeclareTextGlyphY{LinBiolinum_R}{uni01CE}{462}
\DeclareTextGlyphY{LinBiolinum_R}{uni01CF}{463}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D0}{464}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D1}{465}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D2}{466}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D3}{467}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D4}{468}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D5}{469}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D6}{470}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D7}{471}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D8}{472}
\DeclareTextGlyphY{LinBiolinum_R}{uni01D9}{473}
\DeclareTextGlyphY{LinBiolinum_R}{uni01DA}{474}
\DeclareTextGlyphY{LinBiolinum_R}{uni01DB}{475}
\DeclareTextGlyphY{LinBiolinum_R}{uni01DC}{476}
\DeclareTextGlyphY{LinBiolinum_R}{uni01DD}{477}
\DeclareTextGlyphY{LinBiolinum_R}{uni01DE}{478}
\DeclareTextGlyphY{LinBiolinum_R}{uni01DF}{479}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E0}{480}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E1}{481}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E2}{482}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E3}{483}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E4}{484}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E5}{485}
\DeclareTextGlyphY{LinBiolinum_R}{Gcaron}{486}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E6}{486}
\DeclareTextGlyphY{LinBiolinum_R}{gcaron}{487}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E7}{487}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E8}{488}
\DeclareTextGlyphY{LinBiolinum_R}{uni01E9}{489}
\DeclareTextGlyphY{LinBiolinum_R}{uni01EA}{490}
\DeclareTextGlyphY{LinBiolinum_R}{uni01EB}{491}
\DeclareTextGlyphY{LinBiolinum_R}{uni01EC}{492}
\DeclareTextGlyphY{LinBiolinum_R}{uni01ED}{493}
\DeclareTextGlyphY{LinBiolinum_R}{uni01EE}{494}
\DeclareTextGlyphY{LinBiolinum_R}{uni01EF}{495}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F0}{496}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F1}{497}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F2}{498}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F3}{499}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F4}{500}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F5}{501}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F6}{502}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F7}{503}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F8}{504}
\DeclareTextGlyphY{LinBiolinum_R}{uni01F9}{505}
\DeclareTextGlyphY{LinBiolinum_R}{Aringacute}{506}
\DeclareTextGlyphY{LinBiolinum_R}{uni01FA}{506}
\DeclareTextGlyphY{LinBiolinum_R}{aringacute}{507}
\DeclareTextGlyphY{LinBiolinum_R}{uni01FB}{507}
\DeclareTextGlyphY{LinBiolinum_R}{AEacute}{508}
\DeclareTextGlyphY{LinBiolinum_R}{uni01FC}{508}
\DeclareTextGlyphY{LinBiolinum_R}{aeacute}{509}
\DeclareTextGlyphY{LinBiolinum_R}{uni01FD}{509}
\DeclareTextGlyphY{LinBiolinum_R}{Oslashacute}{510}
\DeclareTextGlyphY{LinBiolinum_R}{uni01FE}{510}
\DeclareTextGlyphY{LinBiolinum_R}{oslashacute}{511}
\DeclareTextGlyphY{LinBiolinum_R}{uni01FF}{511}
\DeclareTextGlyphY{LinBiolinum_R}{uni0200}{512}
\DeclareTextGlyphY{LinBiolinum_R}{uni0201}{513}
\DeclareTextGlyphY{LinBiolinum_R}{uni0202}{514}
\DeclareTextGlyphY{LinBiolinum_R}{uni0203}{515}
\DeclareTextGlyphY{LinBiolinum_R}{uni0204}{516}
\DeclareTextGlyphY{LinBiolinum_R}{uni0205}{517}
\DeclareTextGlyphY{LinBiolinum_R}{uni0206}{518}
\DeclareTextGlyphY{LinBiolinum_R}{uni0207}{519}
\DeclareTextGlyphY{LinBiolinum_R}{uni0208}{520}
\DeclareTextGlyphY{LinBiolinum_R}{uni0209}{521}
\DeclareTextGlyphY{LinBiolinum_R}{uni020A}{522}
\DeclareTextGlyphY{LinBiolinum_R}{uni020B}{523}
\DeclareTextGlyphY{LinBiolinum_R}{uni020C}{524}
\DeclareTextGlyphY{LinBiolinum_R}{uni020D}{525}
\DeclareTextGlyphY{LinBiolinum_R}{uni020E}{526}
\DeclareTextGlyphY{LinBiolinum_R}{uni020F}{527}
\DeclareTextGlyphY{LinBiolinum_R}{uni0210}{528}
\DeclareTextGlyphY{LinBiolinum_R}{uni0211}{529}
\DeclareTextGlyphY{LinBiolinum_R}{uni0212}{530}
\DeclareTextGlyphY{LinBiolinum_R}{uni0213}{531}
\DeclareTextGlyphY{LinBiolinum_R}{uni0214}{532}
\DeclareTextGlyphY{LinBiolinum_R}{uni0215}{533}
\DeclareTextGlyphY{LinBiolinum_R}{uni0216}{534}
\DeclareTextGlyphY{LinBiolinum_R}{uni0217}{535}
\DeclareTextGlyphY{LinBiolinum_R}{Scommaaccent}{536}
\DeclareTextGlyphY{LinBiolinum_R}{uni0218}{536}
\DeclareTextGlyphY{LinBiolinum_R}{scommaaccent}{537}
\DeclareTextGlyphY{LinBiolinum_R}{uni0219}{537}
\DeclareTextGlyphY{LinBiolinum_R}{Tcommaaccent}{538}
\DeclareTextGlyphY{LinBiolinum_R}{uni021A}{538}
\DeclareTextGlyphY{LinBiolinum_R}{tcommaaccent}{539}
\DeclareTextGlyphY{LinBiolinum_R}{uni021B}{539}
\DeclareTextGlyphY{LinBiolinum_R}{uni021C}{540}
\DeclareTextGlyphY{LinBiolinum_R}{uni021D}{541}
\DeclareTextGlyphY{LinBiolinum_R}{uni021E}{542}
\DeclareTextGlyphY{LinBiolinum_R}{uni021F}{543}
\DeclareTextGlyphY{LinBiolinum_R}{uni0220}{544}
\DeclareTextGlyphY{LinBiolinum_R}{uni0221}{545}
\DeclareTextGlyphY{LinBiolinum_R}{uni0222}{546}
\DeclareTextGlyphY{LinBiolinum_R}{uni0223}{547}
\DeclareTextGlyphY{LinBiolinum_R}{uni0224}{548}
\DeclareTextGlyphY{LinBiolinum_R}{uni0225}{549}
\DeclareTextGlyphY{LinBiolinum_R}{uni0226}{550}
\DeclareTextGlyphY{LinBiolinum_R}{uni0227}{551}
\DeclareTextGlyphY{LinBiolinum_R}{uni0228}{552}
\DeclareTextGlyphY{LinBiolinum_R}{uni0229}{553}
\DeclareTextGlyphY{LinBiolinum_R}{uni022A}{554}
\DeclareTextGlyphY{LinBiolinum_R}{uni022B}{555}
\DeclareTextGlyphY{LinBiolinum_R}{uni022C}{556}
\DeclareTextGlyphY{LinBiolinum_R}{uni022D}{557}
\DeclareTextGlyphY{LinBiolinum_R}{uni022E}{558}
\DeclareTextGlyphY{LinBiolinum_R}{uni022F}{559}
\DeclareTextGlyphY{LinBiolinum_R}{uni0230}{560}
\DeclareTextGlyphY{LinBiolinum_R}{uni0231}{561}
\DeclareTextGlyphY{LinBiolinum_R}{uni0232}{562}
\DeclareTextGlyphY{LinBiolinum_R}{uni0233}{563}
\DeclareTextGlyphY{LinBiolinum_R}{uni0234}{564}
\DeclareTextGlyphY{LinBiolinum_R}{uni0235}{565}
\DeclareTextGlyphY{LinBiolinum_R}{uni0236}{566}
\DeclareTextGlyphY{LinBiolinum_R}{dotlessj}{567}
\DeclareTextGlyphY{LinBiolinum_R}{uni0237}{567}
\DeclareTextGlyphY{LinBiolinum_R}{uni0238}{568}
\DeclareTextGlyphY{LinBiolinum_R}{uni0239}{569}
\DeclareTextGlyphY{LinBiolinum_R}{uni023A}{570}
\DeclareTextGlyphY{LinBiolinum_R}{uni023B}{571}
\DeclareTextGlyphY{LinBiolinum_R}{uni023C}{572}
\DeclareTextGlyphY{LinBiolinum_R}{uni023D}{573}
\DeclareTextGlyphY{LinBiolinum_R}{uni023E}{574}
\DeclareTextGlyphY{LinBiolinum_R}{uni023F}{575}
\DeclareTextGlyphY{LinBiolinum_R}{uni0241}{577}
\DeclareTextGlyphY{LinBiolinum_R}{uni0243}{579}
\DeclareTextGlyphY{LinBiolinum_R}{uni0250}{592}
\DeclareTextGlyphY{LinBiolinum_R}{uni0251}{593}
\DeclareTextGlyphY{LinBiolinum_R}{uni0252}{594}
\DeclareTextGlyphY{LinBiolinum_R}{uni0253}{595}
\DeclareTextGlyphY{LinBiolinum_R}{uni0254}{596}
\DeclareTextGlyphY{LinBiolinum_R}{uni0255}{597}
\DeclareTextGlyphY{LinBiolinum_R}{uni0256}{598}
\DeclareTextGlyphY{LinBiolinum_R}{uni0257}{599}
\DeclareTextGlyphY{LinBiolinum_R}{uni0258}{600}
\DeclareTextGlyphY{LinBiolinum_R}{uni0259}{601}
\DeclareTextGlyphY{LinBiolinum_R}{uni025A}{602}
\DeclareTextGlyphY{LinBiolinum_R}{uni025B}{603}
\DeclareTextGlyphY{LinBiolinum_R}{uni025C}{604}
\DeclareTextGlyphY{LinBiolinum_R}{uni025D}{605}
\DeclareTextGlyphY{LinBiolinum_R}{uni025E}{606}
\DeclareTextGlyphY{LinBiolinum_R}{uni025F}{607}
\DeclareTextGlyphY{LinBiolinum_R}{uni0260}{608}
\DeclareTextGlyphY{LinBiolinum_R}{uni0261}{609}
\DeclareTextGlyphY{LinBiolinum_R}{uni0262}{610}
\DeclareTextGlyphY{LinBiolinum_R}{gammalatin}{611}
\DeclareTextGlyphY{LinBiolinum_R}{uni0263}{611}
\DeclareTextGlyphY{LinBiolinum_R}{uni0264}{612}
\DeclareTextGlyphY{LinBiolinum_R}{uni0265}{613}
\DeclareTextGlyphY{LinBiolinum_R}{hhook}{614}
\DeclareTextGlyphY{LinBiolinum_R}{uni0266}{614}
\DeclareTextGlyphY{LinBiolinum_R}{uni0267}{615}
\DeclareTextGlyphY{LinBiolinum_R}{uni0268}{616}
\DeclareTextGlyphY{LinBiolinum_R}{uni0269}{617}
\DeclareTextGlyphY{LinBiolinum_R}{uni026A}{618}
\DeclareTextGlyphY{LinBiolinum_R}{uni026B}{619}
\DeclareTextGlyphY{LinBiolinum_R}{uni026C}{620}
\DeclareTextGlyphY{LinBiolinum_R}{uni026D}{621}
\DeclareTextGlyphY{LinBiolinum_R}{uni026E}{622}
\DeclareTextGlyphY{LinBiolinum_R}{uni026F}{623}
\DeclareTextGlyphY{LinBiolinum_R}{uni0270}{624}
\DeclareTextGlyphY{LinBiolinum_R}{uni0271}{625}
\DeclareTextGlyphY{LinBiolinum_R}{uni0272}{626}
\DeclareTextGlyphY{LinBiolinum_R}{uni0273}{627}
\DeclareTextGlyphY{LinBiolinum_R}{uni0274}{628}
\DeclareTextGlyphY{LinBiolinum_R}{uni0275}{629}
\DeclareTextGlyphY{LinBiolinum_R}{uni0276}{630}
\DeclareTextGlyphY{LinBiolinum_R}{uni0277}{631}
\DeclareTextGlyphY{LinBiolinum_R}{uni0278}{632}
\DeclareTextGlyphY{LinBiolinum_R}{rturned}{633}
\DeclareTextGlyphY{LinBiolinum_R}{uni0279}{633}
\DeclareTextGlyphY{LinBiolinum_R}{uni027A}{634}
\DeclareTextGlyphY{LinBiolinum_R}{rhookturned}{635}
\DeclareTextGlyphY{LinBiolinum_R}{uni027B}{635}
\DeclareTextGlyphY{LinBiolinum_R}{uni027C}{636}
\DeclareTextGlyphY{LinBiolinum_R}{uni027D}{637}
\DeclareTextGlyphY{LinBiolinum_R}{uni027E}{638}
\DeclareTextGlyphY{LinBiolinum_R}{uni027F}{639}
\DeclareTextGlyphY{LinBiolinum_R}{Rsmallcap}{640}
\DeclareTextGlyphY{LinBiolinum_R}{uni0280}{640}
\DeclareTextGlyphY{LinBiolinum_R}{Rsmallinverted}{641}
\DeclareTextGlyphY{LinBiolinum_R}{uni0281}{641}
\DeclareTextGlyphY{LinBiolinum_R}{uni0282}{642}
\DeclareTextGlyphY{LinBiolinum_R}{uni0283}{643}
\DeclareTextGlyphY{LinBiolinum_R}{uni0284}{644}
\DeclareTextGlyphY{LinBiolinum_R}{uni0285}{645}
\DeclareTextGlyphY{LinBiolinum_R}{uni0286}{646}
\DeclareTextGlyphY{LinBiolinum_R}{uni0287}{647}
\DeclareTextGlyphY{LinBiolinum_R}{uni0288}{648}
\DeclareTextGlyphY{LinBiolinum_R}{uni0289}{649}
\DeclareTextGlyphY{LinBiolinum_R}{uni028A}{650}
\DeclareTextGlyphY{LinBiolinum_R}{uni028B}{651}
\DeclareTextGlyphY{LinBiolinum_R}{uni028C}{652}
\DeclareTextGlyphY{LinBiolinum_R}{uni028D}{653}
\DeclareTextGlyphY{LinBiolinum_R}{uni028E}{654}
\DeclareTextGlyphY{LinBiolinum_R}{uni028F}{655}
\DeclareTextGlyphY{LinBiolinum_R}{uni0290}{656}
\DeclareTextGlyphY{LinBiolinum_R}{uni0291}{657}
\DeclareTextGlyphY{LinBiolinum_R}{uni0292}{658}
\DeclareTextGlyphY{LinBiolinum_R}{uni0293}{659}
\DeclareTextGlyphY{LinBiolinum_R}{uni0294}{660}
\DeclareTextGlyphY{LinBiolinum_R}{glottalstopreversed}{661}
\DeclareTextGlyphY{LinBiolinum_R}{uni0295}{661}
\DeclareTextGlyphY{LinBiolinum_R}{uni0296}{662}
\DeclareTextGlyphY{LinBiolinum_R}{uni0297}{663}
\DeclareTextGlyphY{LinBiolinum_R}{uni0298}{664}
\DeclareTextGlyphY{LinBiolinum_R}{uni0299}{665}
\DeclareTextGlyphY{LinBiolinum_R}{uni029A}{666}
\DeclareTextGlyphY{LinBiolinum_R}{uni029B}{667}
\DeclareTextGlyphY{LinBiolinum_R}{uni029C}{668}
\DeclareTextGlyphY{LinBiolinum_R}{uni029D}{669}
\DeclareTextGlyphY{LinBiolinum_R}{uni029E}{670}
\DeclareTextGlyphY{LinBiolinum_R}{uni029F}{671}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A0}{672}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A1}{673}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A2}{674}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A3}{675}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A4}{676}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A5}{677}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A6}{678}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A7}{679}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A8}{680}
\DeclareTextGlyphY{LinBiolinum_R}{uni02A9}{681}
\DeclareTextGlyphY{LinBiolinum_R}{uni02AA}{682}
\DeclareTextGlyphY{LinBiolinum_R}{uni02AB}{683}
\DeclareTextGlyphY{LinBiolinum_R}{uni02AC}{684}
\DeclareTextGlyphY{LinBiolinum_R}{uni02AD}{685}
\DeclareTextGlyphY{LinBiolinum_R}{uni02AE}{686}
\DeclareTextGlyphY{LinBiolinum_R}{uni02AF}{687}
\DeclareTextGlyphY{LinBiolinum_R}{h.superior}{688}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B0}{688}
\DeclareTextGlyphY{LinBiolinum_R}{hhook.superior}{689}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B1}{689}
\DeclareTextGlyphY{LinBiolinum_R}{j.superior}{690}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B2}{690}
\DeclareTextGlyphY{LinBiolinum_R}{r.superior}{691}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B3}{691}
\DeclareTextGlyphY{LinBiolinum_R}{rturned.superior}{692}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B4}{692}
\DeclareTextGlyphY{LinBiolinum_R}{rhookturned.superior}{693}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B5}{693}
\DeclareTextGlyphY{LinBiolinum_R}{Rsmallinverted.superior}{694}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B6}{694}
\DeclareTextGlyphY{LinBiolinum_R}{w.superior}{695}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B7}{695}
\DeclareTextGlyphY{LinBiolinum_R}{y.superior}{696}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B8}{696}
\DeclareTextGlyphY{LinBiolinum_R}{uni02B9}{697}
\DeclareTextGlyphY{LinBiolinum_R}{uni02BA}{698}
\DeclareTextGlyphY{LinBiolinum_R}{uni02BB}{699}
\DeclareTextGlyphY{LinBiolinum_R}{afii57929}{700}
\DeclareTextGlyphY{LinBiolinum_R}{uni02BC}{700}
\DeclareTextGlyphY{LinBiolinum_R}{afii64937}{701}
\DeclareTextGlyphY{LinBiolinum_R}{uni02BD}{701}
\DeclareTextGlyphY{LinBiolinum_R}{uni02BE}{702}
\DeclareTextGlyphY{LinBiolinum_R}{uni02BF}{703}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C0}{704}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C1}{705}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C2}{706}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C3}{707}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C4}{708}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C5}{709}
\DeclareTextGlyphY{LinBiolinum_R}{circumflex}{710}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C6}{710}
\DeclareTextGlyphY{LinBiolinum_R}{caron}{711}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C7}{711}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C8}{712}
\DeclareTextGlyphY{LinBiolinum_R}{uni02C9}{713}
\DeclareTextGlyphY{LinBiolinum_R}{uni02CA}{714}
\DeclareTextGlyphY{LinBiolinum_R}{uni02CB}{715}
\DeclareTextGlyphY{LinBiolinum_R}{uni02CC}{716}
\DeclareTextGlyphY{LinBiolinum_R}{uni02CD}{717}
\DeclareTextGlyphY{LinBiolinum_R}{uni02CE}{718}
\DeclareTextGlyphY{LinBiolinum_R}{uni02CF}{719}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D0}{720}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D1}{721}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D2}{722}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D3}{723}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D4}{724}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D5}{725}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D6}{726}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D7}{727}
\DeclareTextGlyphY{LinBiolinum_R}{breve}{728}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D8}{728}
\DeclareTextGlyphY{LinBiolinum_R}{dotaccent}{729}
\DeclareTextGlyphY{LinBiolinum_R}{uni02D9}{729}
\DeclareTextGlyphY{LinBiolinum_R}{ring}{730}
\DeclareTextGlyphY{LinBiolinum_R}{uni02DA}{730}
\DeclareTextGlyphY{LinBiolinum_R}{ogonek}{731}
\DeclareTextGlyphY{LinBiolinum_R}{uni02DB}{731}
\DeclareTextGlyphY{LinBiolinum_R}{tilde}{732}
\DeclareTextGlyphY{LinBiolinum_R}{uni02DC}{732}
\DeclareTextGlyphY{LinBiolinum_R}{hungarumlaut}{733}
\DeclareTextGlyphY{LinBiolinum_R}{uni02DD}{733}
\DeclareTextGlyphY{LinBiolinum_R}{uni02DE}{734}
\DeclareTextGlyphY{LinBiolinum_R}{uni02DF}{735}
\DeclareTextGlyphY{LinBiolinum_R}{gammalatin.superior}{736}
\DeclareTextGlyphY{LinBiolinum_R}{uni02E0}{736}
\DeclareTextGlyphY{LinBiolinum_R}{l.superior}{737}
\DeclareTextGlyphY{LinBiolinum_R}{uni02E1}{737}
\DeclareTextGlyphY{LinBiolinum_R}{s.superior}{738}
\DeclareTextGlyphY{LinBiolinum_R}{uni02E2}{738}
\DeclareTextGlyphY{LinBiolinum_R}{x.superior}{739}
\DeclareTextGlyphY{LinBiolinum_R}{uni02E3}{739}
\DeclareTextGlyphY{LinBiolinum_R}{glottalstopreversed.superior}{740}
\DeclareTextGlyphY{LinBiolinum_R}{uni02E4}{740}
\DeclareTextGlyphY{LinBiolinum_R}{uni02EC}{748}
\DeclareTextGlyphY{LinBiolinum_R}{uni02ED}{749}
\DeclareTextGlyphY{LinBiolinum_R}{uni02EE}{750}
\DeclareTextGlyphY{LinBiolinum_R}{gravecomb}{768}
\DeclareTextGlyphY{LinBiolinum_R}{uni0300}{768}
\DeclareTextGlyphY{LinBiolinum_R}{acutecomb}{769}
\DeclareTextGlyphY{LinBiolinum_R}{uni0301}{769}
\DeclareTextGlyphY{LinBiolinum_R}{uni0302}{770}
\DeclareTextGlyphY{LinBiolinum_R}{tildecomb}{771}
\DeclareTextGlyphY{LinBiolinum_R}{uni0303}{771}
\DeclareTextGlyphY{LinBiolinum_R}{uni0304}{772}
\DeclareTextGlyphY{LinBiolinum_R}{uni0305}{773}
\DeclareTextGlyphY{LinBiolinum_R}{uni0306}{774}
\DeclareTextGlyphY{LinBiolinum_R}{uni0307}{775}
\DeclareTextGlyphY{LinBiolinum_R}{uni0308}{776}
\DeclareTextGlyphY{LinBiolinum_R}{hookabovecomb}{777}
\DeclareTextGlyphY{LinBiolinum_R}{uni0309}{777}
\DeclareTextGlyphY{LinBiolinum_R}{uni030A}{778}
\DeclareTextGlyphY{LinBiolinum_R}{uni030B}{779}
\DeclareTextGlyphY{LinBiolinum_R}{uni030C}{780}
\DeclareTextGlyphY{LinBiolinum_R}{uni030D}{781}
\DeclareTextGlyphY{LinBiolinum_R}{uni030E}{782}
\DeclareTextGlyphY{LinBiolinum_R}{uni030F}{783}
\DeclareTextGlyphY{LinBiolinum_R}{uni0310}{784}
\DeclareTextGlyphY{LinBiolinum_R}{uni0311}{785}
\DeclareTextGlyphY{LinBiolinum_R}{uni0312}{786}
\DeclareTextGlyphY{LinBiolinum_R}{uni0313}{787}
\DeclareTextGlyphY{LinBiolinum_R}{uni0314}{788}
\DeclareTextGlyphY{LinBiolinum_R}{uni0315}{789}
\DeclareTextGlyphY{LinBiolinum_R}{uni0316}{790}
\DeclareTextGlyphY{LinBiolinum_R}{uni0317}{791}
\DeclareTextGlyphY{LinBiolinum_R}{uni0318}{792}
\DeclareTextGlyphY{LinBiolinum_R}{uni0319}{793}
\DeclareTextGlyphY{LinBiolinum_R}{uni031A}{794}
\DeclareTextGlyphY{LinBiolinum_R}{uni031B}{795}
\DeclareTextGlyphY{LinBiolinum_R}{uni031C}{796}
\DeclareTextGlyphY{LinBiolinum_R}{uni031D}{797}
\DeclareTextGlyphY{LinBiolinum_R}{uni031E}{798}
\DeclareTextGlyphY{LinBiolinum_R}{uni031F}{799}
\DeclareTextGlyphY{LinBiolinum_R}{uni0320}{800}
\DeclareTextGlyphY{LinBiolinum_R}{uni0321}{801}
\DeclareTextGlyphY{LinBiolinum_R}{uni0322}{802}
\DeclareTextGlyphY{LinBiolinum_R}{dotbelowcomb}{803}
\DeclareTextGlyphY{LinBiolinum_R}{uni0323}{803}
\DeclareTextGlyphY{LinBiolinum_R}{uni0324}{804}
\DeclareTextGlyphY{LinBiolinum_R}{uni0325}{805}
\DeclareTextGlyphY{LinBiolinum_R}{uni0326}{806}
\DeclareTextGlyphY{LinBiolinum_R}{uni0327}{807}
\DeclareTextGlyphY{LinBiolinum_R}{uni0328}{808}
\DeclareTextGlyphY{LinBiolinum_R}{uni0329}{809}
\DeclareTextGlyphY{LinBiolinum_R}{uni032A}{810}
\DeclareTextGlyphY{LinBiolinum_R}{uni032B}{811}
\DeclareTextGlyphY{LinBiolinum_R}{uni032C}{812}
\DeclareTextGlyphY{LinBiolinum_R}{uni032D}{813}
\DeclareTextGlyphY{LinBiolinum_R}{uni032E}{814}
\DeclareTextGlyphY{LinBiolinum_R}{uni032F}{815}
\DeclareTextGlyphY{LinBiolinum_R}{uni0330}{816}
\DeclareTextGlyphY{LinBiolinum_R}{uni0331}{817}
\DeclareTextGlyphY{LinBiolinum_R}{uni0332}{818}
\DeclareTextGlyphY{LinBiolinum_R}{uni0333}{819}
\DeclareTextGlyphY{LinBiolinum_R}{uni0334}{820}
\DeclareTextGlyphY{LinBiolinum_R}{uni0335}{821}
\DeclareTextGlyphY{LinBiolinum_R}{uni0336}{822}
\DeclareTextGlyphY{LinBiolinum_R}{uni0337}{823}
\DeclareTextGlyphY{LinBiolinum_R}{uni0338}{824}
\DeclareTextGlyphY{LinBiolinum_R}{uni0339}{825}
\DeclareTextGlyphY{LinBiolinum_R}{uni033A}{826}
\DeclareTextGlyphY{LinBiolinum_R}{uni033B}{827}
\DeclareTextGlyphY{LinBiolinum_R}{uni033C}{828}
\DeclareTextGlyphY{LinBiolinum_R}{uni033D}{829}
\DeclareTextGlyphY{LinBiolinum_R}{uni033E}{830}
\DeclareTextGlyphY{LinBiolinum_R}{uni033F}{831}
\DeclareTextGlyphY{LinBiolinum_R}{uni0340}{832}
\DeclareTextGlyphY{LinBiolinum_R}{uni0341}{833}
\DeclareTextGlyphY{LinBiolinum_R}{uni0342}{834}
\DeclareTextGlyphY{LinBiolinum_R}{uni0343}{835}
\DeclareTextGlyphY{LinBiolinum_R}{uni0344}{836}
\DeclareTextGlyphY{LinBiolinum_R}{uni0345}{837}
\DeclareTextGlyphY{LinBiolinum_R}{uni0346}{838}
\DeclareTextGlyphY{LinBiolinum_R}{uni0347}{839}
\DeclareTextGlyphY{LinBiolinum_R}{uni0348}{840}
\DeclareTextGlyphY{LinBiolinum_R}{uni0349}{841}
\DeclareTextGlyphY{LinBiolinum_R}{uni034A}{842}
\DeclareTextGlyphY{LinBiolinum_R}{uni034B}{843}
\DeclareTextGlyphY{LinBiolinum_R}{uni034C}{844}
\DeclareTextGlyphY{LinBiolinum_R}{uni034D}{845}
\DeclareTextGlyphY{LinBiolinum_R}{uni034E}{846}
\DeclareTextGlyphY{LinBiolinum_R}{uni0350}{848}
\DeclareTextGlyphY{LinBiolinum_R}{uni0351}{849}
\DeclareTextGlyphY{LinBiolinum_R}{uni0352}{850}
\DeclareTextGlyphY{LinBiolinum_R}{uni0353}{851}
\DeclareTextGlyphY{LinBiolinum_R}{uni0354}{852}
\DeclareTextGlyphY{LinBiolinum_R}{uni0355}{853}
\DeclareTextGlyphY{LinBiolinum_R}{uni0356}{854}
\DeclareTextGlyphY{LinBiolinum_R}{uni0357}{855}
\DeclareTextGlyphY{LinBiolinum_R}{uni0358}{856}
\DeclareTextGlyphY{LinBiolinum_R}{uni0359}{857}
\DeclareTextGlyphY{LinBiolinum_R}{uni035A}{858}
\DeclareTextGlyphY{LinBiolinum_R}{uni035B}{859}
\DeclareTextGlyphY{LinBiolinum_R}{uni035C}{860}
\DeclareTextGlyphY{LinBiolinum_R}{uni035D}{861}
\DeclareTextGlyphY{LinBiolinum_R}{uni035E}{862}
\DeclareTextGlyphY{LinBiolinum_R}{uni035F}{863}
\DeclareTextGlyphY{LinBiolinum_R}{uni0360}{864}
\DeclareTextGlyphY{LinBiolinum_R}{uni0361}{865}
\DeclareTextGlyphY{LinBiolinum_R}{uni0362}{866}
\DeclareTextGlyphY{LinBiolinum_R}{uni0363}{867}
\DeclareTextGlyphY{LinBiolinum_R}{uni0364}{868}
\DeclareTextGlyphY{LinBiolinum_R}{uni0365}{869}
\DeclareTextGlyphY{LinBiolinum_R}{uni0366}{870}
\DeclareTextGlyphY{LinBiolinum_R}{uni0367}{871}
\DeclareTextGlyphY{LinBiolinum_R}{uni0368}{872}
\DeclareTextGlyphY{LinBiolinum_R}{uni0369}{873}
\DeclareTextGlyphY{LinBiolinum_R}{uni036A}{874}
\DeclareTextGlyphY{LinBiolinum_R}{uni036B}{875}
\DeclareTextGlyphY{LinBiolinum_R}{uni036C}{876}
\DeclareTextGlyphY{LinBiolinum_R}{uni036D}{877}
\DeclareTextGlyphY{LinBiolinum_R}{uni036E}{878}
\DeclareTextGlyphY{LinBiolinum_R}{uni036F}{879}
\DeclareTextGlyphY{LinBiolinum_R}{uni0374}{884}
\DeclareTextGlyphY{LinBiolinum_R}{uni0375}{885}
\DeclareTextGlyphY{LinBiolinum_R}{uni037A}{890}
\DeclareTextGlyphY{LinBiolinum_R}{uni037B}{891}
\DeclareTextGlyphY{LinBiolinum_R}{uni037C}{892}
\DeclareTextGlyphY{LinBiolinum_R}{uni037D}{893}
\DeclareTextGlyphY{LinBiolinum_R}{uni037E}{894}
\DeclareTextGlyphY{LinBiolinum_R}{tonos}{900}
\DeclareTextGlyphY{LinBiolinum_R}{uni0384}{900}
\DeclareTextGlyphY{LinBiolinum_R}{dieresistonos}{901}
\DeclareTextGlyphY{LinBiolinum_R}{uni0385}{901}
\DeclareTextGlyphY{LinBiolinum_R}{Alphatonos}{902}
\DeclareTextGlyphY{LinBiolinum_R}{uni0386}{902}
\DeclareTextGlyphY{LinBiolinum_R}{anoteleia}{903}
\DeclareTextGlyphY{LinBiolinum_R}{uni0387}{903}
\DeclareTextGlyphY{LinBiolinum_R}{Epsilontonos}{904}
\DeclareTextGlyphY{LinBiolinum_R}{uni0388}{904}
\DeclareTextGlyphY{LinBiolinum_R}{Etatonos}{905}
\DeclareTextGlyphY{LinBiolinum_R}{uni0389}{905}
\DeclareTextGlyphY{LinBiolinum_R}{Iotatonos}{906}
\DeclareTextGlyphY{LinBiolinum_R}{uni038A}{906}
\DeclareTextGlyphY{LinBiolinum_R}{Omicrontonos}{908}
\DeclareTextGlyphY{LinBiolinum_R}{uni038C}{908}
\DeclareTextGlyphY{LinBiolinum_R}{Upsilontonos}{910}
\DeclareTextGlyphY{LinBiolinum_R}{uni038E}{910}
\DeclareTextGlyphY{LinBiolinum_R}{Omegatonos}{911}
\DeclareTextGlyphY{LinBiolinum_R}{uni038F}{911}
\DeclareTextGlyphY{LinBiolinum_R}{iotadieresistonos}{912}
\DeclareTextGlyphY{LinBiolinum_R}{uni0390}{912}
\DeclareTextGlyphY{LinBiolinum_R}{Alpha}{913}
\DeclareTextGlyphY{LinBiolinum_R}{uni0391}{913}
\DeclareTextGlyphY{LinBiolinum_R}{Beta}{914}
\DeclareTextGlyphY{LinBiolinum_R}{uni0392}{914}
\DeclareTextGlyphY{LinBiolinum_R}{Gamma}{915}
\DeclareTextGlyphY{LinBiolinum_R}{uni0393}{915}
\DeclareTextGlyphY{LinBiolinum_R}{Delta}{916}
\DeclareTextGlyphY{LinBiolinum_R}{uni0394}{916}
\DeclareTextGlyphY{LinBiolinum_R}{Epsilon}{917}
\DeclareTextGlyphY{LinBiolinum_R}{uni0395}{917}
\DeclareTextGlyphY{LinBiolinum_R}{Zeta}{918}
\DeclareTextGlyphY{LinBiolinum_R}{uni0396}{918}
\DeclareTextGlyphY{LinBiolinum_R}{Eta}{919}
\DeclareTextGlyphY{LinBiolinum_R}{uni0397}{919}
\DeclareTextGlyphY{LinBiolinum_R}{Theta}{920}
\DeclareTextGlyphY{LinBiolinum_R}{uni0398}{920}
\DeclareTextGlyphY{LinBiolinum_R}{Iota}{921}
\DeclareTextGlyphY{LinBiolinum_R}{uni0399}{921}
\DeclareTextGlyphY{LinBiolinum_R}{Kappa}{922}
\DeclareTextGlyphY{LinBiolinum_R}{uni039A}{922}
\DeclareTextGlyphY{LinBiolinum_R}{Lambda}{923}
\DeclareTextGlyphY{LinBiolinum_R}{uni039B}{923}
\DeclareTextGlyphY{LinBiolinum_R}{Mu}{924}
\DeclareTextGlyphY{LinBiolinum_R}{uni039C}{924}
\DeclareTextGlyphY{LinBiolinum_R}{Nu}{925}
\DeclareTextGlyphY{LinBiolinum_R}{uni039D}{925}
\DeclareTextGlyphY{LinBiolinum_R}{Xi}{926}
\DeclareTextGlyphY{LinBiolinum_R}{uni039E}{926}
\DeclareTextGlyphY{LinBiolinum_R}{Omicron}{927}
\DeclareTextGlyphY{LinBiolinum_R}{uni039F}{927}
\DeclareTextGlyphY{LinBiolinum_R}{Pi}{928}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A0}{928}
\DeclareTextGlyphY{LinBiolinum_R}{Rho}{929}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A1}{929}
\DeclareTextGlyphY{LinBiolinum_R}{Sigma}{931}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A3}{931}
\DeclareTextGlyphY{LinBiolinum_R}{Tau}{932}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A4}{932}
\DeclareTextGlyphY{LinBiolinum_R}{Upsilon}{933}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A5}{933}
\DeclareTextGlyphY{LinBiolinum_R}{Phi}{934}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A6}{934}
\DeclareTextGlyphY{LinBiolinum_R}{Chi}{935}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A7}{935}
\DeclareTextGlyphY{LinBiolinum_R}{Psi}{936}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A8}{936}
\DeclareTextGlyphY{LinBiolinum_R}{Omega}{937}
\DeclareTextGlyphY{LinBiolinum_R}{uni03A9}{937}
\DeclareTextGlyphY{LinBiolinum_R}{Iotadieresis}{938}
\DeclareTextGlyphY{LinBiolinum_R}{uni03AA}{938}
\DeclareTextGlyphY{LinBiolinum_R}{Upsilondieresis}{939}
\DeclareTextGlyphY{LinBiolinum_R}{uni03AB}{939}
\DeclareTextGlyphY{LinBiolinum_R}{alphatonos}{940}
\DeclareTextGlyphY{LinBiolinum_R}{uni03AC}{940}
\DeclareTextGlyphY{LinBiolinum_R}{epsilontonos}{941}
\DeclareTextGlyphY{LinBiolinum_R}{uni03AD}{941}
\DeclareTextGlyphY{LinBiolinum_R}{etatonos}{942}
\DeclareTextGlyphY{LinBiolinum_R}{uni03AE}{942}
\DeclareTextGlyphY{LinBiolinum_R}{iotatonos}{943}
\DeclareTextGlyphY{LinBiolinum_R}{uni03AF}{943}
\DeclareTextGlyphY{LinBiolinum_R}{upsilondieresistonos}{944}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B0}{944}
\DeclareTextGlyphY{LinBiolinum_R}{alpha}{945}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B1}{945}
\DeclareTextGlyphY{LinBiolinum_R}{beta}{946}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B2}{946}
\DeclareTextGlyphY{LinBiolinum_R}{gamma}{947}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B3}{947}
\DeclareTextGlyphY{LinBiolinum_R}{delta}{948}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B4}{948}
\DeclareTextGlyphY{LinBiolinum_R}{epsilon}{949}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B5}{949}
\DeclareTextGlyphY{LinBiolinum_R}{zeta}{950}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B6}{950}
\DeclareTextGlyphY{LinBiolinum_R}{eta}{951}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B7}{951}
\DeclareTextGlyphY{LinBiolinum_R}{theta}{952}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B8}{952}
\DeclareTextGlyphY{LinBiolinum_R}{iota}{953}
\DeclareTextGlyphY{LinBiolinum_R}{uni03B9}{953}
\DeclareTextGlyphY{LinBiolinum_R}{kappa}{954}
\DeclareTextGlyphY{LinBiolinum_R}{uni03BA}{954}
\DeclareTextGlyphY{LinBiolinum_R}{lambda}{955}
\DeclareTextGlyphY{LinBiolinum_R}{uni03BB}{955}
\DeclareTextGlyphY{LinBiolinum_R}{mu}{956}
\DeclareTextGlyphY{LinBiolinum_R}{uni03BC}{956}
\DeclareTextGlyphY{LinBiolinum_R}{nu}{957}
\DeclareTextGlyphY{LinBiolinum_R}{uni03BD}{957}
\DeclareTextGlyphY{LinBiolinum_R}{xi}{958}
\DeclareTextGlyphY{LinBiolinum_R}{uni03BE}{958}
\DeclareTextGlyphY{LinBiolinum_R}{omicron}{959}
\DeclareTextGlyphY{LinBiolinum_R}{uni03BF}{959}
\DeclareTextGlyphY{LinBiolinum_R}{pi}{960}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C0}{960}
\DeclareTextGlyphY{LinBiolinum_R}{rho}{961}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C1}{961}
\DeclareTextGlyphY{LinBiolinum_R}{sigma1}{962}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C2}{962}
\DeclareTextGlyphY{LinBiolinum_R}{sigma}{963}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C3}{963}
\DeclareTextGlyphY{LinBiolinum_R}{tau}{964}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C4}{964}
\DeclareTextGlyphY{LinBiolinum_R}{upsilon}{965}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C5}{965}
\DeclareTextGlyphY{LinBiolinum_R}{phi}{966}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C6}{966}
\DeclareTextGlyphY{LinBiolinum_R}{chi}{967}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C7}{967}
\DeclareTextGlyphY{LinBiolinum_R}{psi}{968}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C8}{968}
\DeclareTextGlyphY{LinBiolinum_R}{omega}{969}
\DeclareTextGlyphY{LinBiolinum_R}{uni03C9}{969}
\DeclareTextGlyphY{LinBiolinum_R}{iotadieresis}{970}
\DeclareTextGlyphY{LinBiolinum_R}{uni03CA}{970}
\DeclareTextGlyphY{LinBiolinum_R}{upsilondieresis}{971}
\DeclareTextGlyphY{LinBiolinum_R}{uni03CB}{971}
\DeclareTextGlyphY{LinBiolinum_R}{omicrontonos}{972}
\DeclareTextGlyphY{LinBiolinum_R}{uni03CC}{972}
\DeclareTextGlyphY{LinBiolinum_R}{upsilontonos}{973}
\DeclareTextGlyphY{LinBiolinum_R}{uni03CD}{973}
\DeclareTextGlyphY{LinBiolinum_R}{omegatonos}{974}
\DeclareTextGlyphY{LinBiolinum_R}{uni03CE}{974}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D0}{976}
\DeclareTextGlyphY{LinBiolinum_R}{theta1}{977}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D1}{977}
\DeclareTextGlyphY{LinBiolinum_R}{Upsilon1}{978}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D2}{978}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D3}{979}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D4}{980}
\DeclareTextGlyphY{LinBiolinum_R}{phi1}{981}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D5}{981}
\DeclareTextGlyphY{LinBiolinum_R}{omega1}{982}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D6}{982}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D7}{983}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D8}{984}
\DeclareTextGlyphY{LinBiolinum_R}{uni03D9}{985}
\DeclareTextGlyphY{LinBiolinum_R}{uni03DA}{986}
\DeclareTextGlyphY{LinBiolinum_R}{uni03DB}{987}
\DeclareTextGlyphY{LinBiolinum_R}{uni03DC}{988}
\DeclareTextGlyphY{LinBiolinum_R}{uni03DD}{989}
\DeclareTextGlyphY{LinBiolinum_R}{uni03DE}{990}
\DeclareTextGlyphY{LinBiolinum_R}{uni03DF}{991}
\DeclareTextGlyphY{LinBiolinum_R}{uni03E0}{992}
\DeclareTextGlyphY{LinBiolinum_R}{uni03E1}{993}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F0}{1008}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F1}{1009}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F2}{1010}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F3}{1011}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F4}{1012}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F5}{1013}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F6}{1014}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F8}{1016}
\DeclareTextGlyphY{LinBiolinum_R}{uni03F9}{1017}
\DeclareTextGlyphY{LinBiolinum_R}{uni03FB}{1019}
\DeclareTextGlyphY{LinBiolinum_R}{uni03FD}{1021}
\DeclareTextGlyphY{LinBiolinum_R}{uni03FE}{1022}
\DeclareTextGlyphY{LinBiolinum_R}{uni03FF}{1023}
\DeclareTextGlyphY{LinBiolinum_R}{uni0400}{1024}
\DeclareTextGlyphY{LinBiolinum_R}{afii10023}{1025}
\DeclareTextGlyphY{LinBiolinum_R}{uni0401}{1025}
\DeclareTextGlyphY{LinBiolinum_R}{afii10051}{1026}
\DeclareTextGlyphY{LinBiolinum_R}{uni0402}{1026}
\DeclareTextGlyphY{LinBiolinum_R}{afii10052}{1027}
\DeclareTextGlyphY{LinBiolinum_R}{uni0403}{1027}
\DeclareTextGlyphY{LinBiolinum_R}{afii10053}{1028}
\DeclareTextGlyphY{LinBiolinum_R}{uni0404}{1028}
\DeclareTextGlyphY{LinBiolinum_R}{afii10054}{1029}
\DeclareTextGlyphY{LinBiolinum_R}{uni0405}{1029}
\DeclareTextGlyphY{LinBiolinum_R}{afii10055}{1030}
\DeclareTextGlyphY{LinBiolinum_R}{uni0406}{1030}
\DeclareTextGlyphY{LinBiolinum_R}{afii10056}{1031}
\DeclareTextGlyphY{LinBiolinum_R}{uni0407}{1031}
\DeclareTextGlyphY{LinBiolinum_R}{afii10057}{1032}
\DeclareTextGlyphY{LinBiolinum_R}{uni0408}{1032}
\DeclareTextGlyphY{LinBiolinum_R}{afii10058}{1033}
\DeclareTextGlyphY{LinBiolinum_R}{uni0409}{1033}
\DeclareTextGlyphY{LinBiolinum_R}{afii10059}{1034}
\DeclareTextGlyphY{LinBiolinum_R}{uni040A}{1034}
\DeclareTextGlyphY{LinBiolinum_R}{afii10060}{1035}
\DeclareTextGlyphY{LinBiolinum_R}{uni040B}{1035}
\DeclareTextGlyphY{LinBiolinum_R}{afii10061}{1036}
\DeclareTextGlyphY{LinBiolinum_R}{uni040C}{1036}
\DeclareTextGlyphY{LinBiolinum_R}{uni040D}{1037}
\DeclareTextGlyphY{LinBiolinum_R}{afii10062}{1038}
\DeclareTextGlyphY{LinBiolinum_R}{uni040E}{1038}
\DeclareTextGlyphY{LinBiolinum_R}{afii10145}{1039}
\DeclareTextGlyphY{LinBiolinum_R}{uni040F}{1039}
\DeclareTextGlyphY{LinBiolinum_R}{afii10017}{1040}
\DeclareTextGlyphY{LinBiolinum_R}{uni0410}{1040}
\DeclareTextGlyphY{LinBiolinum_R}{afii10018}{1041}
\DeclareTextGlyphY{LinBiolinum_R}{uni0411}{1041}
\DeclareTextGlyphY{LinBiolinum_R}{afii10019}{1042}
\DeclareTextGlyphY{LinBiolinum_R}{uni0412}{1042}
\DeclareTextGlyphY{LinBiolinum_R}{afii10020}{1043}
\DeclareTextGlyphY{LinBiolinum_R}{uni0413}{1043}
\DeclareTextGlyphY{LinBiolinum_R}{afii10021}{1044}
\DeclareTextGlyphY{LinBiolinum_R}{uni0414}{1044}
\DeclareTextGlyphY{LinBiolinum_R}{afii10022}{1045}
\DeclareTextGlyphY{LinBiolinum_R}{uni0415}{1045}
\DeclareTextGlyphY{LinBiolinum_R}{afii10024}{1046}
\DeclareTextGlyphY{LinBiolinum_R}{uni0416}{1046}
\DeclareTextGlyphY{LinBiolinum_R}{afii10025}{1047}
\DeclareTextGlyphY{LinBiolinum_R}{uni0417}{1047}
\DeclareTextGlyphY{LinBiolinum_R}{afii10026}{1048}
\DeclareTextGlyphY{LinBiolinum_R}{uni0418}{1048}
\DeclareTextGlyphY{LinBiolinum_R}{afii10027}{1049}
\DeclareTextGlyphY{LinBiolinum_R}{uni0419}{1049}
\DeclareTextGlyphY{LinBiolinum_R}{afii10028}{1050}
\DeclareTextGlyphY{LinBiolinum_R}{uni041A}{1050}
\DeclareTextGlyphY{LinBiolinum_R}{afii10029}{1051}
\DeclareTextGlyphY{LinBiolinum_R}{uni041B}{1051}
\DeclareTextGlyphY{LinBiolinum_R}{afii10030}{1052}
\DeclareTextGlyphY{LinBiolinum_R}{uni041C}{1052}
\DeclareTextGlyphY{LinBiolinum_R}{afii10031}{1053}
\DeclareTextGlyphY{LinBiolinum_R}{uni041D}{1053}
\DeclareTextGlyphY{LinBiolinum_R}{afii10032}{1054}
\DeclareTextGlyphY{LinBiolinum_R}{uni041E}{1054}
\DeclareTextGlyphY{LinBiolinum_R}{afii10033}{1055}
\DeclareTextGlyphY{LinBiolinum_R}{uni041F}{1055}
\DeclareTextGlyphY{LinBiolinum_R}{afii10034}{1056}
\DeclareTextGlyphY{LinBiolinum_R}{uni0420}{1056}
\DeclareTextGlyphY{LinBiolinum_R}{afii10035}{1057}
\DeclareTextGlyphY{LinBiolinum_R}{uni0421}{1057}
\DeclareTextGlyphY{LinBiolinum_R}{afii10036}{1058}
\DeclareTextGlyphY{LinBiolinum_R}{uni0422}{1058}
\DeclareTextGlyphY{LinBiolinum_R}{afii10037}{1059}
\DeclareTextGlyphY{LinBiolinum_R}{uni0423}{1059}
\DeclareTextGlyphY{LinBiolinum_R}{afii10038}{1060}
\DeclareTextGlyphY{LinBiolinum_R}{uni0424}{1060}
\DeclareTextGlyphY{LinBiolinum_R}{afii10039}{1061}
\DeclareTextGlyphY{LinBiolinum_R}{uni0425}{1061}
\DeclareTextGlyphY{LinBiolinum_R}{afii10040}{1062}
\DeclareTextGlyphY{LinBiolinum_R}{uni0426}{1062}
\DeclareTextGlyphY{LinBiolinum_R}{afii10041}{1063}
\DeclareTextGlyphY{LinBiolinum_R}{uni0427}{1063}
\DeclareTextGlyphY{LinBiolinum_R}{afii10042}{1064}
\DeclareTextGlyphY{LinBiolinum_R}{uni0428}{1064}
\DeclareTextGlyphY{LinBiolinum_R}{afii10043}{1065}
\DeclareTextGlyphY{LinBiolinum_R}{uni0429}{1065}
\DeclareTextGlyphY{LinBiolinum_R}{afii10044}{1066}
\DeclareTextGlyphY{LinBiolinum_R}{uni042A}{1066}
\DeclareTextGlyphY{LinBiolinum_R}{afii10045}{1067}
\DeclareTextGlyphY{LinBiolinum_R}{uni042B}{1067}
\DeclareTextGlyphY{LinBiolinum_R}{afii10046}{1068}
\DeclareTextGlyphY{LinBiolinum_R}{uni042C}{1068}
\DeclareTextGlyphY{LinBiolinum_R}{afii10047}{1069}
\DeclareTextGlyphY{LinBiolinum_R}{uni042D}{1069}
\DeclareTextGlyphY{LinBiolinum_R}{afii10048}{1070}
\DeclareTextGlyphY{LinBiolinum_R}{uni042E}{1070}
\DeclareTextGlyphY{LinBiolinum_R}{afii10049}{1071}
\DeclareTextGlyphY{LinBiolinum_R}{uni042F}{1071}
\DeclareTextGlyphY{LinBiolinum_R}{afii10065}{1072}
\DeclareTextGlyphY{LinBiolinum_R}{uni0430}{1072}
\DeclareTextGlyphY{LinBiolinum_R}{afii10066}{1073}
\DeclareTextGlyphY{LinBiolinum_R}{uni0431}{1073}
\DeclareTextGlyphY{LinBiolinum_R}{afii10067}{1074}
\DeclareTextGlyphY{LinBiolinum_R}{uni0432}{1074}
\DeclareTextGlyphY{LinBiolinum_R}{afii10068}{1075}
\DeclareTextGlyphY{LinBiolinum_R}{uni0433}{1075}
\DeclareTextGlyphY{LinBiolinum_R}{afii10069}{1076}
\DeclareTextGlyphY{LinBiolinum_R}{uni0434}{1076}
\DeclareTextGlyphY{LinBiolinum_R}{afii10070}{1077}
\DeclareTextGlyphY{LinBiolinum_R}{uni0435}{1077}
\DeclareTextGlyphY{LinBiolinum_R}{afii10072}{1078}
\DeclareTextGlyphY{LinBiolinum_R}{uni0436}{1078}
\DeclareTextGlyphY{LinBiolinum_R}{afii10073}{1079}
\DeclareTextGlyphY{LinBiolinum_R}{uni0437}{1079}
\DeclareTextGlyphY{LinBiolinum_R}{afii10074}{1080}
\DeclareTextGlyphY{LinBiolinum_R}{uni0438}{1080}
\DeclareTextGlyphY{LinBiolinum_R}{afii10075}{1081}
\DeclareTextGlyphY{LinBiolinum_R}{uni0439}{1081}
\DeclareTextGlyphY{LinBiolinum_R}{afii10076}{1082}
\DeclareTextGlyphY{LinBiolinum_R}{uni043A}{1082}
\DeclareTextGlyphY{LinBiolinum_R}{afii10077}{1083}
\DeclareTextGlyphY{LinBiolinum_R}{uni043B}{1083}
\DeclareTextGlyphY{LinBiolinum_R}{afii10078}{1084}
\DeclareTextGlyphY{LinBiolinum_R}{uni043C}{1084}
\DeclareTextGlyphY{LinBiolinum_R}{afii10079}{1085}
\DeclareTextGlyphY{LinBiolinum_R}{uni043D}{1085}
\DeclareTextGlyphY{LinBiolinum_R}{afii10080}{1086}
\DeclareTextGlyphY{LinBiolinum_R}{uni043E}{1086}
\DeclareTextGlyphY{LinBiolinum_R}{afii10081}{1087}
\DeclareTextGlyphY{LinBiolinum_R}{uni043F}{1087}
\DeclareTextGlyphY{LinBiolinum_R}{afii10082}{1088}
\DeclareTextGlyphY{LinBiolinum_R}{uni0440}{1088}
\DeclareTextGlyphY{LinBiolinum_R}{afii10083}{1089}
\DeclareTextGlyphY{LinBiolinum_R}{uni0441}{1089}
\DeclareTextGlyphY{LinBiolinum_R}{afii10084}{1090}
\DeclareTextGlyphY{LinBiolinum_R}{uni0442}{1090}
\DeclareTextGlyphY{LinBiolinum_R}{afii10085}{1091}
\DeclareTextGlyphY{LinBiolinum_R}{uni0443}{1091}
\DeclareTextGlyphY{LinBiolinum_R}{afii10086}{1092}
\DeclareTextGlyphY{LinBiolinum_R}{uni0444}{1092}
\DeclareTextGlyphY{LinBiolinum_R}{afii10087}{1093}
\DeclareTextGlyphY{LinBiolinum_R}{uni0445}{1093}
\DeclareTextGlyphY{LinBiolinum_R}{afii10088}{1094}
\DeclareTextGlyphY{LinBiolinum_R}{uni0446}{1094}
\DeclareTextGlyphY{LinBiolinum_R}{afii10089}{1095}
\DeclareTextGlyphY{LinBiolinum_R}{uni0447}{1095}
\DeclareTextGlyphY{LinBiolinum_R}{afii10090}{1096}
\DeclareTextGlyphY{LinBiolinum_R}{uni0448}{1096}
\DeclareTextGlyphY{LinBiolinum_R}{afii10091}{1097}
\DeclareTextGlyphY{LinBiolinum_R}{uni0449}{1097}
\DeclareTextGlyphY{LinBiolinum_R}{afii10092}{1098}
\DeclareTextGlyphY{LinBiolinum_R}{uni044A}{1098}
\DeclareTextGlyphY{LinBiolinum_R}{afii10093}{1099}
\DeclareTextGlyphY{LinBiolinum_R}{uni044B}{1099}
\DeclareTextGlyphY{LinBiolinum_R}{afii10094}{1100}
\DeclareTextGlyphY{LinBiolinum_R}{uni044C}{1100}
\DeclareTextGlyphY{LinBiolinum_R}{afii10095}{1101}
\DeclareTextGlyphY{LinBiolinum_R}{uni044D}{1101}
\DeclareTextGlyphY{LinBiolinum_R}{afii10096}{1102}
\DeclareTextGlyphY{LinBiolinum_R}{uni044E}{1102}
\DeclareTextGlyphY{LinBiolinum_R}{afii10097}{1103}
\DeclareTextGlyphY{LinBiolinum_R}{uni044F}{1103}
\DeclareTextGlyphY{LinBiolinum_R}{uni0450}{1104}
\DeclareTextGlyphY{LinBiolinum_R}{afii10071}{1105}
\DeclareTextGlyphY{LinBiolinum_R}{uni0451}{1105}
\DeclareTextGlyphY{LinBiolinum_R}{afii10099}{1106}
\DeclareTextGlyphY{LinBiolinum_R}{uni0452}{1106}
\DeclareTextGlyphY{LinBiolinum_R}{afii10100}{1107}
\DeclareTextGlyphY{LinBiolinum_R}{uni0453}{1107}
\DeclareTextGlyphY{LinBiolinum_R}{afii10101}{1108}
\DeclareTextGlyphY{LinBiolinum_R}{uni0454}{1108}
\DeclareTextGlyphY{LinBiolinum_R}{afii10102}{1109}
\DeclareTextGlyphY{LinBiolinum_R}{uni0455}{1109}
\DeclareTextGlyphY{LinBiolinum_R}{afii10103}{1110}
\DeclareTextGlyphY{LinBiolinum_R}{uni0456}{1110}
\DeclareTextGlyphY{LinBiolinum_R}{afii10104}{1111}
\DeclareTextGlyphY{LinBiolinum_R}{uni0457}{1111}
\DeclareTextGlyphY{LinBiolinum_R}{afii10105}{1112}
\DeclareTextGlyphY{LinBiolinum_R}{uni0458}{1112}
\DeclareTextGlyphY{LinBiolinum_R}{afii10106}{1113}
\DeclareTextGlyphY{LinBiolinum_R}{uni0459}{1113}
\DeclareTextGlyphY{LinBiolinum_R}{afii10107}{1114}
\DeclareTextGlyphY{LinBiolinum_R}{uni045A}{1114}
\DeclareTextGlyphY{LinBiolinum_R}{afii10108}{1115}
\DeclareTextGlyphY{LinBiolinum_R}{uni045B}{1115}
\DeclareTextGlyphY{LinBiolinum_R}{afii10109}{1116}
\DeclareTextGlyphY{LinBiolinum_R}{uni045C}{1116}
\DeclareTextGlyphY{LinBiolinum_R}{uni045D}{1117}
\DeclareTextGlyphY{LinBiolinum_R}{afii10110}{1118}
\DeclareTextGlyphY{LinBiolinum_R}{uni045E}{1118}
\DeclareTextGlyphY{LinBiolinum_R}{afii10193}{1119}
\DeclareTextGlyphY{LinBiolinum_R}{uni045F}{1119}
\DeclareTextGlyphY{LinBiolinum_R}{afii10050}{1168}
\DeclareTextGlyphY{LinBiolinum_R}{uni0490}{1168}
\DeclareTextGlyphY{LinBiolinum_R}{afii10098}{1169}
\DeclareTextGlyphY{LinBiolinum_R}{uni0491}{1169}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D0}{1232}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D1}{1233}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D2}{1234}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D3}{1235}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D4}{1236}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D5}{1237}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D6}{1238}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D7}{1239}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D8}{1240}
\DeclareTextGlyphY{LinBiolinum_R}{afii10846}{1241}
\DeclareTextGlyphY{LinBiolinum_R}{uni04D9}{1241}
\DeclareTextGlyphY{LinBiolinum_R}{uni04DA}{1242}
\DeclareTextGlyphY{LinBiolinum_R}{uni04DB}{1243}
\DeclareTextGlyphY{LinBiolinum_R}{uni04DC}{1244}
\DeclareTextGlyphY{LinBiolinum_R}{uni04DD}{1245}
\DeclareTextGlyphY{LinBiolinum_R}{uni04DE}{1246}
\DeclareTextGlyphY{LinBiolinum_R}{uni04DF}{1247}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E0}{1248}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E1}{1249}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E2}{1250}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E3}{1251}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E4}{1252}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E5}{1253}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E6}{1254}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E7}{1255}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E8}{1256}
\DeclareTextGlyphY{LinBiolinum_R}{uni04E9}{1257}
\DeclareTextGlyphY{LinBiolinum_R}{uni04EA}{1258}
\DeclareTextGlyphY{LinBiolinum_R}{uni04EB}{1259}
\DeclareTextGlyphY{LinBiolinum_R}{uni04EC}{1260}
\DeclareTextGlyphY{LinBiolinum_R}{uni04ED}{1261}
\DeclareTextGlyphY{LinBiolinum_R}{uni04EE}{1262}
\DeclareTextGlyphY{LinBiolinum_R}{uni04EF}{1263}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F0}{1264}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F1}{1265}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F2}{1266}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F3}{1267}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F4}{1268}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F5}{1269}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F6}{1270}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F7}{1271}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F8}{1272}
\DeclareTextGlyphY{LinBiolinum_R}{uni04F9}{1273}
\DeclareTextGlyphY{LinBiolinum_R}{afii57799}{1456}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B0}{1456}
\DeclareTextGlyphY{LinBiolinum_R}{afii57801}{1457}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B1}{1457}
\DeclareTextGlyphY{LinBiolinum_R}{afii57800}{1458}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B2}{1458}
\DeclareTextGlyphY{LinBiolinum_R}{afii57802}{1459}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B3}{1459}
\DeclareTextGlyphY{LinBiolinum_R}{afii57793}{1460}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B4}{1460}
\DeclareTextGlyphY{LinBiolinum_R}{afii57794}{1461}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B5}{1461}
\DeclareTextGlyphY{LinBiolinum_R}{afii57795}{1462}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B6}{1462}
\DeclareTextGlyphY{LinBiolinum_R}{afii57798}{1463}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B7}{1463}
\DeclareTextGlyphY{LinBiolinum_R}{afii57797}{1464}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B8}{1464}
\DeclareTextGlyphY{LinBiolinum_R}{afii57806}{1465}
\DeclareTextGlyphY{LinBiolinum_R}{uni05B9}{1465}
\DeclareTextGlyphY{LinBiolinum_R}{uni05BA}{1466}
\DeclareTextGlyphY{LinBiolinum_R}{afii57796}{1467}
\DeclareTextGlyphY{LinBiolinum_R}{uni05BB}{1467}
\DeclareTextGlyphY{LinBiolinum_R}{afii57807}{1468}
\DeclareTextGlyphY{LinBiolinum_R}{uni05BC}{1468}
\DeclareTextGlyphY{LinBiolinum_R}{afii57839}{1469}
\DeclareTextGlyphY{LinBiolinum_R}{uni05BD}{1469}
\DeclareTextGlyphY{LinBiolinum_R}{afii57645}{1470}
\DeclareTextGlyphY{LinBiolinum_R}{uni05BE}{1470}
\DeclareTextGlyphY{LinBiolinum_R}{afii57841}{1471}
\DeclareTextGlyphY{LinBiolinum_R}{uni05BF}{1471}
\DeclareTextGlyphY{LinBiolinum_R}{afii57842}{1472}
\DeclareTextGlyphY{LinBiolinum_R}{uni05C0}{1472}
\DeclareTextGlyphY{LinBiolinum_R}{afii57804}{1473}
\DeclareTextGlyphY{LinBiolinum_R}{uni05C1}{1473}
\DeclareTextGlyphY{LinBiolinum_R}{afii57803}{1474}
\DeclareTextGlyphY{LinBiolinum_R}{uni05C2}{1474}
\DeclareTextGlyphY{LinBiolinum_R}{afii57658}{1475}
\DeclareTextGlyphY{LinBiolinum_R}{uni05C3}{1475}
\DeclareTextGlyphY{LinBiolinum_R}{uni05C6}{1478}
\DeclareTextGlyphY{LinBiolinum_R}{afii57664}{1488}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D0}{1488}
\DeclareTextGlyphY{LinBiolinum_R}{afii57665}{1489}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D1}{1489}
\DeclareTextGlyphY{LinBiolinum_R}{afii57666}{1490}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D2}{1490}
\DeclareTextGlyphY{LinBiolinum_R}{afii57667}{1491}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D3}{1491}
\DeclareTextGlyphY{LinBiolinum_R}{afii57668}{1492}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D4}{1492}
\DeclareTextGlyphY{LinBiolinum_R}{afii57669}{1493}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D5}{1493}
\DeclareTextGlyphY{LinBiolinum_R}{afii57670}{1494}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D6}{1494}
\DeclareTextGlyphY{LinBiolinum_R}{afii57671}{1495}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D7}{1495}
\DeclareTextGlyphY{LinBiolinum_R}{afii57672}{1496}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D8}{1496}
\DeclareTextGlyphY{LinBiolinum_R}{afii57673}{1497}
\DeclareTextGlyphY{LinBiolinum_R}{uni05D9}{1497}
\DeclareTextGlyphY{LinBiolinum_R}{afii57674}{1498}
\DeclareTextGlyphY{LinBiolinum_R}{uni05DA}{1498}
\DeclareTextGlyphY{LinBiolinum_R}{afii57675}{1499}
\DeclareTextGlyphY{LinBiolinum_R}{uni05DB}{1499}
\DeclareTextGlyphY{LinBiolinum_R}{afii57676}{1500}
\DeclareTextGlyphY{LinBiolinum_R}{uni05DC}{1500}
\DeclareTextGlyphY{LinBiolinum_R}{afii57677}{1501}
\DeclareTextGlyphY{LinBiolinum_R}{uni05DD}{1501}
\DeclareTextGlyphY{LinBiolinum_R}{afii57678}{1502}
\DeclareTextGlyphY{LinBiolinum_R}{uni05DE}{1502}
\DeclareTextGlyphY{LinBiolinum_R}{afii57679}{1503}
\DeclareTextGlyphY{LinBiolinum_R}{uni05DF}{1503}
\DeclareTextGlyphY{LinBiolinum_R}{afii57680}{1504}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E0}{1504}
\DeclareTextGlyphY{LinBiolinum_R}{afii57681}{1505}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E1}{1505}
\DeclareTextGlyphY{LinBiolinum_R}{afii57682}{1506}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E2}{1506}
\DeclareTextGlyphY{LinBiolinum_R}{afii57683}{1507}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E3}{1507}
\DeclareTextGlyphY{LinBiolinum_R}{afii57684}{1508}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E4}{1508}
\DeclareTextGlyphY{LinBiolinum_R}{afii57685}{1509}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E5}{1509}
\DeclareTextGlyphY{LinBiolinum_R}{afii57686}{1510}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E6}{1510}
\DeclareTextGlyphY{LinBiolinum_R}{afii57687}{1511}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E7}{1511}
\DeclareTextGlyphY{LinBiolinum_R}{afii57688}{1512}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E8}{1512}
\DeclareTextGlyphY{LinBiolinum_R}{afii57689}{1513}
\DeclareTextGlyphY{LinBiolinum_R}{uni05E9}{1513}
\DeclareTextGlyphY{LinBiolinum_R}{afii57690}{1514}
\DeclareTextGlyphY{LinBiolinum_R}{uni05EA}{1514}
\DeclareTextGlyphY{LinBiolinum_R}{afii57716}{1520}
\DeclareTextGlyphY{LinBiolinum_R}{uni05F0}{1520}
\DeclareTextGlyphY{LinBiolinum_R}{afii57717}{1521}
\DeclareTextGlyphY{LinBiolinum_R}{uni05F1}{1521}
\DeclareTextGlyphY{LinBiolinum_R}{afii57718}{1522}
\DeclareTextGlyphY{LinBiolinum_R}{uni05F2}{1522}
\DeclareTextGlyphY{LinBiolinum_R}{uni05F3}{1523}
\DeclareTextGlyphY{LinBiolinum_R}{uni05F4}{1524}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D15}{7445}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D43}{7491}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D44}{7492}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D47}{7495}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D48}{7496}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D49}{7497}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D4A}{7498}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D4D}{7501}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D4E}{7502}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D4F}{7503}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D50}{7504}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D52}{7506}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D53}{7507}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D56}{7510}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D57}{7511}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D58}{7512}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D5A}{7514}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D5B}{7515}
\DeclareTextGlyphY{LinBiolinum_R}{uni1D9C}{7580}
\DeclareTextGlyphY{LinBiolinum_R}{uni1DA0}{7584}
\DeclareTextGlyphY{LinBiolinum_R}{uni1DBB}{7611}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E00}{7680}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E01}{7681}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E02}{7682}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E03}{7683}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E04}{7684}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E05}{7685}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E06}{7686}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E07}{7687}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E08}{7688}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E09}{7689}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E0A}{7690}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E0B}{7691}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E0C}{7692}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E0D}{7693}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E0E}{7694}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E0F}{7695}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E10}{7696}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E11}{7697}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E12}{7698}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E13}{7699}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E14}{7700}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E15}{7701}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E16}{7702}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E17}{7703}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E18}{7704}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E19}{7705}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E1A}{7706}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E1B}{7707}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E1C}{7708}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E1D}{7709}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E1E}{7710}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E1F}{7711}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E20}{7712}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E21}{7713}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E22}{7714}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E23}{7715}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E24}{7716}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E25}{7717}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E26}{7718}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E27}{7719}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E28}{7720}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E29}{7721}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E2A}{7722}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E2B}{7723}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E2C}{7724}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E2D}{7725}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E2E}{7726}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E2F}{7727}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E30}{7728}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E31}{7729}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E32}{7730}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E33}{7731}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E34}{7732}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E35}{7733}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E36}{7734}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E37}{7735}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E38}{7736}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E39}{7737}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E3A}{7738}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E3B}{7739}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E3C}{7740}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E3D}{7741}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E3E}{7742}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E3F}{7743}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E40}{7744}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E41}{7745}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E42}{7746}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E43}{7747}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E44}{7748}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E45}{7749}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E46}{7750}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E47}{7751}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E48}{7752}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E49}{7753}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E4A}{7754}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E4B}{7755}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E4C}{7756}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E4D}{7757}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E4E}{7758}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E4F}{7759}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E50}{7760}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E51}{7761}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E52}{7762}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E53}{7763}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E54}{7764}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E55}{7765}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E56}{7766}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E57}{7767}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E58}{7768}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E59}{7769}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E5A}{7770}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E5B}{7771}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E5C}{7772}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E5D}{7773}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E5E}{7774}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E5F}{7775}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E60}{7776}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E61}{7777}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E62}{7778}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E63}{7779}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E64}{7780}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E65}{7781}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E66}{7782}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E67}{7783}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E68}{7784}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E69}{7785}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E6A}{7786}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E6B}{7787}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E6C}{7788}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E6D}{7789}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E6E}{7790}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E6F}{7791}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E70}{7792}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E71}{7793}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E72}{7794}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E73}{7795}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E74}{7796}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E75}{7797}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E76}{7798}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E77}{7799}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E78}{7800}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E79}{7801}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E7A}{7802}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E7B}{7803}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E7C}{7804}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E7D}{7805}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E7E}{7806}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E7F}{7807}
\DeclareTextGlyphY{LinBiolinum_R}{Wgrave}{7808}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E80}{7808}
\DeclareTextGlyphY{LinBiolinum_R}{wgrave}{7809}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E81}{7809}
\DeclareTextGlyphY{LinBiolinum_R}{Wacute}{7810}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E82}{7810}
\DeclareTextGlyphY{LinBiolinum_R}{wacute}{7811}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E83}{7811}
\DeclareTextGlyphY{LinBiolinum_R}{Wdieresis}{7812}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E84}{7812}
\DeclareTextGlyphY{LinBiolinum_R}{wdieresis}{7813}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E85}{7813}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E86}{7814}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E87}{7815}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E88}{7816}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E89}{7817}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E8A}{7818}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E8B}{7819}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E8C}{7820}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E8D}{7821}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E8E}{7822}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E8F}{7823}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E90}{7824}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E91}{7825}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E92}{7826}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E93}{7827}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E94}{7828}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E95}{7829}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E96}{7830}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E97}{7831}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E98}{7832}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E99}{7833}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E9A}{7834}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E9B}{7835}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E9C}{7836}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E9D}{7837}
\DeclareTextGlyphY{LinBiolinum_R}{Germandbls}{7838}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E9E}{7838}
\DeclareTextGlyphY{LinBiolinum_R}{uni1E9F}{7839}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA0}{7840}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA1}{7841}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA2}{7842}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA3}{7843}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA4}{7844}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA5}{7845}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA6}{7846}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA7}{7847}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA8}{7848}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EA9}{7849}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EAA}{7850}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EAB}{7851}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EAC}{7852}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EAD}{7853}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EAE}{7854}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EAF}{7855}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB0}{7856}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB1}{7857}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB2}{7858}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB3}{7859}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB4}{7860}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB5}{7861}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB6}{7862}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB7}{7863}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB8}{7864}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EB9}{7865}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EBA}{7866}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EBB}{7867}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EBC}{7868}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EBD}{7869}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EBE}{7870}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EBF}{7871}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC0}{7872}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC1}{7873}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC2}{7874}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC3}{7875}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC4}{7876}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC5}{7877}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC6}{7878}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC7}{7879}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC8}{7880}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EC9}{7881}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ECA}{7882}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ECB}{7883}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ECC}{7884}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ECD}{7885}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ECE}{7886}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ECF}{7887}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED0}{7888}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED1}{7889}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED2}{7890}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED3}{7891}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED4}{7892}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED5}{7893}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED6}{7894}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED7}{7895}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED8}{7896}
\DeclareTextGlyphY{LinBiolinum_R}{uni1ED9}{7897}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EDA}{7898}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EDB}{7899}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EDC}{7900}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EDD}{7901}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EDE}{7902}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EDF}{7903}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE0}{7904}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE1}{7905}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE2}{7906}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE3}{7907}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE4}{7908}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE5}{7909}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE6}{7910}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE7}{7911}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE8}{7912}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EE9}{7913}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EEA}{7914}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EEB}{7915}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EEC}{7916}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EED}{7917}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EEE}{7918}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EEF}{7919}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF0}{7920}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF1}{7921}
\DeclareTextGlyphY{LinBiolinum_R}{Ygrave}{7922}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF2}{7922}
\DeclareTextGlyphY{LinBiolinum_R}{ygrave}{7923}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF3}{7923}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF4}{7924}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF5}{7925}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF6}{7926}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF7}{7927}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF8}{7928}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EF9}{7929}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EFA}{7930}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EFB}{7931}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EFC}{7932}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EFD}{7933}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EFE}{7934}
\DeclareTextGlyphY{LinBiolinum_R}{uni1EFF}{7935}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F00}{7936}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F01}{7937}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F02}{7938}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F03}{7939}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F04}{7940}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F05}{7941}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F06}{7942}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F07}{7943}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F08}{7944}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F09}{7945}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F0A}{7946}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F0B}{7947}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F0C}{7948}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F0D}{7949}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F0E}{7950}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F0F}{7951}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F10}{7952}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F11}{7953}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F12}{7954}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F13}{7955}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F14}{7956}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F15}{7957}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F18}{7960}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F19}{7961}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F1A}{7962}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F1B}{7963}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F1C}{7964}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F1D}{7965}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F20}{7968}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F21}{7969}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F22}{7970}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F23}{7971}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F24}{7972}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F25}{7973}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F26}{7974}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F27}{7975}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F28}{7976}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F29}{7977}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F2A}{7978}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F2B}{7979}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F2C}{7980}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F2D}{7981}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F2E}{7982}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F2F}{7983}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F30}{7984}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F31}{7985}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F32}{7986}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F33}{7987}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F34}{7988}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F35}{7989}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F36}{7990}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F37}{7991}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F38}{7992}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F39}{7993}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F3A}{7994}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F3B}{7995}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F3C}{7996}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F3D}{7997}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F3E}{7998}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F3F}{7999}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F40}{8000}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F41}{8001}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F42}{8002}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F43}{8003}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F44}{8004}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F45}{8005}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F48}{8008}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F49}{8009}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F4A}{8010}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F4B}{8011}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F4C}{8012}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F4D}{8013}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F50}{8016}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F51}{8017}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F52}{8018}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F53}{8019}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F54}{8020}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F55}{8021}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F56}{8022}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F57}{8023}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F59}{8025}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F5B}{8027}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F5D}{8029}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F5F}{8031}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F60}{8032}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F61}{8033}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F62}{8034}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F63}{8035}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F64}{8036}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F65}{8037}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F66}{8038}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F67}{8039}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F68}{8040}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F69}{8041}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F6A}{8042}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F6B}{8043}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F6C}{8044}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F6D}{8045}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F6E}{8046}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F6F}{8047}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F70}{8048}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F71}{8049}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F72}{8050}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F73}{8051}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F74}{8052}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F75}{8053}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F76}{8054}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F77}{8055}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F78}{8056}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F79}{8057}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F7A}{8058}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F7B}{8059}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F7C}{8060}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F7D}{8061}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F80}{8064}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F81}{8065}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F82}{8066}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F83}{8067}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F84}{8068}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F85}{8069}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F86}{8070}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F87}{8071}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F88}{8072}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F89}{8073}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F8A}{8074}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F8B}{8075}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F8C}{8076}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F8D}{8077}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F8E}{8078}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F8F}{8079}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F90}{8080}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F91}{8081}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F92}{8082}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F93}{8083}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F94}{8084}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F95}{8085}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F96}{8086}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F97}{8087}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F98}{8088}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F99}{8089}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F9A}{8090}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F9B}{8091}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F9C}{8092}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F9D}{8093}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F9E}{8094}
\DeclareTextGlyphY{LinBiolinum_R}{uni1F9F}{8095}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA0}{8096}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA1}{8097}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA2}{8098}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA3}{8099}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA4}{8100}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA5}{8101}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA6}{8102}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA7}{8103}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA8}{8104}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FA9}{8105}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FAA}{8106}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FAB}{8107}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FAC}{8108}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FAD}{8109}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FAE}{8110}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FAF}{8111}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB0}{8112}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB1}{8113}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB2}{8114}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB3}{8115}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB4}{8116}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB6}{8118}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB7}{8119}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB8}{8120}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FB9}{8121}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FBA}{8122}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FBB}{8123}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FBC}{8124}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FBD}{8125}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FBE}{8126}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FBF}{8127}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC0}{8128}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC1}{8129}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC2}{8130}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC3}{8131}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC4}{8132}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC6}{8134}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC7}{8135}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC8}{8136}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FC9}{8137}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FCA}{8138}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FCB}{8139}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FCC}{8140}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FCD}{8141}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FCE}{8142}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FCF}{8143}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FD0}{8144}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FD1}{8145}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FD2}{8146}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FD3}{8147}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FD6}{8150}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FD7}{8151}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FD8}{8152}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FD9}{8153}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FDA}{8154}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FDB}{8155}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FDD}{8157}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FDE}{8158}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FDF}{8159}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE0}{8160}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE1}{8161}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE2}{8162}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE3}{8163}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE4}{8164}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE5}{8165}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE6}{8166}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE7}{8167}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE8}{8168}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FE9}{8169}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FEA}{8170}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FEB}{8171}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FEC}{8172}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FED}{8173}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FEE}{8174}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FEF}{8175}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FF2}{8178}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FF3}{8179}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FF4}{8180}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FF6}{8182}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FF7}{8183}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FF8}{8184}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FF9}{8185}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FFA}{8186}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FFB}{8187}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FFC}{8188}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FFD}{8189}
\DeclareTextGlyphY{LinBiolinum_R}{uni1FFE}{8190}
\DeclareTextGlyphY{LinBiolinum_R}{enquad}{8192}
\DeclareTextGlyphY{LinBiolinum_R}{uni2000}{8192}
\DeclareTextGlyphY{LinBiolinum_R}{emquad}{8193}
\DeclareTextGlyphY{LinBiolinum_R}{uni2001}{8193}
\DeclareTextGlyphY{LinBiolinum_R}{enspace}{8194}
\DeclareTextGlyphY{LinBiolinum_R}{uni2002}{8194}
\DeclareTextGlyphY{LinBiolinum_R}{emspace}{8195}
\DeclareTextGlyphY{LinBiolinum_R}{uni2003}{8195}
\DeclareTextGlyphY{LinBiolinum_R}{threeperemspace}{8196}
\DeclareTextGlyphY{LinBiolinum_R}{uni2004}{8196}
\DeclareTextGlyphY{LinBiolinum_R}{fourperemspace}{8197}
\DeclareTextGlyphY{LinBiolinum_R}{uni2005}{8197}
\DeclareTextGlyphY{LinBiolinum_R}{sixperemspace}{8198}
\DeclareTextGlyphY{LinBiolinum_R}{uni2006}{8198}
\DeclareTextGlyphY{LinBiolinum_R}{figurespace}{8199}
\DeclareTextGlyphY{LinBiolinum_R}{uni2007}{8199}
\DeclareTextGlyphY{LinBiolinum_R}{punctuationspace}{8200}
\DeclareTextGlyphY{LinBiolinum_R}{uni2008}{8200}
\DeclareTextGlyphY{LinBiolinum_R}{thinspace}{8201}
\DeclareTextGlyphY{LinBiolinum_R}{uni2009}{8201}
\DeclareTextGlyphY{LinBiolinum_R}{hairspace}{8202}
\DeclareTextGlyphY{LinBiolinum_R}{uni200A}{8202}
\DeclareTextGlyphY{LinBiolinum_R}{zerowidthspace}{8203}
\DeclareTextGlyphY{LinBiolinum_R}{uni200B}{8203}
\DeclareTextGlyphY{LinBiolinum_R}{hyphentwo}{8208}
\DeclareTextGlyphY{LinBiolinum_R}{uni2010}{8208}
\DeclareTextGlyphY{LinBiolinum_R}{hyphennobreak}{8209}
\DeclareTextGlyphY{LinBiolinum_R}{uni2011}{8209}
\DeclareTextGlyphY{LinBiolinum_R}{figuredash}{8210}
\DeclareTextGlyphY{LinBiolinum_R}{uni2012}{8210}
\DeclareTextGlyphY{LinBiolinum_R}{endash}{8211}
\DeclareTextGlyphY{LinBiolinum_R}{uni2013}{8211}
\DeclareTextGlyphY{LinBiolinum_R}{emdash}{8212}
\DeclareTextGlyphY{LinBiolinum_R}{uni2014}{8212}
\DeclareTextGlyphY{LinBiolinum_R}{horizontalbar}{8213}
\DeclareTextGlyphY{LinBiolinum_R}{uni2015}{8213}
\DeclareTextGlyphY{LinBiolinum_R}{uni2016}{8214}
\DeclareTextGlyphY{LinBiolinum_R}{underscoredbl}{8215}
\DeclareTextGlyphY{LinBiolinum_R}{uni2017}{8215}
\DeclareTextGlyphY{LinBiolinum_R}{quoteleft}{8216}
\DeclareTextGlyphY{LinBiolinum_R}{uni2018}{8216}
\DeclareTextGlyphY{LinBiolinum_R}{quoteright}{8217}
\DeclareTextGlyphY{LinBiolinum_R}{uni2019}{8217}
\DeclareTextGlyphY{LinBiolinum_R}{quotesinglbase}{8218}
\DeclareTextGlyphY{LinBiolinum_R}{uni201A}{8218}
\DeclareTextGlyphY{LinBiolinum_R}{quotereversed}{8219}
\DeclareTextGlyphY{LinBiolinum_R}{uni201B}{8219}
\DeclareTextGlyphY{LinBiolinum_R}{quotedblleft}{8220}
\DeclareTextGlyphY{LinBiolinum_R}{uni201C}{8220}
\DeclareTextGlyphY{LinBiolinum_R}{quotedblright}{8221}
\DeclareTextGlyphY{LinBiolinum_R}{uni201D}{8221}
\DeclareTextGlyphY{LinBiolinum_R}{quotedblbase}{8222}
\DeclareTextGlyphY{LinBiolinum_R}{uni201E}{8222}
\DeclareTextGlyphY{LinBiolinum_R}{quotedblrev}{8223}
\DeclareTextGlyphY{LinBiolinum_R}{uni201F}{8223}
\DeclareTextGlyphY{LinBiolinum_R}{dagger}{8224}
\DeclareTextGlyphY{LinBiolinum_R}{uni2020}{8224}
\DeclareTextGlyphY{LinBiolinum_R}{daggerdbl}{8225}
\DeclareTextGlyphY{LinBiolinum_R}{uni2021}{8225}
\DeclareTextGlyphY{LinBiolinum_R}{bullet}{8226}
\DeclareTextGlyphY{LinBiolinum_R}{uni2022}{8226}
\DeclareTextGlyphY{LinBiolinum_R}{trianglebullet}{8227}
\DeclareTextGlyphY{LinBiolinum_R}{uni2023}{8227}
\DeclareTextGlyphY{LinBiolinum_R}{onedotenleader}{8228}
\DeclareTextGlyphY{LinBiolinum_R}{uni2024}{8228}
\DeclareTextGlyphY{LinBiolinum_R}{twodotenleader}{8229}
\DeclareTextGlyphY{LinBiolinum_R}{uni2025}{8229}
\DeclareTextGlyphY{LinBiolinum_R}{ellipsis}{8230}
\DeclareTextGlyphY{LinBiolinum_R}{uni2026}{8230}
\DeclareTextGlyphY{LinBiolinum_R}{hyphendot}{8231}
\DeclareTextGlyphY{LinBiolinum_R}{uni2027}{8231}
\DeclareTextGlyphY{LinBiolinum_R}{uni202F}{8239}
\DeclareTextGlyphY{LinBiolinum_R}{perthousand}{8240}
\DeclareTextGlyphY{LinBiolinum_R}{uni2030}{8240}
\DeclareTextGlyphY{LinBiolinum_R}{uni2031}{8241}
\DeclareTextGlyphY{LinBiolinum_R}{minute}{8242}
\DeclareTextGlyphY{LinBiolinum_R}{uni2032}{8242}
\DeclareTextGlyphY{LinBiolinum_R}{second}{8243}
\DeclareTextGlyphY{LinBiolinum_R}{uni2033}{8243}
\DeclareTextGlyphY{LinBiolinum_R}{primetriple}{8244}
\DeclareTextGlyphY{LinBiolinum_R}{uni2034}{8244}
\DeclareTextGlyphY{LinBiolinum_R}{primereversed}{8245}
\DeclareTextGlyphY{LinBiolinum_R}{uni2035}{8245}
\DeclareTextGlyphY{LinBiolinum_R}{uni2036}{8246}
\DeclareTextGlyphY{LinBiolinum_R}{uni2037}{8247}
\DeclareTextGlyphY{LinBiolinum_R}{guilsinglleft}{8249}
\DeclareTextGlyphY{LinBiolinum_R}{uni2039}{8249}
\DeclareTextGlyphY{LinBiolinum_R}{guilsinglright}{8250}
\DeclareTextGlyphY{LinBiolinum_R}{uni203A}{8250}
\DeclareTextGlyphY{LinBiolinum_R}{uni203B}{8251}
\DeclareTextGlyphY{LinBiolinum_R}{exclamdbl}{8252}
\DeclareTextGlyphY{LinBiolinum_R}{uni203C}{8252}
\DeclareTextGlyphY{LinBiolinum_R}{interrobang}{8253}
\DeclareTextGlyphY{LinBiolinum_R}{uni203D}{8253}
\DeclareTextGlyphY{LinBiolinum_R}{uni203E}{8254}
\DeclareTextGlyphY{LinBiolinum_R}{uni2042}{8258}
\DeclareTextGlyphY{LinBiolinum_R}{fraction}{8260}
\DeclareTextGlyphY{LinBiolinum_R}{uni2044}{8260}
\DeclareTextGlyphY{LinBiolinum_R}{question_question}{8263}
\DeclareTextGlyphY{LinBiolinum_R}{uni2047}{8263}
\DeclareTextGlyphY{LinBiolinum_R}{question_exclam}{8264}
\DeclareTextGlyphY{LinBiolinum_R}{uni2048}{8264}
\DeclareTextGlyphY{LinBiolinum_R}{exclam_question}{8265}
\DeclareTextGlyphY{LinBiolinum_R}{uni2049}{8265}
\DeclareTextGlyphY{LinBiolinum_R}{uni204A}{8266}
\DeclareTextGlyphY{LinBiolinum_R}{uni204B}{8267}
\DeclareTextGlyphY{LinBiolinum_R}{uni204F}{8271}
\DeclareTextGlyphY{LinBiolinum_R}{zero.superior}{8304}
\DeclareTextGlyphY{LinBiolinum_R}{uni2070}{8304}
\DeclareTextGlyphY{LinBiolinum_R}{i.superior}{8305}
\DeclareTextGlyphY{LinBiolinum_R}{uni2071}{8305}
\DeclareTextGlyphY{LinBiolinum_R}{four.superior}{8308}
\DeclareTextGlyphY{LinBiolinum_R}{uni2074}{8308}
\DeclareTextGlyphY{LinBiolinum_R}{five.superior}{8309}
\DeclareTextGlyphY{LinBiolinum_R}{uni2075}{8309}
\DeclareTextGlyphY{LinBiolinum_R}{six.superior}{8310}
\DeclareTextGlyphY{LinBiolinum_R}{uni2076}{8310}
\DeclareTextGlyphY{LinBiolinum_R}{seven.superior}{8311}
\DeclareTextGlyphY{LinBiolinum_R}{uni2077}{8311}
\DeclareTextGlyphY{LinBiolinum_R}{eight.superior}{8312}
\DeclareTextGlyphY{LinBiolinum_R}{uni2078}{8312}
\DeclareTextGlyphY{LinBiolinum_R}{nine.superior}{8313}
\DeclareTextGlyphY{LinBiolinum_R}{uni2079}{8313}
\DeclareTextGlyphY{LinBiolinum_R}{plus.superior}{8314}
\DeclareTextGlyphY{LinBiolinum_R}{uni207A}{8314}
\DeclareTextGlyphY{LinBiolinum_R}{minus.superior}{8315}
\DeclareTextGlyphY{LinBiolinum_R}{uni207B}{8315}
\DeclareTextGlyphY{LinBiolinum_R}{equal.superior}{8316}
\DeclareTextGlyphY{LinBiolinum_R}{uni207C}{8316}
\DeclareTextGlyphY{LinBiolinum_R}{parenleft.superior}{8317}
\DeclareTextGlyphY{LinBiolinum_R}{uni207D}{8317}
\DeclareTextGlyphY{LinBiolinum_R}{parenright.superior}{8318}
\DeclareTextGlyphY{LinBiolinum_R}{uni207E}{8318}
\DeclareTextGlyphY{LinBiolinum_R}{n.superior}{8319}
\DeclareTextGlyphY{LinBiolinum_R}{uni207F}{8319}
\DeclareTextGlyphY{LinBiolinum_R}{zero.inferior}{8320}
\DeclareTextGlyphY{LinBiolinum_R}{uni2080}{8320}
\DeclareTextGlyphY{LinBiolinum_R}{one.inferior}{8321}
\DeclareTextGlyphY{LinBiolinum_R}{uni2081}{8321}
\DeclareTextGlyphY{LinBiolinum_R}{two.inferior}{8322}
\DeclareTextGlyphY{LinBiolinum_R}{uni2082}{8322}
\DeclareTextGlyphY{LinBiolinum_R}{three.inferior}{8323}
\DeclareTextGlyphY{LinBiolinum_R}{uni2083}{8323}
\DeclareTextGlyphY{LinBiolinum_R}{four.inferior}{8324}
\DeclareTextGlyphY{LinBiolinum_R}{uni2084}{8324}
\DeclareTextGlyphY{LinBiolinum_R}{five.inferior}{8325}
\DeclareTextGlyphY{LinBiolinum_R}{uni2085}{8325}
\DeclareTextGlyphY{LinBiolinum_R}{six.inferior}{8326}
\DeclareTextGlyphY{LinBiolinum_R}{uni2086}{8326}
\DeclareTextGlyphY{LinBiolinum_R}{seven.inferior}{8327}
\DeclareTextGlyphY{LinBiolinum_R}{uni2087}{8327}
\DeclareTextGlyphY{LinBiolinum_R}{eight.inferior}{8328}
\DeclareTextGlyphY{LinBiolinum_R}{uni2088}{8328}
\DeclareTextGlyphY{LinBiolinum_R}{nine.inferior}{8329}
\DeclareTextGlyphY{LinBiolinum_R}{uni2089}{8329}
\DeclareTextGlyphY{LinBiolinum_R}{plus.inferior}{8330}
\DeclareTextGlyphY{LinBiolinum_R}{uni208A}{8330}
\DeclareTextGlyphY{LinBiolinum_R}{minus.inferior}{8331}
\DeclareTextGlyphY{LinBiolinum_R}{uni208B}{8331}
\DeclareTextGlyphY{LinBiolinum_R}{equal.inferior}{8332}
\DeclareTextGlyphY{LinBiolinum_R}{uni208C}{8332}
\DeclareTextGlyphY{LinBiolinum_R}{parenleft.inferior}{8333}
\DeclareTextGlyphY{LinBiolinum_R}{uni208D}{8333}
\DeclareTextGlyphY{LinBiolinum_R}{parenright.inferior}{8334}
\DeclareTextGlyphY{LinBiolinum_R}{uni208E}{8334}
\DeclareTextGlyphY{LinBiolinum_R}{a.inferior}{8336}
\DeclareTextGlyphY{LinBiolinum_R}{uni2090}{8336}
\DeclareTextGlyphY{LinBiolinum_R}{e.inferior}{8337}
\DeclareTextGlyphY{LinBiolinum_R}{uni2091}{8337}
\DeclareTextGlyphY{LinBiolinum_R}{o.inferior}{8338}
\DeclareTextGlyphY{LinBiolinum_R}{uni2092}{8338}
\DeclareTextGlyphY{LinBiolinum_R}{x.inferior}{8339}
\DeclareTextGlyphY{LinBiolinum_R}{uni2093}{8339}
\DeclareTextGlyphY{LinBiolinum_R}{uni2094}{8340}
\DeclareTextGlyphY{LinBiolinum_R}{uni2095}{8341}
\DeclareTextGlyphY{LinBiolinum_R}{uni2096}{8342}
\DeclareTextGlyphY{LinBiolinum_R}{uni2097}{8343}
\DeclareTextGlyphY{LinBiolinum_R}{uni2098}{8344}
\DeclareTextGlyphY{LinBiolinum_R}{uni2099}{8345}
\DeclareTextGlyphY{LinBiolinum_R}{uni209A}{8346}
\DeclareTextGlyphY{LinBiolinum_R}{uni209B}{8347}
\DeclareTextGlyphY{LinBiolinum_R}{uni209C}{8348}
\DeclareTextGlyphY{LinBiolinum_R}{uni20A2}{8354}
\DeclareTextGlyphY{LinBiolinum_R}{franc}{8355}
\DeclareTextGlyphY{LinBiolinum_R}{uni20A3}{8355}
\DeclareTextGlyphY{LinBiolinum_R}{lira}{8356}
\DeclareTextGlyphY{LinBiolinum_R}{uni20A4}{8356}
\DeclareTextGlyphY{LinBiolinum_R}{peseta}{8359}
\DeclareTextGlyphY{LinBiolinum_R}{uni20A7}{8359}
\DeclareTextGlyphY{LinBiolinum_R}{uni20A8}{8360}
\DeclareTextGlyphY{LinBiolinum_R}{dong}{8363}
\DeclareTextGlyphY{LinBiolinum_R}{uni20AB}{8363}
\DeclareTextGlyphY{LinBiolinum_R}{Euro}{8364}
\DeclareTextGlyphY{LinBiolinum_R}{uni20AC}{8364}
\DeclareTextGlyphY{LinBiolinum_R}{uni20AF}{8367}
\DeclareTextGlyphY{LinBiolinum_R}{uni20B1}{8369}
\DeclareTextGlyphY{LinBiolinum_R}{uni2100}{8448}
\DeclareTextGlyphY{LinBiolinum_R}{uni2101}{8449}
\DeclareTextGlyphY{LinBiolinum_R}{uni2102}{8450}
\DeclareTextGlyphY{LinBiolinum_R}{centigrade}{8451}
\DeclareTextGlyphY{LinBiolinum_R}{uni2103}{8451}
\DeclareTextGlyphY{LinBiolinum_R}{afii61248}{8453}
\DeclareTextGlyphY{LinBiolinum_R}{uni2105}{8453}
\DeclareTextGlyphY{LinBiolinum_R}{uni2106}{8454}
\DeclareTextGlyphY{LinBiolinum_R}{fahrenheit}{8457}
\DeclareTextGlyphY{LinBiolinum_R}{uni2109}{8457}
\DeclareTextGlyphY{LinBiolinum_R}{uni210C}{8460}
\DeclareTextGlyphY{LinBiolinum_R}{uni210D}{8461}
\DeclareTextGlyphY{LinBiolinum_R}{uni210E}{8462}
\DeclareTextGlyphY{LinBiolinum_R}{uni210F}{8463}
\DeclareTextGlyphY{LinBiolinum_R}{Ifraktur}{8465}
\DeclareTextGlyphY{LinBiolinum_R}{uni2111}{8465}
\DeclareTextGlyphY{LinBiolinum_R}{afii61289}{8467}
\DeclareTextGlyphY{LinBiolinum_R}{uni2113}{8467}
\DeclareTextGlyphY{LinBiolinum_R}{uni2115}{8469}
\DeclareTextGlyphY{LinBiolinum_R}{afii61352}{8470}
\DeclareTextGlyphY{LinBiolinum_R}{uni2116}{8470}
\DeclareTextGlyphY{LinBiolinum_R}{uni2119}{8473}
\DeclareTextGlyphY{LinBiolinum_R}{uni211A}{8474}
\DeclareTextGlyphY{LinBiolinum_R}{Rfraktur}{8476}
\DeclareTextGlyphY{LinBiolinum_R}{uni211C}{8476}
\DeclareTextGlyphY{LinBiolinum_R}{uni211D}{8477}
\DeclareTextGlyphY{LinBiolinum_R}{uni2120}{8480}
\DeclareTextGlyphY{LinBiolinum_R}{trademark}{8482}
\DeclareTextGlyphY{LinBiolinum_R}{uni2122}{8482}
\DeclareTextGlyphY{LinBiolinum_R}{uni2124}{8484}
\DeclareTextGlyphY{LinBiolinum_R}{uni2126}{8486}
\DeclareTextGlyphY{LinBiolinum_R}{uni2127}{8487}
\DeclareTextGlyphY{LinBiolinum_R}{estimated}{8494}
\DeclareTextGlyphY{LinBiolinum_R}{uni212E}{8494}
\DeclareTextGlyphY{LinBiolinum_R}{aleph}{8501}
\DeclareTextGlyphY{LinBiolinum_R}{uni2135}{8501}
\DeclareTextGlyphY{LinBiolinum_R}{uni2136}{8502}
\DeclareTextGlyphY{LinBiolinum_R}{uni2137}{8503}
\DeclareTextGlyphY{LinBiolinum_R}{uni2138}{8504}
\DeclareTextGlyphY{LinBiolinum_R}{uni2139}{8505}
\DeclareTextGlyphY{LinBiolinum_R}{uni214F}{8527}
\DeclareTextGlyphY{LinBiolinum_R}{onethird}{8531}
\DeclareTextGlyphY{LinBiolinum_R}{uni2153}{8531}
\DeclareTextGlyphY{LinBiolinum_R}{twothirds}{8532}
\DeclareTextGlyphY{LinBiolinum_R}{uni2154}{8532}
\DeclareTextGlyphY{LinBiolinum_R}{onefifth}{8533}
\DeclareTextGlyphY{LinBiolinum_R}{uni2155}{8533}
\DeclareTextGlyphY{LinBiolinum_R}{twofifths}{8534}
\DeclareTextGlyphY{LinBiolinum_R}{uni2156}{8534}
\DeclareTextGlyphY{LinBiolinum_R}{threefifths}{8535}
\DeclareTextGlyphY{LinBiolinum_R}{uni2157}{8535}
\DeclareTextGlyphY{LinBiolinum_R}{fourfifths}{8536}
\DeclareTextGlyphY{LinBiolinum_R}{uni2158}{8536}
\DeclareTextGlyphY{LinBiolinum_R}{onesixth}{8537}
\DeclareTextGlyphY{LinBiolinum_R}{uni2159}{8537}
\DeclareTextGlyphY{LinBiolinum_R}{fivesixths}{8538}
\DeclareTextGlyphY{LinBiolinum_R}{uni215A}{8538}
\DeclareTextGlyphY{LinBiolinum_R}{oneeighth}{8539}
\DeclareTextGlyphY{LinBiolinum_R}{uni215B}{8539}
\DeclareTextGlyphY{LinBiolinum_R}{threeeighths}{8540}
\DeclareTextGlyphY{LinBiolinum_R}{uni215C}{8540}
\DeclareTextGlyphY{LinBiolinum_R}{fiveeighths}{8541}
\DeclareTextGlyphY{LinBiolinum_R}{uni215D}{8541}
\DeclareTextGlyphY{LinBiolinum_R}{seveneighths}{8542}
\DeclareTextGlyphY{LinBiolinum_R}{uni215E}{8542}
\DeclareTextGlyphY{LinBiolinum_R}{onenumerator}{8543}
\DeclareTextGlyphY{LinBiolinum_R}{uni215F}{8543}
\DeclareTextGlyphY{LinBiolinum_R}{Oneroman}{8544}
\DeclareTextGlyphY{LinBiolinum_R}{uni2160}{8544}
\DeclareTextGlyphY{LinBiolinum_R}{Tworoman}{8545}
\DeclareTextGlyphY{LinBiolinum_R}{uni2161}{8545}
\DeclareTextGlyphY{LinBiolinum_R}{Threeroman}{8546}
\DeclareTextGlyphY{LinBiolinum_R}{uni2162}{8546}
\DeclareTextGlyphY{LinBiolinum_R}{Fourroman}{8547}
\DeclareTextGlyphY{LinBiolinum_R}{uni2163}{8547}
\DeclareTextGlyphY{LinBiolinum_R}{Fiveroman}{8548}
\DeclareTextGlyphY{LinBiolinum_R}{uni2164}{8548}
\DeclareTextGlyphY{LinBiolinum_R}{Sixroman}{8549}
\DeclareTextGlyphY{LinBiolinum_R}{uni2165}{8549}
\DeclareTextGlyphY{LinBiolinum_R}{Sevenroman}{8550}
\DeclareTextGlyphY{LinBiolinum_R}{uni2166}{8550}
\DeclareTextGlyphY{LinBiolinum_R}{Eightroman}{8551}
\DeclareTextGlyphY{LinBiolinum_R}{uni2167}{8551}
\DeclareTextGlyphY{LinBiolinum_R}{Nineroman}{8552}
\DeclareTextGlyphY{LinBiolinum_R}{uni2168}{8552}
\DeclareTextGlyphY{LinBiolinum_R}{Tenroman}{8553}
\DeclareTextGlyphY{LinBiolinum_R}{uni2169}{8553}
\DeclareTextGlyphY{LinBiolinum_R}{Elevenroman}{8554}
\DeclareTextGlyphY{LinBiolinum_R}{uni216A}{8554}
\DeclareTextGlyphY{LinBiolinum_R}{Twelveroman}{8555}
\DeclareTextGlyphY{LinBiolinum_R}{uni216B}{8555}
\DeclareTextGlyphY{LinBiolinum_R}{uni216C}{8556}
\DeclareTextGlyphY{LinBiolinum_R}{uni216D}{8557}
\DeclareTextGlyphY{LinBiolinum_R}{uni216E}{8558}
\DeclareTextGlyphY{LinBiolinum_R}{uni216F}{8559}
\DeclareTextGlyphY{LinBiolinum_R}{oneroman}{8560}
\DeclareTextGlyphY{LinBiolinum_R}{uni2170}{8560}
\DeclareTextGlyphY{LinBiolinum_R}{tworoman}{8561}
\DeclareTextGlyphY{LinBiolinum_R}{uni2171}{8561}
\DeclareTextGlyphY{LinBiolinum_R}{threeroman}{8562}
\DeclareTextGlyphY{LinBiolinum_R}{uni2172}{8562}
\DeclareTextGlyphY{LinBiolinum_R}{fourroman}{8563}
\DeclareTextGlyphY{LinBiolinum_R}{uni2173}{8563}
\DeclareTextGlyphY{LinBiolinum_R}{fiveroman}{8564}
\DeclareTextGlyphY{LinBiolinum_R}{uni2174}{8564}
\DeclareTextGlyphY{LinBiolinum_R}{sixroman}{8565}
\DeclareTextGlyphY{LinBiolinum_R}{uni2175}{8565}
\DeclareTextGlyphY{LinBiolinum_R}{sevenroman}{8566}
\DeclareTextGlyphY{LinBiolinum_R}{uni2176}{8566}
\DeclareTextGlyphY{LinBiolinum_R}{eightroman}{8567}
\DeclareTextGlyphY{LinBiolinum_R}{uni2177}{8567}
\DeclareTextGlyphY{LinBiolinum_R}{nineroman}{8568}
\DeclareTextGlyphY{LinBiolinum_R}{uni2178}{8568}
\DeclareTextGlyphY{LinBiolinum_R}{tenroman}{8569}
\DeclareTextGlyphY{LinBiolinum_R}{uni2179}{8569}
\DeclareTextGlyphY{LinBiolinum_R}{elevenroman}{8570}
\DeclareTextGlyphY{LinBiolinum_R}{uni217A}{8570}
\DeclareTextGlyphY{LinBiolinum_R}{twelveroman}{8571}
\DeclareTextGlyphY{LinBiolinum_R}{uni217B}{8571}
\DeclareTextGlyphY{LinBiolinum_R}{uni217C}{8572}
\DeclareTextGlyphY{LinBiolinum_R}{uni217D}{8573}
\DeclareTextGlyphY{LinBiolinum_R}{uni217E}{8574}
\DeclareTextGlyphY{LinBiolinum_R}{uni217F}{8575}
\DeclareTextGlyphY{LinBiolinum_R}{arrowleft}{8592}
\DeclareTextGlyphY{LinBiolinum_R}{uni2190}{8592}
\DeclareTextGlyphY{LinBiolinum_R}{arrowup}{8593}
\DeclareTextGlyphY{LinBiolinum_R}{uni2191}{8593}
\DeclareTextGlyphY{LinBiolinum_R}{arrowright}{8594}
\DeclareTextGlyphY{LinBiolinum_R}{uni2192}{8594}
\DeclareTextGlyphY{LinBiolinum_R}{arrowdown}{8595}
\DeclareTextGlyphY{LinBiolinum_R}{uni2193}{8595}
\DeclareTextGlyphY{LinBiolinum_R}{arrowboth}{8596}
\DeclareTextGlyphY{LinBiolinum_R}{uni2194}{8596}
\DeclareTextGlyphY{LinBiolinum_R}{arrowupdn}{8597}
\DeclareTextGlyphY{LinBiolinum_R}{uni2195}{8597}
\DeclareTextGlyphY{LinBiolinum_R}{uni2196}{8598}
\DeclareTextGlyphY{LinBiolinum_R}{uni2197}{8599}
\DeclareTextGlyphY{LinBiolinum_R}{uni2198}{8600}
\DeclareTextGlyphY{LinBiolinum_R}{uni2199}{8601}
\DeclareTextGlyphY{LinBiolinum_R}{uni219A}{8602}
\DeclareTextGlyphY{LinBiolinum_R}{uni219B}{8603}
\DeclareTextGlyphY{LinBiolinum_R}{uni21A6}{8614}
\DeclareTextGlyphY{LinBiolinum_R}{arrowupdnbse}{8616}
\DeclareTextGlyphY{LinBiolinum_R}{uni21A8}{8616}
\DeclareTextGlyphY{LinBiolinum_R}{uni21AE}{8622}
\DeclareTextGlyphY{LinBiolinum_R}{uni21BC}{8636}
\DeclareTextGlyphY{LinBiolinum_R}{uni21BD}{8637}
\DeclareTextGlyphY{LinBiolinum_R}{uni21C0}{8640}
\DeclareTextGlyphY{LinBiolinum_R}{uni21C1}{8641}
\DeclareTextGlyphY{LinBiolinum_R}{uni21CB}{8651}
\DeclareTextGlyphY{LinBiolinum_R}{uni21CC}{8652}
\DeclareTextGlyphY{LinBiolinum_R}{uni21CD}{8653}
\DeclareTextGlyphY{LinBiolinum_R}{uni21CE}{8654}
\DeclareTextGlyphY{LinBiolinum_R}{uni21CF}{8655}
\DeclareTextGlyphY{LinBiolinum_R}{arrowdblleft}{8656}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D0}{8656}
\DeclareTextGlyphY{LinBiolinum_R}{arrowdblup}{8657}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D1}{8657}
\DeclareTextGlyphY{LinBiolinum_R}{arrowdblright}{8658}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D2}{8658}
\DeclareTextGlyphY{LinBiolinum_R}{arrowdbldown}{8659}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D3}{8659}
\DeclareTextGlyphY{LinBiolinum_R}{arrowdblboth}{8660}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D4}{8660}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D5}{8661}
\DeclareTextGlyphY{LinBiolinum_R}{Nwarrow}{8662}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D6}{8662}
\DeclareTextGlyphY{LinBiolinum_R}{Nearrow}{8663}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D7}{8663}
\DeclareTextGlyphY{LinBiolinum_R}{Searrow}{8664}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D8}{8664}
\DeclareTextGlyphY{LinBiolinum_R}{Swarrow}{8665}
\DeclareTextGlyphY{LinBiolinum_R}{uni21D9}{8665}
\DeclareTextGlyphY{LinBiolinum_R}{uni2200}{8704}
\DeclareTextGlyphY{LinBiolinum_R}{uni2201}{8705}
\DeclareTextGlyphY{LinBiolinum_R}{partialdiff}{8706}
\DeclareTextGlyphY{LinBiolinum_R}{uni2202}{8706}
\DeclareTextGlyphY{LinBiolinum_R}{existential}{8707}
\DeclareTextGlyphY{LinBiolinum_R}{uni2203}{8707}
\DeclareTextGlyphY{LinBiolinum_R}{uni2204}{8708}
\DeclareTextGlyphY{LinBiolinum_R}{emptyset}{8709}
\DeclareTextGlyphY{LinBiolinum_R}{uni2205}{8709}
\DeclareTextGlyphY{LinBiolinum_R}{uni2206}{8710}
\DeclareTextGlyphY{LinBiolinum_R}{gradient}{8711}
\DeclareTextGlyphY{LinBiolinum_R}{uni2207}{8711}
\DeclareTextGlyphY{LinBiolinum_R}{element}{8712}
\DeclareTextGlyphY{LinBiolinum_R}{uni2208}{8712}
\DeclareTextGlyphY{LinBiolinum_R}{notelement}{8713}
\DeclareTextGlyphY{LinBiolinum_R}{uni2209}{8713}
\DeclareTextGlyphY{LinBiolinum_R}{uni220A}{8714}
\DeclareTextGlyphY{LinBiolinum_R}{suchthat}{8715}
\DeclareTextGlyphY{LinBiolinum_R}{uni220B}{8715}
\DeclareTextGlyphY{LinBiolinum_R}{uni220C}{8716}
\DeclareTextGlyphY{LinBiolinum_R}{uni220D}{8717}
\DeclareTextGlyphY{LinBiolinum_R}{product}{8719}
\DeclareTextGlyphY{LinBiolinum_R}{uni220F}{8719}
\DeclareTextGlyphY{LinBiolinum_R}{uni2210}{8720}
\DeclareTextGlyphY{LinBiolinum_R}{summation}{8721}
\DeclareTextGlyphY{LinBiolinum_R}{uni2211}{8721}
\DeclareTextGlyphY{LinBiolinum_R}{minus}{8722}
\DeclareTextGlyphY{LinBiolinum_R}{uni2212}{8722}
\DeclareTextGlyphY{LinBiolinum_R}{uni2213}{8723}
\DeclareTextGlyphY{LinBiolinum_R}{uni2214}{8724}
\DeclareTextGlyphY{LinBiolinum_R}{uni2215}{8725}
\DeclareTextGlyphY{LinBiolinum_R}{uni2216}{8726}
\DeclareTextGlyphY{LinBiolinum_R}{asteriskmath}{8727}
\DeclareTextGlyphY{LinBiolinum_R}{uni2217}{8727}
\DeclareTextGlyphY{LinBiolinum_R}{uni2218}{8728}
\DeclareTextGlyphY{LinBiolinum_R}{uni2219}{8729}
\DeclareTextGlyphY{LinBiolinum_R}{radical}{8730}
\DeclareTextGlyphY{LinBiolinum_R}{uni221A}{8730}
\DeclareTextGlyphY{LinBiolinum_R}{uni221B}{8731}
\DeclareTextGlyphY{LinBiolinum_R}{uni221C}{8732}
\DeclareTextGlyphY{LinBiolinum_R}{proportional}{8733}
\DeclareTextGlyphY{LinBiolinum_R}{uni221D}{8733}
\DeclareTextGlyphY{LinBiolinum_R}{infinity}{8734}
\DeclareTextGlyphY{LinBiolinum_R}{uni221E}{8734}
\DeclareTextGlyphY{LinBiolinum_R}{uni221F}{8735}
\DeclareTextGlyphY{LinBiolinum_R}{uni2223}{8739}
\DeclareTextGlyphY{LinBiolinum_R}{uni2224}{8740}
\DeclareTextGlyphY{LinBiolinum_R}{uni2225}{8741}
\DeclareTextGlyphY{LinBiolinum_R}{uni2226}{8742}
\DeclareTextGlyphY{LinBiolinum_R}{logicaland}{8743}
\DeclareTextGlyphY{LinBiolinum_R}{uni2227}{8743}
\DeclareTextGlyphY{LinBiolinum_R}{logicalor}{8744}
\DeclareTextGlyphY{LinBiolinum_R}{uni2228}{8744}
\DeclareTextGlyphY{LinBiolinum_R}{intersection}{8745}
\DeclareTextGlyphY{LinBiolinum_R}{uni2229}{8745}
\DeclareTextGlyphY{LinBiolinum_R}{uni222A}{8746}
\DeclareTextGlyphY{LinBiolinum_R}{integral}{8747}
\DeclareTextGlyphY{LinBiolinum_R}{uni222B}{8747}
\DeclareTextGlyphY{LinBiolinum_R}{uni2236}{8758}
\DeclareTextGlyphY{LinBiolinum_R}{similar}{8764}
\DeclareTextGlyphY{LinBiolinum_R}{uni223C}{8764}
\DeclareTextGlyphY{LinBiolinum_R}{uni2241}{8769}
\DeclareTextGlyphY{LinBiolinum_R}{congruent}{8773}
\DeclareTextGlyphY{LinBiolinum_R}{uni2245}{8773}
\DeclareTextGlyphY{LinBiolinum_R}{approxequal}{8776}
\DeclareTextGlyphY{LinBiolinum_R}{uni2248}{8776}
\DeclareTextGlyphY{LinBiolinum_R}{uni2249}{8777}
\DeclareTextGlyphY{LinBiolinum_R}{uni2259}{8793}
\DeclareTextGlyphY{LinBiolinum_R}{notequal}{8800}
\DeclareTextGlyphY{LinBiolinum_R}{uni2260}{8800}
\DeclareTextGlyphY{LinBiolinum_R}{equivalence}{8801}
\DeclareTextGlyphY{LinBiolinum_R}{uni2261}{8801}
\DeclareTextGlyphY{LinBiolinum_R}{uni2262}{8802}
\DeclareTextGlyphY{LinBiolinum_R}{lessequal}{8804}
\DeclareTextGlyphY{LinBiolinum_R}{uni2264}{8804}
\DeclareTextGlyphY{LinBiolinum_R}{greaterequal}{8805}
\DeclareTextGlyphY{LinBiolinum_R}{uni2265}{8805}
\DeclareTextGlyphY{LinBiolinum_R}{uni226A}{8810}
\DeclareTextGlyphY{LinBiolinum_R}{uni226B}{8811}
\DeclareTextGlyphY{LinBiolinum_R}{uni226E}{8814}
\DeclareTextGlyphY{LinBiolinum_R}{uni226F}{8815}
\DeclareTextGlyphY{LinBiolinum_R}{uni2270}{8816}
\DeclareTextGlyphY{LinBiolinum_R}{uni2271}{8817}
\DeclareTextGlyphY{LinBiolinum_R}{propersubset}{8834}
\DeclareTextGlyphY{LinBiolinum_R}{uni2282}{8834}
\DeclareTextGlyphY{LinBiolinum_R}{propersuperset}{8835}
\DeclareTextGlyphY{LinBiolinum_R}{uni2283}{8835}
\DeclareTextGlyphY{LinBiolinum_R}{notsubset}{8836}
\DeclareTextGlyphY{LinBiolinum_R}{uni2284}{8836}
\DeclareTextGlyphY{LinBiolinum_R}{uni2285}{8837}
\DeclareTextGlyphY{LinBiolinum_R}{circleplus}{8853}
\DeclareTextGlyphY{LinBiolinum_R}{uni2295}{8853}
\DeclareTextGlyphY{LinBiolinum_R}{uni2296}{8854}
\DeclareTextGlyphY{LinBiolinum_R}{circlemultiply}{8855}
\DeclareTextGlyphY{LinBiolinum_R}{uni2297}{8855}
\DeclareTextGlyphY{LinBiolinum_R}{uni2298}{8856}
\DeclareTextGlyphY{LinBiolinum_R}{uni22A2}{8866}
\DeclareTextGlyphY{LinBiolinum_R}{uni22A3}{8867}
\DeclareTextGlyphY{LinBiolinum_R}{uni22A4}{8868}
\DeclareTextGlyphY{LinBiolinum_R}{perpendicular}{8869}
\DeclareTextGlyphY{LinBiolinum_R}{uni22A5}{8869}
\DeclareTextGlyphY{LinBiolinum_R}{uni22A6}{8870}
\DeclareTextGlyphY{LinBiolinum_R}{dotmath}{8901}
\DeclareTextGlyphY{LinBiolinum_R}{uni22C5}{8901}
\DeclareTextGlyphY{LinBiolinum_R}{uni22EE}{8942}
\DeclareTextGlyphY{LinBiolinum_R}{uni22EF}{8943}
\DeclareTextGlyphY{LinBiolinum_R}{uni2300}{8960}
\DeclareTextGlyphY{LinBiolinum_R}{uni2302}{8962}
\DeclareTextGlyphY{LinBiolinum_R}{uni2303}{8963}
\DeclareTextGlyphY{LinBiolinum_R}{uni2310}{8976}
\DeclareTextGlyphY{LinBiolinum_R}{uni2320}{8992}
\DeclareTextGlyphY{LinBiolinum_R}{uni2321}{8993}
\DeclareTextGlyphY{LinBiolinum_R}{uni2326}{8998}
\DeclareTextGlyphY{LinBiolinum_R}{uni2327}{8999}
\DeclareTextGlyphY{LinBiolinum_R}{uni2329}{9001}
\DeclareTextGlyphY{LinBiolinum_R}{uni232A}{9002}
\DeclareTextGlyphY{LinBiolinum_R}{uni232B}{9003}
\DeclareTextGlyphY{LinBiolinum_R}{uni237D}{9085}
\DeclareTextGlyphY{LinBiolinum_R}{uni2380}{9088}
\DeclareTextGlyphY{LinBiolinum_R}{uni23D3}{9171}
\DeclareTextGlyphY{LinBiolinum_R}{uni2423}{9251}
\DeclareTextGlyphY{LinBiolinum_R}{uni2460}{9312}
\DeclareTextGlyphY{LinBiolinum_R}{uni2461}{9313}
\DeclareTextGlyphY{LinBiolinum_R}{uni2462}{9314}
\DeclareTextGlyphY{LinBiolinum_R}{uni2463}{9315}
\DeclareTextGlyphY{LinBiolinum_R}{uni2464}{9316}
\DeclareTextGlyphY{LinBiolinum_R}{uni2465}{9317}
\DeclareTextGlyphY{LinBiolinum_R}{uni2466}{9318}
\DeclareTextGlyphY{LinBiolinum_R}{uni2467}{9319}
\DeclareTextGlyphY{LinBiolinum_R}{uni2468}{9320}
\DeclareTextGlyphY{LinBiolinum_R}{uni2469}{9321}
\DeclareTextGlyphY{LinBiolinum_R}{uni246A}{9322}
\DeclareTextGlyphY{LinBiolinum_R}{uni246B}{9323}
\DeclareTextGlyphY{LinBiolinum_R}{uni246C}{9324}
\DeclareTextGlyphY{LinBiolinum_R}{uni246D}{9325}
\DeclareTextGlyphY{LinBiolinum_R}{uni246E}{9326}
\DeclareTextGlyphY{LinBiolinum_R}{uni246F}{9327}
\DeclareTextGlyphY{LinBiolinum_R}{uni2470}{9328}
\DeclareTextGlyphY{LinBiolinum_R}{uni2471}{9329}
\DeclareTextGlyphY{LinBiolinum_R}{uni2472}{9330}
\DeclareTextGlyphY{LinBiolinum_R}{uni2473}{9331}
\DeclareTextGlyphY{LinBiolinum_R}{uni2474}{9332}
\DeclareTextGlyphY{LinBiolinum_R}{uni2475}{9333}
\DeclareTextGlyphY{LinBiolinum_R}{uni2476}{9334}
\DeclareTextGlyphY{LinBiolinum_R}{uni2477}{9335}
\DeclareTextGlyphY{LinBiolinum_R}{uni2478}{9336}
\DeclareTextGlyphY{LinBiolinum_R}{uni2479}{9337}
\DeclareTextGlyphY{LinBiolinum_R}{uni247A}{9338}
\DeclareTextGlyphY{LinBiolinum_R}{uni247B}{9339}
\DeclareTextGlyphY{LinBiolinum_R}{uni247C}{9340}
\DeclareTextGlyphY{LinBiolinum_R}{uni247D}{9341}
\DeclareTextGlyphY{LinBiolinum_R}{uni247E}{9342}
\DeclareTextGlyphY{LinBiolinum_R}{uni247F}{9343}
\DeclareTextGlyphY{LinBiolinum_R}{uni2480}{9344}
\DeclareTextGlyphY{LinBiolinum_R}{uni2481}{9345}
\DeclareTextGlyphY{LinBiolinum_R}{uni2482}{9346}
\DeclareTextGlyphY{LinBiolinum_R}{uni2483}{9347}
\DeclareTextGlyphY{LinBiolinum_R}{uni2484}{9348}
\DeclareTextGlyphY{LinBiolinum_R}{uni2485}{9349}
\DeclareTextGlyphY{LinBiolinum_R}{uni2486}{9350}
\DeclareTextGlyphY{LinBiolinum_R}{uni2487}{9351}
\DeclareTextGlyphY{LinBiolinum_R}{uni24B6}{9398}
\DeclareTextGlyphY{LinBiolinum_R}{uni24B7}{9399}
\DeclareTextGlyphY{LinBiolinum_R}{uni24B8}{9400}
\DeclareTextGlyphY{LinBiolinum_R}{uni24B9}{9401}
\DeclareTextGlyphY{LinBiolinum_R}{uni24BA}{9402}
\DeclareTextGlyphY{LinBiolinum_R}{uni24BB}{9403}
\DeclareTextGlyphY{LinBiolinum_R}{uni24BC}{9404}
\DeclareTextGlyphY{LinBiolinum_R}{uni24BD}{9405}
\DeclareTextGlyphY{LinBiolinum_R}{uni24BE}{9406}
\DeclareTextGlyphY{LinBiolinum_R}{uni24BF}{9407}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C0}{9408}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C1}{9409}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C2}{9410}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C3}{9411}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C4}{9412}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C5}{9413}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C6}{9414}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C7}{9415}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C8}{9416}
\DeclareTextGlyphY{LinBiolinum_R}{uni24C9}{9417}
\DeclareTextGlyphY{LinBiolinum_R}{uni24CA}{9418}
\DeclareTextGlyphY{LinBiolinum_R}{uni24CB}{9419}
\DeclareTextGlyphY{LinBiolinum_R}{uni24CC}{9420}
\DeclareTextGlyphY{LinBiolinum_R}{uni24CD}{9421}
\DeclareTextGlyphY{LinBiolinum_R}{uni24CE}{9422}
\DeclareTextGlyphY{LinBiolinum_R}{uni24CF}{9423}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D0}{9424}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D1}{9425}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D2}{9426}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D3}{9427}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D4}{9428}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D5}{9429}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D6}{9430}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D7}{9431}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D8}{9432}
\DeclareTextGlyphY{LinBiolinum_R}{uni24D9}{9433}
\DeclareTextGlyphY{LinBiolinum_R}{uni24DA}{9434}
\DeclareTextGlyphY{LinBiolinum_R}{uni24DB}{9435}
\DeclareTextGlyphY{LinBiolinum_R}{uni24DC}{9436}
\DeclareTextGlyphY{LinBiolinum_R}{uni24DD}{9437}
\DeclareTextGlyphY{LinBiolinum_R}{uni24DE}{9438}
\DeclareTextGlyphY{LinBiolinum_R}{uni24DF}{9439}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E0}{9440}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E1}{9441}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E2}{9442}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E3}{9443}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E4}{9444}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E5}{9445}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E6}{9446}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E7}{9447}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E8}{9448}
\DeclareTextGlyphY{LinBiolinum_R}{uni24E9}{9449}
\DeclareTextGlyphY{LinBiolinum_R}{uni24EA}{9450}
\DeclareTextGlyphY{LinBiolinum_R}{uni24EB}{9451}
\DeclareTextGlyphY{LinBiolinum_R}{uni24EC}{9452}
\DeclareTextGlyphY{LinBiolinum_R}{uni24ED}{9453}
\DeclareTextGlyphY{LinBiolinum_R}{uni24EE}{9454}
\DeclareTextGlyphY{LinBiolinum_R}{uni24EF}{9455}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F0}{9456}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F1}{9457}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F2}{9458}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F3}{9459}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F4}{9460}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F5}{9461}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F6}{9462}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F7}{9463}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F8}{9464}
\DeclareTextGlyphY{LinBiolinum_R}{uni24F9}{9465}
\DeclareTextGlyphY{LinBiolinum_R}{uni24FA}{9466}
\DeclareTextGlyphY{LinBiolinum_R}{uni24FB}{9467}
\DeclareTextGlyphY{LinBiolinum_R}{uni24FC}{9468}
\DeclareTextGlyphY{LinBiolinum_R}{uni24FD}{9469}
\DeclareTextGlyphY{LinBiolinum_R}{uni24FE}{9470}
\DeclareTextGlyphY{LinBiolinum_R}{uni24FF}{9471}
\DeclareTextGlyphY{LinBiolinum_R}{filledbox}{9632}
\DeclareTextGlyphY{LinBiolinum_R}{uni25A0}{9632}
\DeclareTextGlyphY{LinBiolinum_R}{H22073}{9633}
\DeclareTextGlyphY{LinBiolinum_R}{uni25A1}{9633}
\DeclareTextGlyphY{LinBiolinum_R}{triagup}{9650}
\DeclareTextGlyphY{LinBiolinum_R}{uni25B2}{9650}
\DeclareTextGlyphY{LinBiolinum_R}{uni25B3}{9651}
\DeclareTextGlyphY{LinBiolinum_R}{uni25B6}{9654}
\DeclareTextGlyphY{LinBiolinum_R}{uni25B7}{9655}
\DeclareTextGlyphY{LinBiolinum_R}{triagdn}{9660}
\DeclareTextGlyphY{LinBiolinum_R}{uni25BC}{9660}
\DeclareTextGlyphY{LinBiolinum_R}{uni25BD}{9661}
\DeclareTextGlyphY{LinBiolinum_R}{uni25C0}{9664}
\DeclareTextGlyphY{LinBiolinum_R}{uni25C1}{9665}
\DeclareTextGlyphY{LinBiolinum_R}{uni25C6}{9670}
\DeclareTextGlyphY{LinBiolinum_R}{uni25C7}{9671}
\DeclareTextGlyphY{LinBiolinum_R}{uni25C9}{9673}
\DeclareTextGlyphY{LinBiolinum_R}{lozenge}{9674}
\DeclareTextGlyphY{LinBiolinum_R}{uni25CA}{9674}
\DeclareTextGlyphY{LinBiolinum_R}{circle}{9675}
\DeclareTextGlyphY{LinBiolinum_R}{uni25CB}{9675}
\DeclareTextGlyphY{LinBiolinum_R}{uni25CE}{9678}
\DeclareTextGlyphY{LinBiolinum_R}{H18533}{9679}
\DeclareTextGlyphY{LinBiolinum_R}{uni25CF}{9679}
\DeclareTextGlyphY{LinBiolinum_R}{uni25D0}{9680}
\DeclareTextGlyphY{LinBiolinum_R}{uni25D1}{9681}
\DeclareTextGlyphY{LinBiolinum_R}{uni25D2}{9682}
\DeclareTextGlyphY{LinBiolinum_R}{uni25D3}{9683}
\DeclareTextGlyphY{LinBiolinum_R}{uni25D4}{9684}
\DeclareTextGlyphY{LinBiolinum_R}{uni25D5}{9685}
\DeclareTextGlyphY{LinBiolinum_R}{uni25D6}{9686}
\DeclareTextGlyphY{LinBiolinum_R}{uni25D7}{9687}
\DeclareTextGlyphY{LinBiolinum_R}{openbullet}{9702}
\DeclareTextGlyphY{LinBiolinum_R}{uni25E6}{9702}
\DeclareTextGlyphY{LinBiolinum_R}{uni2605}{9733}
\DeclareTextGlyphY{LinBiolinum_R}{uni2619}{9753}
\DeclareTextGlyphY{LinBiolinum_R}{uni261B}{9755}
\DeclareTextGlyphY{LinBiolinum_R}{uni261E}{9758}
\DeclareTextGlyphY{LinBiolinum_R}{uni2627}{9767}
\DeclareTextGlyphY{LinBiolinum_R}{uni262F}{9775}
\DeclareTextGlyphY{LinBiolinum_R}{uni2639}{9785}
\DeclareTextGlyphY{LinBiolinum_R}{uni263A}{9786}
\DeclareTextGlyphY{LinBiolinum_R}{uni263B}{9787}
\DeclareTextGlyphY{LinBiolinum_R}{uni263C}{9788}
\DeclareTextGlyphY{LinBiolinum_R}{uni263D}{9789}
\DeclareTextGlyphY{LinBiolinum_R}{uni263E}{9790}
\DeclareTextGlyphY{LinBiolinum_R}{uni263F}{9791}
\DeclareTextGlyphY{LinBiolinum_R}{female}{9792}
\DeclareTextGlyphY{LinBiolinum_R}{uni2640}{9792}
\DeclareTextGlyphY{LinBiolinum_R}{uni2641}{9793}
\DeclareTextGlyphY{LinBiolinum_R}{male}{9794}
\DeclareTextGlyphY{LinBiolinum_R}{uni2642}{9794}
\DeclareTextGlyphY{LinBiolinum_R}{uni2643}{9795}
\DeclareTextGlyphY{LinBiolinum_R}{uni2644}{9796}
\DeclareTextGlyphY{LinBiolinum_R}{uni2645}{9797}
\DeclareTextGlyphY{LinBiolinum_R}{uni2646}{9798}
\DeclareTextGlyphY{LinBiolinum_R}{uni2647}{9799}
\DeclareTextGlyphY{LinBiolinum_R}{uni2648}{9800}
\DeclareTextGlyphY{LinBiolinum_R}{uni2649}{9801}
\DeclareTextGlyphY{LinBiolinum_R}{uni264A}{9802}
\DeclareTextGlyphY{LinBiolinum_R}{uni264B}{9803}
\DeclareTextGlyphY{LinBiolinum_R}{uni264C}{9804}
\DeclareTextGlyphY{LinBiolinum_R}{uni264D}{9805}
\DeclareTextGlyphY{LinBiolinum_R}{uni264E}{9806}
\DeclareTextGlyphY{LinBiolinum_R}{uni264F}{9807}
\DeclareTextGlyphY{LinBiolinum_R}{uni2650}{9808}
\DeclareTextGlyphY{LinBiolinum_R}{uni2651}{9809}
\DeclareTextGlyphY{LinBiolinum_R}{uni2652}{9810}
\DeclareTextGlyphY{LinBiolinum_R}{uni2653}{9811}
\DeclareTextGlyphY{LinBiolinum_R}{uni2660}{9824}
\DeclareTextGlyphY{LinBiolinum_R}{uni2663}{9827}
\DeclareTextGlyphY{LinBiolinum_R}{uni2665}{9829}
\DeclareTextGlyphY{LinBiolinum_R}{uni2666}{9830}
\DeclareTextGlyphY{LinBiolinum_R}{uni2669}{9833}
\DeclareTextGlyphY{LinBiolinum_R}{musicalnote}{9834}
\DeclareTextGlyphY{LinBiolinum_R}{uni266A}{9834}
\DeclareTextGlyphY{LinBiolinum_R}{musicalnotedbl}{9835}
\DeclareTextGlyphY{LinBiolinum_R}{uni266B}{9835}
\DeclareTextGlyphY{LinBiolinum_R}{uni266C}{9836}
\DeclareTextGlyphY{LinBiolinum_R}{uni2695}{9877}
\DeclareTextGlyphY{LinBiolinum_R}{uni2698}{9880}
\DeclareTextGlyphY{LinBiolinum_R}{uni26A2}{9890}
\DeclareTextGlyphY{LinBiolinum_R}{uni26A3}{9891}
\DeclareTextGlyphY{LinBiolinum_R}{uni26A4}{9892}
\DeclareTextGlyphY{LinBiolinum_R}{uni26A5}{9893}
\DeclareTextGlyphY{LinBiolinum_R}{uni26AD}{9901}
\DeclareTextGlyphY{LinBiolinum_R}{uni2767}{10087}
\DeclareTextGlyphY{LinBiolinum_R}{uni2776}{10102}
\DeclareTextGlyphY{LinBiolinum_R}{uni2777}{10103}
\DeclareTextGlyphY{LinBiolinum_R}{uni2778}{10104}
\DeclareTextGlyphY{LinBiolinum_R}{uni2779}{10105}
\DeclareTextGlyphY{LinBiolinum_R}{uni277A}{10106}
\DeclareTextGlyphY{LinBiolinum_R}{uni277B}{10107}
\DeclareTextGlyphY{LinBiolinum_R}{uni277C}{10108}
\DeclareTextGlyphY{LinBiolinum_R}{uni277D}{10109}
\DeclareTextGlyphY{LinBiolinum_R}{uni277E}{10110}
\DeclareTextGlyphY{LinBiolinum_R}{uni277F}{10111}
\DeclareTextGlyphY{LinBiolinum_R}{uni27C2}{10178}
\DeclareTextGlyphY{LinBiolinum_R}{uni27E6}{10214}
\DeclareTextGlyphY{LinBiolinum_R}{uni27E7}{10215}
\DeclareTextGlyphY{LinBiolinum_R}{uni27E8}{10216}
\DeclareTextGlyphY{LinBiolinum_R}{uni27E9}{10217}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C60}{11360}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C61}{11361}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C62}{11362}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C63}{11363}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C64}{11364}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C65}{11365}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C66}{11366}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C67}{11367}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C68}{11368}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C69}{11369}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C6A}{11370}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C6B}{11371}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C6C}{11372}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C74}{11380}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C75}{11381}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C76}{11382}
\DeclareTextGlyphY{LinBiolinum_R}{uni2C77}{11383}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E02}{11778}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E03}{11779}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E04}{11780}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E05}{11781}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E08}{11784}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E09}{11785}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E0A}{11786}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E17}{11799}
\DeclareTextGlyphY{LinBiolinum_R}{uni2E18}{11800}
\DeclareTextGlyphY{LinBiolinum_R}{uniA720}{42784}
\DeclareTextGlyphY{LinBiolinum_R}{uniA721}{42785}
\DeclareTextGlyphY{LinBiolinum_R}{Tux}{57344}
\DeclareTextGlyphY{LinBiolinum_R}{uniE000}{57344}
\DeclareTextGlyphY{LinBiolinum_R}{uniE001}{57345}
\DeclareTextGlyphY{LinBiolinum_R}{uniE002}{57346}
\DeclareTextGlyphY{LinBiolinum_R}{uniE003}{57347}
\DeclareTextGlyphY{LinBiolinum_R}{uniE004}{57348}
\DeclareTextGlyphY{LinBiolinum_R}{uniE005}{57349}
\DeclareTextGlyphY{LinBiolinum_R}{uniE006}{57350}
\DeclareTextGlyphY{LinBiolinum_R}{uniE007}{57351}
\DeclareTextGlyphY{LinBiolinum_R}{uniE008}{57352}
\DeclareTextGlyphY{LinBiolinum_R}{uniE009}{57353}
\DeclareTextGlyphY{LinBiolinum_R}{uniE00A}{57354}
\DeclareTextGlyphY{LinBiolinum_R}{uniE00B}{57355}
\DeclareTextGlyphY{LinBiolinum_R}{zero.slashfitted}{57359}
\DeclareTextGlyphY{LinBiolinum_R}{uniE00F}{57359}
\DeclareTextGlyphY{LinBiolinum_R}{zero.fitted}{57360}
\DeclareTextGlyphY{LinBiolinum_R}{uniE010}{57360}
\DeclareTextGlyphY{LinBiolinum_R}{one.fitted}{57361}
\DeclareTextGlyphY{LinBiolinum_R}{uniE011}{57361}
\DeclareTextGlyphY{LinBiolinum_R}{two.fitted}{57362}
\DeclareTextGlyphY{LinBiolinum_R}{uniE012}{57362}
\DeclareTextGlyphY{LinBiolinum_R}{three.fitted}{57363}
\DeclareTextGlyphY{LinBiolinum_R}{uniE013}{57363}
\DeclareTextGlyphY{LinBiolinum_R}{four.fitted}{57364}
\DeclareTextGlyphY{LinBiolinum_R}{uniE014}{57364}
\DeclareTextGlyphY{LinBiolinum_R}{five.fitted}{57365}
\DeclareTextGlyphY{LinBiolinum_R}{uniE015}{57365}
\DeclareTextGlyphY{LinBiolinum_R}{six.fitted}{57366}
\DeclareTextGlyphY{LinBiolinum_R}{uniE016}{57366}
\DeclareTextGlyphY{LinBiolinum_R}{seven.fitted}{57367}
\DeclareTextGlyphY{LinBiolinum_R}{uniE017}{57367}
\DeclareTextGlyphY{LinBiolinum_R}{eight.fitted}{57368}
\DeclareTextGlyphY{LinBiolinum_R}{uniE018}{57368}
\DeclareTextGlyphY{LinBiolinum_R}{nine.fitted}{57369}
\DeclareTextGlyphY{LinBiolinum_R}{uniE019}{57369}
\DeclareTextGlyphY{LinBiolinum_R}{Euro.fitted}{57370}
\DeclareTextGlyphY{LinBiolinum_R}{uniE01A}{57370}
\DeclareTextGlyphY{LinBiolinum_R}{Yen.fitted}{57371}
\DeclareTextGlyphY{LinBiolinum_R}{uniE01B}{57371}
\DeclareTextGlyphY{LinBiolinum_R}{perthousandzero}{57375}
\DeclareTextGlyphY{LinBiolinum_R}{uniE01F}{57375}
\DeclareTextGlyphY{LinBiolinum_R}{zero.oldstyle}{57376}
\DeclareTextGlyphY{LinBiolinum_R}{uniE020}{57376}
\DeclareTextGlyphY{LinBiolinum_R}{one.oldstyle}{57377}
\DeclareTextGlyphY{LinBiolinum_R}{uniE021}{57377}
\DeclareTextGlyphY{LinBiolinum_R}{two.oldstyle}{57378}
\DeclareTextGlyphY{LinBiolinum_R}{uniE022}{57378}
\DeclareTextGlyphY{LinBiolinum_R}{three.oldstyle}{57379}
\DeclareTextGlyphY{LinBiolinum_R}{uniE023}{57379}
\DeclareTextGlyphY{LinBiolinum_R}{four.oldstyle}{57380}
\DeclareTextGlyphY{LinBiolinum_R}{uniE024}{57380}
\DeclareTextGlyphY{LinBiolinum_R}{five.oldstyle}{57381}
\DeclareTextGlyphY{LinBiolinum_R}{uniE025}{57381}
\DeclareTextGlyphY{LinBiolinum_R}{six.oldstyle}{57382}
\DeclareTextGlyphY{LinBiolinum_R}{uniE026}{57382}
\DeclareTextGlyphY{LinBiolinum_R}{seven.oldstyle}{57383}
\DeclareTextGlyphY{LinBiolinum_R}{uniE027}{57383}
\DeclareTextGlyphY{LinBiolinum_R}{eight.oldstyle}{57384}
\DeclareTextGlyphY{LinBiolinum_R}{uniE028}{57384}
\DeclareTextGlyphY{LinBiolinum_R}{nine.oldstyle}{57385}
\DeclareTextGlyphY{LinBiolinum_R}{uniE029}{57385}
\DeclareTextGlyphY{LinBiolinum_R}{Adieresis.alt}{57388}
\DeclareTextGlyphY{LinBiolinum_R}{uniE02C}{57388}
\DeclareTextGlyphY{LinBiolinum_R}{Odieresis.alt}{57389}
\DeclareTextGlyphY{LinBiolinum_R}{uniE02D}{57389}
\DeclareTextGlyphY{LinBiolinum_R}{Udieresis.alt}{57390}
\DeclareTextGlyphY{LinBiolinum_R}{uniE02E}{57390}
\DeclareTextGlyphY{LinBiolinum_R}{f_t}{57401}
\DeclareTextGlyphY{LinBiolinum_R}{uniE039}{57401}
\DeclareTextGlyphY{LinBiolinum_R}{t_t}{57404}
\DeclareTextGlyphY{LinBiolinum_R}{uniE03C}{57404}
\DeclareTextGlyphY{LinBiolinum_R}{c_t}{57405}
\DeclareTextGlyphY{LinBiolinum_R}{uniE03D}{57405}
\DeclareTextGlyphY{LinBiolinum_R}{uniE040}{57408}
\DeclareTextGlyphY{LinBiolinum_R}{uniE041}{57409}
\DeclareTextGlyphY{LinBiolinum_R}{uniE042}{57410}
\DeclareTextGlyphY{LinBiolinum_R}{Q_u}{57416}
\DeclareTextGlyphY{LinBiolinum_R}{uniE048}{57416}
\DeclareTextGlyphY{LinBiolinum_R}{t_z}{57418}
\DeclareTextGlyphY{LinBiolinum_R}{uniE04A}{57418}
\DeclareTextGlyphY{LinBiolinum_R}{h.alt}{57419}
\DeclareTextGlyphY{LinBiolinum_R}{uniE04B}{57419}
\DeclareTextGlyphY{LinBiolinum_R}{germandbls.alt}{57420}
\DeclareTextGlyphY{LinBiolinum_R}{uniE04C}{57420}
\DeclareTextGlyphY{LinBiolinum_R}{Germandbls.alt}{57422}
\DeclareTextGlyphY{LinBiolinum_R}{uniE04E}{57422}
\DeclareTextGlyphY{LinBiolinum_R}{ampersand.alt}{57424}
\DeclareTextGlyphY{LinBiolinum_R}{uniE050}{57424}
\DeclareTextGlyphY{LinBiolinum_R}{a.sc}{57425}
\DeclareTextGlyphY{LinBiolinum_R}{uniE051}{57425}
\DeclareTextGlyphY{LinBiolinum_R}{b.sc}{57426}
\DeclareTextGlyphY{LinBiolinum_R}{uniE052}{57426}
\DeclareTextGlyphY{LinBiolinum_R}{c.sc}{57427}
\DeclareTextGlyphY{LinBiolinum_R}{uniE053}{57427}
\DeclareTextGlyphY{LinBiolinum_R}{d.sc}{57428}
\DeclareTextGlyphY{LinBiolinum_R}{uniE054}{57428}
\DeclareTextGlyphY{LinBiolinum_R}{e.sc}{57429}
\DeclareTextGlyphY{LinBiolinum_R}{uniE055}{57429}
\DeclareTextGlyphY{LinBiolinum_R}{f.sc}{57430}
\DeclareTextGlyphY{LinBiolinum_R}{uniE056}{57430}
\DeclareTextGlyphY{LinBiolinum_R}{g.sc}{57431}
\DeclareTextGlyphY{LinBiolinum_R}{uniE057}{57431}
\DeclareTextGlyphY{LinBiolinum_R}{h.sc}{57432}
\DeclareTextGlyphY{LinBiolinum_R}{uniE058}{57432}
\DeclareTextGlyphY{LinBiolinum_R}{i.sc}{57433}
\DeclareTextGlyphY{LinBiolinum_R}{uniE059}{57433}
\DeclareTextGlyphY{LinBiolinum_R}{j.sc}{57434}
\DeclareTextGlyphY{LinBiolinum_R}{uniE05A}{57434}
\DeclareTextGlyphY{LinBiolinum_R}{k.sc}{57435}
\DeclareTextGlyphY{LinBiolinum_R}{uniE05B}{57435}
\DeclareTextGlyphY{LinBiolinum_R}{l.sc}{57436}
\DeclareTextGlyphY{LinBiolinum_R}{uniE05C}{57436}
\DeclareTextGlyphY{LinBiolinum_R}{m.sc}{57437}
\DeclareTextGlyphY{LinBiolinum_R}{uniE05D}{57437}
\DeclareTextGlyphY{LinBiolinum_R}{n.sc}{57438}
\DeclareTextGlyphY{LinBiolinum_R}{uniE05E}{57438}
\DeclareTextGlyphY{LinBiolinum_R}{o.sc}{57439}
\DeclareTextGlyphY{LinBiolinum_R}{uniE05F}{57439}
\DeclareTextGlyphY{LinBiolinum_R}{p.sc}{57440}
\DeclareTextGlyphY{LinBiolinum_R}{uniE060}{57440}
\DeclareTextGlyphY{LinBiolinum_R}{q.sc}{57441}
\DeclareTextGlyphY{LinBiolinum_R}{uniE061}{57441}
\DeclareTextGlyphY{LinBiolinum_R}{r.sc}{57442}
\DeclareTextGlyphY{LinBiolinum_R}{uniE062}{57442}
\DeclareTextGlyphY{LinBiolinum_R}{s.sc}{57443}
\DeclareTextGlyphY{LinBiolinum_R}{uniE063}{57443}
\DeclareTextGlyphY{LinBiolinum_R}{t.sc}{57444}
\DeclareTextGlyphY{LinBiolinum_R}{uniE064}{57444}
\DeclareTextGlyphY{LinBiolinum_R}{u.sc}{57445}
\DeclareTextGlyphY{LinBiolinum_R}{uniE065}{57445}
\DeclareTextGlyphY{LinBiolinum_R}{v.sc}{57446}
\DeclareTextGlyphY{LinBiolinum_R}{uniE066}{57446}
\DeclareTextGlyphY{LinBiolinum_R}{w.sc}{57447}
\DeclareTextGlyphY{LinBiolinum_R}{uniE067}{57447}
\DeclareTextGlyphY{LinBiolinum_R}{x.sc}{57448}
\DeclareTextGlyphY{LinBiolinum_R}{uniE068}{57448}
\DeclareTextGlyphY{LinBiolinum_R}{y.sc}{57449}
\DeclareTextGlyphY{LinBiolinum_R}{uniE069}{57449}
\DeclareTextGlyphY{LinBiolinum_R}{z.sc}{57450}
\DeclareTextGlyphY{LinBiolinum_R}{uniE06A}{57450}
\DeclareTextGlyphY{LinBiolinum_R}{uniE06B}{57451}
\DeclareTextGlyphY{LinBiolinum_R}{hyphen.sc}{57453}
\DeclareTextGlyphY{LinBiolinum_R}{uniE06D}{57453}
\DeclareTextGlyphY{LinBiolinum_R}{agrave.sc}{57456}
\DeclareTextGlyphY{LinBiolinum_R}{uniE070}{57456}
\DeclareTextGlyphY{LinBiolinum_R}{aacute.sc}{57457}
\DeclareTextGlyphY{LinBiolinum_R}{uniE071}{57457}
\DeclareTextGlyphY{LinBiolinum_R}{acircumflex.sc}{57458}
\DeclareTextGlyphY{LinBiolinum_R}{uniE072}{57458}
\DeclareTextGlyphY{LinBiolinum_R}{atilde.sc}{57459}
\DeclareTextGlyphY{LinBiolinum_R}{uniE073}{57459}
\DeclareTextGlyphY{LinBiolinum_R}{adieresis.sc}{57460}
\DeclareTextGlyphY{LinBiolinum_R}{uniE074}{57460}
\DeclareTextGlyphY{LinBiolinum_R}{aring.sc}{57461}
\DeclareTextGlyphY{LinBiolinum_R}{uniE075}{57461}
\DeclareTextGlyphY{LinBiolinum_R}{ae.sc}{57462}
\DeclareTextGlyphY{LinBiolinum_R}{uniE076}{57462}
\DeclareTextGlyphY{LinBiolinum_R}{ccedilla.sc}{57463}
\DeclareTextGlyphY{LinBiolinum_R}{uniE077}{57463}
\DeclareTextGlyphY{LinBiolinum_R}{egrave.sc}{57464}
\DeclareTextGlyphY{LinBiolinum_R}{uniE078}{57464}
\DeclareTextGlyphY{LinBiolinum_R}{eacute.sc}{57465}
\DeclareTextGlyphY{LinBiolinum_R}{uniE079}{57465}
\DeclareTextGlyphY{LinBiolinum_R}{ecircumflex.sc}{57466}
\DeclareTextGlyphY{LinBiolinum_R}{uniE07A}{57466}
\DeclareTextGlyphY{LinBiolinum_R}{edieresis.sc}{57467}
\DeclareTextGlyphY{LinBiolinum_R}{uniE07B}{57467}
\DeclareTextGlyphY{LinBiolinum_R}{igrave.sc}{57468}
\DeclareTextGlyphY{LinBiolinum_R}{uniE07C}{57468}
\DeclareTextGlyphY{LinBiolinum_R}{iacute.sc}{57469}
\DeclareTextGlyphY{LinBiolinum_R}{uniE07D}{57469}
\DeclareTextGlyphY{LinBiolinum_R}{icircumflex.sc}{57470}
\DeclareTextGlyphY{LinBiolinum_R}{uniE07E}{57470}
\DeclareTextGlyphY{LinBiolinum_R}{idieresis.sc}{57471}
\DeclareTextGlyphY{LinBiolinum_R}{uniE07F}{57471}
\DeclareTextGlyphY{LinBiolinum_R}{eth.sc}{57472}
\DeclareTextGlyphY{LinBiolinum_R}{uniE080}{57472}
\DeclareTextGlyphY{LinBiolinum_R}{ntilde.sc}{57473}
\DeclareTextGlyphY{LinBiolinum_R}{uniE081}{57473}
\DeclareTextGlyphY{LinBiolinum_R}{ograve.sc}{57474}
\DeclareTextGlyphY{LinBiolinum_R}{uniE082}{57474}
\DeclareTextGlyphY{LinBiolinum_R}{oacute.sc}{57475}
\DeclareTextGlyphY{LinBiolinum_R}{uniE083}{57475}
\DeclareTextGlyphY{LinBiolinum_R}{ocircumflex.sc}{57476}
\DeclareTextGlyphY{LinBiolinum_R}{uniE084}{57476}
\DeclareTextGlyphY{LinBiolinum_R}{otilde.sc}{57477}
\DeclareTextGlyphY{LinBiolinum_R}{uniE085}{57477}
\DeclareTextGlyphY{LinBiolinum_R}{odieresis.sc}{57478}
\DeclareTextGlyphY{LinBiolinum_R}{uniE086}{57478}
\DeclareTextGlyphY{LinBiolinum_R}{oe.sc}{57479}
\DeclareTextGlyphY{LinBiolinum_R}{uniE087}{57479}
\DeclareTextGlyphY{LinBiolinum_R}{oslash.sc}{57480}
\DeclareTextGlyphY{LinBiolinum_R}{uniE088}{57480}
\DeclareTextGlyphY{LinBiolinum_R}{ugrave.sc}{57481}
\DeclareTextGlyphY{LinBiolinum_R}{uniE089}{57481}
\DeclareTextGlyphY{LinBiolinum_R}{uacute.sc}{57482}
\DeclareTextGlyphY{LinBiolinum_R}{uniE08A}{57482}
\DeclareTextGlyphY{LinBiolinum_R}{ucircumflex.sc}{57483}
\DeclareTextGlyphY{LinBiolinum_R}{uniE08B}{57483}
\DeclareTextGlyphY{LinBiolinum_R}{udieresis.sc}{57484}
\DeclareTextGlyphY{LinBiolinum_R}{uniE08C}{57484}
\DeclareTextGlyphY{LinBiolinum_R}{yacute.sc}{57485}
\DeclareTextGlyphY{LinBiolinum_R}{uniE08D}{57485}
\DeclareTextGlyphY{LinBiolinum_R}{thorn.sc}{57486}
\DeclareTextGlyphY{LinBiolinum_R}{uniE08E}{57486}
\DeclareTextGlyphY{LinBiolinum_R}{ydieresis.sc}{57487}
\DeclareTextGlyphY{LinBiolinum_R}{uniE08F}{57487}
\DeclareTextGlyphY{LinBiolinum_R}{ij.sc}{57488}
\DeclareTextGlyphY{LinBiolinum_R}{uniE090}{57488}
\DeclareTextGlyphY{LinBiolinum_R}{germandbls.scalt}{57489}
\DeclareTextGlyphY{LinBiolinum_R}{uniE091}{57489}
\DeclareTextGlyphY{LinBiolinum_R}{germandbls.sc}{57490}
\DeclareTextGlyphY{LinBiolinum_R}{uniE092}{57490}
\DeclareTextGlyphY{LinBiolinum_R}{dcroat.sc}{57495}
\DeclareTextGlyphY{LinBiolinum_R}{uniE097}{57495}
\DeclareTextGlyphY{LinBiolinum_R}{abreve.sc}{57496}
\DeclareTextGlyphY{LinBiolinum_R}{uniE098}{57496}
\DeclareTextGlyphY{LinBiolinum_R}{aogonek.sc}{57497}
\DeclareTextGlyphY{LinBiolinum_R}{uniE099}{57497}
\DeclareTextGlyphY{LinBiolinum_R}{cacute.sc}{57498}
\DeclareTextGlyphY{LinBiolinum_R}{uniE09A}{57498}
\DeclareTextGlyphY{LinBiolinum_R}{ccaron.sc}{57499}
\DeclareTextGlyphY{LinBiolinum_R}{uniE09B}{57499}
\DeclareTextGlyphY{LinBiolinum_R}{dcaron.sc}{57500}
\DeclareTextGlyphY{LinBiolinum_R}{uniE09C}{57500}
\DeclareTextGlyphY{LinBiolinum_R}{eogonek.sc}{57501}
\DeclareTextGlyphY{LinBiolinum_R}{uniE09D}{57501}
\DeclareTextGlyphY{LinBiolinum_R}{ecaron.sc}{57502}
\DeclareTextGlyphY{LinBiolinum_R}{uniE09E}{57502}
\DeclareTextGlyphY{LinBiolinum_R}{gbreve.sc}{57503}
\DeclareTextGlyphY{LinBiolinum_R}{uniE09F}{57503}
\DeclareTextGlyphY{LinBiolinum_R}{lacute.sc}{57504}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A0}{57504}
\DeclareTextGlyphY{LinBiolinum_R}{lslash.sc}{57505}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A1}{57505}
\DeclareTextGlyphY{LinBiolinum_R}{nacute.sc}{57506}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A2}{57506}
\DeclareTextGlyphY{LinBiolinum_R}{ncaron.sc}{57507}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A3}{57507}
\DeclareTextGlyphY{LinBiolinum_R}{eng.sc}{57508}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A4}{57508}
\DeclareTextGlyphY{LinBiolinum_R}{ohungarumlaut.sc}{57509}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A5}{57509}
\DeclareTextGlyphY{LinBiolinum_R}{racute.sc}{57510}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A6}{57510}
\DeclareTextGlyphY{LinBiolinum_R}{rcaron.sc}{57511}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A7}{57511}
\DeclareTextGlyphY{LinBiolinum_R}{sacute.sc}{57512}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A8}{57512}
\DeclareTextGlyphY{LinBiolinum_R}{scedilla.sc}{57513}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0A9}{57513}
\DeclareTextGlyphY{LinBiolinum_R}{scaron.sc}{57514}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0AA}{57514}
\DeclareTextGlyphY{LinBiolinum_R}{tcedilla.sc}{57515}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0AB}{57515}
\DeclareTextGlyphY{LinBiolinum_R}{tbar.sc}{57516}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0AC}{57516}
\DeclareTextGlyphY{LinBiolinum_R}{uring.sc}{57517}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0AD}{57517}
\DeclareTextGlyphY{LinBiolinum_R}{uhungarumlaut.sc}{57518}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0AE}{57518}
\DeclareTextGlyphY{LinBiolinum_R}{zacute.sc}{57519}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0AF}{57519}
\DeclareTextGlyphY{LinBiolinum_R}{zdotaccent.sc}{57520}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0B0}{57520}
\DeclareTextGlyphY{LinBiolinum_R}{zcaron.sc}{57521}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0B1}{57521}
\DeclareTextGlyphY{LinBiolinum_R}{lcaron.sc}{57522}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0B2}{57522}
\DeclareTextGlyphY{LinBiolinum_R}{tcaron.sc}{57523}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0B3}{57523}
\DeclareTextGlyphY{LinBiolinum_R}{tcommaaccent.sc}{57524}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0B4}{57524}
\DeclareTextGlyphY{LinBiolinum_R}{scommaaccent.sc}{57525}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0B5}{57525}
\DeclareTextGlyphY{LinBiolinum_R}{idotaccent.sc}{57526}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0B6}{57526}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0BC}{57532}
\DeclareTextGlyphY{LinBiolinum_R}{ampersand.sc}{57533}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0BD}{57533}
\DeclareTextGlyphY{LinBiolinum_R}{a.scalt}{57534}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0BE}{57534}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0BF}{57535}
\DeclareTextGlyphY{LinBiolinum_R}{a.superior}{57536}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0C0}{57536}
\DeclareTextGlyphY{LinBiolinum_R}{b.superior}{57537}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0C1}{57537}
\DeclareTextGlyphY{LinBiolinum_R}{c.superior}{57538}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0C2}{57538}
\DeclareTextGlyphY{LinBiolinum_R}{d.superior}{57539}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0C3}{57539}
\DeclareTextGlyphY{LinBiolinum_R}{e.superior}{57540}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0C4}{57540}
\DeclareTextGlyphY{LinBiolinum_R}{f.superior}{57541}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0C5}{57541}
\DeclareTextGlyphY{LinBiolinum_R}{g.superior}{57542}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0C6}{57542}
\DeclareTextGlyphY{LinBiolinum_R}{k.superior}{57546}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0CA}{57546}
\DeclareTextGlyphY{LinBiolinum_R}{m.superior}{57548}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0CC}{57548}
\DeclareTextGlyphY{LinBiolinum_R}{o.superior}{57550}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0CE}{57550}
\DeclareTextGlyphY{LinBiolinum_R}{p.superior}{57551}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0CF}{57551}
\DeclareTextGlyphY{LinBiolinum_R}{q.superior}{57552}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0D0}{57552}
\DeclareTextGlyphY{LinBiolinum_R}{t.superior}{57555}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0D3}{57555}
\DeclareTextGlyphY{LinBiolinum_R}{u.superior}{57556}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0D4}{57556}
\DeclareTextGlyphY{LinBiolinum_R}{v.superior}{57557}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0D5}{57557}
\DeclareTextGlyphY{LinBiolinum_R}{z.superior}{57561}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0D9}{57561}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0DA}{57562}
\DeclareTextGlyphY{LinBiolinum_R}{f.short}{57568}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0E0}{57568}
\DeclareTextGlyphY{LinBiolinum_R}{f_f.short}{57569}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0E1}{57569}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0E8}{57576}
\DeclareTextGlyphY{LinBiolinum_R}{W.alt}{57577}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0E9}{57577}
\DeclareTextGlyphY{LinBiolinum_R}{V.alt}{57578}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0EA}{57578}
\DeclareTextGlyphY{LinBiolinum_R}{K.alt}{57579}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0EB}{57579}
\DeclareTextGlyphY{LinBiolinum_R}{R.alt}{57580}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0EC}{57580}
\DeclareTextGlyphY{LinBiolinum_R}{J.alt}{57581}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0ED}{57581}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0EE}{57582}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0EF}{57583}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0F0}{57584}
\DeclareTextGlyphY{LinBiolinum_R}{w.alt}{57585}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0F1}{57585}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0F2}{57586}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0F3}{57587}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0F4}{57588}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0F5}{57589}
\DeclareTextGlyphY{LinBiolinum_R}{y.alt}{57590}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0F6}{57590}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0F9}{57593}
\DeclareTextGlyphY{LinBiolinum_R}{uniE0FB}{57595}
\DeclareTextGlyphY{LinBiolinum_R}{kreis}{57600}
\DeclareTextGlyphY{LinBiolinum_R}{uniE100}{57600}
\DeclareTextGlyphY{LinBiolinum_R}{uniE101}{57601}
\DeclareTextGlyphY{LinBiolinum_R}{uniE104}{57604}
\DeclareTextGlyphY{LinBiolinum_R}{uniE105}{57605}
\DeclareTextGlyphY{LinBiolinum_R}{uniE106}{57606}
\DeclareTextGlyphY{LinBiolinum_R}{uniE107}{57607}
\DeclareTextGlyphY{LinBiolinum_R}{zero.taboldstyle}{57624}
\DeclareTextGlyphY{LinBiolinum_R}{uniE118}{57624}
\DeclareTextGlyphY{LinBiolinum_R}{one.taboldstyle}{57625}
\DeclareTextGlyphY{LinBiolinum_R}{uniE119}{57625}
\DeclareTextGlyphY{LinBiolinum_R}{two.taboldstyle}{57626}
\DeclareTextGlyphY{LinBiolinum_R}{uniE11A}{57626}
\DeclareTextGlyphY{LinBiolinum_R}{three.taboldstyle}{57627}
\DeclareTextGlyphY{LinBiolinum_R}{uniE11B}{57627}
\DeclareTextGlyphY{LinBiolinum_R}{four.taboldstyle}{57628}
\DeclareTextGlyphY{LinBiolinum_R}{uniE11C}{57628}
\DeclareTextGlyphY{LinBiolinum_R}{five.taboldstyle}{57629}
\DeclareTextGlyphY{LinBiolinum_R}{uniE11D}{57629}
\DeclareTextGlyphY{LinBiolinum_R}{six.taboldstyle}{57630}
\DeclareTextGlyphY{LinBiolinum_R}{uniE11E}{57630}
\DeclareTextGlyphY{LinBiolinum_R}{seven.taboldstyle}{57631}
\DeclareTextGlyphY{LinBiolinum_R}{uniE11F}{57631}
\DeclareTextGlyphY{LinBiolinum_R}{eight.taboldstyle}{57632}
\DeclareTextGlyphY{LinBiolinum_R}{uniE120}{57632}
\DeclareTextGlyphY{LinBiolinum_R}{nine.taboldstyle}{57633}
\DeclareTextGlyphY{LinBiolinum_R}{uniE121}{57633}
\DeclareTextGlyphY{LinBiolinum_R}{uniE128}{57640}
\DeclareTextGlyphY{LinBiolinum_R}{uniE129}{57641}
\DeclareTextGlyphY{LinBiolinum_R}{uniE12A}{57642}
\DeclareTextGlyphY{LinBiolinum_R}{uniE130}{57648}
\DeclareTextGlyphY{LinBiolinum_R}{b.inferior}{57673}
\DeclareTextGlyphY{LinBiolinum_R}{uniE149}{57673}
\DeclareTextGlyphY{LinBiolinum_R}{c.inferior}{57674}
\DeclareTextGlyphY{LinBiolinum_R}{uniE14A}{57674}
\DeclareTextGlyphY{LinBiolinum_R}{d.inferior}{57675}
\DeclareTextGlyphY{LinBiolinum_R}{uniE14B}{57675}
\DeclareTextGlyphY{LinBiolinum_R}{uniE14C}{57676}
\DeclareTextGlyphY{LinBiolinum_R}{f.inferior}{57677}
\DeclareTextGlyphY{LinBiolinum_R}{uniE14D}{57677}
\DeclareTextGlyphY{LinBiolinum_R}{g.inferior}{57678}
\DeclareTextGlyphY{LinBiolinum_R}{uniE14E}{57678}
\DeclareTextGlyphY{LinBiolinum_R}{h.inferior}{57679}
\DeclareTextGlyphY{LinBiolinum_R}{uniE14F}{57679}
\DeclareTextGlyphY{LinBiolinum_R}{i.inferior}{57680}
\DeclareTextGlyphY{LinBiolinum_R}{uniE150}{57680}
\DeclareTextGlyphY{LinBiolinum_R}{j.inferior}{57681}
\DeclareTextGlyphY{LinBiolinum_R}{uniE151}{57681}
\DeclareTextGlyphY{LinBiolinum_R}{k.inferior}{57682}
\DeclareTextGlyphY{LinBiolinum_R}{uniE152}{57682}
\DeclareTextGlyphY{LinBiolinum_R}{l.inferior}{57683}
\DeclareTextGlyphY{LinBiolinum_R}{uniE153}{57683}
\DeclareTextGlyphY{LinBiolinum_R}{m.inferior}{57684}
\DeclareTextGlyphY{LinBiolinum_R}{uniE154}{57684}
\DeclareTextGlyphY{LinBiolinum_R}{n.inferior}{57685}
\DeclareTextGlyphY{LinBiolinum_R}{uniE155}{57685}
\DeclareTextGlyphY{LinBiolinum_R}{p.inferior}{57687}
\DeclareTextGlyphY{LinBiolinum_R}{uniE157}{57687}
\DeclareTextGlyphY{LinBiolinum_R}{q.inferior}{57688}
\DeclareTextGlyphY{LinBiolinum_R}{uniE158}{57688}
\DeclareTextGlyphY{LinBiolinum_R}{r.inferior}{57689}
\DeclareTextGlyphY{LinBiolinum_R}{uniE159}{57689}
\DeclareTextGlyphY{LinBiolinum_R}{s.inferior}{57690}
\DeclareTextGlyphY{LinBiolinum_R}{uniE15A}{57690}
\DeclareTextGlyphY{LinBiolinum_R}{t.inferior}{57691}
\DeclareTextGlyphY{LinBiolinum_R}{uniE15B}{57691}
\DeclareTextGlyphY{LinBiolinum_R}{u.inferior}{57692}
\DeclareTextGlyphY{LinBiolinum_R}{uniE15C}{57692}
\DeclareTextGlyphY{LinBiolinum_R}{v.inferior}{57693}
\DeclareTextGlyphY{LinBiolinum_R}{uniE15D}{57693}
\DeclareTextGlyphY{LinBiolinum_R}{w.inferior}{57694}
\DeclareTextGlyphY{LinBiolinum_R}{uniE15E}{57694}
\DeclareTextGlyphY{LinBiolinum_R}{y.inferior}{57696}
\DeclareTextGlyphY{LinBiolinum_R}{uniE160}{57696}
\DeclareTextGlyphY{LinBiolinum_R}{z.inferior}{57697}
\DeclareTextGlyphY{LinBiolinum_R}{uniE161}{57697}
\DeclareTextGlyphY{LinBiolinum_R}{uniE162}{57698}
\DeclareTextGlyphY{LinBiolinum_R}{uniE163}{57699}
\DeclareTextGlyphY{LinBiolinum_R}{uniE164}{57700}
\DeclareTextGlyphY{LinBiolinum_R}{uniE165}{57701}
\DeclareTextGlyphY{LinBiolinum_R}{grave.cap}{58200}
\DeclareTextGlyphY{LinBiolinum_R}{uniE358}{58200}
\DeclareTextGlyphY{LinBiolinum_R}{acute.cap}{58201}
\DeclareTextGlyphY{LinBiolinum_R}{uniE359}{58201}
\DeclareTextGlyphY{LinBiolinum_R}{circumflex.cap}{58202}
\DeclareTextGlyphY{LinBiolinum_R}{uniE35A}{58202}
\DeclareTextGlyphY{LinBiolinum_R}{caron.cap}{58203}
\DeclareTextGlyphY{LinBiolinum_R}{uniE35B}{58203}
\DeclareTextGlyphY{LinBiolinum_R}{breve.cap}{58204}
\DeclareTextGlyphY{LinBiolinum_R}{uniE35C}{58204}
\DeclareTextGlyphY{LinBiolinum_R}{hungarumlaut.cap}{58205}
\DeclareTextGlyphY{LinBiolinum_R}{uniE35D}{58205}
\DeclareTextGlyphY{LinBiolinum_R}{space_uni030F.cap}{58206}
\DeclareTextGlyphY{LinBiolinum_R}{uniE35E}{58206}
\DeclareTextGlyphY{LinBiolinum_R}{breveinvertedcmb.cap}{58207}
\DeclareTextGlyphY{LinBiolinum_R}{uniE35F}{58207}
\DeclareTextGlyphY{LinBiolinum_R}{breve.cyrcap}{58208}
\DeclareTextGlyphY{LinBiolinum_R}{uniE360}{58208}
\DeclareTextGlyphY{LinBiolinum_R}{breve.cyr}{58209}
\DeclareTextGlyphY{LinBiolinum_R}{uniE361}{58209}
\DeclareTextGlyphY{LinBiolinum_R}{dieresis.cap}{58210}
\DeclareTextGlyphY{LinBiolinum_R}{uniE362}{58210}
\DeclareTextGlyphY{LinBiolinum_R}{hookabovecomb.cap}{58211}
\DeclareTextGlyphY{LinBiolinum_R}{uniE363}{58211}
\DeclareTextGlyphY{LinBiolinum_R}{dotaccent.cap}{58212}
\DeclareTextGlyphY{LinBiolinum_R}{uniE364}{58212}
\DeclareTextGlyphY{LinBiolinum_R}{uniE420}{58400}
\DeclareTextGlyphY{LinBiolinum_R}{zero.slash}{63032}
\DeclareTextGlyphY{LinBiolinum_R}{uniF638}{63032}
\DeclareTextGlyphY{LinBiolinum_R}{parenleft.sc}{63150}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6AE}{63150}
\DeclareTextGlyphY{LinBiolinum_R}{parenright.sc}{63151}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6AF}{63151}
\DeclareTextGlyphY{LinBiolinum_R}{bracketleft.sc}{63152}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B0}{63152}
\DeclareTextGlyphY{LinBiolinum_R}{bracketright.sc}{63153}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B1}{63153}
\DeclareTextGlyphY{LinBiolinum_R}{braceleft.sc}{63154}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B2}{63154}
\DeclareTextGlyphY{LinBiolinum_R}{braceright.sc}{63155}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B3}{63155}
\DeclareTextGlyphY{LinBiolinum_R}{exclamdown.sc}{63156}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B4}{63156}
\DeclareTextGlyphY{LinBiolinum_R}{questiondown.sc}{63157}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B5}{63157}
\DeclareTextGlyphY{LinBiolinum_R}{guillemotleft.sc}{63158}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B6}{63158}
\DeclareTextGlyphY{LinBiolinum_R}{guillemotright.sc}{63159}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B7}{63159}
\DeclareTextGlyphY{LinBiolinum_R}{guilsinglleft.sc}{63160}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B8}{63160}
\DeclareTextGlyphY{LinBiolinum_R}{guilsinglright.sc}{63161}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6B9}{63161}
\DeclareTextGlyphY{LinBiolinum_R}{hyphen.cap}{63162}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6BA}{63162}
\DeclareTextGlyphY{LinBiolinum_R}{uniF6BE}{63166}
\DeclareTextGlyphY{LinBiolinum_R}{f_f}{64256}
\DeclareTextGlyphY{LinBiolinum_R}{uniFB00}{64256}
\DeclareTextGlyphY{LinBiolinum_R}{f_i}{64257}
\DeclareTextGlyphY{LinBiolinum_R}{uniFB01}{64257}
\DeclareTextGlyphY{LinBiolinum_R}{f_l}{64258}
\DeclareTextGlyphY{LinBiolinum_R}{uniFB02}{64258}
\DeclareTextGlyphY{LinBiolinum_R}{f_f_i}{64259}
\DeclareTextGlyphY{LinBiolinum_R}{uniFB03}{64259}
\DeclareTextGlyphY{LinBiolinum_R}{f_f_l}{64260}
\DeclareTextGlyphY{LinBiolinum_R}{uniFB04}{64260}
\DeclareTextGlyphY{LinBiolinum_R}{longs_t}{64261}
\DeclareTextGlyphY{LinBiolinum_R}{uniFB05}{64261}
\DeclareTextGlyphY{LinBiolinum_R}{s_t}{64262}
\DeclareTextGlyphY{LinBiolinum_R}{uniFB06}{64262}
\DeclareTextGlyphY{LinBiolinum_R}{uniFFFD}{65533}


==> LinLibertine_I.tex <==
\DeclareTextGlyphY{LinLibertine_I}{space}{32}
\DeclareTextGlyphY{LinLibertine_I}{uni0020}{32}
\DeclareTextGlyphY{LinLibertine_I}{zero}{48}
\DeclareTextGlyphY{LinLibertine_I}{uni0030}{48}
\DeclareTextGlyphY{LinLibertine_I}{one}{49}
\DeclareTextGlyphY{LinLibertine_I}{uni0031}{49}
\DeclareTextGlyphY{LinLibertine_I}{two}{50}
\DeclareTextGlyphY{LinLibertine_I}{uni0032}{50}
\DeclareTextGlyphY{LinLibertine_I}{three}{51}
\DeclareTextGlyphY{LinLibertine_I}{uni0033}{51}
\DeclareTextGlyphY{LinLibertine_I}{four}{52}
\DeclareTextGlyphY{LinLibertine_I}{uni0034}{52}
\DeclareTextGlyphY{LinLibertine_I}{five}{53}
\DeclareTextGlyphY{LinLibertine_I}{uni0035}{53}
\DeclareTextGlyphY{LinLibertine_I}{six}{54}
\DeclareTextGlyphY{LinLibertine_I}{uni0036}{54}
\DeclareTextGlyphY{LinLibertine_I}{seven}{55}
\DeclareTextGlyphY{LinLibertine_I}{uni0037}{55}
\DeclareTextGlyphY{LinLibertine_I}{eight}{56}
\DeclareTextGlyphY{LinLibertine_I}{uni0038}{56}
\DeclareTextGlyphY{LinLibertine_I}{nine}{57}
\DeclareTextGlyphY{LinLibertine_I}{uni0039}{57}
\DeclareTextGlyphY{LinLibertine_I}{A}{65}
\DeclareTextGlyphY{LinLibertine_I}{uni0041}{65}
\DeclareTextGlyphY{LinLibertine_I}{B}{66}
\DeclareTextGlyphY{LinLibertine_I}{uni0042}{66}
\DeclareTextGlyphY{LinLibertine_I}{C}{67}
\DeclareTextGlyphY{LinLibertine_I}{uni0043}{67}
\DeclareTextGlyphY{LinLibertine_I}{D}{68}
\DeclareTextGlyphY{LinLibertine_I}{uni0044}{68}
\DeclareTextGlyphY{LinLibertine_I}{E}{69}
\DeclareTextGlyphY{LinLibertine_I}{uni0045}{69}
\DeclareTextGlyphY{LinLibertine_I}{F}{70}
\DeclareTextGlyphY{LinLibertine_I}{uni0046}{70}
\DeclareTextGlyphY{LinLibertine_I}{G}{71}
\DeclareTextGlyphY{LinLibertine_I}{uni0047}{71}
\DeclareTextGlyphY{LinLibertine_I}{H}{72}
\DeclareTextGlyphY{LinLibertine_I}{uni0048}{72}
\DeclareTextGlyphY{LinLibertine_I}{I}{73}
\DeclareTextGlyphY{LinLibertine_I}{uni0049}{73}
\DeclareTextGlyphY{LinLibertine_I}{J}{74}
\DeclareTextGlyphY{LinLibertine_I}{uni004A}{74}
\DeclareTextGlyphY{LinLibertine_I}{K}{75}
\DeclareTextGlyphY{LinLibertine_I}{uni004B}{75}
\DeclareTextGlyphY{LinLibertine_I}{L}{76}
\DeclareTextGlyphY{LinLibertine_I}{uni004C}{76}
\DeclareTextGlyphY{LinLibertine_I}{M}{77}
\DeclareTextGlyphY{LinLibertine_I}{uni004D}{77}
\DeclareTextGlyphY{LinLibertine_I}{N}{78}
\DeclareTextGlyphY{LinLibertine_I}{uni004E}{78}
\DeclareTextGlyphY{LinLibertine_I}{O}{79}
\DeclareTextGlyphY{LinLibertine_I}{uni004F}{79}
\DeclareTextGlyphY{LinLibertine_I}{P}{80}
\DeclareTextGlyphY{LinLibertine_I}{uni0050}{80}
\DeclareTextGlyphY{LinLibertine_I}{Q}{81}
\DeclareTextGlyphY{LinLibertine_I}{uni0051}{81}
\DeclareTextGlyphY{LinLibertine_I}{R}{82}
\DeclareTextGlyphY{LinLibertine_I}{uni0052}{82}
\DeclareTextGlyphY{LinLibertine_I}{S}{83}
\DeclareTextGlyphY{LinLibertine_I}{uni0053}{83}
\DeclareTextGlyphY{LinLibertine_I}{T}{84}
\DeclareTextGlyphY{LinLibertine_I}{uni0054}{84}
\DeclareTextGlyphY{LinLibertine_I}{U}{85}
\DeclareTextGlyphY{LinLibertine_I}{uni0055}{85}
\DeclareTextGlyphY{LinLibertine_I}{V}{86}
\DeclareTextGlyphY{LinLibertine_I}{uni0056}{86}
\DeclareTextGlyphY{LinLibertine_I}{W}{87}
\DeclareTextGlyphY{LinLibertine_I}{uni0057}{87}
\DeclareTextGlyphY{LinLibertine_I}{X}{88}
\DeclareTextGlyphY{LinLibertine_I}{uni0058}{88}
\DeclareTextGlyphY{LinLibertine_I}{Y}{89}
\DeclareTextGlyphY{LinLibertine_I}{uni0059}{89}
\DeclareTextGlyphY{LinLibertine_I}{Z}{90}
\DeclareTextGlyphY{LinLibertine_I}{uni005A}{90}
\DeclareTextGlyphY{LinLibertine_I}{asciicircum}{94}
\DeclareTextGlyphY{LinLibertine_I}{uni005E}{94}
\DeclareTextGlyphY{LinLibertine_I}{Adieresis}{196}
\DeclareTextGlyphY{LinLibertine_I}{uni00C4}{196}
\DeclareTextGlyphY{LinLibertine_I}{Aring}{197}
\DeclareTextGlyphY{LinLibertine_I}{uni00C5}{197}
\DeclareTextGlyphY{LinLibertine_I}{AE}{198}
\DeclareTextGlyphY{LinLibertine_I}{uni00C6}{198}
\DeclareTextGlyphY{LinLibertine_I}{Ccedilla}{199}
\DeclareTextGlyphY{LinLibertine_I}{uni00C7}{199}
\DeclareTextGlyphY{LinLibertine_I}{Odieresis}{214}
\DeclareTextGlyphY{LinLibertine_I}{uni00D6}{214}
\DeclareTextGlyphY{LinLibertine_I}{Oslash}{216}
\DeclareTextGlyphY{LinLibertine_I}{uni00D8}{216}
\DeclareTextGlyphY{LinLibertine_I}{Udieresis}{220}
\DeclareTextGlyphY{LinLibertine_I}{uni00DC}{220}
\DeclareTextGlyphY{LinLibertine_I}{Thorn}{222}
\DeclareTextGlyphY{LinLibertine_I}{uni00DE}{222}
\DeclareTextGlyphY{LinLibertine_I}{iogonek}{303}
\DeclareTextGlyphY{LinLibertine_I}{uni012F}{303}
\DeclareTextGlyphY{LinLibertine_I}{IJ}{306}
\DeclareTextGlyphY{LinLibertine_I}{uni0132}{306}
\DeclareTextGlyphY{LinLibertine_I}{Eng}{330}
\DeclareTextGlyphY{LinLibertine_I}{uni014A}{330}
\DeclareTextGlyphY{LinLibertine_I}{Ohungarumlaut}{336}
\DeclareTextGlyphY{LinLibertine_I}{uni0150}{336}
\DeclareTextGlyphY{LinLibertine_I}{OE}{338}
\DeclareTextGlyphY{LinLibertine_I}{uni0152}{338}
\DeclareTextGlyphY{LinLibertine_I}{Uhungarumlaut}{368}
\DeclareTextGlyphY{LinLibertine_I}{uni0170}{368}
\DeclareTextGlyphY{LinLibertine_I}{Alpha}{913}
\DeclareTextGlyphY{LinLibertine_I}{uni0391}{913}
\DeclareTextGlyphY{LinLibertine_I}{Beta}{914}
\DeclareTextGlyphY{LinLibertine_I}{uni0392}{914}
\DeclareTextGlyphY{LinLibertine_I}{Gamma}{915}
\DeclareTextGlyphY{LinLibertine_I}{uni0393}{915}
\DeclareTextGlyphY{LinLibertine_I}{Delta}{916}
\DeclareTextGlyphY{LinLibertine_I}{uni0394}{916}
\DeclareTextGlyphY{LinLibertine_I}{Epsilon}{917}
\DeclareTextGlyphY{LinLibertine_I}{uni0395}{917}
\DeclareTextGlyphY{LinLibertine_I}{Zeta}{918}
\DeclareTextGlyphY{LinLibertine_I}{uni0396}{918}
\DeclareTextGlyphY{LinLibertine_I}{Eta}{919}
\DeclareTextGlyphY{LinLibertine_I}{uni0397}{919}
\DeclareTextGlyphY{LinLibertine_I}{Theta}{920}
\DeclareTextGlyphY{LinLibertine_I}{uni0398}{920}
\DeclareTextGlyphY{LinLibertine_I}{Iota}{921}
\DeclareTextGlyphY{LinLibertine_I}{uni0399}{921}
\DeclareTextGlyphY{LinLibertine_I}{Kappa}{922}
\DeclareTextGlyphY{LinLibertine_I}{uni039A}{922}
\DeclareTextGlyphY{LinLibertine_I}{Lambda}{923}
\DeclareTextGlyphY{LinLibertine_I}{uni039B}{923}
\DeclareTextGlyphY{LinLibertine_I}{Mu}{924}
\DeclareTextGlyphY{LinLibertine_I}{uni039C}{924}
\DeclareTextGlyphY{LinLibertine_I}{Nu}{925}
\DeclareTextGlyphY{LinLibertine_I}{uni039D}{925}
\DeclareTextGlyphY{LinLibertine_I}{Xi}{926}
\DeclareTextGlyphY{LinLibertine_I}{uni039E}{926}
\DeclareTextGlyphY{LinLibertine_I}{Omicron}{927}
\DeclareTextGlyphY{LinLibertine_I}{uni039F}{927}
\DeclareTextGlyphY{LinLibertine_I}{Pi}{928}
\DeclareTextGlyphY{LinLibertine_I}{uni03A0}{928}
\DeclareTextGlyphY{LinLibertine_I}{Rho}{929}
\DeclareTextGlyphY{LinLibertine_I}{uni03A1}{929}
\DeclareTextGlyphY{LinLibertine_I}{Sigma}{931}
\DeclareTextGlyphY{LinLibertine_I}{uni03A3}{931}
\DeclareTextGlyphY{LinLibertine_I}{Tau}{932}
\DeclareTextGlyphY{LinLibertine_I}{uni03A4}{932}
\DeclareTextGlyphY{LinLibertine_I}{Upsilon}{933}
\DeclareTextGlyphY{LinLibertine_I}{uni03A5}{933}
\DeclareTextGlyphY{LinLibertine_I}{Phi}{934}
\DeclareTextGlyphY{LinLibertine_I}{uni03A6}{934}
\DeclareTextGlyphY{LinLibertine_I}{Chi}{935}
\DeclareTextGlyphY{LinLibertine_I}{uni03A7}{935}
\DeclareTextGlyphY{LinLibertine_I}{Psi}{936}
\DeclareTextGlyphY{LinLibertine_I}{uni03A8}{936}
\DeclareTextGlyphY{LinLibertine_I}{Omega}{937}
\DeclareTextGlyphY{LinLibertine_I}{uni03A9}{937}
\DeclareTextGlyphY{LinLibertine_I}{Iotadieresis}{938}
\DeclareTextGlyphY{LinLibertine_I}{uni03AA}{938}
\DeclareTextGlyphY{LinLibertine_I}{Upsilon1}{978}
\DeclareTextGlyphY{LinLibertine_I}{uni03D2}{978}
\DeclareTextGlyphY{LinLibertine_I}{afii10051}{1026}
\DeclareTextGlyphY{LinLibertine_I}{uni0402}{1026}
\DeclareTextGlyphY{LinLibertine_I}{afii10053}{1028}
\DeclareTextGlyphY{LinLibertine_I}{uni0404}{1028}
\DeclareTextGlyphY{LinLibertine_I}{afii10054}{1029}
\DeclareTextGlyphY{LinLibertine_I}{uni0405}{1029}
\DeclareTextGlyphY{LinLibertine_I}{afii10055}{1030}
\DeclareTextGlyphY{LinLibertine_I}{uni0406}{1030}
\DeclareTextGlyphY{LinLibertine_I}{afii10056}{1031}
\DeclareTextGlyphY{LinLibertine_I}{uni0407}{1031}
\DeclareTextGlyphY{LinLibertine_I}{afii10057}{1032}
\DeclareTextGlyphY{LinLibertine_I}{uni0408}{1032}
\DeclareTextGlyphY{LinLibertine_I}{afii10058}{1033}
\DeclareTextGlyphY{LinLibertine_I}{uni0409}{1033}
\DeclareTextGlyphY{LinLibertine_I}{afii10059}{1034}
\DeclareTextGlyphY{LinLibertine_I}{uni040A}{1034}
\DeclareTextGlyphY{LinLibertine_I}{afii10060}{1035}
\DeclareTextGlyphY{LinLibertine_I}{uni040B}{1035}
\DeclareTextGlyphY{LinLibertine_I}{afii10061}{1036}
\DeclareTextGlyphY{LinLibertine_I}{uni040C}{1036}
\DeclareTextGlyphY{LinLibertine_I}{uni040D}{1037}
\DeclareTextGlyphY{LinLibertine_I}{afii10062}{1038}
\DeclareTextGlyphY{LinLibertine_I}{uni040E}{1038}
\DeclareTextGlyphY{LinLibertine_I}{afii10145}{1039}
\DeclareTextGlyphY{LinLibertine_I}{uni040F}{1039}
\DeclareTextGlyphY{LinLibertine_I}{afii10017}{1040}
\DeclareTextGlyphY{LinLibertine_I}{uni0410}{1040}
\DeclareTextGlyphY{LinLibertine_I}{afii10018}{1041}
\DeclareTextGlyphY{LinLibertine_I}{uni0411}{1041}
\DeclareTextGlyphY{LinLibertine_I}{afii10019}{1042}
\DeclareTextGlyphY{LinLibertine_I}{uni0412}{1042}
\DeclareTextGlyphY{LinLibertine_I}{afii10020}{1043}
\DeclareTextGlyphY{LinLibertine_I}{uni0413}{1043}
\DeclareTextGlyphY{LinLibertine_I}{afii10021}{1044}
\DeclareTextGlyphY{LinLibertine_I}{uni0414}{1044}
\DeclareTextGlyphY{LinLibertine_I}{afii10022}{1045}
\DeclareTextGlyphY{LinLibertine_I}{uni0415}{1045}
\DeclareTextGlyphY{LinLibertine_I}{afii10024}{1046}
\DeclareTextGlyphY{LinLibertine_I}{uni0416}{1046}
\DeclareTextGlyphY{LinLibertine_I}{afii10025}{1047}
\DeclareTextGlyphY{LinLibertine_I}{uni0417}{1047}
\DeclareTextGlyphY{LinLibertine_I}{afii10026}{1048}
\DeclareTextGlyphY{LinLibertine_I}{uni0418}{1048}
\DeclareTextGlyphY{LinLibertine_I}{afii10027}{1049}
\DeclareTextGlyphY{LinLibertine_I}{uni0419}{1049}
\DeclareTextGlyphY{LinLibertine_I}{afii10028}{1050}
\DeclareTextGlyphY{LinLibertine_I}{uni041A}{1050}
\DeclareTextGlyphY{LinLibertine_I}{afii10029}{1051}
\DeclareTextGlyphY{LinLibertine_I}{uni041B}{1051}
\DeclareTextGlyphY{LinLibertine_I}{afii10030}{1052}
\DeclareTextGlyphY{LinLibertine_I}{uni041C}{1052}
\DeclareTextGlyphY{LinLibertine_I}{afii10031}{1053}
\DeclareTextGlyphY{LinLibertine_I}{uni041D}{1053}
\DeclareTextGlyphY{LinLibertine_I}{afii10032}{1054}
\DeclareTextGlyphY{LinLibertine_I}{uni041E}{1054}
\DeclareTextGlyphY{LinLibertine_I}{afii10033}{1055}
\DeclareTextGlyphY{LinLibertine_I}{uni041F}{1055}
\DeclareTextGlyphY{LinLibertine_I}{afii10034}{1056}
\DeclareTextGlyphY{LinLibertine_I}{uni0420}{1056}
\DeclareTextGlyphY{LinLibertine_I}{afii10035}{1057}
\DeclareTextGlyphY{LinLibertine_I}{uni0421}{1057}
\DeclareTextGlyphY{LinLibertine_I}{afii10036}{1058}
\DeclareTextGlyphY{LinLibertine_I}{uni0422}{1058}
\DeclareTextGlyphY{LinLibertine_I}{afii10037}{1059}
\DeclareTextGlyphY{LinLibertine_I}{uni0423}{1059}
\DeclareTextGlyphY{LinLibertine_I}{afii10038}{1060}
\DeclareTextGlyphY{LinLibertine_I}{uni0424}{1060}
\DeclareTextGlyphY{LinLibertine_I}{afii10039}{1061}
\DeclareTextGlyphY{LinLibertine_I}{uni0425}{1061}
\DeclareTextGlyphY{LinLibertine_I}{afii10040}{1062}
\DeclareTextGlyphY{LinLibertine_I}{uni0426}{1062}
\DeclareTextGlyphY{LinLibertine_I}{afii10041}{1063}
\DeclareTextGlyphY{LinLibertine_I}{uni0427}{1063}
\DeclareTextGlyphY{LinLibertine_I}{afii10042}{1064}
\DeclareTextGlyphY{LinLibertine_I}{uni0428}{1064}
\DeclareTextGlyphY{LinLibertine_I}{afii10043}{1065}
\DeclareTextGlyphY{LinLibertine_I}{uni0429}{1065}
\DeclareTextGlyphY{LinLibertine_I}{afii10044}{1066}
\DeclareTextGlyphY{LinLibertine_I}{uni042A}{1066}
\DeclareTextGlyphY{LinLibertine_I}{afii10045}{1067}
\DeclareTextGlyphY{LinLibertine_I}{uni042B}{1067}
\DeclareTextGlyphY{LinLibertine_I}{afii10046}{1068}
\DeclareTextGlyphY{LinLibertine_I}{uni042C}{1068}
\DeclareTextGlyphY{LinLibertine_I}{afii10047}{1069}
\DeclareTextGlyphY{LinLibertine_I}{uni042D}{1069}
\DeclareTextGlyphY{LinLibertine_I}{afii10048}{1070}
\DeclareTextGlyphY{LinLibertine_I}{uni042E}{1070}
\DeclareTextGlyphY{LinLibertine_I}{afii10049}{1071}
\DeclareTextGlyphY{LinLibertine_I}{uni042F}{1071}
\DeclareTextGlyphY{LinLibertine_I}{uni05C6}{1478}
\DeclareTextGlyphY{LinLibertine_I}{afii57664}{1488}
\DeclareTextGlyphY{LinLibertine_I}{uni05D0}{1488}
\DeclareTextGlyphY{LinLibertine_I}{afii57665}{1489}
\DeclareTextGlyphY{LinLibertine_I}{uni05D1}{1489}
\DeclareTextGlyphY{LinLibertine_I}{afii57666}{1490}
\DeclareTextGlyphY{LinLibertine_I}{uni05D2}{1490}
\DeclareTextGlyphY{LinLibertine_I}{afii57667}{1491}
\DeclareTextGlyphY{LinLibertine_I}{uni05D3}{1491}
\DeclareTextGlyphY{LinLibertine_I}{afii57668}{1492}
\DeclareTextGlyphY{LinLibertine_I}{uni05D4}{1492}
\DeclareTextGlyphY{LinLibertine_I}{afii57669}{1493}
\DeclareTextGlyphY{LinLibertine_I}{uni05D5}{1493}
\DeclareTextGlyphY{LinLibertine_I}{afii57670}{1494}
\DeclareTextGlyphY{LinLibertine_I}{uni05D6}{1494}
\DeclareTextGlyphY{LinLibertine_I}{afii57671}{1495}
\DeclareTextGlyphY{LinLibertine_I}{uni05D7}{1495}
\DeclareTextGlyphY{LinLibertine_I}{afii57672}{1496}
\DeclareTextGlyphY{LinLibertine_I}{uni05D8}{1496}
\DeclareTextGlyphY{LinLibertine_I}{afii57673}{1497}
\DeclareTextGlyphY{LinLibertine_I}{uni05D9}{1497}
\DeclareTextGlyphY{LinLibertine_I}{afii57674}{1498}
\DeclareTextGlyphY{LinLibertine_I}{uni05DA}{1498}
\DeclareTextGlyphY{LinLibertine_I}{afii57675}{1499}
\DeclareTextGlyphY{LinLibertine_I}{uni05DB}{1499}
\DeclareTextGlyphY{LinLibertine_I}{afii57676}{1500}
\DeclareTextGlyphY{LinLibertine_I}{uni05DC}{1500}
\DeclareTextGlyphY{LinLibertine_I}{afii57677}{1501}
\DeclareTextGlyphY{LinLibertine_I}{uni05DD}{1501}
\DeclareTextGlyphY{LinLibertine_I}{afii57678}{1502}
\DeclareTextGlyphY{LinLibertine_I}{uni05DE}{1502}
\DeclareTextGlyphY{LinLibertine_I}{afii57679}{1503}
\DeclareTextGlyphY{LinLibertine_I}{uni05DF}{1503}
\DeclareTextGlyphY{LinLibertine_I}{afii57680}{1504}
\DeclareTextGlyphY{LinLibertine_I}{uni05E0}{1504}
\DeclareTextGlyphY{LinLibertine_I}{afii57681}{1505}
\DeclareTextGlyphY{LinLibertine_I}{uni05E1}{1505}
\DeclareTextGlyphY{LinLibertine_I}{afii57682}{1506}
\DeclareTextGlyphY{LinLibertine_I}{uni05E2}{1506}
\DeclareTextGlyphY{LinLibertine_I}{afii57683}{1507}
\DeclareTextGlyphY{LinLibertine_I}{uni05E3}{1507}
\DeclareTextGlyphY{LinLibertine_I}{afii57684}{1508}
\DeclareTextGlyphY{LinLibertine_I}{uni05E4}{1508}
\DeclareTextGlyphY{LinLibertine_I}{afii57685}{1509}
\DeclareTextGlyphY{LinLibertine_I}{uni05E5}{1509}
\DeclareTextGlyphY{LinLibertine_I}{afii57686}{1510}
\DeclareTextGlyphY{LinLibertine_I}{uni05E6}{1510}
\DeclareTextGlyphY{LinLibertine_I}{afii57687}{1511}
\DeclareTextGlyphY{LinLibertine_I}{uni05E7}{1511}
\DeclareTextGlyphY{LinLibertine_I}{afii57688}{1512}
\DeclareTextGlyphY{LinLibertine_I}{uni05E8}{1512}
\DeclareTextGlyphY{LinLibertine_I}{afii57689}{1513}
\DeclareTextGlyphY{LinLibertine_I}{uni05E9}{1513}
\DeclareTextGlyphY{LinLibertine_I}{afii57690}{1514}
\DeclareTextGlyphY{LinLibertine_I}{uni05EA}{1514}
\DeclareTextGlyphY{LinLibertine_I}{afii57716}{1520}
\DeclareTextGlyphY{LinLibertine_I}{uni05F0}{1520}
\DeclareTextGlyphY{LinLibertine_I}{afii57717}{1521}
\DeclareTextGlyphY{LinLibertine_I}{uni05F1}{1521}
\DeclareTextGlyphY{LinLibertine_I}{afii57718}{1522}
\DeclareTextGlyphY{LinLibertine_I}{uni05F2}{1522}
\DeclareTextGlyphY{LinLibertine_I}{uni05F3}{1523}
\DeclareTextGlyphY{LinLibertine_I}{uni05F4}{1524}
\DeclareTextGlyphY{LinLibertine_I}{Germandbls}{7838}
\DeclareTextGlyphY{LinLibertine_I}{uni1E9E}{7838}
\DeclareTextGlyphY{LinLibertine_I}{Oneroman}{8544}
\DeclareTextGlyphY{LinLibertine_I}{uni2160}{8544}
\DeclareTextGlyphY{LinLibertine_I}{Tworoman}{8545}
\DeclareTextGlyphY{LinLibertine_I}{uni2161}{8545}
\DeclareTextGlyphY{LinLibertine_I}{Threeroman}{8546}
\DeclareTextGlyphY{LinLibertine_I}{uni2162}{8546}
\DeclareTextGlyphY{LinLibertine_I}{Fourroman}{8547}
\DeclareTextGlyphY{LinLibertine_I}{uni2163}{8547}
\DeclareTextGlyphY{LinLibertine_I}{Fiveroman}{8548}
\DeclareTextGlyphY{LinLibertine_I}{uni2164}{8548}
\DeclareTextGlyphY{LinLibertine_I}{Sixroman}{8549}
\DeclareTextGlyphY{LinLibertine_I}{uni2165}{8549}
\DeclareTextGlyphY{LinLibertine_I}{Sevenroman}{8550}
\DeclareTextGlyphY{LinLibertine_I}{uni2166}{8550}
\DeclareTextGlyphY{LinLibertine_I}{Eightroman}{8551}
\DeclareTextGlyphY{LinLibertine_I}{uni2167}{8551}
\DeclareTextGlyphY{LinLibertine_I}{Nineroman}{8552}
\DeclareTextGlyphY{LinLibertine_I}{uni2168}{8552}
\DeclareTextGlyphY{LinLibertine_I}{Tenroman}{8553}
\DeclareTextGlyphY{LinLibertine_I}{uni2169}{8553}
\DeclareTextGlyphY{LinLibertine_I}{Elevenroman}{8554}
\DeclareTextGlyphY{LinLibertine_I}{uni216A}{8554}
\DeclareTextGlyphY{LinLibertine_I}{Twelveroman}{8555}
\DeclareTextGlyphY{LinLibertine_I}{uni216B}{8555}
\DeclareTextGlyphY{LinLibertine_I}{uni216C}{8556}
\DeclareTextGlyphY{LinLibertine_I}{uni216D}{8557}
\DeclareTextGlyphY{LinLibertine_I}{uni216E}{8558}
\DeclareTextGlyphY{LinLibertine_I}{uni216F}{8559}
\DeclareTextGlyphY{LinLibertine_I}{uni24B6}{9398}
\DeclareTextGlyphY{LinLibertine_I}{uni24B7}{9399}
\DeclareTextGlyphY{LinLibertine_I}{uni24B8}{9400}
\DeclareTextGlyphY{LinLibertine_I}{uni24B9}{9401}
\DeclareTextGlyphY{LinLibertine_I}{uni24BA}{9402}
\DeclareTextGlyphY{LinLibertine_I}{uni24BB}{9403}
\DeclareTextGlyphY{LinLibertine_I}{uni24BC}{9404}
\DeclareTextGlyphY{LinLibertine_I}{uni24BE}{9406}
\DeclareTextGlyphY{LinLibertine_I}{uni24BF}{9407}
\DeclareTextGlyphY{LinLibertine_I}{uni24C0}{9408}
\DeclareTextGlyphY{LinLibertine_I}{uni24C1}{9409}
\DeclareTextGlyphY{LinLibertine_I}{uni24C2}{9410}
\DeclareTextGlyphY{LinLibertine_I}{uni24C3}{9411}
\DeclareTextGlyphY{LinLibertine_I}{uni24C4}{9412}
\DeclareTextGlyphY{LinLibertine_I}{uni24C5}{9413}
\DeclareTextGlyphY{LinLibertine_I}{uni24C6}{9414}
\DeclareTextGlyphY{LinLibertine_I}{uni24C7}{9415}
\DeclareTextGlyphY{LinLibertine_I}{uni24C8}{9416}
\DeclareTextGlyphY{LinLibertine_I}{uni24CA}{9418}
\DeclareTextGlyphY{LinLibertine_I}{uni24CB}{9419}
\DeclareTextGlyphY{LinLibertine_I}{uni24CC}{9420}
\DeclareTextGlyphY{LinLibertine_I}{uni24CD}{9421}
\DeclareTextGlyphY{LinLibertine_I}{uni24CE}{9422}
\DeclareTextGlyphY{LinLibertine_I}{uni24CF}{9423}
\DeclareTextGlyphY{LinLibertine_I}{Tux}{57344}
\DeclareTextGlyphY{LinLibertine_I}{uniE000}{57344}
\DeclareTextGlyphY{LinLibertine_I}{uniE001}{57345}
\DeclareTextGlyphY{LinLibertine_I}{uniE002}{57346}
\DeclareTextGlyphY{LinLibertine_I}{uniE003}{57347}
\DeclareTextGlyphY{LinLibertine_I}{uniE004}{57348}
\DeclareTextGlyphY{LinLibertine_I}{uniE005}{57349}
\DeclareTextGlyphY{LinLibertine_I}{uniE006}{57350}
\DeclareTextGlyphY{LinLibertine_I}{uniE007}{57351}
\DeclareTextGlyphY{LinLibertine_I}{uniE008}{57352}
\DeclareTextGlyphY{LinLibertine_I}{uniE009}{57353}
\DeclareTextGlyphY{LinLibertine_I}{uniE00A}{57354}
\DeclareTextGlyphY{LinLibertine_I}{uniE00B}{57355}
\DeclareTextGlyphY{LinLibertine_I}{copyleft}{57356}
\DeclareTextGlyphY{LinLibertine_I}{uniE00C}{57356}
\DeclareTextGlyphY{LinLibertine_I}{publicdomain}{57357}
\DeclareTextGlyphY{LinLibertine_I}{uniE00D}{57357}
\DeclareTextGlyphY{LinLibertine_I}{creativecommons}{57358}
\DeclareTextGlyphY{LinLibertine_I}{uniE00E}{57358}
\DeclareTextGlyphY{LinLibertine_I}{zero.fitted}{57360}
\DeclareTextGlyphY{LinLibertine_I}{uniE010}{57360}
\DeclareTextGlyphY{LinLibertine_I}{one.fitted}{57361}
\DeclareTextGlyphY{LinLibertine_I}{uniE011}{57361}
\DeclareTextGlyphY{LinLibertine_I}{two.fitted}{57362}
\DeclareTextGlyphY{LinLibertine_I}{uniE012}{57362}
\DeclareTextGlyphY{LinLibertine_I}{three.fitted}{57363}
\DeclareTextGlyphY{LinLibertine_I}{uniE013}{57363}
\DeclareTextGlyphY{LinLibertine_I}{four.fitted}{57364}
\DeclareTextGlyphY{LinLibertine_I}{uniE014}{57364}
\DeclareTextGlyphY{LinLibertine_I}{five.fitted}{57365}
\DeclareTextGlyphY{LinLibertine_I}{uniE015}{57365}
\DeclareTextGlyphY{LinLibertine_I}{six.fitted}{57366}
\DeclareTextGlyphY{LinLibertine_I}{uniE016}{57366}
\DeclareTextGlyphY{LinLibertine_I}{seven.fitted}{57367}
\DeclareTextGlyphY{LinLibertine_I}{uniE017}{57367}
\DeclareTextGlyphY{LinLibertine_I}{eight.fitted}{57368}
\DeclareTextGlyphY{LinLibertine_I}{uniE018}{57368}
\DeclareTextGlyphY{LinLibertine_I}{nine.fitted}{57369}
\DeclareTextGlyphY{LinLibertine_I}{uniE019}{57369}
\DeclareTextGlyphY{LinLibertine_I}{W.alt}{57391}
\DeclareTextGlyphY{LinLibertine_I}{uniE02F}{57391}
\DeclareTextGlyphY{LinLibertine_I}{uniE040}{57408}
\DeclareTextGlyphY{LinLibertine_I}{uniE041}{57409}
\DeclareTextGlyphY{LinLibertine_I}{uniE042}{57410}
\DeclareTextGlyphY{LinLibertine_I}{ampersand.alt}{57424}
\DeclareTextGlyphY{LinLibertine_I}{uniE050}{57424}
\DeclareTextGlyphY{LinLibertine_I}{a.sc}{57425}
\DeclareTextGlyphY{LinLibertine_I}{uniE051}{57425}
\DeclareTextGlyphY{LinLibertine_I}{b.sc}{57426}
\DeclareTextGlyphY{LinLibertine_I}{uniE052}{57426}
\DeclareTextGlyphY{LinLibertine_I}{c.sc}{57427}
\DeclareTextGlyphY{LinLibertine_I}{uniE053}{57427}
\DeclareTextGlyphY{LinLibertine_I}{d.sc}{57428}
\DeclareTextGlyphY{LinLibertine_I}{uniE054}{57428}
\DeclareTextGlyphY{LinLibertine_I}{e.sc}{57429}
\DeclareTextGlyphY{LinLibertine_I}{uniE055}{57429}
\DeclareTextGlyphY{LinLibertine_I}{f.sc}{57430}
\DeclareTextGlyphY{LinLibertine_I}{uniE056}{57430}
\DeclareTextGlyphY{LinLibertine_I}{g.sc}{57431}
\DeclareTextGlyphY{LinLibertine_I}{uniE057}{57431}
\DeclareTextGlyphY{LinLibertine_I}{h.sc}{57432}
\DeclareTextGlyphY{LinLibertine_I}{uniE058}{57432}
\DeclareTextGlyphY{LinLibertine_I}{i.sc}{57433}
\DeclareTextGlyphY{LinLibertine_I}{uniE059}{57433}
\DeclareTextGlyphY{LinLibertine_I}{j.sc}{57434}
\DeclareTextGlyphY{LinLibertine_I}{uniE05A}{57434}
\DeclareTextGlyphY{LinLibertine_I}{k.sc}{57435}
\DeclareTextGlyphY{LinLibertine_I}{uniE05B}{57435}
\DeclareTextGlyphY{LinLibertine_I}{l.sc}{57436}
\DeclareTextGlyphY{LinLibertine_I}{uniE05C}{57436}
\DeclareTextGlyphY{LinLibertine_I}{m.sc}{57437}
\DeclareTextGlyphY{LinLibertine_I}{uniE05D}{57437}
\DeclareTextGlyphY{LinLibertine_I}{n.sc}{57438}
\DeclareTextGlyphY{LinLibertine_I}{uniE05E}{57438}
\DeclareTextGlyphY{LinLibertine_I}{o.sc}{57439}
\DeclareTextGlyphY{LinLibertine_I}{uniE05F}{57439}
\DeclareTextGlyphY{LinLibertine_I}{p.sc}{57440}
\DeclareTextGlyphY{LinLibertine_I}{uniE060}{57440}
\DeclareTextGlyphY{LinLibertine_I}{q.sc}{57441}
\DeclareTextGlyphY{LinLibertine_I}{uniE061}{57441}
\DeclareTextGlyphY{LinLibertine_I}{r.sc}{57442}
\DeclareTextGlyphY{LinLibertine_I}{uniE062}{57442}
\DeclareTextGlyphY{LinLibertine_I}{s.sc}{57443}
\DeclareTextGlyphY{LinLibertine_I}{uniE063}{57443}
\DeclareTextGlyphY{LinLibertine_I}{t.sc}{57444}
\DeclareTextGlyphY{LinLibertine_I}{uniE064}{57444}
\DeclareTextGlyphY{LinLibertine_I}{u.sc}{57445}
\DeclareTextGlyphY{LinLibertine_I}{uniE065}{57445}
\DeclareTextGlyphY{LinLibertine_I}{v.sc}{57446}
\DeclareTextGlyphY{LinLibertine_I}{uniE066}{57446}
\DeclareTextGlyphY{LinLibertine_I}{w.sc}{57447}
\DeclareTextGlyphY{LinLibertine_I}{uniE067}{57447}
\DeclareTextGlyphY{LinLibertine_I}{x.sc}{57448}
\DeclareTextGlyphY{LinLibertine_I}{uniE068}{57448}
\DeclareTextGlyphY{LinLibertine_I}{y.sc}{57449}
\DeclareTextGlyphY{LinLibertine_I}{uniE069}{57449}
\DeclareTextGlyphY{LinLibertine_I}{z.sc}{57450}
\DeclareTextGlyphY{LinLibertine_I}{uniE06A}{57450}
\DeclareTextGlyphY{LinLibertine_I}{uniE06B}{57451}
\DeclareTextGlyphY{LinLibertine_I}{hyphen.sc}{57453}
\DeclareTextGlyphY{LinLibertine_I}{uniE06D}{57453}
\DeclareTextGlyphY{LinLibertine_I}{adieresis.sc}{57460}
\DeclareTextGlyphY{LinLibertine_I}{uniE074}{57460}
\DeclareTextGlyphY{LinLibertine_I}{ae.sc}{57462}
\DeclareTextGlyphY{LinLibertine_I}{uniE076}{57462}
\DeclareTextGlyphY{LinLibertine_I}{odieresis.sc}{57478}
\DeclareTextGlyphY{LinLibertine_I}{uniE086}{57478}
\DeclareTextGlyphY{LinLibertine_I}{oe.sc}{57479}
\DeclareTextGlyphY{LinLibertine_I}{uniE087}{57479}
\DeclareTextGlyphY{LinLibertine_I}{thorn.sc}{57486}
\DeclareTextGlyphY{LinLibertine_I}{uniE08E}{57486}
\DeclareTextGlyphY{LinLibertine_I}{ij.sc}{57488}
\DeclareTextGlyphY{LinLibertine_I}{uniE090}{57488}
\DeclareTextGlyphY{LinLibertine_I}{germandbls.sc}{57490}
\DeclareTextGlyphY{LinLibertine_I}{uniE092}{57490}
\DeclareTextGlyphY{LinLibertine_I}{Q_u.sc}{57491}
\DeclareTextGlyphY{LinLibertine_I}{uniE093}{57491}
\DeclareTextGlyphY{LinLibertine_I}{eng.sc}{57508}
\DeclareTextGlyphY{LinLibertine_I}{uniE0A4}{57508}
\DeclareTextGlyphY{LinLibertine_I}{ohungarumlaut.sc}{57509}
\DeclareTextGlyphY{LinLibertine_I}{uniE0A5}{57509}
\DeclareTextGlyphY{LinLibertine_I}{uhungarumlaut.sc}{57518}
\DeclareTextGlyphY{LinLibertine_I}{uniE0AE}{57518}
\DeclareTextGlyphY{LinLibertine_I}{uniE104}{57604}
\DeclareTextGlyphY{LinLibertine_I}{uniE105}{57605}
\DeclareTextGlyphY{LinLibertine_I}{uniE106}{57606}
\DeclareTextGlyphY{LinLibertine_I}{uniE107}{57607}
\DeclareTextGlyphY{LinLibertine_I}{leaf}{57656}
\DeclareTextGlyphY{LinLibertine_I}{uniE138}{57656}
\DeclareTextGlyphY{LinLibertine_I}{hungarumlaut.cap}{58205}
\DeclareTextGlyphY{LinLibertine_I}{uniE35D}{58205}
\DeclareTextGlyphY{LinLibertine_I}{breve.cyrcap}{58208}
\DeclareTextGlyphY{LinLibertine_I}{uniE360}{58208}
\DeclareTextGlyphY{LinLibertine_I}{breve.cyr}{58209}
\DeclareTextGlyphY{LinLibertine_I}{uniE361}{58209}
\DeclareTextGlyphY{LinLibertine_I}{dieresis.cap}{58210}
\DeclareTextGlyphY{LinLibertine_I}{uniE362}{58210}
\DeclareTextGlyphY{LinLibertine_I}{metric}{58400}
\DeclareTextGlyphY{LinLibertine_I}{uniE420}{58400}
\DeclareTextGlyphY{LinLibertine_I}{uniFFFD}{65533}


==> LinLibertine_R.tex <==
\DeclareTextGlyphY{LinLibertine_R}{space}{32}
\DeclareTextGlyphY{LinLibertine_R}{uni0020}{32}
\DeclareTextGlyphY{LinLibertine_R}{exclam}{33}
\DeclareTextGlyphY{LinLibertine_R}{uni0021}{33}
\DeclareTextGlyphY{LinLibertine_R}{quotedbl}{34}
\DeclareTextGlyphY{LinLibertine_R}{uni0022}{34}
\DeclareTextGlyphY{LinLibertine_R}{numbersign}{35}
\DeclareTextGlyphY{LinLibertine_R}{uni0023}{35}
\DeclareTextGlyphY{LinLibertine_R}{dollar}{36}
\DeclareTextGlyphY{LinLibertine_R}{uni0024}{36}
\DeclareTextGlyphY{LinLibertine_R}{percent}{37}
\DeclareTextGlyphY{LinLibertine_R}{uni0025}{37}
\DeclareTextGlyphY{LinLibertine_R}{ampersand}{38}
\DeclareTextGlyphY{LinLibertine_R}{uni0026}{38}
\DeclareTextGlyphY{LinLibertine_R}{quotesingle}{39}
\DeclareTextGlyphY{LinLibertine_R}{uni0027}{39}
\DeclareTextGlyphY{LinLibertine_R}{parenleft}{40}
\DeclareTextGlyphY{LinLibertine_R}{uni0028}{40}
\DeclareTextGlyphY{LinLibertine_R}{parenright}{41}
\DeclareTextGlyphY{LinLibertine_R}{uni0029}{41}
\DeclareTextGlyphY{LinLibertine_R}{asterisk}{42}
\DeclareTextGlyphY{LinLibertine_R}{uni002A}{42}
\DeclareTextGlyphY{LinLibertine_R}{plus}{43}
\DeclareTextGlyphY{LinLibertine_R}{uni002B}{43}
\DeclareTextGlyphY{LinLibertine_R}{comma}{44}
\DeclareTextGlyphY{LinLibertine_R}{uni002C}{44}
\DeclareTextGlyphY{LinLibertine_R}{hyphen}{45}
\DeclareTextGlyphY{LinLibertine_R}{uni002D}{45}
\DeclareTextGlyphY{LinLibertine_R}{period}{46}
\DeclareTextGlyphY{LinLibertine_R}{uni002E}{46}
\DeclareTextGlyphY{LinLibertine_R}{slash}{47}
\DeclareTextGlyphY{LinLibertine_R}{uni002F}{47}
\DeclareTextGlyphY{LinLibertine_R}{zero}{48}
\DeclareTextGlyphY{LinLibertine_R}{uni0030}{48}
\DeclareTextGlyphY{LinLibertine_R}{one}{49}
\DeclareTextGlyphY{LinLibertine_R}{uni0031}{49}
\DeclareTextGlyphY{LinLibertine_R}{two}{50}
\DeclareTextGlyphY{LinLibertine_R}{uni0032}{50}
\DeclareTextGlyphY{LinLibertine_R}{three}{51}
\DeclareTextGlyphY{LinLibertine_R}{uni0033}{51}
\DeclareTextGlyphY{LinLibertine_R}{four}{52}
\DeclareTextGlyphY{LinLibertine_R}{uni0034}{52}
\DeclareTextGlyphY{LinLibertine_R}{five}{53}
\DeclareTextGlyphY{LinLibertine_R}{uni0035}{53}
\DeclareTextGlyphY{LinLibertine_R}{six}{54}
\DeclareTextGlyphY{LinLibertine_R}{uni0036}{54}
\DeclareTextGlyphY{LinLibertine_R}{seven}{55}
\DeclareTextGlyphY{LinLibertine_R}{uni0037}{55}
\DeclareTextGlyphY{LinLibertine_R}{eight}{56}
\DeclareTextGlyphY{LinLibertine_R}{uni0038}{56}
\DeclareTextGlyphY{LinLibertine_R}{nine}{57}
\DeclareTextGlyphY{LinLibertine_R}{uni0039}{57}
\DeclareTextGlyphY{LinLibertine_R}{colon}{58}
\DeclareTextGlyphY{LinLibertine_R}{uni003A}{58}
\DeclareTextGlyphY{LinLibertine_R}{semicolon}{59}
\DeclareTextGlyphY{LinLibertine_R}{uni003B}{59}
\DeclareTextGlyphY{LinLibertine_R}{less}{60}
\DeclareTextGlyphY{LinLibertine_R}{uni003C}{60}
\DeclareTextGlyphY{LinLibertine_R}{equal}{61}
\DeclareTextGlyphY{LinLibertine_R}{uni003D}{61}
\DeclareTextGlyphY{LinLibertine_R}{greater}{62}
\DeclareTextGlyphY{LinLibertine_R}{uni003E}{62}
\DeclareTextGlyphY{LinLibertine_R}{question}{63}
\DeclareTextGlyphY{LinLibertine_R}{uni003F}{63}
\DeclareTextGlyphY{LinLibertine_R}{at}{64}
\DeclareTextGlyphY{LinLibertine_R}{uni0040}{64}
\DeclareTextGlyphY{LinLibertine_R}{A}{65}
\DeclareTextGlyphY{LinLibertine_R}{uni0041}{65}
\DeclareTextGlyphY{LinLibertine_R}{B}{66}
\DeclareTextGlyphY{LinLibertine_R}{uni0042}{66}
\DeclareTextGlyphY{LinLibertine_R}{C}{67}
\DeclareTextGlyphY{LinLibertine_R}{uni0043}{67}
\DeclareTextGlyphY{LinLibertine_R}{D}{68}
\DeclareTextGlyphY{LinLibertine_R}{uni0044}{68}
\DeclareTextGlyphY{LinLibertine_R}{E}{69}
\DeclareTextGlyphY{LinLibertine_R}{uni0045}{69}
\DeclareTextGlyphY{LinLibertine_R}{F}{70}
\DeclareTextGlyphY{LinLibertine_R}{uni0046}{70}
\DeclareTextGlyphY{LinLibertine_R}{G}{71}
\DeclareTextGlyphY{LinLibertine_R}{uni0047}{71}
\DeclareTextGlyphY{LinLibertine_R}{H}{72}
\DeclareTextGlyphY{LinLibertine_R}{uni0048}{72}
\DeclareTextGlyphY{LinLibertine_R}{I}{73}
\DeclareTextGlyphY{LinLibertine_R}{uni0049}{73}
\DeclareTextGlyphY{LinLibertine_R}{J}{74}
\DeclareTextGlyphY{LinLibertine_R}{uni004A}{74}
\DeclareTextGlyphY{LinLibertine_R}{K}{75}
\DeclareTextGlyphY{LinLibertine_R}{uni004B}{75}
\DeclareTextGlyphY{LinLibertine_R}{L}{76}
\DeclareTextGlyphY{LinLibertine_R}{uni004C}{76}
\DeclareTextGlyphY{LinLibertine_R}{M}{77}
\DeclareTextGlyphY{LinLibertine_R}{uni004D}{77}
\DeclareTextGlyphY{LinLibertine_R}{N}{78}
\DeclareTextGlyphY{LinLibertine_R}{uni004E}{78}
\DeclareTextGlyphY{LinLibertine_R}{O}{79}
\DeclareTextGlyphY{LinLibertine_R}{uni004F}{79}
\DeclareTextGlyphY{LinLibertine_R}{P}{80}
\DeclareTextGlyphY{LinLibertine_R}{uni0050}{80}
\DeclareTextGlyphY{LinLibertine_R}{Q}{81}
\DeclareTextGlyphY{LinLibertine_R}{uni0051}{81}
\DeclareTextGlyphY{LinLibertine_R}{R}{82}
\DeclareTextGlyphY{LinLibertine_R}{uni0052}{82}
\DeclareTextGlyphY{LinLibertine_R}{S}{83}
\DeclareTextGlyphY{LinLibertine_R}{uni0053}{83}
\DeclareTextGlyphY{LinLibertine_R}{T}{84}
\DeclareTextGlyphY{LinLibertine_R}{uni0054}{84}
\DeclareTextGlyphY{LinLibertine_R}{U}{85}
\DeclareTextGlyphY{LinLibertine_R}{uni0055}{85}
\DeclareTextGlyphY{LinLibertine_R}{V}{86}
\DeclareTextGlyphY{LinLibertine_R}{uni0056}{86}
\DeclareTextGlyphY{LinLibertine_R}{W}{87}
\DeclareTextGlyphY{LinLibertine_R}{uni0057}{87}
\DeclareTextGlyphY{LinLibertine_R}{X}{88}
\DeclareTextGlyphY{LinLibertine_R}{uni0058}{88}
\DeclareTextGlyphY{LinLibertine_R}{Y}{89}
\DeclareTextGlyphY{LinLibertine_R}{uni0059}{89}
\DeclareTextGlyphY{LinLibertine_R}{Z}{90}
\DeclareTextGlyphY{LinLibertine_R}{uni005A}{90}
\DeclareTextGlyphY{LinLibertine_R}{bracketleft}{91}
\DeclareTextGlyphY{LinLibertine_R}{uni005B}{91}
\DeclareTextGlyphY{LinLibertine_R}{backslash}{92}
\DeclareTextGlyphY{LinLibertine_R}{uni005C}{92}
\DeclareTextGlyphY{LinLibertine_R}{bracketright}{93}
\DeclareTextGlyphY{LinLibertine_R}{uni005D}{93}
\DeclareTextGlyphY{LinLibertine_R}{asciicircum}{94}
\DeclareTextGlyphY{LinLibertine_R}{uni005E}{94}
\DeclareTextGlyphY{LinLibertine_R}{underscore}{95}
\DeclareTextGlyphY{LinLibertine_R}{uni005F}{95}
\DeclareTextGlyphY{LinLibertine_R}{grave}{96}
\DeclareTextGlyphY{LinLibertine_R}{uni0060}{96}
\DeclareTextGlyphY{LinLibertine_R}{a}{97}
\DeclareTextGlyphY{LinLibertine_R}{uni0061}{97}
\DeclareTextGlyphY{LinLibertine_R}{b}{98}
\DeclareTextGlyphY{LinLibertine_R}{uni0062}{98}
\DeclareTextGlyphY{LinLibertine_R}{c}{99}
\DeclareTextGlyphY{LinLibertine_R}{uni0063}{99}
\DeclareTextGlyphY{LinLibertine_R}{d}{100}
\DeclareTextGlyphY{LinLibertine_R}{uni0064}{100}
\DeclareTextGlyphY{LinLibertine_R}{e}{101}
\DeclareTextGlyphY{LinLibertine_R}{uni0065}{101}
\DeclareTextGlyphY{LinLibertine_R}{f}{102}
\DeclareTextGlyphY{LinLibertine_R}{uni0066}{102}
\DeclareTextGlyphY{LinLibertine_R}{g}{103}
\DeclareTextGlyphY{LinLibertine_R}{uni0067}{103}
\DeclareTextGlyphY{LinLibertine_R}{h}{104}
\DeclareTextGlyphY{LinLibertine_R}{uni0068}{104}
\DeclareTextGlyphY{LinLibertine_R}{i}{105}
\DeclareTextGlyphY{LinLibertine_R}{uni0069}{105}
\DeclareTextGlyphY{LinLibertine_R}{j}{106}
\DeclareTextGlyphY{LinLibertine_R}{uni006A}{106}
\DeclareTextGlyphY{LinLibertine_R}{k}{107}
\DeclareTextGlyphY{LinLibertine_R}{uni006B}{107}
\DeclareTextGlyphY{LinLibertine_R}{l}{108}
\DeclareTextGlyphY{LinLibertine_R}{uni006C}{108}
\DeclareTextGlyphY{LinLibertine_R}{m}{109}
\DeclareTextGlyphY{LinLibertine_R}{uni006D}{109}
\DeclareTextGlyphY{LinLibertine_R}{n}{110}
\DeclareTextGlyphY{LinLibertine_R}{uni006E}{110}
\DeclareTextGlyphY{LinLibertine_R}{o}{111}
\DeclareTextGlyphY{LinLibertine_R}{uni006F}{111}
\DeclareTextGlyphY{LinLibertine_R}{p}{112}
\DeclareTextGlyphY{LinLibertine_R}{uni0070}{112}
\DeclareTextGlyphY{LinLibertine_R}{q}{113}
\DeclareTextGlyphY{LinLibertine_R}{uni0071}{113}
\DeclareTextGlyphY{LinLibertine_R}{r}{114}
\DeclareTextGlyphY{LinLibertine_R}{uni0072}{114}
\DeclareTextGlyphY{LinLibertine_R}{s}{115}
\DeclareTextGlyphY{LinLibertine_R}{uni0073}{115}
\DeclareTextGlyphY{LinLibertine_R}{t}{116}
\DeclareTextGlyphY{LinLibertine_R}{uni0074}{116}
\DeclareTextGlyphY{LinLibertine_R}{u}{117}
\DeclareTextGlyphY{LinLibertine_R}{uni0075}{117}
\DeclareTextGlyphY{LinLibertine_R}{v}{118}
\DeclareTextGlyphY{LinLibertine_R}{uni0076}{118}
\DeclareTextGlyphY{LinLibertine_R}{w}{119}
\DeclareTextGlyphY{LinLibertine_R}{uni0077}{119}
\DeclareTextGlyphY{LinLibertine_R}{x}{120}
\DeclareTextGlyphY{LinLibertine_R}{uni0078}{120}
\DeclareTextGlyphY{LinLibertine_R}{y}{121}
\DeclareTextGlyphY{LinLibertine_R}{uni0079}{121}
\DeclareTextGlyphY{LinLibertine_R}{z}{122}
\DeclareTextGlyphY{LinLibertine_R}{uni007A}{122}
\DeclareTextGlyphY{LinLibertine_R}{braceleft}{123}
\DeclareTextGlyphY{LinLibertine_R}{uni007B}{123}
\DeclareTextGlyphY{LinLibertine_R}{bar}{124}
\DeclareTextGlyphY{LinLibertine_R}{uni007C}{124}
\DeclareTextGlyphY{LinLibertine_R}{braceright}{125}
\DeclareTextGlyphY{LinLibertine_R}{uni007D}{125}
\DeclareTextGlyphY{LinLibertine_R}{asciitilde}{126}
\DeclareTextGlyphY{LinLibertine_R}{uni007E}{126}
\DeclareTextGlyphY{LinLibertine_R}{uni00A0}{160}
\DeclareTextGlyphY{LinLibertine_R}{exclamdown}{161}
\DeclareTextGlyphY{LinLibertine_R}{uni00A1}{161}
\DeclareTextGlyphY{LinLibertine_R}{cent}{162}
\DeclareTextGlyphY{LinLibertine_R}{uni00A2}{162}
\DeclareTextGlyphY{LinLibertine_R}{sterling}{163}
\DeclareTextGlyphY{LinLibertine_R}{uni00A3}{163}
\DeclareTextGlyphY{LinLibertine_R}{currency}{164}
\DeclareTextGlyphY{LinLibertine_R}{uni00A4}{164}
\DeclareTextGlyphY{LinLibertine_R}{yen}{165}
\DeclareTextGlyphY{LinLibertine_R}{uni00A5}{165}
\DeclareTextGlyphY{LinLibertine_R}{brokenbar}{166}
\DeclareTextGlyphY{LinLibertine_R}{uni00A6}{166}
\DeclareTextGlyphY{LinLibertine_R}{section}{167}
\DeclareTextGlyphY{LinLibertine_R}{uni00A7}{167}
\DeclareTextGlyphY{LinLibertine_R}{dieresis}{168}
\DeclareTextGlyphY{LinLibertine_R}{uni00A8}{168}
\DeclareTextGlyphY{LinLibertine_R}{copyright}{169}
\DeclareTextGlyphY{LinLibertine_R}{uni00A9}{169}
\DeclareTextGlyphY{LinLibertine_R}{ordfeminine}{170}
\DeclareTextGlyphY{LinLibertine_R}{uni00AA}{170}
\DeclareTextGlyphY{LinLibertine_R}{guillemotleft}{171}
\DeclareTextGlyphY{LinLibertine_R}{uni00AB}{171}
\DeclareTextGlyphY{LinLibertine_R}{logicalnot}{172}
\DeclareTextGlyphY{LinLibertine_R}{uni00AC}{172}
\DeclareTextGlyphY{LinLibertine_R}{uni00AD}{173}
\DeclareTextGlyphY{LinLibertine_R}{registered}{174}
\DeclareTextGlyphY{LinLibertine_R}{uni00AE}{174}
\DeclareTextGlyphY{LinLibertine_R}{macron}{175}
\DeclareTextGlyphY{LinLibertine_R}{uni00AF}{175}
\DeclareTextGlyphY{LinLibertine_R}{degree}{176}
\DeclareTextGlyphY{LinLibertine_R}{uni00B0}{176}
\DeclareTextGlyphY{LinLibertine_R}{plusminus}{177}
\DeclareTextGlyphY{LinLibertine_R}{uni00B1}{177}
\DeclareTextGlyphY{LinLibertine_R}{two.superior}{178}
\DeclareTextGlyphY{LinLibertine_R}{uni00B2}{178}
\DeclareTextGlyphY{LinLibertine_R}{three.superior}{179}
\DeclareTextGlyphY{LinLibertine_R}{uni00B3}{179}
\DeclareTextGlyphY{LinLibertine_R}{acute}{180}
\DeclareTextGlyphY{LinLibertine_R}{uni00B4}{180}
\DeclareTextGlyphY{LinLibertine_R}{uni00B5}{181}
\DeclareTextGlyphY{LinLibertine_R}{pilcrow}{182}
\DeclareTextGlyphY{LinLibertine_R}{uni00B6}{182}
\DeclareTextGlyphY{LinLibertine_R}{periodcentered}{183}
\DeclareTextGlyphY{LinLibertine_R}{uni00B7}{183}
\DeclareTextGlyphY{LinLibertine_R}{cedilla}{184}
\DeclareTextGlyphY{LinLibertine_R}{uni00B8}{184}
\DeclareTextGlyphY{LinLibertine_R}{one.superior}{185}
\DeclareTextGlyphY{LinLibertine_R}{uni00B9}{185}
\DeclareTextGlyphY{LinLibertine_R}{ordmasculine}{186}
\DeclareTextGlyphY{LinLibertine_R}{uni00BA}{186}
\DeclareTextGlyphY{LinLibertine_R}{guillemotright}{187}
\DeclareTextGlyphY{LinLibertine_R}{uni00BB}{187}
\DeclareTextGlyphY{LinLibertine_R}{onequarter}{188}
\DeclareTextGlyphY{LinLibertine_R}{uni00BC}{188}
\DeclareTextGlyphY{LinLibertine_R}{onehalf}{189}
\DeclareTextGlyphY{LinLibertine_R}{uni00BD}{189}
\DeclareTextGlyphY{LinLibertine_R}{threequarters}{190}
\DeclareTextGlyphY{LinLibertine_R}{uni00BE}{190}
\DeclareTextGlyphY{LinLibertine_R}{questiondown}{191}
\DeclareTextGlyphY{LinLibertine_R}{uni00BF}{191}
\DeclareTextGlyphY{LinLibertine_R}{Agrave}{192}
\DeclareTextGlyphY{LinLibertine_R}{uni00C0}{192}
\DeclareTextGlyphY{LinLibertine_R}{Aacute}{193}
\DeclareTextGlyphY{LinLibertine_R}{uni00C1}{193}
\DeclareTextGlyphY{LinLibertine_R}{Acircumflex}{194}
\DeclareTextGlyphY{LinLibertine_R}{uni00C2}{194}
\DeclareTextGlyphY{LinLibertine_R}{Atilde}{195}
\DeclareTextGlyphY{LinLibertine_R}{uni00C3}{195}
\DeclareTextGlyphY{LinLibertine_R}{Adieresis}{196}
\DeclareTextGlyphY{LinLibertine_R}{uni00C4}{196}
\DeclareTextGlyphY{LinLibertine_R}{Aring}{197}
\DeclareTextGlyphY{LinLibertine_R}{uni00C5}{197}
\DeclareTextGlyphY{LinLibertine_R}{AE}{198}
\DeclareTextGlyphY{LinLibertine_R}{uni00C6}{198}
\DeclareTextGlyphY{LinLibertine_R}{Ccedilla}{199}
\DeclareTextGlyphY{LinLibertine_R}{uni00C7}{199}
\DeclareTextGlyphY{LinLibertine_R}{Egrave}{200}
\DeclareTextGlyphY{LinLibertine_R}{uni00C8}{200}
\DeclareTextGlyphY{LinLibertine_R}{Eacute}{201}
\DeclareTextGlyphY{LinLibertine_R}{uni00C9}{201}
\DeclareTextGlyphY{LinLibertine_R}{Ecircumflex}{202}
\DeclareTextGlyphY{LinLibertine_R}{uni00CA}{202}
\DeclareTextGlyphY{LinLibertine_R}{Edieresis}{203}
\DeclareTextGlyphY{LinLibertine_R}{uni00CB}{203}
\DeclareTextGlyphY{LinLibertine_R}{Igrave}{204}
\DeclareTextGlyphY{LinLibertine_R}{uni00CC}{204}
\DeclareTextGlyphY{LinLibertine_R}{Iacute}{205}
\DeclareTextGlyphY{LinLibertine_R}{uni00CD}{205}
\DeclareTextGlyphY{LinLibertine_R}{Icircumflex}{206}
\DeclareTextGlyphY{LinLibertine_R}{uni00CE}{206}
\DeclareTextGlyphY{LinLibertine_R}{Idieresis}{207}
\DeclareTextGlyphY{LinLibertine_R}{uni00CF}{207}
\DeclareTextGlyphY{LinLibertine_R}{Eth}{208}
\DeclareTextGlyphY{LinLibertine_R}{uni00D0}{208}
\DeclareTextGlyphY{LinLibertine_R}{Ntilde}{209}
\DeclareTextGlyphY{LinLibertine_R}{uni00D1}{209}
\DeclareTextGlyphY{LinLibertine_R}{Ograve}{210}
\DeclareTextGlyphY{LinLibertine_R}{uni00D2}{210}
\DeclareTextGlyphY{LinLibertine_R}{Oacute}{211}
\DeclareTextGlyphY{LinLibertine_R}{uni00D3}{211}
\DeclareTextGlyphY{LinLibertine_R}{Ocircumflex}{212}
\DeclareTextGlyphY{LinLibertine_R}{uni00D4}{212}
\DeclareTextGlyphY{LinLibertine_R}{Otilde}{213}
\DeclareTextGlyphY{LinLibertine_R}{uni00D5}{213}
\DeclareTextGlyphY{LinLibertine_R}{Odieresis}{214}
\DeclareTextGlyphY{LinLibertine_R}{uni00D6}{214}
\DeclareTextGlyphY{LinLibertine_R}{multiply}{215}
\DeclareTextGlyphY{LinLibertine_R}{uni00D7}{215}
\DeclareTextGlyphY{LinLibertine_R}{Oslash}{216}
\DeclareTextGlyphY{LinLibertine_R}{uni00D8}{216}
\DeclareTextGlyphY{LinLibertine_R}{Ugrave}{217}
\DeclareTextGlyphY{LinLibertine_R}{uni00D9}{217}
\DeclareTextGlyphY{LinLibertine_R}{Uacute}{218}
\DeclareTextGlyphY{LinLibertine_R}{uni00DA}{218}
\DeclareTextGlyphY{LinLibertine_R}{Ucircumflex}{219}
\DeclareTextGlyphY{LinLibertine_R}{uni00DB}{219}
\DeclareTextGlyphY{LinLibertine_R}{Udieresis}{220}
\DeclareTextGlyphY{LinLibertine_R}{uni00DC}{220}
\DeclareTextGlyphY{LinLibertine_R}{Yacute}{221}
\DeclareTextGlyphY{LinLibertine_R}{uni00DD}{221}
\DeclareTextGlyphY{LinLibertine_R}{Thorn}{222}
\DeclareTextGlyphY{LinLibertine_R}{uni00DE}{222}
\DeclareTextGlyphY{LinLibertine_R}{germandbls}{223}
\DeclareTextGlyphY{LinLibertine_R}{uni00DF}{223}
\DeclareTextGlyphY{LinLibertine_R}{agrave}{224}
\DeclareTextGlyphY{LinLibertine_R}{uni00E0}{224}
\DeclareTextGlyphY{LinLibertine_R}{aacute}{225}
\DeclareTextGlyphY{LinLibertine_R}{uni00E1}{225}
\DeclareTextGlyphY{LinLibertine_R}{acircumflex}{226}
\DeclareTextGlyphY{LinLibertine_R}{uni00E2}{226}
\DeclareTextGlyphY{LinLibertine_R}{atilde}{227}
\DeclareTextGlyphY{LinLibertine_R}{uni00E3}{227}
\DeclareTextGlyphY{LinLibertine_R}{adieresis}{228}
\DeclareTextGlyphY{LinLibertine_R}{uni00E4}{228}
\DeclareTextGlyphY{LinLibertine_R}{aring}{229}
\DeclareTextGlyphY{LinLibertine_R}{uni00E5}{229}
\DeclareTextGlyphY{LinLibertine_R}{ae}{230}
\DeclareTextGlyphY{LinLibertine_R}{uni00E6}{230}
\DeclareTextGlyphY{LinLibertine_R}{ccedilla}{231}
\DeclareTextGlyphY{LinLibertine_R}{uni00E7}{231}
\DeclareTextGlyphY{LinLibertine_R}{egrave}{232}
\DeclareTextGlyphY{LinLibertine_R}{uni00E8}{232}
\DeclareTextGlyphY{LinLibertine_R}{eacute}{233}
\DeclareTextGlyphY{LinLibertine_R}{uni00E9}{233}
\DeclareTextGlyphY{LinLibertine_R}{ecircumflex}{234}
\DeclareTextGlyphY{LinLibertine_R}{uni00EA}{234}
\DeclareTextGlyphY{LinLibertine_R}{edieresis}{235}
\DeclareTextGlyphY{LinLibertine_R}{uni00EB}{235}
\DeclareTextGlyphY{LinLibertine_R}{igrave}{236}
\DeclareTextGlyphY{LinLibertine_R}{uni00EC}{236}
\DeclareTextGlyphY{LinLibertine_R}{iacute}{237}
\DeclareTextGlyphY{LinLibertine_R}{uni00ED}{237}
\DeclareTextGlyphY{LinLibertine_R}{icircumflex}{238}
\DeclareTextGlyphY{LinLibertine_R}{uni00EE}{238}
\DeclareTextGlyphY{LinLibertine_R}{idieresis}{239}
\DeclareTextGlyphY{LinLibertine_R}{uni00EF}{239}
\DeclareTextGlyphY{LinLibertine_R}{eth}{240}
\DeclareTextGlyphY{LinLibertine_R}{uni00F0}{240}
\DeclareTextGlyphY{LinLibertine_R}{ntilde}{241}
\DeclareTextGlyphY{LinLibertine_R}{uni00F1}{241}
\DeclareTextGlyphY{LinLibertine_R}{ograve}{242}
\DeclareTextGlyphY{LinLibertine_R}{uni00F2}{242}
\DeclareTextGlyphY{LinLibertine_R}{oacute}{243}
\DeclareTextGlyphY{LinLibertine_R}{uni00F3}{243}
\DeclareTextGlyphY{LinLibertine_R}{ocircumflex}{244}
\DeclareTextGlyphY{LinLibertine_R}{uni00F4}{244}
\DeclareTextGlyphY{LinLibertine_R}{otilde}{245}
\DeclareTextGlyphY{LinLibertine_R}{uni00F5}{245}
\DeclareTextGlyphY{LinLibertine_R}{odieresis}{246}
\DeclareTextGlyphY{LinLibertine_R}{uni00F6}{246}
\DeclareTextGlyphY{LinLibertine_R}{divide}{247}
\DeclareTextGlyphY{LinLibertine_R}{uni00F7}{247}
\DeclareTextGlyphY{LinLibertine_R}{oslash}{248}
\DeclareTextGlyphY{LinLibertine_R}{uni00F8}{248}
\DeclareTextGlyphY{LinLibertine_R}{ugrave}{249}
\DeclareTextGlyphY{LinLibertine_R}{uni00F9}{249}
\DeclareTextGlyphY{LinLibertine_R}{uacute}{250}
\DeclareTextGlyphY{LinLibertine_R}{uni00FA}{250}
\DeclareTextGlyphY{LinLibertine_R}{ucircumflex}{251}
\DeclareTextGlyphY{LinLibertine_R}{uni00FB}{251}
\DeclareTextGlyphY{LinLibertine_R}{udieresis}{252}
\DeclareTextGlyphY{LinLibertine_R}{uni00FC}{252}
\DeclareTextGlyphY{LinLibertine_R}{yacute}{253}
\DeclareTextGlyphY{LinLibertine_R}{uni00FD}{253}
\DeclareTextGlyphY{LinLibertine_R}{thorn}{254}
\DeclareTextGlyphY{LinLibertine_R}{uni00FE}{254}
\DeclareTextGlyphY{LinLibertine_R}{ydieresis}{255}
\DeclareTextGlyphY{LinLibertine_R}{uni00FF}{255}
\DeclareTextGlyphY{LinLibertine_R}{Amacron}{256}
\DeclareTextGlyphY{LinLibertine_R}{uni0100}{256}
\DeclareTextGlyphY{LinLibertine_R}{amacron}{257}
\DeclareTextGlyphY{LinLibertine_R}{uni0101}{257}
\DeclareTextGlyphY{LinLibertine_R}{Abreve}{258}
\DeclareTextGlyphY{LinLibertine_R}{uni0102}{258}
\DeclareTextGlyphY{LinLibertine_R}{abreve}{259}
\DeclareTextGlyphY{LinLibertine_R}{uni0103}{259}
\DeclareTextGlyphY{LinLibertine_R}{Aogonek}{260}
\DeclareTextGlyphY{LinLibertine_R}{uni0104}{260}
\DeclareTextGlyphY{LinLibertine_R}{aogonek}{261}
\DeclareTextGlyphY{LinLibertine_R}{uni0105}{261}
\DeclareTextGlyphY{LinLibertine_R}{Cacute}{262}
\DeclareTextGlyphY{LinLibertine_R}{uni0106}{262}
\DeclareTextGlyphY{LinLibertine_R}{cacute}{263}
\DeclareTextGlyphY{LinLibertine_R}{uni0107}{263}
\DeclareTextGlyphY{LinLibertine_R}{Ccircumflex}{264}
\DeclareTextGlyphY{LinLibertine_R}{uni0108}{264}
\DeclareTextGlyphY{LinLibertine_R}{ccircumflex}{265}
\DeclareTextGlyphY{LinLibertine_R}{uni0109}{265}
\DeclareTextGlyphY{LinLibertine_R}{Cdotaccent}{266}
\DeclareTextGlyphY{LinLibertine_R}{uni010A}{266}
\DeclareTextGlyphY{LinLibertine_R}{cdotaccent}{267}
\DeclareTextGlyphY{LinLibertine_R}{uni010B}{267}
\DeclareTextGlyphY{LinLibertine_R}{Ccaron}{268}
\DeclareTextGlyphY{LinLibertine_R}{uni010C}{268}
\DeclareTextGlyphY{LinLibertine_R}{ccaron}{269}
\DeclareTextGlyphY{LinLibertine_R}{uni010D}{269}
\DeclareTextGlyphY{LinLibertine_R}{Dcaron}{270}
\DeclareTextGlyphY{LinLibertine_R}{uni010E}{270}
\DeclareTextGlyphY{LinLibertine_R}{dcaron}{271}
\DeclareTextGlyphY{LinLibertine_R}{uni010F}{271}
\DeclareTextGlyphY{LinLibertine_R}{Dcroat}{272}
\DeclareTextGlyphY{LinLibertine_R}{uni0110}{272}
\DeclareTextGlyphY{LinLibertine_R}{dcroat}{273}
\DeclareTextGlyphY{LinLibertine_R}{uni0111}{273}
\DeclareTextGlyphY{LinLibertine_R}{Emacron}{274}
\DeclareTextGlyphY{LinLibertine_R}{uni0112}{274}
\DeclareTextGlyphY{LinLibertine_R}{emacron}{275}
\DeclareTextGlyphY{LinLibertine_R}{uni0113}{275}
\DeclareTextGlyphY{LinLibertine_R}{Ebreve}{276}
\DeclareTextGlyphY{LinLibertine_R}{uni0114}{276}
\DeclareTextGlyphY{LinLibertine_R}{ebreve}{277}
\DeclareTextGlyphY{LinLibertine_R}{uni0115}{277}
\DeclareTextGlyphY{LinLibertine_R}{Edotaccent}{278}
\DeclareTextGlyphY{LinLibertine_R}{uni0116}{278}
\DeclareTextGlyphY{LinLibertine_R}{edotaccent}{279}
\DeclareTextGlyphY{LinLibertine_R}{uni0117}{279}
\DeclareTextGlyphY{LinLibertine_R}{Eogonek}{280}
\DeclareTextGlyphY{LinLibertine_R}{uni0118}{280}
\DeclareTextGlyphY{LinLibertine_R}{eogonek}{281}
\DeclareTextGlyphY{LinLibertine_R}{uni0119}{281}
\DeclareTextGlyphY{LinLibertine_R}{Ecaron}{282}
\DeclareTextGlyphY{LinLibertine_R}{uni011A}{282}
\DeclareTextGlyphY{LinLibertine_R}{ecaron}{283}
\DeclareTextGlyphY{LinLibertine_R}{uni011B}{283}
\DeclareTextGlyphY{LinLibertine_R}{Gcircumflex}{284}
\DeclareTextGlyphY{LinLibertine_R}{uni011C}{284}
\DeclareTextGlyphY{LinLibertine_R}{gcircumflex}{285}
\DeclareTextGlyphY{LinLibertine_R}{uni011D}{285}
\DeclareTextGlyphY{LinLibertine_R}{Gbreve}{286}
\DeclareTextGlyphY{LinLibertine_R}{uni011E}{286}
\DeclareTextGlyphY{LinLibertine_R}{gbreve}{287}
\DeclareTextGlyphY{LinLibertine_R}{uni011F}{287}
\DeclareTextGlyphY{LinLibertine_R}{Gdotaccent}{288}
\DeclareTextGlyphY{LinLibertine_R}{uni0120}{288}
\DeclareTextGlyphY{LinLibertine_R}{gdotaccent}{289}
\DeclareTextGlyphY{LinLibertine_R}{uni0121}{289}
\DeclareTextGlyphY{LinLibertine_R}{Gcommaaccent}{290}
\DeclareTextGlyphY{LinLibertine_R}{uni0122}{290}
\DeclareTextGlyphY{LinLibertine_R}{gcommaaccent}{291}
\DeclareTextGlyphY{LinLibertine_R}{uni0123}{291}
\DeclareTextGlyphY{LinLibertine_R}{Hcircumflex}{292}
\DeclareTextGlyphY{LinLibertine_R}{uni0124}{292}
\DeclareTextGlyphY{LinLibertine_R}{hcircumflex}{293}
\DeclareTextGlyphY{LinLibertine_R}{uni0125}{293}
\DeclareTextGlyphY{LinLibertine_R}{Hbar}{294}
\DeclareTextGlyphY{LinLibertine_R}{uni0126}{294}
\DeclareTextGlyphY{LinLibertine_R}{hbar}{295}
\DeclareTextGlyphY{LinLibertine_R}{uni0127}{295}
\DeclareTextGlyphY{LinLibertine_R}{Itilde}{296}
\DeclareTextGlyphY{LinLibertine_R}{uni0128}{296}
\DeclareTextGlyphY{LinLibertine_R}{itilde}{297}
\DeclareTextGlyphY{LinLibertine_R}{uni0129}{297}
\DeclareTextGlyphY{LinLibertine_R}{Imacron}{298}
\DeclareTextGlyphY{LinLibertine_R}{uni012A}{298}
\DeclareTextGlyphY{LinLibertine_R}{imacron}{299}
\DeclareTextGlyphY{LinLibertine_R}{uni012B}{299}
\DeclareTextGlyphY{LinLibertine_R}{Ibreve}{300}
\DeclareTextGlyphY{LinLibertine_R}{uni012C}{300}
\DeclareTextGlyphY{LinLibertine_R}{ibreve}{301}
\DeclareTextGlyphY{LinLibertine_R}{uni012D}{301}
\DeclareTextGlyphY{LinLibertine_R}{Iogonek}{302}
\DeclareTextGlyphY{LinLibertine_R}{uni012E}{302}
\DeclareTextGlyphY{LinLibertine_R}{iogonek}{303}
\DeclareTextGlyphY{LinLibertine_R}{uni012F}{303}
\DeclareTextGlyphY{LinLibertine_R}{Idotaccent}{304}
\DeclareTextGlyphY{LinLibertine_R}{uni0130}{304}
\DeclareTextGlyphY{LinLibertine_R}{dotlessi}{305}
\DeclareTextGlyphY{LinLibertine_R}{uni0131}{305}
\DeclareTextGlyphY{LinLibertine_R}{IJ}{306}
\DeclareTextGlyphY{LinLibertine_R}{uni0132}{306}
\DeclareTextGlyphY{LinLibertine_R}{ij}{307}
\DeclareTextGlyphY{LinLibertine_R}{uni0133}{307}
\DeclareTextGlyphY{LinLibertine_R}{Jcircumflex}{308}
\DeclareTextGlyphY{LinLibertine_R}{uni0134}{308}
\DeclareTextGlyphY{LinLibertine_R}{jcircumflex}{309}
\DeclareTextGlyphY{LinLibertine_R}{uni0135}{309}
\DeclareTextGlyphY{LinLibertine_R}{Kcommaaccent}{310}
\DeclareTextGlyphY{LinLibertine_R}{uni0136}{310}
\DeclareTextGlyphY{LinLibertine_R}{kcommaaccent}{311}
\DeclareTextGlyphY{LinLibertine_R}{uni0137}{311}
\DeclareTextGlyphY{LinLibertine_R}{kgreenlandic}{312}
\DeclareTextGlyphY{LinLibertine_R}{uni0138}{312}
\DeclareTextGlyphY{LinLibertine_R}{Lacute}{313}
\DeclareTextGlyphY{LinLibertine_R}{uni0139}{313}
\DeclareTextGlyphY{LinLibertine_R}{lacute}{314}
\DeclareTextGlyphY{LinLibertine_R}{uni013A}{314}
\DeclareTextGlyphY{LinLibertine_R}{Lcommaaccent}{315}
\DeclareTextGlyphY{LinLibertine_R}{uni013B}{315}
\DeclareTextGlyphY{LinLibertine_R}{lcommaaccent}{316}
\DeclareTextGlyphY{LinLibertine_R}{uni013C}{316}
\DeclareTextGlyphY{LinLibertine_R}{Lcaron}{317}
\DeclareTextGlyphY{LinLibertine_R}{uni013D}{317}
\DeclareTextGlyphY{LinLibertine_R}{lcaron}{318}
\DeclareTextGlyphY{LinLibertine_R}{uni013E}{318}
\DeclareTextGlyphY{LinLibertine_R}{Ldot}{319}
\DeclareTextGlyphY{LinLibertine_R}{uni013F}{319}
\DeclareTextGlyphY{LinLibertine_R}{ldot}{320}
\DeclareTextGlyphY{LinLibertine_R}{uni0140}{320}
\DeclareTextGlyphY{LinLibertine_R}{Lslash}{321}
\DeclareTextGlyphY{LinLibertine_R}{uni0141}{321}
\DeclareTextGlyphY{LinLibertine_R}{lslash}{322}
\DeclareTextGlyphY{LinLibertine_R}{uni0142}{322}
\DeclareTextGlyphY{LinLibertine_R}{Nacute}{323}
\DeclareTextGlyphY{LinLibertine_R}{uni0143}{323}
\DeclareTextGlyphY{LinLibertine_R}{nacute}{324}
\DeclareTextGlyphY{LinLibertine_R}{uni0144}{324}
\DeclareTextGlyphY{LinLibertine_R}{Ncommaaccent}{325}
\DeclareTextGlyphY{LinLibertine_R}{uni0145}{325}
\DeclareTextGlyphY{LinLibertine_R}{ncommaaccent}{326}
\DeclareTextGlyphY{LinLibertine_R}{uni0146}{326}
\DeclareTextGlyphY{LinLibertine_R}{Ncaron}{327}
\DeclareTextGlyphY{LinLibertine_R}{uni0147}{327}
\DeclareTextGlyphY{LinLibertine_R}{ncaron}{328}
\DeclareTextGlyphY{LinLibertine_R}{uni0148}{328}
\DeclareTextGlyphY{LinLibertine_R}{napostrophe}{329}
\DeclareTextGlyphY{LinLibertine_R}{uni0149}{329}
\DeclareTextGlyphY{LinLibertine_R}{Eng}{330}
\DeclareTextGlyphY{LinLibertine_R}{uni014A}{330}
\DeclareTextGlyphY{LinLibertine_R}{eng}{331}
\DeclareTextGlyphY{LinLibertine_R}{uni014B}{331}
\DeclareTextGlyphY{LinLibertine_R}{Omacron}{332}
\DeclareTextGlyphY{LinLibertine_R}{uni014C}{332}
\DeclareTextGlyphY{LinLibertine_R}{omacron}{333}
\DeclareTextGlyphY{LinLibertine_R}{uni014D}{333}
\DeclareTextGlyphY{LinLibertine_R}{Obreve}{334}
\DeclareTextGlyphY{LinLibertine_R}{uni014E}{334}
\DeclareTextGlyphY{LinLibertine_R}{obreve}{335}
\DeclareTextGlyphY{LinLibertine_R}{uni014F}{335}
\DeclareTextGlyphY{LinLibertine_R}{Ohungarumlaut}{336}
\DeclareTextGlyphY{LinLibertine_R}{uni0150}{336}
\DeclareTextGlyphY{LinLibertine_R}{ohungarumlaut}{337}
\DeclareTextGlyphY{LinLibertine_R}{uni0151}{337}
\DeclareTextGlyphY{LinLibertine_R}{OE}{338}
\DeclareTextGlyphY{LinLibertine_R}{uni0152}{338}
\DeclareTextGlyphY{LinLibertine_R}{oe}{339}
\DeclareTextGlyphY{LinLibertine_R}{uni0153}{339}
\DeclareTextGlyphY{LinLibertine_R}{Racute}{340}
\DeclareTextGlyphY{LinLibertine_R}{uni0154}{340}
\DeclareTextGlyphY{LinLibertine_R}{racute}{341}
\DeclareTextGlyphY{LinLibertine_R}{uni0155}{341}
\DeclareTextGlyphY{LinLibertine_R}{Rcommaaccent}{342}
\DeclareTextGlyphY{LinLibertine_R}{uni0156}{342}
\DeclareTextGlyphY{LinLibertine_R}{rcommaaccent}{343}
\DeclareTextGlyphY{LinLibertine_R}{uni0157}{343}
\DeclareTextGlyphY{LinLibertine_R}{Rcaron}{344}
\DeclareTextGlyphY{LinLibertine_R}{uni0158}{344}
\DeclareTextGlyphY{LinLibertine_R}{rcaron}{345}
\DeclareTextGlyphY{LinLibertine_R}{uni0159}{345}
\DeclareTextGlyphY{LinLibertine_R}{Sacute}{346}
\DeclareTextGlyphY{LinLibertine_R}{uni015A}{346}
\DeclareTextGlyphY{LinLibertine_R}{sacute}{347}
\DeclareTextGlyphY{LinLibertine_R}{uni015B}{347}
\DeclareTextGlyphY{LinLibertine_R}{Scircumflex}{348}
\DeclareTextGlyphY{LinLibertine_R}{uni015C}{348}
\DeclareTextGlyphY{LinLibertine_R}{scircumflex}{349}
\DeclareTextGlyphY{LinLibertine_R}{uni015D}{349}
\DeclareTextGlyphY{LinLibertine_R}{Scedilla}{350}
\DeclareTextGlyphY{LinLibertine_R}{uni015E}{350}
\DeclareTextGlyphY{LinLibertine_R}{scedilla}{351}
\DeclareTextGlyphY{LinLibertine_R}{uni015F}{351}
\DeclareTextGlyphY{LinLibertine_R}{Scaron}{352}
\DeclareTextGlyphY{LinLibertine_R}{uni0160}{352}
\DeclareTextGlyphY{LinLibertine_R}{scaron}{353}
\DeclareTextGlyphY{LinLibertine_R}{uni0161}{353}
\DeclareTextGlyphY{LinLibertine_R}{Tcedilla}{354}
\DeclareTextGlyphY{LinLibertine_R}{uni0162}{354}
\DeclareTextGlyphY{LinLibertine_R}{tcedilla}{355}
\DeclareTextGlyphY{LinLibertine_R}{uni0163}{355}
\DeclareTextGlyphY{LinLibertine_R}{Tcaron}{356}
\DeclareTextGlyphY{LinLibertine_R}{uni0164}{356}
\DeclareTextGlyphY{LinLibertine_R}{tcaron}{357}
\DeclareTextGlyphY{LinLibertine_R}{uni0165}{357}
\DeclareTextGlyphY{LinLibertine_R}{Tbar}{358}
\DeclareTextGlyphY{LinLibertine_R}{uni0166}{358}
\DeclareTextGlyphY{LinLibertine_R}{tbar}{359}
\DeclareTextGlyphY{LinLibertine_R}{uni0167}{359}
\DeclareTextGlyphY{LinLibertine_R}{Utilde}{360}
\DeclareTextGlyphY{LinLibertine_R}{uni0168}{360}
\DeclareTextGlyphY{LinLibertine_R}{utilde}{361}
\DeclareTextGlyphY{LinLibertine_R}{uni0169}{361}
\DeclareTextGlyphY{LinLibertine_R}{Umacron}{362}
\DeclareTextGlyphY{LinLibertine_R}{uni016A}{362}
\DeclareTextGlyphY{LinLibertine_R}{umacron}{363}
\DeclareTextGlyphY{LinLibertine_R}{uni016B}{363}
\DeclareTextGlyphY{LinLibertine_R}{Ubreve}{364}
\DeclareTextGlyphY{LinLibertine_R}{uni016C}{364}
\DeclareTextGlyphY{LinLibertine_R}{ubreve}{365}
\DeclareTextGlyphY{LinLibertine_R}{uni016D}{365}
\DeclareTextGlyphY{LinLibertine_R}{Uring}{366}
\DeclareTextGlyphY{LinLibertine_R}{uni016E}{366}
\DeclareTextGlyphY{LinLibertine_R}{uring}{367}
\DeclareTextGlyphY{LinLibertine_R}{uni016F}{367}
\DeclareTextGlyphY{LinLibertine_R}{Uhungarumlaut}{368}
\DeclareTextGlyphY{LinLibertine_R}{uni0170}{368}
\DeclareTextGlyphY{LinLibertine_R}{uhungarumlaut}{369}
\DeclareTextGlyphY{LinLibertine_R}{uni0171}{369}
\DeclareTextGlyphY{LinLibertine_R}{Uogonek}{370}
\DeclareTextGlyphY{LinLibertine_R}{uni0172}{370}
\DeclareTextGlyphY{LinLibertine_R}{uogonek}{371}
\DeclareTextGlyphY{LinLibertine_R}{uni0173}{371}
\DeclareTextGlyphY{LinLibertine_R}{Wcircumflex}{372}
\DeclareTextGlyphY{LinLibertine_R}{uni0174}{372}
\DeclareTextGlyphY{LinLibertine_R}{wcircumflex}{373}
\DeclareTextGlyphY{LinLibertine_R}{uni0175}{373}
\DeclareTextGlyphY{LinLibertine_R}{Ycircumflex}{374}
\DeclareTextGlyphY{LinLibertine_R}{uni0176}{374}
\DeclareTextGlyphY{LinLibertine_R}{ycircumflex}{375}
\DeclareTextGlyphY{LinLibertine_R}{uni0177}{375}
\DeclareTextGlyphY{LinLibertine_R}{Ydieresis}{376}
\DeclareTextGlyphY{LinLibertine_R}{uni0178}{376}
\DeclareTextGlyphY{LinLibertine_R}{Zacute}{377}
\DeclareTextGlyphY{LinLibertine_R}{uni0179}{377}
\DeclareTextGlyphY{LinLibertine_R}{zacute}{378}
\DeclareTextGlyphY{LinLibertine_R}{uni017A}{378}
\DeclareTextGlyphY{LinLibertine_R}{Zdotaccent}{379}
\DeclareTextGlyphY{LinLibertine_R}{uni017B}{379}
\DeclareTextGlyphY{LinLibertine_R}{zdotaccent}{380}
\DeclareTextGlyphY{LinLibertine_R}{uni017C}{380}
\DeclareTextGlyphY{LinLibertine_R}{Zcaron}{381}
\DeclareTextGlyphY{LinLibertine_R}{uni017D}{381}
\DeclareTextGlyphY{LinLibertine_R}{zcaron}{382}
\DeclareTextGlyphY{LinLibertine_R}{uni017E}{382}
\DeclareTextGlyphY{LinLibertine_R}{longs}{383}
\DeclareTextGlyphY{LinLibertine_R}{uni017F}{383}
\DeclareTextGlyphY{LinLibertine_R}{uni0180}{384}
\DeclareTextGlyphY{LinLibertine_R}{uni0181}{385}
\DeclareTextGlyphY{LinLibertine_R}{uni0182}{386}
\DeclareTextGlyphY{LinLibertine_R}{uni0183}{387}
\DeclareTextGlyphY{LinLibertine_R}{uni0184}{388}
\DeclareTextGlyphY{LinLibertine_R}{uni0185}{389}
\DeclareTextGlyphY{LinLibertine_R}{uni0186}{390}
\DeclareTextGlyphY{LinLibertine_R}{uni0187}{391}
\DeclareTextGlyphY{LinLibertine_R}{uni0188}{392}
\DeclareTextGlyphY{LinLibertine_R}{uni0189}{393}
\DeclareTextGlyphY{LinLibertine_R}{uni018A}{394}
\DeclareTextGlyphY{LinLibertine_R}{uni018B}{395}
\DeclareTextGlyphY{LinLibertine_R}{uni018C}{396}
\DeclareTextGlyphY{LinLibertine_R}{uni018D}{397}
\DeclareTextGlyphY{LinLibertine_R}{uni018E}{398}
\DeclareTextGlyphY{LinLibertine_R}{uni018F}{399}
\DeclareTextGlyphY{LinLibertine_R}{uni0190}{400}
\DeclareTextGlyphY{LinLibertine_R}{uni0191}{401}
\DeclareTextGlyphY{LinLibertine_R}{florin}{402}
\DeclareTextGlyphY{LinLibertine_R}{uni0192}{402}
\DeclareTextGlyphY{LinLibertine_R}{uni0193}{403}
\DeclareTextGlyphY{LinLibertine_R}{uni0194}{404}
\DeclareTextGlyphY{LinLibertine_R}{uni0195}{405}
\DeclareTextGlyphY{LinLibertine_R}{uni0196}{406}
\DeclareTextGlyphY{LinLibertine_R}{uni0197}{407}
\DeclareTextGlyphY{LinLibertine_R}{uni0198}{408}
\DeclareTextGlyphY{LinLibertine_R}{uni0199}{409}
\DeclareTextGlyphY{LinLibertine_R}{uni019A}{410}
\DeclareTextGlyphY{LinLibertine_R}{uni019B}{411}
\DeclareTextGlyphY{LinLibertine_R}{uni019C}{412}
\DeclareTextGlyphY{LinLibertine_R}{uni019D}{413}
\DeclareTextGlyphY{LinLibertine_R}{uni019E}{414}
\DeclareTextGlyphY{LinLibertine_R}{uni019F}{415}
\DeclareTextGlyphY{LinLibertine_R}{Ohorn}{416}
\DeclareTextGlyphY{LinLibertine_R}{uni01A0}{416}
\DeclareTextGlyphY{LinLibertine_R}{ohorn}{417}
\DeclareTextGlyphY{LinLibertine_R}{uni01A1}{417}
\DeclareTextGlyphY{LinLibertine_R}{uni01A2}{418}
\DeclareTextGlyphY{LinLibertine_R}{uni01A3}{419}
\DeclareTextGlyphY{LinLibertine_R}{uni01A4}{420}
\DeclareTextGlyphY{LinLibertine_R}{uni01A5}{421}
\DeclareTextGlyphY{LinLibertine_R}{uni01A6}{422}
\DeclareTextGlyphY{LinLibertine_R}{uni01A7}{423}
\DeclareTextGlyphY{LinLibertine_R}{uni01A8}{424}
\DeclareTextGlyphY{LinLibertine_R}{uni01A9}{425}
\DeclareTextGlyphY{LinLibertine_R}{uni01AA}{426}
\DeclareTextGlyphY{LinLibertine_R}{uni01AB}{427}
\DeclareTextGlyphY{LinLibertine_R}{uni01AC}{428}
\DeclareTextGlyphY{LinLibertine_R}{uni01AD}{429}
\DeclareTextGlyphY{LinLibertine_R}{uni01AE}{430}
\DeclareTextGlyphY{LinLibertine_R}{Uhorn}{431}
\DeclareTextGlyphY{LinLibertine_R}{uni01AF}{431}
\DeclareTextGlyphY{LinLibertine_R}{uhorn}{432}
\DeclareTextGlyphY{LinLibertine_R}{uni01B0}{432}
\DeclareTextGlyphY{LinLibertine_R}{uni01B1}{433}
\DeclareTextGlyphY{LinLibertine_R}{uni01B2}{434}
\DeclareTextGlyphY{LinLibertine_R}{uni01B3}{435}
\DeclareTextGlyphY{LinLibertine_R}{uni01B4}{436}
\DeclareTextGlyphY{LinLibertine_R}{uni01B5}{437}
\DeclareTextGlyphY{LinLibertine_R}{uni01B6}{438}
\DeclareTextGlyphY{LinLibertine_R}{uni01B7}{439}
\DeclareTextGlyphY{LinLibertine_R}{uni01B8}{440}
\DeclareTextGlyphY{LinLibertine_R}{uni01B9}{441}
\DeclareTextGlyphY{LinLibertine_R}{uni01BA}{442}
\DeclareTextGlyphY{LinLibertine_R}{uni01BB}{443}
\DeclareTextGlyphY{LinLibertine_R}{uni01BC}{444}
\DeclareTextGlyphY{LinLibertine_R}{uni01BD}{445}
\DeclareTextGlyphY{LinLibertine_R}{uni01BE}{446}
\DeclareTextGlyphY{LinLibertine_R}{uni01BF}{447}
\DeclareTextGlyphY{LinLibertine_R}{uni01C0}{448}
\DeclareTextGlyphY{LinLibertine_R}{uni01C1}{449}
\DeclareTextGlyphY{LinLibertine_R}{uni01C2}{450}
\DeclareTextGlyphY{LinLibertine_R}{uni01C3}{451}
\DeclareTextGlyphY{LinLibertine_R}{uni01C4}{452}
\DeclareTextGlyphY{LinLibertine_R}{uni01C5}{453}
\DeclareTextGlyphY{LinLibertine_R}{uni01C6}{454}
\DeclareTextGlyphY{LinLibertine_R}{uni01C7}{455}
\DeclareTextGlyphY{LinLibertine_R}{uni01C8}{456}
\DeclareTextGlyphY{LinLibertine_R}{uni01C9}{457}
\DeclareTextGlyphY{LinLibertine_R}{uni01CA}{458}
\DeclareTextGlyphY{LinLibertine_R}{uni01CB}{459}
\DeclareTextGlyphY{LinLibertine_R}{uni01CC}{460}
\DeclareTextGlyphY{LinLibertine_R}{uni01CD}{461}
\DeclareTextGlyphY{LinLibertine_R}{uni01CE}{462}
\DeclareTextGlyphY{LinLibertine_R}{uni01CF}{463}
\DeclareTextGlyphY{LinLibertine_R}{uni01D0}{464}
\DeclareTextGlyphY{LinLibertine_R}{uni01D1}{465}
\DeclareTextGlyphY{LinLibertine_R}{uni01D2}{466}
\DeclareTextGlyphY{LinLibertine_R}{uni01D3}{467}
\DeclareTextGlyphY{LinLibertine_R}{uni01D4}{468}
\DeclareTextGlyphY{LinLibertine_R}{uni01D5}{469}
\DeclareTextGlyphY{LinLibertine_R}{uni01D6}{470}
\DeclareTextGlyphY{LinLibertine_R}{uni01D7}{471}
\DeclareTextGlyphY{LinLibertine_R}{uni01D8}{472}
\DeclareTextGlyphY{LinLibertine_R}{uni01D9}{473}
\DeclareTextGlyphY{LinLibertine_R}{uni01DA}{474}
\DeclareTextGlyphY{LinLibertine_R}{uni01DB}{475}
\DeclareTextGlyphY{LinLibertine_R}{uni01DC}{476}
\DeclareTextGlyphY{LinLibertine_R}{eturned}{477}
\DeclareTextGlyphY{LinLibertine_R}{uni01DD}{477}
\DeclareTextGlyphY{LinLibertine_R}{uni01DE}{478}
\DeclareTextGlyphY{LinLibertine_R}{uni01DF}{479}
\DeclareTextGlyphY{LinLibertine_R}{uni01E0}{480}
\DeclareTextGlyphY{LinLibertine_R}{uni01E1}{481}
\DeclareTextGlyphY{LinLibertine_R}{uni01E2}{482}
\DeclareTextGlyphY{LinLibertine_R}{uni01E3}{483}
\DeclareTextGlyphY{LinLibertine_R}{uni01E4}{484}
\DeclareTextGlyphY{LinLibertine_R}{uni01E5}{485}
\DeclareTextGlyphY{LinLibertine_R}{Gcaron}{486}
\DeclareTextGlyphY{LinLibertine_R}{uni01E6}{486}
\DeclareTextGlyphY{LinLibertine_R}{gcaron}{487}
\DeclareTextGlyphY{LinLibertine_R}{uni01E7}{487}
\DeclareTextGlyphY{LinLibertine_R}{uni01E8}{488}
\DeclareTextGlyphY{LinLibertine_R}{uni01E9}{489}
\DeclareTextGlyphY{LinLibertine_R}{uni01EA}{490}
\DeclareTextGlyphY{LinLibertine_R}{uni01EB}{491}
\DeclareTextGlyphY{LinLibertine_R}{uni01EC}{492}
\DeclareTextGlyphY{LinLibertine_R}{uni01ED}{493}
\DeclareTextGlyphY{LinLibertine_R}{uni01EE}{494}
\DeclareTextGlyphY{LinLibertine_R}{uni01EF}{495}
\DeclareTextGlyphY{LinLibertine_R}{uni01F0}{496}
\DeclareTextGlyphY{LinLibertine_R}{uni01F1}{497}
\DeclareTextGlyphY{LinLibertine_R}{uni01F2}{498}
\DeclareTextGlyphY{LinLibertine_R}{uni01F3}{499}
\DeclareTextGlyphY{LinLibertine_R}{uni01F4}{500}
\DeclareTextGlyphY{LinLibertine_R}{uni01F5}{501}
\DeclareTextGlyphY{LinLibertine_R}{uni01F6}{502}
\DeclareTextGlyphY{LinLibertine_R}{uni01F7}{503}
\DeclareTextGlyphY{LinLibertine_R}{uni01F8}{504}
\DeclareTextGlyphY{LinLibertine_R}{uni01F9}{505}
\DeclareTextGlyphY{LinLibertine_R}{Aringacute}{506}
\DeclareTextGlyphY{LinLibertine_R}{uni01FA}{506}
\DeclareTextGlyphY{LinLibertine_R}{aringacute}{507}
\DeclareTextGlyphY{LinLibertine_R}{uni01FB}{507}
\DeclareTextGlyphY{LinLibertine_R}{AEacute}{508}
\DeclareTextGlyphY{LinLibertine_R}{uni01FC}{508}
\DeclareTextGlyphY{LinLibertine_R}{aeacute}{509}
\DeclareTextGlyphY{LinLibertine_R}{uni01FD}{509}
\DeclareTextGlyphY{LinLibertine_R}{Oslashacute}{510}
\DeclareTextGlyphY{LinLibertine_R}{uni01FE}{510}
\DeclareTextGlyphY{LinLibertine_R}{oslashacute}{511}
\DeclareTextGlyphY{LinLibertine_R}{uni01FF}{511}
\DeclareTextGlyphY{LinLibertine_R}{uni0200}{512}
\DeclareTextGlyphY{LinLibertine_R}{uni0201}{513}
\DeclareTextGlyphY{LinLibertine_R}{uni0202}{514}
\DeclareTextGlyphY{LinLibertine_R}{uni0203}{515}
\DeclareTextGlyphY{LinLibertine_R}{uni0204}{516}
\DeclareTextGlyphY{LinLibertine_R}{uni0205}{517}
\DeclareTextGlyphY{LinLibertine_R}{uni0206}{518}
\DeclareTextGlyphY{LinLibertine_R}{uni0207}{519}
\DeclareTextGlyphY{LinLibertine_R}{uni0208}{520}
\DeclareTextGlyphY{LinLibertine_R}{uni0209}{521}
\DeclareTextGlyphY{LinLibertine_R}{uni020A}{522}
\DeclareTextGlyphY{LinLibertine_R}{uni020B}{523}
\DeclareTextGlyphY{LinLibertine_R}{uni020C}{524}
\DeclareTextGlyphY{LinLibertine_R}{uni020D}{525}
\DeclareTextGlyphY{LinLibertine_R}{uni020E}{526}
\DeclareTextGlyphY{LinLibertine_R}{uni020F}{527}
\DeclareTextGlyphY{LinLibertine_R}{uni0210}{528}
\DeclareTextGlyphY{LinLibertine_R}{uni0211}{529}
\DeclareTextGlyphY{LinLibertine_R}{uni0212}{530}
\DeclareTextGlyphY{LinLibertine_R}{uni0213}{531}
\DeclareTextGlyphY{LinLibertine_R}{uni0214}{532}
\DeclareTextGlyphY{LinLibertine_R}{uni0215}{533}
\DeclareTextGlyphY{LinLibertine_R}{uni0216}{534}
\DeclareTextGlyphY{LinLibertine_R}{uni0217}{535}
\DeclareTextGlyphY{LinLibertine_R}{Scommaaccent}{536}
\DeclareTextGlyphY{LinLibertine_R}{uni0218}{536}
\DeclareTextGlyphY{LinLibertine_R}{scommaaccent}{537}
\DeclareTextGlyphY{LinLibertine_R}{uni0219}{537}
\DeclareTextGlyphY{LinLibertine_R}{Tcommaaccent}{538}
\DeclareTextGlyphY{LinLibertine_R}{uni021A}{538}
\DeclareTextGlyphY{LinLibertine_R}{tcommaaccent}{539}
\DeclareTextGlyphY{LinLibertine_R}{uni021B}{539}
\DeclareTextGlyphY{LinLibertine_R}{uni021C}{540}
\DeclareTextGlyphY{LinLibertine_R}{uni021D}{541}
\DeclareTextGlyphY{LinLibertine_R}{uni021E}{542}
\DeclareTextGlyphY{LinLibertine_R}{uni021F}{543}
\DeclareTextGlyphY{LinLibertine_R}{uni0220}{544}
\DeclareTextGlyphY{LinLibertine_R}{uni0221}{545}
\DeclareTextGlyphY{LinLibertine_R}{uni0222}{546}
\DeclareTextGlyphY{LinLibertine_R}{uni0223}{547}
\DeclareTextGlyphY{LinLibertine_R}{uni0224}{548}
\DeclareTextGlyphY{LinLibertine_R}{uni0225}{549}
\DeclareTextGlyphY{LinLibertine_R}{uni0226}{550}
\DeclareTextGlyphY{LinLibertine_R}{uni0227}{551}
\DeclareTextGlyphY{LinLibertine_R}{uni0228}{552}
\DeclareTextGlyphY{LinLibertine_R}{uni0229}{553}
\DeclareTextGlyphY{LinLibertine_R}{uni022A}{554}
\DeclareTextGlyphY{LinLibertine_R}{uni022B}{555}
\DeclareTextGlyphY{LinLibertine_R}{uni022C}{556}
\DeclareTextGlyphY{LinLibertine_R}{uni022D}{557}
\DeclareTextGlyphY{LinLibertine_R}{uni022E}{558}
\DeclareTextGlyphY{LinLibertine_R}{uni022F}{559}
\DeclareTextGlyphY{LinLibertine_R}{uni0230}{560}
\DeclareTextGlyphY{LinLibertine_R}{uni0231}{561}
\DeclareTextGlyphY{LinLibertine_R}{uni0232}{562}
\DeclareTextGlyphY{LinLibertine_R}{uni0233}{563}
\DeclareTextGlyphY{LinLibertine_R}{uni0234}{564}
\DeclareTextGlyphY{LinLibertine_R}{uni0235}{565}
\DeclareTextGlyphY{LinLibertine_R}{uni0236}{566}
\DeclareTextGlyphY{LinLibertine_R}{dotlessj}{567}
\DeclareTextGlyphY{LinLibertine_R}{uni0237}{567}
\DeclareTextGlyphY{LinLibertine_R}{uni0238}{568}
\DeclareTextGlyphY{LinLibertine_R}{uni0239}{569}
\DeclareTextGlyphY{LinLibertine_R}{uni023A}{570}
\DeclareTextGlyphY{LinLibertine_R}{uni023B}{571}
\DeclareTextGlyphY{LinLibertine_R}{uni023C}{572}
\DeclareTextGlyphY{LinLibertine_R}{uni023D}{573}
\DeclareTextGlyphY{LinLibertine_R}{uni023E}{574}
\DeclareTextGlyphY{LinLibertine_R}{uni023F}{575}
\DeclareTextGlyphY{LinLibertine_R}{uni0240}{576}
\DeclareTextGlyphY{LinLibertine_R}{uni0241}{577}
\DeclareTextGlyphY{LinLibertine_R}{uni0242}{578}
\DeclareTextGlyphY{LinLibertine_R}{uni0243}{579}
\DeclareTextGlyphY{LinLibertine_R}{uni0244}{580}
\DeclareTextGlyphY{LinLibertine_R}{uni0245}{581}
\DeclareTextGlyphY{LinLibertine_R}{uni0246}{582}
\DeclareTextGlyphY{LinLibertine_R}{uni0247}{583}
\DeclareTextGlyphY{LinLibertine_R}{uni0248}{584}
\DeclareTextGlyphY{LinLibertine_R}{uni0249}{585}
\DeclareTextGlyphY{LinLibertine_R}{uni024A}{586}
\DeclareTextGlyphY{LinLibertine_R}{uni024B}{587}
\DeclareTextGlyphY{LinLibertine_R}{uni024C}{588}
\DeclareTextGlyphY{LinLibertine_R}{uni024D}{589}
\DeclareTextGlyphY{LinLibertine_R}{uni024E}{590}
\DeclareTextGlyphY{LinLibertine_R}{uni024F}{591}
\DeclareTextGlyphY{LinLibertine_R}{aturned}{592}
\DeclareTextGlyphY{LinLibertine_R}{uni0250}{592}
\DeclareTextGlyphY{LinLibertine_R}{uni0251}{593}
\DeclareTextGlyphY{LinLibertine_R}{uni0252}{594}
\DeclareTextGlyphY{LinLibertine_R}{uni0253}{595}
\DeclareTextGlyphY{LinLibertine_R}{cturned}{596}
\DeclareTextGlyphY{LinLibertine_R}{uni0254}{596}
\DeclareTextGlyphY{LinLibertine_R}{uni0255}{597}
\DeclareTextGlyphY{LinLibertine_R}{uni0256}{598}
\DeclareTextGlyphY{LinLibertine_R}{uni0257}{599}
\DeclareTextGlyphY{LinLibertine_R}{uni0258}{600}
\DeclareTextGlyphY{LinLibertine_R}{uni0259}{601}
\DeclareTextGlyphY{LinLibertine_R}{uni025A}{602}
\DeclareTextGlyphY{LinLibertine_R}{uni025B}{603}
\DeclareTextGlyphY{LinLibertine_R}{uni025C}{604}
\DeclareTextGlyphY{LinLibertine_R}{uni025D}{605}
\DeclareTextGlyphY{LinLibertine_R}{uni025E}{606}
\DeclareTextGlyphY{LinLibertine_R}{uni025F}{607}
\DeclareTextGlyphY{LinLibertine_R}{uni0260}{608}
\DeclareTextGlyphY{LinLibertine_R}{uni0261}{609}
\DeclareTextGlyphY{LinLibertine_R}{uni0262}{610}
\DeclareTextGlyphY{LinLibertine_R}{gammalatin}{611}
\DeclareTextGlyphY{LinLibertine_R}{uni0263}{611}
\DeclareTextGlyphY{LinLibertine_R}{uni0264}{612}
\DeclareTextGlyphY{LinLibertine_R}{uni0265}{613}
\DeclareTextGlyphY{LinLibertine_R}{hhook}{614}
\DeclareTextGlyphY{LinLibertine_R}{uni0266}{614}
\DeclareTextGlyphY{LinLibertine_R}{uni0267}{615}
\DeclareTextGlyphY{LinLibertine_R}{uni0268}{616}
\DeclareTextGlyphY{LinLibertine_R}{uni0269}{617}
\DeclareTextGlyphY{LinLibertine_R}{uni026A}{618}
\DeclareTextGlyphY{LinLibertine_R}{uni026B}{619}
\DeclareTextGlyphY{LinLibertine_R}{uni026C}{620}
\DeclareTextGlyphY{LinLibertine_R}{uni026D}{621}
\DeclareTextGlyphY{LinLibertine_R}{uni026E}{622}
\DeclareTextGlyphY{LinLibertine_R}{mturned}{623}
\DeclareTextGlyphY{LinLibertine_R}{uni026F}{623}
\DeclareTextGlyphY{LinLibertine_R}{uni0270}{624}
\DeclareTextGlyphY{LinLibertine_R}{uni0271}{625}
\DeclareTextGlyphY{LinLibertine_R}{uni0272}{626}
\DeclareTextGlyphY{LinLibertine_R}{uni0273}{627}
\DeclareTextGlyphY{LinLibertine_R}{uni0274}{628}
\DeclareTextGlyphY{LinLibertine_R}{uni0275}{629}
\DeclareTextGlyphY{LinLibertine_R}{uni0276}{630}
\DeclareTextGlyphY{LinLibertine_R}{uni0277}{631}
\DeclareTextGlyphY{LinLibertine_R}{uni0278}{632}
\DeclareTextGlyphY{LinLibertine_R}{rturned}{633}
\DeclareTextGlyphY{LinLibertine_R}{uni0279}{633}
\DeclareTextGlyphY{LinLibertine_R}{uni027A}{634}
\DeclareTextGlyphY{LinLibertine_R}{rhookturned}{635}
\DeclareTextGlyphY{LinLibertine_R}{uni027B}{635}
\DeclareTextGlyphY{LinLibertine_R}{uni027C}{636}
\DeclareTextGlyphY{LinLibertine_R}{uni027D}{637}
\DeclareTextGlyphY{LinLibertine_R}{uni027E}{638}
\DeclareTextGlyphY{LinLibertine_R}{uni027F}{639}
\DeclareTextGlyphY{LinLibertine_R}{Rsmallcap}{640}
\DeclareTextGlyphY{LinLibertine_R}{uni0280}{640}
\DeclareTextGlyphY{LinLibertine_R}{Rsmallinverted}{641}
\DeclareTextGlyphY{LinLibertine_R}{uni0281}{641}
\DeclareTextGlyphY{LinLibertine_R}{uni0282}{642}
\DeclareTextGlyphY{LinLibertine_R}{uni0283}{643}
\DeclareTextGlyphY{LinLibertine_R}{uni0284}{644}
\DeclareTextGlyphY{LinLibertine_R}{uni0285}{645}
\DeclareTextGlyphY{LinLibertine_R}{uni0286}{646}
\DeclareTextGlyphY{LinLibertine_R}{uni0287}{647}
\DeclareTextGlyphY{LinLibertine_R}{uni0288}{648}
\DeclareTextGlyphY{LinLibertine_R}{uni0289}{649}
\DeclareTextGlyphY{LinLibertine_R}{uni028A}{650}
\DeclareTextGlyphY{LinLibertine_R}{uni028B}{651}
\DeclareTextGlyphY{LinLibertine_R}{uni028C}{652}
\DeclareTextGlyphY{LinLibertine_R}{uni028D}{653}
\DeclareTextGlyphY{LinLibertine_R}{uni028E}{654}
\DeclareTextGlyphY{LinLibertine_R}{uni028F}{655}
\DeclareTextGlyphY{LinLibertine_R}{uni0290}{656}
\DeclareTextGlyphY{LinLibertine_R}{uni0291}{657}
\DeclareTextGlyphY{LinLibertine_R}{uni0292}{658}
\DeclareTextGlyphY{LinLibertine_R}{uni0293}{659}
\DeclareTextGlyphY{LinLibertine_R}{uni0294}{660}
\DeclareTextGlyphY{LinLibertine_R}{glottalstopreversed}{661}
\DeclareTextGlyphY{LinLibertine_R}{uni0295}{661}
\DeclareTextGlyphY{LinLibertine_R}{uni0296}{662}
\DeclareTextGlyphY{LinLibertine_R}{uni0297}{663}
\DeclareTextGlyphY{LinLibertine_R}{uni0298}{664}
\DeclareTextGlyphY{LinLibertine_R}{uni0299}{665}
\DeclareTextGlyphY{LinLibertine_R}{uni029A}{666}
\DeclareTextGlyphY{LinLibertine_R}{uni029B}{667}
\DeclareTextGlyphY{LinLibertine_R}{uni029C}{668}
\DeclareTextGlyphY{LinLibertine_R}{uni029D}{669}
\DeclareTextGlyphY{LinLibertine_R}{uni029E}{670}
\DeclareTextGlyphY{LinLibertine_R}{uni029F}{671}
\DeclareTextGlyphY{LinLibertine_R}{uni02A0}{672}
\DeclareTextGlyphY{LinLibertine_R}{uni02A1}{673}
\DeclareTextGlyphY{LinLibertine_R}{uni02A2}{674}
\DeclareTextGlyphY{LinLibertine_R}{uni02A3}{675}
\DeclareTextGlyphY{LinLibertine_R}{uni02A4}{676}
\DeclareTextGlyphY{LinLibertine_R}{uni02A5}{677}
\DeclareTextGlyphY{LinLibertine_R}{uni02A6}{678}
\DeclareTextGlyphY{LinLibertine_R}{uni02A7}{679}
\DeclareTextGlyphY{LinLibertine_R}{uni02A8}{680}
\DeclareTextGlyphY{LinLibertine_R}{uni02A9}{681}
\DeclareTextGlyphY{LinLibertine_R}{uni02AA}{682}
\DeclareTextGlyphY{LinLibertine_R}{uni02AB}{683}
\DeclareTextGlyphY{LinLibertine_R}{uni02AC}{684}
\DeclareTextGlyphY{LinLibertine_R}{uni02AD}{685}
\DeclareTextGlyphY{LinLibertine_R}{uni02AE}{686}
\DeclareTextGlyphY{LinLibertine_R}{uni02AF}{687}
\DeclareTextGlyphY{LinLibertine_R}{h.superior}{688}
\DeclareTextGlyphY{LinLibertine_R}{uni02B0}{688}
\DeclareTextGlyphY{LinLibertine_R}{hhook.superior}{689}
\DeclareTextGlyphY{LinLibertine_R}{uni02B1}{689}
\DeclareTextGlyphY{LinLibertine_R}{j.superior}{690}
\DeclareTextGlyphY{LinLibertine_R}{uni02B2}{690}
\DeclareTextGlyphY{LinLibertine_R}{r.superior}{691}
\DeclareTextGlyphY{LinLibertine_R}{uni02B3}{691}
\DeclareTextGlyphY{LinLibertine_R}{rturned.superior}{692}
\DeclareTextGlyphY{LinLibertine_R}{uni02B4}{692}
\DeclareTextGlyphY{LinLibertine_R}{rhookturned.superior}{693}
\DeclareTextGlyphY{LinLibertine_R}{uni02B5}{693}
\DeclareTextGlyphY{LinLibertine_R}{Rsmallinverted.superior}{694}
\DeclareTextGlyphY{LinLibertine_R}{uni02B6}{694}
\DeclareTextGlyphY{LinLibertine_R}{w.superior}{695}
\DeclareTextGlyphY{LinLibertine_R}{uni02B7}{695}
\DeclareTextGlyphY{LinLibertine_R}{y.superior}{696}
\DeclareTextGlyphY{LinLibertine_R}{uni02B8}{696}
\DeclareTextGlyphY{LinLibertine_R}{uni02B9}{697}
\DeclareTextGlyphY{LinLibertine_R}{uni02BA}{698}
\DeclareTextGlyphY{LinLibertine_R}{uni02BB}{699}
\DeclareTextGlyphY{LinLibertine_R}{afii57929}{700}
\DeclareTextGlyphY{LinLibertine_R}{uni02BC}{700}
\DeclareTextGlyphY{LinLibertine_R}{afii64937}{701}
\DeclareTextGlyphY{LinLibertine_R}{uni02BD}{701}
\DeclareTextGlyphY{LinLibertine_R}{uni02BE}{702}
\DeclareTextGlyphY{LinLibertine_R}{uni02BF}{703}
\DeclareTextGlyphY{LinLibertine_R}{uni02C0}{704}
\DeclareTextGlyphY{LinLibertine_R}{uni02C1}{705}
\DeclareTextGlyphY{LinLibertine_R}{uni02C2}{706}
\DeclareTextGlyphY{LinLibertine_R}{uni02C3}{707}
\DeclareTextGlyphY{LinLibertine_R}{uni02C4}{708}
\DeclareTextGlyphY{LinLibertine_R}{uni02C5}{709}
\DeclareTextGlyphY{LinLibertine_R}{circumflex}{710}
\DeclareTextGlyphY{LinLibertine_R}{uni02C6}{710}
\DeclareTextGlyphY{LinLibertine_R}{caron}{711}
\DeclareTextGlyphY{LinLibertine_R}{uni02C7}{711}
\DeclareTextGlyphY{LinLibertine_R}{uni02C8}{712}
\DeclareTextGlyphY{LinLibertine_R}{uni02C9}{713}
\DeclareTextGlyphY{LinLibertine_R}{uni02CA}{714}
\DeclareTextGlyphY{LinLibertine_R}{uni02CB}{715}
\DeclareTextGlyphY{LinLibertine_R}{uni02CC}{716}
\DeclareTextGlyphY{LinLibertine_R}{uni02CD}{717}
\DeclareTextGlyphY{LinLibertine_R}{uni02CE}{718}
\DeclareTextGlyphY{LinLibertine_R}{uni02CF}{719}
\DeclareTextGlyphY{LinLibertine_R}{uni02D0}{720}
\DeclareTextGlyphY{LinLibertine_R}{uni02D1}{721}
\DeclareTextGlyphY{LinLibertine_R}{uni02D2}{722}
\DeclareTextGlyphY{LinLibertine_R}{uni02D3}{723}
\DeclareTextGlyphY{LinLibertine_R}{uni02D4}{724}
\DeclareTextGlyphY{LinLibertine_R}{uni02D5}{725}
\DeclareTextGlyphY{LinLibertine_R}{uni02D6}{726}
\DeclareTextGlyphY{LinLibertine_R}{uni02D7}{727}
\DeclareTextGlyphY{LinLibertine_R}{breve}{728}
\DeclareTextGlyphY{LinLibertine_R}{uni02D8}{728}
\DeclareTextGlyphY{LinLibertine_R}{dotaccent}{729}
\DeclareTextGlyphY{LinLibertine_R}{uni02D9}{729}
\DeclareTextGlyphY{LinLibertine_R}{ring}{730}
\DeclareTextGlyphY{LinLibertine_R}{uni02DA}{730}
\DeclareTextGlyphY{LinLibertine_R}{ogonek}{731}
\DeclareTextGlyphY{LinLibertine_R}{uni02DB}{731}
\DeclareTextGlyphY{LinLibertine_R}{tilde}{732}
\DeclareTextGlyphY{LinLibertine_R}{uni02DC}{732}
\DeclareTextGlyphY{LinLibertine_R}{hungarumlaut}{733}
\DeclareTextGlyphY{LinLibertine_R}{uni02DD}{733}
\DeclareTextGlyphY{LinLibertine_R}{uni02DE}{734}
\DeclareTextGlyphY{LinLibertine_R}{uni02DF}{735}
\DeclareTextGlyphY{LinLibertine_R}{gammalatin.superior}{736}
\DeclareTextGlyphY{LinLibertine_R}{uni02E0}{736}
\DeclareTextGlyphY{LinLibertine_R}{l.superior}{737}
\DeclareTextGlyphY{LinLibertine_R}{uni02E1}{737}
\DeclareTextGlyphY{LinLibertine_R}{s.superior}{738}
\DeclareTextGlyphY{LinLibertine_R}{uni02E2}{738}
\DeclareTextGlyphY{LinLibertine_R}{x.superior}{739}
\DeclareTextGlyphY{LinLibertine_R}{uni02E3}{739}
\DeclareTextGlyphY{LinLibertine_R}{glottalstopreversed.superior}{740}
\DeclareTextGlyphY{LinLibertine_R}{uni02E4}{740}
\DeclareTextGlyphY{LinLibertine_R}{uni02E5}{741}
\DeclareTextGlyphY{LinLibertine_R}{uni02E6}{742}
\DeclareTextGlyphY{LinLibertine_R}{uni02E7}{743}
\DeclareTextGlyphY{LinLibertine_R}{uni02E8}{744}
\DeclareTextGlyphY{LinLibertine_R}{uni02E9}{745}
\DeclareTextGlyphY{LinLibertine_R}{uni02EA}{746}
\DeclareTextGlyphY{LinLibertine_R}{uni02EB}{747}
\DeclareTextGlyphY{LinLibertine_R}{uni02EC}{748}
\DeclareTextGlyphY{LinLibertine_R}{uni02ED}{749}
\DeclareTextGlyphY{LinLibertine_R}{uni02EE}{750}
\DeclareTextGlyphY{LinLibertine_R}{uni02EF}{751}
\DeclareTextGlyphY{LinLibertine_R}{uni02F0}{752}
\DeclareTextGlyphY{LinLibertine_R}{uni02F1}{753}
\DeclareTextGlyphY{LinLibertine_R}{uni02F2}{754}
\DeclareTextGlyphY{LinLibertine_R}{uni02F3}{755}
\DeclareTextGlyphY{LinLibertine_R}{uni02F4}{756}
\DeclareTextGlyphY{LinLibertine_R}{uni02F5}{757}
\DeclareTextGlyphY{LinLibertine_R}{uni02F6}{758}
\DeclareTextGlyphY{LinLibertine_R}{uni02F7}{759}
\DeclareTextGlyphY{LinLibertine_R}{uni02F8}{760}
\DeclareTextGlyphY{LinLibertine_R}{uni02F9}{761}
\DeclareTextGlyphY{LinLibertine_R}{uni02FA}{762}
\DeclareTextGlyphY{LinLibertine_R}{uni02FB}{763}
\DeclareTextGlyphY{LinLibertine_R}{uni02FC}{764}
\DeclareTextGlyphY{LinLibertine_R}{uni02FD}{765}
\DeclareTextGlyphY{LinLibertine_R}{uni02FE}{766}
\DeclareTextGlyphY{LinLibertine_R}{uni02FF}{767}
\DeclareTextGlyphY{LinLibertine_R}{gravecomb}{768}
\DeclareTextGlyphY{LinLibertine_R}{uni0300}{768}
\DeclareTextGlyphY{LinLibertine_R}{acutecomb}{769}
\DeclareTextGlyphY{LinLibertine_R}{uni0301}{769}
\DeclareTextGlyphY{LinLibertine_R}{circumflexcomb}{770}
\DeclareTextGlyphY{LinLibertine_R}{uni0302}{770}
\DeclareTextGlyphY{LinLibertine_R}{tildecomb}{771}
\DeclareTextGlyphY{LinLibertine_R}{uni0303}{771}
\DeclareTextGlyphY{LinLibertine_R}{macroncomb}{772}
\DeclareTextGlyphY{LinLibertine_R}{uni0304}{772}
\DeclareTextGlyphY{LinLibertine_R}{uni0305}{773}
\DeclareTextGlyphY{LinLibertine_R}{brevecomb}{774}
\DeclareTextGlyphY{LinLibertine_R}{uni0306}{774}
\DeclareTextGlyphY{LinLibertine_R}{uni0307}{775}
\DeclareTextGlyphY{LinLibertine_R}{uni0308}{776}
\DeclareTextGlyphY{LinLibertine_R}{hookabovecomb}{777}
\DeclareTextGlyphY{LinLibertine_R}{uni0309}{777}
\DeclareTextGlyphY{LinLibertine_R}{uni030A}{778}
\DeclareTextGlyphY{LinLibertine_R}{uni030B}{779}
\DeclareTextGlyphY{LinLibertine_R}{uni030C}{780}
\DeclareTextGlyphY{LinLibertine_R}{uni030D}{781}
\DeclareTextGlyphY{LinLibertine_R}{uni030E}{782}
\DeclareTextGlyphY{LinLibertine_R}{uni030F}{783}
\DeclareTextGlyphY{LinLibertine_R}{uni0310}{784}
\DeclareTextGlyphY{LinLibertine_R}{uni0311}{785}
\DeclareTextGlyphY{LinLibertine_R}{uni0312}{786}
\DeclareTextGlyphY{LinLibertine_R}{uni0313}{787}
\DeclareTextGlyphY{LinLibertine_R}{uni0314}{788}
\DeclareTextGlyphY{LinLibertine_R}{uni0315}{789}
\DeclareTextGlyphY{LinLibertine_R}{uni0316}{790}
\DeclareTextGlyphY{LinLibertine_R}{uni0317}{791}
\DeclareTextGlyphY{LinLibertine_R}{uni0318}{792}
\DeclareTextGlyphY{LinLibertine_R}{uni0319}{793}
\DeclareTextGlyphY{LinLibertine_R}{uni031A}{794}
\DeclareTextGlyphY{LinLibertine_R}{uni031B}{795}
\DeclareTextGlyphY{LinLibertine_R}{uni031C}{796}
\DeclareTextGlyphY{LinLibertine_R}{uni031D}{797}
\DeclareTextGlyphY{LinLibertine_R}{uni031E}{798}
\DeclareTextGlyphY{LinLibertine_R}{uni031F}{799}
\DeclareTextGlyphY{LinLibertine_R}{uni0320}{800}
\DeclareTextGlyphY{LinLibertine_R}{uni0321}{801}
\DeclareTextGlyphY{LinLibertine_R}{uni0322}{802}
\DeclareTextGlyphY{LinLibertine_R}{dotbelowcomb}{803}
\DeclareTextGlyphY{LinLibertine_R}{uni0323}{803}
\DeclareTextGlyphY{LinLibertine_R}{uni0324}{804}
\DeclareTextGlyphY{LinLibertine_R}{uni0325}{805}
\DeclareTextGlyphY{LinLibertine_R}{uni0326}{806}
\DeclareTextGlyphY{LinLibertine_R}{uni0327}{807}
\DeclareTextGlyphY{LinLibertine_R}{uni0328}{808}
\DeclareTextGlyphY{LinLibertine_R}{uni0329}{809}
\DeclareTextGlyphY{LinLibertine_R}{uni032A}{810}
\DeclareTextGlyphY{LinLibertine_R}{uni032B}{811}
\DeclareTextGlyphY{LinLibertine_R}{uni032C}{812}
\DeclareTextGlyphY{LinLibertine_R}{uni032D}{813}
\DeclareTextGlyphY{LinLibertine_R}{uni032E}{814}
\DeclareTextGlyphY{LinLibertine_R}{uni032F}{815}
\DeclareTextGlyphY{LinLibertine_R}{uni0330}{816}
\DeclareTextGlyphY{LinLibertine_R}{uni0331}{817}
\DeclareTextGlyphY{LinLibertine_R}{uni0332}{818}
\DeclareTextGlyphY{LinLibertine_R}{uni0333}{819}
\DeclareTextGlyphY{LinLibertine_R}{uni0334}{820}
\DeclareTextGlyphY{LinLibertine_R}{uni0335}{821}
\DeclareTextGlyphY{LinLibertine_R}{uni0336}{822}
\DeclareTextGlyphY{LinLibertine_R}{uni0337}{823}
\DeclareTextGlyphY{LinLibertine_R}{uni0338}{824}
\DeclareTextGlyphY{LinLibertine_R}{uni0339}{825}
\DeclareTextGlyphY{LinLibertine_R}{uni033A}{826}
\DeclareTextGlyphY{LinLibertine_R}{uni033B}{827}
\DeclareTextGlyphY{LinLibertine_R}{uni033C}{828}
\DeclareTextGlyphY{LinLibertine_R}{uni033D}{829}
\DeclareTextGlyphY{LinLibertine_R}{uni033E}{830}
\DeclareTextGlyphY{LinLibertine_R}{uni033F}{831}
\DeclareTextGlyphY{LinLibertine_R}{uni0340}{832}
\DeclareTextGlyphY{LinLibertine_R}{uni0341}{833}
\DeclareTextGlyphY{LinLibertine_R}{uni0342}{834}
\DeclareTextGlyphY{LinLibertine_R}{uni0343}{835}
\DeclareTextGlyphY{LinLibertine_R}{uni0344}{836}
\DeclareTextGlyphY{LinLibertine_R}{uni0345}{837}
\DeclareTextGlyphY{LinLibertine_R}{uni0346}{838}
\DeclareTextGlyphY{LinLibertine_R}{uni0347}{839}
\DeclareTextGlyphY{LinLibertine_R}{uni0348}{840}
\DeclareTextGlyphY{LinLibertine_R}{uni0349}{841}
\DeclareTextGlyphY{LinLibertine_R}{uni034A}{842}
\DeclareTextGlyphY{LinLibertine_R}{uni034B}{843}
\DeclareTextGlyphY{LinLibertine_R}{uni034C}{844}
\DeclareTextGlyphY{LinLibertine_R}{uni034D}{845}
\DeclareTextGlyphY{LinLibertine_R}{uni034E}{846}
\DeclareTextGlyphY{LinLibertine_R}{uni0350}{848}
\DeclareTextGlyphY{LinLibertine_R}{uni0351}{849}
\DeclareTextGlyphY{LinLibertine_R}{uni0352}{850}
\DeclareTextGlyphY{LinLibertine_R}{uni0353}{851}
\DeclareTextGlyphY{LinLibertine_R}{uni0354}{852}
\DeclareTextGlyphY{LinLibertine_R}{uni0355}{853}
\DeclareTextGlyphY{LinLibertine_R}{uni0356}{854}
\DeclareTextGlyphY{LinLibertine_R}{uni0357}{855}
\DeclareTextGlyphY{LinLibertine_R}{uni0358}{856}
\DeclareTextGlyphY{LinLibertine_R}{uni0359}{857}
\DeclareTextGlyphY{LinLibertine_R}{uni035A}{858}
\DeclareTextGlyphY{LinLibertine_R}{uni035B}{859}
\DeclareTextGlyphY{LinLibertine_R}{uni035C}{860}
\DeclareTextGlyphY{LinLibertine_R}{uni035D}{861}
\DeclareTextGlyphY{LinLibertine_R}{uni035E}{862}
\DeclareTextGlyphY{LinLibertine_R}{uni035F}{863}
\DeclareTextGlyphY{LinLibertine_R}{uni0360}{864}
\DeclareTextGlyphY{LinLibertine_R}{uni0361}{865}
\DeclareTextGlyphY{LinLibertine_R}{uni0362}{866}
\DeclareTextGlyphY{LinLibertine_R}{uni0363}{867}
\DeclareTextGlyphY{LinLibertine_R}{uni0364}{868}
\DeclareTextGlyphY{LinLibertine_R}{uni0365}{869}
\DeclareTextGlyphY{LinLibertine_R}{uni0366}{870}
\DeclareTextGlyphY{LinLibertine_R}{uni0367}{871}
\DeclareTextGlyphY{LinLibertine_R}{uni0368}{872}
\DeclareTextGlyphY{LinLibertine_R}{uni0369}{873}
\DeclareTextGlyphY{LinLibertine_R}{uni036A}{874}
\DeclareTextGlyphY{LinLibertine_R}{uni036B}{875}
\DeclareTextGlyphY{LinLibertine_R}{uni036C}{876}
\DeclareTextGlyphY{LinLibertine_R}{uni036D}{877}
\DeclareTextGlyphY{LinLibertine_R}{uni036E}{878}
\DeclareTextGlyphY{LinLibertine_R}{uni036F}{879}
\DeclareTextGlyphY{LinLibertine_R}{uni0374}{884}
\DeclareTextGlyphY{LinLibertine_R}{uni0375}{885}
\DeclareTextGlyphY{LinLibertine_R}{uni037A}{890}
\DeclareTextGlyphY{LinLibertine_R}{uni037B}{891}
\DeclareTextGlyphY{LinLibertine_R}{uni037C}{892}
\DeclareTextGlyphY{LinLibertine_R}{uni037D}{893}
\DeclareTextGlyphY{LinLibertine_R}{uni037E}{894}
\DeclareTextGlyphY{LinLibertine_R}{tonos}{900}
\DeclareTextGlyphY{LinLibertine_R}{uni0384}{900}
\DeclareTextGlyphY{LinLibertine_R}{dieresistonos}{901}
\DeclareTextGlyphY{LinLibertine_R}{uni0385}{901}
\DeclareTextGlyphY{LinLibertine_R}{Alphatonos}{902}
\DeclareTextGlyphY{LinLibertine_R}{uni0386}{902}
\DeclareTextGlyphY{LinLibertine_R}{anoteleia}{903}
\DeclareTextGlyphY{LinLibertine_R}{uni0387}{903}
\DeclareTextGlyphY{LinLibertine_R}{Epsilontonos}{904}
\DeclareTextGlyphY{LinLibertine_R}{uni0388}{904}
\DeclareTextGlyphY{LinLibertine_R}{Etatonos}{905}
\DeclareTextGlyphY{LinLibertine_R}{uni0389}{905}
\DeclareTextGlyphY{LinLibertine_R}{Iotatonos}{906}
\DeclareTextGlyphY{LinLibertine_R}{uni038A}{906}
\DeclareTextGlyphY{LinLibertine_R}{Omicrontonos}{908}
\DeclareTextGlyphY{LinLibertine_R}{uni038C}{908}
\DeclareTextGlyphY{LinLibertine_R}{Upsilontonos}{910}
\DeclareTextGlyphY{LinLibertine_R}{uni038E}{910}
\DeclareTextGlyphY{LinLibertine_R}{Omegatonos}{911}
\DeclareTextGlyphY{LinLibertine_R}{uni038F}{911}
\DeclareTextGlyphY{LinLibertine_R}{iotadieresistonos}{912}
\DeclareTextGlyphY{LinLibertine_R}{uni0390}{912}
\DeclareTextGlyphY{LinLibertine_R}{Alpha}{913}
\DeclareTextGlyphY{LinLibertine_R}{uni0391}{913}
\DeclareTextGlyphY{LinLibertine_R}{Beta}{914}
\DeclareTextGlyphY{LinLibertine_R}{uni0392}{914}
\DeclareTextGlyphY{LinLibertine_R}{Gamma}{915}
\DeclareTextGlyphY{LinLibertine_R}{uni0393}{915}
\DeclareTextGlyphY{LinLibertine_R}{Delta}{916}
\DeclareTextGlyphY{LinLibertine_R}{uni0394}{916}
\DeclareTextGlyphY{LinLibertine_R}{Epsilon}{917}
\DeclareTextGlyphY{LinLibertine_R}{uni0395}{917}
\DeclareTextGlyphY{LinLibertine_R}{Zeta}{918}
\DeclareTextGlyphY{LinLibertine_R}{uni0396}{918}
\DeclareTextGlyphY{LinLibertine_R}{Eta}{919}
\DeclareTextGlyphY{LinLibertine_R}{uni0397}{919}
\DeclareTextGlyphY{LinLibertine_R}{Theta}{920}
\DeclareTextGlyphY{LinLibertine_R}{uni0398}{920}
\DeclareTextGlyphY{LinLibertine_R}{Iota}{921}
\DeclareTextGlyphY{LinLibertine_R}{uni0399}{921}
\DeclareTextGlyphY{LinLibertine_R}{Kappa}{922}
\DeclareTextGlyphY{LinLibertine_R}{uni039A}{922}
\DeclareTextGlyphY{LinLibertine_R}{Lambda}{923}
\DeclareTextGlyphY{LinLibertine_R}{uni039B}{923}
\DeclareTextGlyphY{LinLibertine_R}{Mu}{924}
\DeclareTextGlyphY{LinLibertine_R}{uni039C}{924}
\DeclareTextGlyphY{LinLibertine_R}{Nu}{925}
\DeclareTextGlyphY{LinLibertine_R}{uni039D}{925}
\DeclareTextGlyphY{LinLibertine_R}{Xi}{926}
\DeclareTextGlyphY{LinLibertine_R}{uni039E}{926}
\DeclareTextGlyphY{LinLibertine_R}{Omicron}{927}
\DeclareTextGlyphY{LinLibertine_R}{uni039F}{927}
\DeclareTextGlyphY{LinLibertine_R}{Pi}{928}
\DeclareTextGlyphY{LinLibertine_R}{uni03A0}{928}
\DeclareTextGlyphY{LinLibertine_R}{Rho}{929}
\DeclareTextGlyphY{LinLibertine_R}{uni03A1}{929}
\DeclareTextGlyphY{LinLibertine_R}{Sigma}{931}
\DeclareTextGlyphY{LinLibertine_R}{uni03A3}{931}
\DeclareTextGlyphY{LinLibertine_R}{Tau}{932}
\DeclareTextGlyphY{LinLibertine_R}{uni03A4}{932}
\DeclareTextGlyphY{LinLibertine_R}{Upsilon}{933}
\DeclareTextGlyphY{LinLibertine_R}{uni03A5}{933}
\DeclareTextGlyphY{LinLibertine_R}{Phi}{934}
\DeclareTextGlyphY{LinLibertine_R}{uni03A6}{934}
\DeclareTextGlyphY{LinLibertine_R}{Chi}{935}
\DeclareTextGlyphY{LinLibertine_R}{uni03A7}{935}
\DeclareTextGlyphY{LinLibertine_R}{Psi}{936}
\DeclareTextGlyphY{LinLibertine_R}{uni03A8}{936}
\DeclareTextGlyphY{LinLibertine_R}{Omega}{937}
\DeclareTextGlyphY{LinLibertine_R}{uni03A9}{937}
\DeclareTextGlyphY{LinLibertine_R}{Iotadieresis}{938}
\DeclareTextGlyphY{LinLibertine_R}{uni03AA}{938}
\DeclareTextGlyphY{LinLibertine_R}{Upsilondieresis}{939}
\DeclareTextGlyphY{LinLibertine_R}{uni03AB}{939}
\DeclareTextGlyphY{LinLibertine_R}{alphatonos}{940}
\DeclareTextGlyphY{LinLibertine_R}{uni03AC}{940}
\DeclareTextGlyphY{LinLibertine_R}{epsilontonos}{941}
\DeclareTextGlyphY{LinLibertine_R}{uni03AD}{941}
\DeclareTextGlyphY{LinLibertine_R}{etatonos}{942}
\DeclareTextGlyphY{LinLibertine_R}{uni03AE}{942}
\DeclareTextGlyphY{LinLibertine_R}{iotatonos}{943}
\DeclareTextGlyphY{LinLibertine_R}{uni03AF}{943}
\DeclareTextGlyphY{LinLibertine_R}{upsilondieresistonos}{944}
\DeclareTextGlyphY{LinLibertine_R}{uni03B0}{944}
\DeclareTextGlyphY{LinLibertine_R}{alpha}{945}
\DeclareTextGlyphY{LinLibertine_R}{uni03B1}{945}
\DeclareTextGlyphY{LinLibertine_R}{beta}{946}
\DeclareTextGlyphY{LinLibertine_R}{uni03B2}{946}
\DeclareTextGlyphY{LinLibertine_R}{gamma}{947}
\DeclareTextGlyphY{LinLibertine_R}{uni03B3}{947}
\DeclareTextGlyphY{LinLibertine_R}{delta}{948}
\DeclareTextGlyphY{LinLibertine_R}{uni03B4}{948}
\DeclareTextGlyphY{LinLibertine_R}{epsilon}{949}
\DeclareTextGlyphY{LinLibertine_R}{uni03B5}{949}
\DeclareTextGlyphY{LinLibertine_R}{zeta}{950}
\DeclareTextGlyphY{LinLibertine_R}{uni03B6}{950}
\DeclareTextGlyphY{LinLibertine_R}{eta}{951}
\DeclareTextGlyphY{LinLibertine_R}{uni03B7}{951}
\DeclareTextGlyphY{LinLibertine_R}{theta}{952}
\DeclareTextGlyphY{LinLibertine_R}{uni03B8}{952}
\DeclareTextGlyphY{LinLibertine_R}{iota}{953}
\DeclareTextGlyphY{LinLibertine_R}{uni03B9}{953}
\DeclareTextGlyphY{LinLibertine_R}{kappa}{954}
\DeclareTextGlyphY{LinLibertine_R}{uni03BA}{954}
\DeclareTextGlyphY{LinLibertine_R}{lambda}{955}
\DeclareTextGlyphY{LinLibertine_R}{uni03BB}{955}
\DeclareTextGlyphY{LinLibertine_R}{mu}{956}
\DeclareTextGlyphY{LinLibertine_R}{uni03BC}{956}
\DeclareTextGlyphY{LinLibertine_R}{nu}{957}
\DeclareTextGlyphY{LinLibertine_R}{uni03BD}{957}
\DeclareTextGlyphY{LinLibertine_R}{xi}{958}
\DeclareTextGlyphY{LinLibertine_R}{uni03BE}{958}
\DeclareTextGlyphY{LinLibertine_R}{omicron}{959}
\DeclareTextGlyphY{LinLibertine_R}{uni03BF}{959}
\DeclareTextGlyphY{LinLibertine_R}{pi}{960}
\DeclareTextGlyphY{LinLibertine_R}{uni03C0}{960}
\DeclareTextGlyphY{LinLibertine_R}{rho}{961}
\DeclareTextGlyphY{LinLibertine_R}{uni03C1}{961}
\DeclareTextGlyphY{LinLibertine_R}{sigma1}{962}
\DeclareTextGlyphY{LinLibertine_R}{uni03C2}{962}
\DeclareTextGlyphY{LinLibertine_R}{sigma}{963}
\DeclareTextGlyphY{LinLibertine_R}{uni03C3}{963}
\DeclareTextGlyphY{LinLibertine_R}{tau}{964}
\DeclareTextGlyphY{LinLibertine_R}{uni03C4}{964}
\DeclareTextGlyphY{LinLibertine_R}{upsilon}{965}
\DeclareTextGlyphY{LinLibertine_R}{uni03C5}{965}
\DeclareTextGlyphY{LinLibertine_R}{phi}{966}
\DeclareTextGlyphY{LinLibertine_R}{uni03C6}{966}
\DeclareTextGlyphY{LinLibertine_R}{chi}{967}
\DeclareTextGlyphY{LinLibertine_R}{uni03C7}{967}
\DeclareTextGlyphY{LinLibertine_R}{psi}{968}
\DeclareTextGlyphY{LinLibertine_R}{uni03C8}{968}
\DeclareTextGlyphY{LinLibertine_R}{omega}{969}
\DeclareTextGlyphY{LinLibertine_R}{uni03C9}{969}
\DeclareTextGlyphY{LinLibertine_R}{iotadieresis}{970}
\DeclareTextGlyphY{LinLibertine_R}{uni03CA}{970}
\DeclareTextGlyphY{LinLibertine_R}{upsilondieresis}{971}
\DeclareTextGlyphY{LinLibertine_R}{uni03CB}{971}
\DeclareTextGlyphY{LinLibertine_R}{omicrontonos}{972}
\DeclareTextGlyphY{LinLibertine_R}{uni03CC}{972}
\DeclareTextGlyphY{LinLibertine_R}{upsilontonos}{973}
\DeclareTextGlyphY{LinLibertine_R}{uni03CD}{973}
\DeclareTextGlyphY{LinLibertine_R}{omegatonos}{974}
\DeclareTextGlyphY{LinLibertine_R}{uni03CE}{974}
\DeclareTextGlyphY{LinLibertine_R}{uni03D0}{976}
\DeclareTextGlyphY{LinLibertine_R}{theta1}{977}
\DeclareTextGlyphY{LinLibertine_R}{uni03D1}{977}
\DeclareTextGlyphY{LinLibertine_R}{Upsilon1}{978}
\DeclareTextGlyphY{LinLibertine_R}{uni03D2}{978}
\DeclareTextGlyphY{LinLibertine_R}{uni03D3}{979}
\DeclareTextGlyphY{LinLibertine_R}{uni03D4}{980}
\DeclareTextGlyphY{LinLibertine_R}{phi1}{981}
\DeclareTextGlyphY{LinLibertine_R}{uni03D5}{981}
\DeclareTextGlyphY{LinLibertine_R}{omega1}{982}
\DeclareTextGlyphY{LinLibertine_R}{uni03D6}{982}
\DeclareTextGlyphY{LinLibertine_R}{uni03D7}{983}
\DeclareTextGlyphY{LinLibertine_R}{uni03D8}{984}
\DeclareTextGlyphY{LinLibertine_R}{uni03D9}{985}
\DeclareTextGlyphY{LinLibertine_R}{uni03DA}{986}
\DeclareTextGlyphY{LinLibertine_R}{uni03DB}{987}
\DeclareTextGlyphY{LinLibertine_R}{uni03DC}{988}
\DeclareTextGlyphY{LinLibertine_R}{uni03DD}{989}
\DeclareTextGlyphY{LinLibertine_R}{uni03DE}{990}
\DeclareTextGlyphY{LinLibertine_R}{uni03DF}{991}
\DeclareTextGlyphY{LinLibertine_R}{uni03E0}{992}
\DeclareTextGlyphY{LinLibertine_R}{uni03E1}{993}
\DeclareTextGlyphY{LinLibertine_R}{uni03F0}{1008}
\DeclareTextGlyphY{LinLibertine_R}{uni03F1}{1009}
\DeclareTextGlyphY{LinLibertine_R}{uni03F2}{1010}
\DeclareTextGlyphY{LinLibertine_R}{uni03F3}{1011}
\DeclareTextGlyphY{LinLibertine_R}{uni03F4}{1012}
\DeclareTextGlyphY{LinLibertine_R}{uni03F5}{1013}
\DeclareTextGlyphY{LinLibertine_R}{uni03F6}{1014}
\DeclareTextGlyphY{LinLibertine_R}{uni03F8}{1016}
\DeclareTextGlyphY{LinLibertine_R}{uni03F9}{1017}
\DeclareTextGlyphY{LinLibertine_R}{uni03FB}{1019}
\DeclareTextGlyphY{LinLibertine_R}{uni03FD}{1021}
\DeclareTextGlyphY{LinLibertine_R}{uni03FE}{1022}
\DeclareTextGlyphY{LinLibertine_R}{uni03FF}{1023}
\DeclareTextGlyphY{LinLibertine_R}{uni0400}{1024}
\DeclareTextGlyphY{LinLibertine_R}{afii10023}{1025}
\DeclareTextGlyphY{LinLibertine_R}{uni0401}{1025}
\DeclareTextGlyphY{LinLibertine_R}{afii10051}{1026}
\DeclareTextGlyphY{LinLibertine_R}{uni0402}{1026}
\DeclareTextGlyphY{LinLibertine_R}{afii10052}{1027}
\DeclareTextGlyphY{LinLibertine_R}{uni0403}{1027}
\DeclareTextGlyphY{LinLibertine_R}{afii10053}{1028}
\DeclareTextGlyphY{LinLibertine_R}{uni0404}{1028}
\DeclareTextGlyphY{LinLibertine_R}{afii10054}{1029}
\DeclareTextGlyphY{LinLibertine_R}{uni0405}{1029}
\DeclareTextGlyphY{LinLibertine_R}{afii10055}{1030}
\DeclareTextGlyphY{LinLibertine_R}{uni0406}{1030}
\DeclareTextGlyphY{LinLibertine_R}{afii10056}{1031}
\DeclareTextGlyphY{LinLibertine_R}{uni0407}{1031}
\DeclareTextGlyphY{LinLibertine_R}{afii10057}{1032}
\DeclareTextGlyphY{LinLibertine_R}{uni0408}{1032}
\DeclareTextGlyphY{LinLibertine_R}{afii10058}{1033}
\DeclareTextGlyphY{LinLibertine_R}{uni0409}{1033}
\DeclareTextGlyphY{LinLibertine_R}{afii10059}{1034}
\DeclareTextGlyphY{LinLibertine_R}{uni040A}{1034}
\DeclareTextGlyphY{LinLibertine_R}{afii10060}{1035}
\DeclareTextGlyphY{LinLibertine_R}{uni040B}{1035}
\DeclareTextGlyphY{LinLibertine_R}{afii10061}{1036}
\DeclareTextGlyphY{LinLibertine_R}{uni040C}{1036}
\DeclareTextGlyphY{LinLibertine_R}{uni040D}{1037}
\DeclareTextGlyphY{LinLibertine_R}{afii10062}{1038}
\DeclareTextGlyphY{LinLibertine_R}{uni040E}{1038}
\DeclareTextGlyphY{LinLibertine_R}{afii10145}{1039}
\DeclareTextGlyphY{LinLibertine_R}{uni040F}{1039}
\DeclareTextGlyphY{LinLibertine_R}{afii10017}{1040}
\DeclareTextGlyphY{LinLibertine_R}{uni0410}{1040}
\DeclareTextGlyphY{LinLibertine_R}{afii10018}{1041}
\DeclareTextGlyphY{LinLibertine_R}{uni0411}{1041}
\DeclareTextGlyphY{LinLibertine_R}{afii10019}{1042}
\DeclareTextGlyphY{LinLibertine_R}{uni0412}{1042}
\DeclareTextGlyphY{LinLibertine_R}{afii10020}{1043}
\DeclareTextGlyphY{LinLibertine_R}{uni0413}{1043}
\DeclareTextGlyphY{LinLibertine_R}{afii10021}{1044}
\DeclareTextGlyphY{LinLibertine_R}{uni0414}{1044}
\DeclareTextGlyphY{LinLibertine_R}{afii10022}{1045}
\DeclareTextGlyphY{LinLibertine_R}{uni0415}{1045}
\DeclareTextGlyphY{LinLibertine_R}{afii10024}{1046}
\DeclareTextGlyphY{LinLibertine_R}{uni0416}{1046}
\DeclareTextGlyphY{LinLibertine_R}{afii10025}{1047}
\DeclareTextGlyphY{LinLibertine_R}{uni0417}{1047}
\DeclareTextGlyphY{LinLibertine_R}{afii10026}{1048}
\DeclareTextGlyphY{LinLibertine_R}{uni0418}{1048}
\DeclareTextGlyphY{LinLibertine_R}{afii10027}{1049}
\DeclareTextGlyphY{LinLibertine_R}{uni0419}{1049}
\DeclareTextGlyphY{LinLibertine_R}{afii10028}{1050}
\DeclareTextGlyphY{LinLibertine_R}{uni041A}{1050}
\DeclareTextGlyphY{LinLibertine_R}{afii10029}{1051}
\DeclareTextGlyphY{LinLibertine_R}{uni041B}{1051}
\DeclareTextGlyphY{LinLibertine_R}{afii10030}{1052}
\DeclareTextGlyphY{LinLibertine_R}{uni041C}{1052}
\DeclareTextGlyphY{LinLibertine_R}{afii10031}{1053}
\DeclareTextGlyphY{LinLibertine_R}{uni041D}{1053}
\DeclareTextGlyphY{LinLibertine_R}{afii10032}{1054}
\DeclareTextGlyphY{LinLibertine_R}{uni041E}{1054}
\DeclareTextGlyphY{LinLibertine_R}{afii10033}{1055}
\DeclareTextGlyphY{LinLibertine_R}{uni041F}{1055}
\DeclareTextGlyphY{LinLibertine_R}{afii10034}{1056}
\DeclareTextGlyphY{LinLibertine_R}{uni0420}{1056}
\DeclareTextGlyphY{LinLibertine_R}{afii10035}{1057}
\DeclareTextGlyphY{LinLibertine_R}{uni0421}{1057}
\DeclareTextGlyphY{LinLibertine_R}{afii10036}{1058}
\DeclareTextGlyphY{LinLibertine_R}{uni0422}{1058}
\DeclareTextGlyphY{LinLibertine_R}{afii10037}{1059}
\DeclareTextGlyphY{LinLibertine_R}{uni0423}{1059}
\DeclareTextGlyphY{LinLibertine_R}{afii10038}{1060}
\DeclareTextGlyphY{LinLibertine_R}{uni0424}{1060}
\DeclareTextGlyphY{LinLibertine_R}{afii10039}{1061}
\DeclareTextGlyphY{LinLibertine_R}{uni0425}{1061}
\DeclareTextGlyphY{LinLibertine_R}{afii10040}{1062}
\DeclareTextGlyphY{LinLibertine_R}{uni0426}{1062}
\DeclareTextGlyphY{LinLibertine_R}{afii10041}{1063}
\DeclareTextGlyphY{LinLibertine_R}{uni0427}{1063}
\DeclareTextGlyphY{LinLibertine_R}{afii10042}{1064}
\DeclareTextGlyphY{LinLibertine_R}{uni0428}{1064}
\DeclareTextGlyphY{LinLibertine_R}{afii10043}{1065}
\DeclareTextGlyphY{LinLibertine_R}{uni0429}{1065}
\DeclareTextGlyphY{LinLibertine_R}{afii10044}{1066}
\DeclareTextGlyphY{LinLibertine_R}{uni042A}{1066}
\DeclareTextGlyphY{LinLibertine_R}{afii10045}{1067}
\DeclareTextGlyphY{LinLibertine_R}{uni042B}{1067}
\DeclareTextGlyphY{LinLibertine_R}{afii10046}{1068}
\DeclareTextGlyphY{LinLibertine_R}{uni042C}{1068}
\DeclareTextGlyphY{LinLibertine_R}{afii10047}{1069}
\DeclareTextGlyphY{LinLibertine_R}{uni042D}{1069}
\DeclareTextGlyphY{LinLibertine_R}{afii10048}{1070}
\DeclareTextGlyphY{LinLibertine_R}{uni042E}{1070}
\DeclareTextGlyphY{LinLibertine_R}{afii10049}{1071}
\DeclareTextGlyphY{LinLibertine_R}{uni042F}{1071}
\DeclareTextGlyphY{LinLibertine_R}{afii10065}{1072}
\DeclareTextGlyphY{LinLibertine_R}{uni0430}{1072}
\DeclareTextGlyphY{LinLibertine_R}{afii10066}{1073}
\DeclareTextGlyphY{LinLibertine_R}{uni0431}{1073}
\DeclareTextGlyphY{LinLibertine_R}{afii10067}{1074}
\DeclareTextGlyphY{LinLibertine_R}{uni0432}{1074}
\DeclareTextGlyphY{LinLibertine_R}{afii10068}{1075}
\DeclareTextGlyphY{LinLibertine_R}{uni0433}{1075}
\DeclareTextGlyphY{LinLibertine_R}{afii10069}{1076}
\DeclareTextGlyphY{LinLibertine_R}{uni0434}{1076}
\DeclareTextGlyphY{LinLibertine_R}{afii10070}{1077}
\DeclareTextGlyphY{LinLibertine_R}{uni0435}{1077}
\DeclareTextGlyphY{LinLibertine_R}{afii10072}{1078}
\DeclareTextGlyphY{LinLibertine_R}{uni0436}{1078}
\DeclareTextGlyphY{LinLibertine_R}{afii10073}{1079}
\DeclareTextGlyphY{LinLibertine_R}{uni0437}{1079}
\DeclareTextGlyphY{LinLibertine_R}{afii10074}{1080}
\DeclareTextGlyphY{LinLibertine_R}{uni0438}{1080}
\DeclareTextGlyphY{LinLibertine_R}{afii10075}{1081}
\DeclareTextGlyphY{LinLibertine_R}{uni0439}{1081}
\DeclareTextGlyphY{LinLibertine_R}{afii10076}{1082}
\DeclareTextGlyphY{LinLibertine_R}{uni043A}{1082}
\DeclareTextGlyphY{LinLibertine_R}{afii10077}{1083}
\DeclareTextGlyphY{LinLibertine_R}{uni043B}{1083}
\DeclareTextGlyphY{LinLibertine_R}{afii10078}{1084}
\DeclareTextGlyphY{LinLibertine_R}{uni043C}{1084}
\DeclareTextGlyphY{LinLibertine_R}{afii10079}{1085}
\DeclareTextGlyphY{LinLibertine_R}{uni043D}{1085}
\DeclareTextGlyphY{LinLibertine_R}{afii10080}{1086}
\DeclareTextGlyphY{LinLibertine_R}{uni043E}{1086}
\DeclareTextGlyphY{LinLibertine_R}{afii10081}{1087}
\DeclareTextGlyphY{LinLibertine_R}{uni043F}{1087}
\DeclareTextGlyphY{LinLibertine_R}{afii10082}{1088}
\DeclareTextGlyphY{LinLibertine_R}{uni0440}{1088}
\DeclareTextGlyphY{LinLibertine_R}{afii10083}{1089}
\DeclareTextGlyphY{LinLibertine_R}{uni0441}{1089}
\DeclareTextGlyphY{LinLibertine_R}{afii10084}{1090}
\DeclareTextGlyphY{LinLibertine_R}{uni0442}{1090}
\DeclareTextGlyphY{LinLibertine_R}{afii10085}{1091}
\DeclareTextGlyphY{LinLibertine_R}{uni0443}{1091}
\DeclareTextGlyphY{LinLibertine_R}{afii10086}{1092}
\DeclareTextGlyphY{LinLibertine_R}{uni0444}{1092}
\DeclareTextGlyphY{LinLibertine_R}{afii10087}{1093}
\DeclareTextGlyphY{LinLibertine_R}{uni0445}{1093}
\DeclareTextGlyphY{LinLibertine_R}{afii10088}{1094}
\DeclareTextGlyphY{LinLibertine_R}{uni0446}{1094}
\DeclareTextGlyphY{LinLibertine_R}{afii10089}{1095}
\DeclareTextGlyphY{LinLibertine_R}{uni0447}{1095}
\DeclareTextGlyphY{LinLibertine_R}{afii10090}{1096}
\DeclareTextGlyphY{LinLibertine_R}{uni0448}{1096}
\DeclareTextGlyphY{LinLibertine_R}{afii10091}{1097}
\DeclareTextGlyphY{LinLibertine_R}{uni0449}{1097}
\DeclareTextGlyphY{LinLibertine_R}{afii10092}{1098}
\DeclareTextGlyphY{LinLibertine_R}{uni044A}{1098}
\DeclareTextGlyphY{LinLibertine_R}{afii10093}{1099}
\DeclareTextGlyphY{LinLibertine_R}{uni044B}{1099}
\DeclareTextGlyphY{LinLibertine_R}{afii10094}{1100}
\DeclareTextGlyphY{LinLibertine_R}{uni044C}{1100}
\DeclareTextGlyphY{LinLibertine_R}{afii10095}{1101}
\DeclareTextGlyphY{LinLibertine_R}{uni044D}{1101}
\DeclareTextGlyphY{LinLibertine_R}{afii10096}{1102}
\DeclareTextGlyphY{LinLibertine_R}{uni044E}{1102}
\DeclareTextGlyphY{LinLibertine_R}{afii10097}{1103}
\DeclareTextGlyphY{LinLibertine_R}{uni044F}{1103}
\DeclareTextGlyphY{LinLibertine_R}{uni0450}{1104}
\DeclareTextGlyphY{LinLibertine_R}{afii10071}{1105}
\DeclareTextGlyphY{LinLibertine_R}{uni0451}{1105}
\DeclareTextGlyphY{LinLibertine_R}{afii10099}{1106}
\DeclareTextGlyphY{LinLibertine_R}{uni0452}{1106}
\DeclareTextGlyphY{LinLibertine_R}{afii10100}{1107}
\DeclareTextGlyphY{LinLibertine_R}{uni0453}{1107}
\DeclareTextGlyphY{LinLibertine_R}{afii10101}{1108}
\DeclareTextGlyphY{LinLibertine_R}{uni0454}{1108}
\DeclareTextGlyphY{LinLibertine_R}{afii10102}{1109}
\DeclareTextGlyphY{LinLibertine_R}{uni0455}{1109}
\DeclareTextGlyphY{LinLibertine_R}{afii10103}{1110}
\DeclareTextGlyphY{LinLibertine_R}{uni0456}{1110}
\DeclareTextGlyphY{LinLibertine_R}{afii10104}{1111}
\DeclareTextGlyphY{LinLibertine_R}{uni0457}{1111}
\DeclareTextGlyphY{LinLibertine_R}{afii10105}{1112}
\DeclareTextGlyphY{LinLibertine_R}{uni0458}{1112}
\DeclareTextGlyphY{LinLibertine_R}{afii10106}{1113}
\DeclareTextGlyphY{LinLibertine_R}{uni0459}{1113}
\DeclareTextGlyphY{LinLibertine_R}{afii10107}{1114}
\DeclareTextGlyphY{LinLibertine_R}{uni045A}{1114}
\DeclareTextGlyphY{LinLibertine_R}{afii10108}{1115}
\DeclareTextGlyphY{LinLibertine_R}{uni045B}{1115}
\DeclareTextGlyphY{LinLibertine_R}{afii10109}{1116}
\DeclareTextGlyphY{LinLibertine_R}{uni045C}{1116}
\DeclareTextGlyphY{LinLibertine_R}{uni045D}{1117}
\DeclareTextGlyphY{LinLibertine_R}{afii10110}{1118}
\DeclareTextGlyphY{LinLibertine_R}{uni045E}{1118}
\DeclareTextGlyphY{LinLibertine_R}{afii10193}{1119}
\DeclareTextGlyphY{LinLibertine_R}{uni045F}{1119}
\DeclareTextGlyphY{LinLibertine_R}{uni0460}{1120}
\DeclareTextGlyphY{LinLibertine_R}{uni0461}{1121}
\DeclareTextGlyphY{LinLibertine_R}{afii10146}{1122}
\DeclareTextGlyphY{LinLibertine_R}{uni0462}{1122}
\DeclareTextGlyphY{LinLibertine_R}{afii10194}{1123}
\DeclareTextGlyphY{LinLibertine_R}{uni0463}{1123}
\DeclareTextGlyphY{LinLibertine_R}{uni0464}{1124}
\DeclareTextGlyphY{LinLibertine_R}{uni0465}{1125}
\DeclareTextGlyphY{LinLibertine_R}{uni0466}{1126}
\DeclareTextGlyphY{LinLibertine_R}{uni0467}{1127}
\DeclareTextGlyphY{LinLibertine_R}{uni0468}{1128}
\DeclareTextGlyphY{LinLibertine_R}{uni0469}{1129}
\DeclareTextGlyphY{LinLibertine_R}{uni046A}{1130}
\DeclareTextGlyphY{LinLibertine_R}{uni046B}{1131}
\DeclareTextGlyphY{LinLibertine_R}{uni046C}{1132}
\DeclareTextGlyphY{LinLibertine_R}{uni046D}{1133}
\DeclareTextGlyphY{LinLibertine_R}{uni046E}{1134}
\DeclareTextGlyphY{LinLibertine_R}{uni046F}{1135}
\DeclareTextGlyphY{LinLibertine_R}{uni0470}{1136}
\DeclareTextGlyphY{LinLibertine_R}{uni0471}{1137}
\DeclareTextGlyphY{LinLibertine_R}{afii10147}{1138}
\DeclareTextGlyphY{LinLibertine_R}{uni0472}{1138}
\DeclareTextGlyphY{LinLibertine_R}{afii10195}{1139}
\DeclareTextGlyphY{LinLibertine_R}{uni0473}{1139}
\DeclareTextGlyphY{LinLibertine_R}{afii10148}{1140}
\DeclareTextGlyphY{LinLibertine_R}{uni0474}{1140}
\DeclareTextGlyphY{LinLibertine_R}{afii10196}{1141}
\DeclareTextGlyphY{LinLibertine_R}{uni0475}{1141}
\DeclareTextGlyphY{LinLibertine_R}{uni0476}{1142}
\DeclareTextGlyphY{LinLibertine_R}{uni0477}{1143}
\DeclareTextGlyphY{LinLibertine_R}{uni047C}{1148}
\DeclareTextGlyphY{LinLibertine_R}{uni047D}{1149}
\DeclareTextGlyphY{LinLibertine_R}{uni047E}{1150}
\DeclareTextGlyphY{LinLibertine_R}{uni047F}{1151}
\DeclareTextGlyphY{LinLibertine_R}{uni0483}{1155}
\DeclareTextGlyphY{LinLibertine_R}{uni048C}{1164}
\DeclareTextGlyphY{LinLibertine_R}{uni048D}{1165}
\DeclareTextGlyphY{LinLibertine_R}{uni048E}{1166}
\DeclareTextGlyphY{LinLibertine_R}{uni048F}{1167}
\DeclareTextGlyphY{LinLibertine_R}{afii10050}{1168}
\DeclareTextGlyphY{LinLibertine_R}{uni0490}{1168}
\DeclareTextGlyphY{LinLibertine_R}{afii10098}{1169}
\DeclareTextGlyphY{LinLibertine_R}{uni0491}{1169}
\DeclareTextGlyphY{LinLibertine_R}{uni0492}{1170}
\DeclareTextGlyphY{LinLibertine_R}{uni0493}{1171}
\DeclareTextGlyphY{LinLibertine_R}{uni0494}{1172}
\DeclareTextGlyphY{LinLibertine_R}{uni0495}{1173}
\DeclareTextGlyphY{LinLibertine_R}{uni0496}{1174}
\DeclareTextGlyphY{LinLibertine_R}{uni0497}{1175}
\DeclareTextGlyphY{LinLibertine_R}{uni0498}{1176}
\DeclareTextGlyphY{LinLibertine_R}{uni0499}{1177}
\DeclareTextGlyphY{LinLibertine_R}{uni049A}{1178}
\DeclareTextGlyphY{LinLibertine_R}{uni049B}{1179}
\DeclareTextGlyphY{LinLibertine_R}{uni049C}{1180}
\DeclareTextGlyphY{LinLibertine_R}{uni049D}{1181}
\DeclareTextGlyphY{LinLibertine_R}{uni049E}{1182}
\DeclareTextGlyphY{LinLibertine_R}{uni049F}{1183}
\DeclareTextGlyphY{LinLibertine_R}{uni04A0}{1184}
\DeclareTextGlyphY{LinLibertine_R}{uni04A1}{1185}
\DeclareTextGlyphY{LinLibertine_R}{uni04A2}{1186}
\DeclareTextGlyphY{LinLibertine_R}{uni04A3}{1187}
\DeclareTextGlyphY{LinLibertine_R}{uni04A4}{1188}
\DeclareTextGlyphY{LinLibertine_R}{uni04A5}{1189}
\DeclareTextGlyphY{LinLibertine_R}{uni04A6}{1190}
\DeclareTextGlyphY{LinLibertine_R}{uni04A7}{1191}
\DeclareTextGlyphY{LinLibertine_R}{uni04A8}{1192}
\DeclareTextGlyphY{LinLibertine_R}{uni04A9}{1193}
\DeclareTextGlyphY{LinLibertine_R}{uni04AA}{1194}
\DeclareTextGlyphY{LinLibertine_R}{uni04AB}{1195}
\DeclareTextGlyphY{LinLibertine_R}{uni04AC}{1196}
\DeclareTextGlyphY{LinLibertine_R}{uni04AD}{1197}
\DeclareTextGlyphY{LinLibertine_R}{uni04AE}{1198}
\DeclareTextGlyphY{LinLibertine_R}{uni04AF}{1199}
\DeclareTextGlyphY{LinLibertine_R}{uni04B0}{1200}
\DeclareTextGlyphY{LinLibertine_R}{uni04B1}{1201}
\DeclareTextGlyphY{LinLibertine_R}{uni04B2}{1202}
\DeclareTextGlyphY{LinLibertine_R}{uni04B3}{1203}
\DeclareTextGlyphY{LinLibertine_R}{uni04B4}{1204}
\DeclareTextGlyphY{LinLibertine_R}{uni04B5}{1205}
\DeclareTextGlyphY{LinLibertine_R}{uni04B6}{1206}
\DeclareTextGlyphY{LinLibertine_R}{uni04B7}{1207}
\DeclareTextGlyphY{LinLibertine_R}{uni04B8}{1208}
\DeclareTextGlyphY{LinLibertine_R}{uni04B9}{1209}
\DeclareTextGlyphY{LinLibertine_R}{uni04BA}{1210}
\DeclareTextGlyphY{LinLibertine_R}{uni04BB}{1211}
\DeclareTextGlyphY{LinLibertine_R}{uni04BC}{1212}
\DeclareTextGlyphY{LinLibertine_R}{uni04BD}{1213}
\DeclareTextGlyphY{LinLibertine_R}{uni04BE}{1214}
\DeclareTextGlyphY{LinLibertine_R}{uni04BF}{1215}
\DeclareTextGlyphY{LinLibertine_R}{uni04C0}{1216}
\DeclareTextGlyphY{LinLibertine_R}{uni04C1}{1217}
\DeclareTextGlyphY{LinLibertine_R}{uni04C2}{1218}
\DeclareTextGlyphY{LinLibertine_R}{uni04C3}{1219}
\DeclareTextGlyphY{LinLibertine_R}{uni04C4}{1220}
\DeclareTextGlyphY{LinLibertine_R}{uni04C7}{1223}
\DeclareTextGlyphY{LinLibertine_R}{uni04C8}{1224}
\DeclareTextGlyphY{LinLibertine_R}{uni04C9}{1225}
\DeclareTextGlyphY{LinLibertine_R}{uni04CA}{1226}
\DeclareTextGlyphY{LinLibertine_R}{uni04CB}{1227}
\DeclareTextGlyphY{LinLibertine_R}{uni04CC}{1228}
\DeclareTextGlyphY{LinLibertine_R}{uni04D0}{1232}
\DeclareTextGlyphY{LinLibertine_R}{uni04D1}{1233}
\DeclareTextGlyphY{LinLibertine_R}{uni04D2}{1234}
\DeclareTextGlyphY{LinLibertine_R}{uni04D3}{1235}
\DeclareTextGlyphY{LinLibertine_R}{uni04D4}{1236}
\DeclareTextGlyphY{LinLibertine_R}{uni04D5}{1237}
\DeclareTextGlyphY{LinLibertine_R}{uni04D6}{1238}
\DeclareTextGlyphY{LinLibertine_R}{uni04D7}{1239}
\DeclareTextGlyphY{LinLibertine_R}{uni04D8}{1240}
\DeclareTextGlyphY{LinLibertine_R}{afii10846}{1241}
\DeclareTextGlyphY{LinLibertine_R}{uni04D9}{1241}
\DeclareTextGlyphY{LinLibertine_R}{uni04DA}{1242}
\DeclareTextGlyphY{LinLibertine_R}{uni04DB}{1243}
\DeclareTextGlyphY{LinLibertine_R}{uni04DC}{1244}
\DeclareTextGlyphY{LinLibertine_R}{uni04DD}{1245}
\DeclareTextGlyphY{LinLibertine_R}{uni04DE}{1246}
\DeclareTextGlyphY{LinLibertine_R}{uni04DF}{1247}
\DeclareTextGlyphY{LinLibertine_R}{uni04E0}{1248}
\DeclareTextGlyphY{LinLibertine_R}{uni04E1}{1249}
\DeclareTextGlyphY{LinLibertine_R}{uni04E2}{1250}
\DeclareTextGlyphY{LinLibertine_R}{uni04E3}{1251}
\DeclareTextGlyphY{LinLibertine_R}{uni04E4}{1252}
\DeclareTextGlyphY{LinLibertine_R}{uni04E5}{1253}
\DeclareTextGlyphY{LinLibertine_R}{uni04E6}{1254}
\DeclareTextGlyphY{LinLibertine_R}{uni04E7}{1255}
\DeclareTextGlyphY{LinLibertine_R}{uni04E8}{1256}
\DeclareTextGlyphY{LinLibertine_R}{uni04E9}{1257}
\DeclareTextGlyphY{LinLibertine_R}{uni04EA}{1258}
\DeclareTextGlyphY{LinLibertine_R}{uni04EB}{1259}
\DeclareTextGlyphY{LinLibertine_R}{uni04EC}{1260}
\DeclareTextGlyphY{LinLibertine_R}{uni04ED}{1261}
\DeclareTextGlyphY{LinLibertine_R}{uni04EE}{1262}
\DeclareTextGlyphY{LinLibertine_R}{uni04EF}{1263}
\DeclareTextGlyphY{LinLibertine_R}{uni04F0}{1264}
\DeclareTextGlyphY{LinLibertine_R}{uni04F1}{1265}
\DeclareTextGlyphY{LinLibertine_R}{uni04F2}{1266}
\DeclareTextGlyphY{LinLibertine_R}{uni04F3}{1267}
\DeclareTextGlyphY{LinLibertine_R}{uni04F4}{1268}
\DeclareTextGlyphY{LinLibertine_R}{uni04F5}{1269}
\DeclareTextGlyphY{LinLibertine_R}{uni04F6}{1270}
\DeclareTextGlyphY{LinLibertine_R}{uni04F7}{1271}
\DeclareTextGlyphY{LinLibertine_R}{uni04F8}{1272}
\DeclareTextGlyphY{LinLibertine_R}{uni04F9}{1273}
\DeclareTextGlyphY{LinLibertine_R}{afii57799}{1456}
\DeclareTextGlyphY{LinLibertine_R}{uni05B0}{1456}
\DeclareTextGlyphY{LinLibertine_R}{afii57801}{1457}
\DeclareTextGlyphY{LinLibertine_R}{uni05B1}{1457}
\DeclareTextGlyphY{LinLibertine_R}{afii57800}{1458}
\DeclareTextGlyphY{LinLibertine_R}{uni05B2}{1458}
\DeclareTextGlyphY{LinLibertine_R}{afii57802}{1459}
\DeclareTextGlyphY{LinLibertine_R}{uni05B3}{1459}
\DeclareTextGlyphY{LinLibertine_R}{afii57793}{1460}
\DeclareTextGlyphY{LinLibertine_R}{uni05B4}{1460}
\DeclareTextGlyphY{LinLibertine_R}{afii57794}{1461}
\DeclareTextGlyphY{LinLibertine_R}{uni05B5}{1461}
\DeclareTextGlyphY{LinLibertine_R}{afii57795}{1462}
\DeclareTextGlyphY{LinLibertine_R}{uni05B6}{1462}
\DeclareTextGlyphY{LinLibertine_R}{afii57798}{1463}
\DeclareTextGlyphY{LinLibertine_R}{uni05B7}{1463}
\DeclareTextGlyphY{LinLibertine_R}{afii57797}{1464}
\DeclareTextGlyphY{LinLibertine_R}{uni05B8}{1464}
\DeclareTextGlyphY{LinLibertine_R}{afii57806}{1465}
\DeclareTextGlyphY{LinLibertine_R}{uni05B9}{1465}
\DeclareTextGlyphY{LinLibertine_R}{uni05BA}{1466}
\DeclareTextGlyphY{LinLibertine_R}{afii57796}{1467}
\DeclareTextGlyphY{LinLibertine_R}{uni05BB}{1467}
\DeclareTextGlyphY{LinLibertine_R}{afii57807}{1468}
\DeclareTextGlyphY{LinLibertine_R}{uni05BC}{1468}
\DeclareTextGlyphY{LinLibertine_R}{afii57839}{1469}
\DeclareTextGlyphY{LinLibertine_R}{uni05BD}{1469}
\DeclareTextGlyphY{LinLibertine_R}{afii57645}{1470}
\DeclareTextGlyphY{LinLibertine_R}{uni05BE}{1470}
\DeclareTextGlyphY{LinLibertine_R}{afii57841}{1471}
\DeclareTextGlyphY{LinLibertine_R}{uni05BF}{1471}
\DeclareTextGlyphY{LinLibertine_R}{afii57842}{1472}
\DeclareTextGlyphY{LinLibertine_R}{uni05C0}{1472}
\DeclareTextGlyphY{LinLibertine_R}{afii57804}{1473}
\DeclareTextGlyphY{LinLibertine_R}{uni05C1}{1473}
\DeclareTextGlyphY{LinLibertine_R}{afii57803}{1474}
\DeclareTextGlyphY{LinLibertine_R}{uni05C2}{1474}
\DeclareTextGlyphY{LinLibertine_R}{afii57658}{1475}
\DeclareTextGlyphY{LinLibertine_R}{uni05C3}{1475}
\DeclareTextGlyphY{LinLibertine_R}{uni05C6}{1478}
\DeclareTextGlyphY{LinLibertine_R}{afii57664}{1488}
\DeclareTextGlyphY{LinLibertine_R}{uni05D0}{1488}
\DeclareTextGlyphY{LinLibertine_R}{afii57665}{1489}
\DeclareTextGlyphY{LinLibertine_R}{uni05D1}{1489}
\DeclareTextGlyphY{LinLibertine_R}{afii57666}{1490}
\DeclareTextGlyphY{LinLibertine_R}{uni05D2}{1490}
\DeclareTextGlyphY{LinLibertine_R}{afii57667}{1491}
\DeclareTextGlyphY{LinLibertine_R}{uni05D3}{1491}
\DeclareTextGlyphY{LinLibertine_R}{afii57668}{1492}
\DeclareTextGlyphY{LinLibertine_R}{uni05D4}{1492}
\DeclareTextGlyphY{LinLibertine_R}{afii57669}{1493}
\DeclareTextGlyphY{LinLibertine_R}{uni05D5}{1493}
\DeclareTextGlyphY{LinLibertine_R}{afii57670}{1494}
\DeclareTextGlyphY{LinLibertine_R}{uni05D6}{1494}
\DeclareTextGlyphY{LinLibertine_R}{afii57671}{1495}
\DeclareTextGlyphY{LinLibertine_R}{uni05D7}{1495}
\DeclareTextGlyphY{LinLibertine_R}{afii57672}{1496}
\DeclareTextGlyphY{LinLibertine_R}{uni05D8}{1496}
\DeclareTextGlyphY{LinLibertine_R}{afii57673}{1497}
\DeclareTextGlyphY{LinLibertine_R}{uni05D9}{1497}
\DeclareTextGlyphY{LinLibertine_R}{afii57674}{1498}
\DeclareTextGlyphY{LinLibertine_R}{uni05DA}{1498}
\DeclareTextGlyphY{LinLibertine_R}{afii57675}{1499}
\DeclareTextGlyphY{LinLibertine_R}{uni05DB}{1499}
\DeclareTextGlyphY{LinLibertine_R}{afii57676}{1500}
\DeclareTextGlyphY{LinLibertine_R}{uni05DC}{1500}
\DeclareTextGlyphY{LinLibertine_R}{afii57677}{1501}
\DeclareTextGlyphY{LinLibertine_R}{uni05DD}{1501}
\DeclareTextGlyphY{LinLibertine_R}{afii57678}{1502}
\DeclareTextGlyphY{LinLibertine_R}{uni05DE}{1502}
\DeclareTextGlyphY{LinLibertine_R}{afii57679}{1503}
\DeclareTextGlyphY{LinLibertine_R}{uni05DF}{1503}
\DeclareTextGlyphY{LinLibertine_R}{afii57680}{1504}
\DeclareTextGlyphY{LinLibertine_R}{uni05E0}{1504}
\DeclareTextGlyphY{LinLibertine_R}{afii57681}{1505}
\DeclareTextGlyphY{LinLibertine_R}{uni05E1}{1505}
\DeclareTextGlyphY{LinLibertine_R}{afii57682}{1506}
\DeclareTextGlyphY{LinLibertine_R}{uni05E2}{1506}
\DeclareTextGlyphY{LinLibertine_R}{afii57683}{1507}
\DeclareTextGlyphY{LinLibertine_R}{uni05E3}{1507}
\DeclareTextGlyphY{LinLibertine_R}{afii57684}{1508}
\DeclareTextGlyphY{LinLibertine_R}{uni05E4}{1508}
\DeclareTextGlyphY{LinLibertine_R}{afii57685}{1509}
\DeclareTextGlyphY{LinLibertine_R}{uni05E5}{1509}
\DeclareTextGlyphY{LinLibertine_R}{afii57686}{1510}
\DeclareTextGlyphY{LinLibertine_R}{uni05E6}{1510}
\DeclareTextGlyphY{LinLibertine_R}{afii57687}{1511}
\DeclareTextGlyphY{LinLibertine_R}{uni05E7}{1511}
\DeclareTextGlyphY{LinLibertine_R}{afii57688}{1512}
\DeclareTextGlyphY{LinLibertine_R}{uni05E8}{1512}
\DeclareTextGlyphY{LinLibertine_R}{afii57689}{1513}
\DeclareTextGlyphY{LinLibertine_R}{uni05E9}{1513}
\DeclareTextGlyphY{LinLibertine_R}{afii57690}{1514}
\DeclareTextGlyphY{LinLibertine_R}{uni05EA}{1514}
\DeclareTextGlyphY{LinLibertine_R}{afii57716}{1520}
\DeclareTextGlyphY{LinLibertine_R}{uni05F0}{1520}
\DeclareTextGlyphY{LinLibertine_R}{afii57717}{1521}
\DeclareTextGlyphY{LinLibertine_R}{uni05F1}{1521}
\DeclareTextGlyphY{LinLibertine_R}{afii57718}{1522}
\DeclareTextGlyphY{LinLibertine_R}{uni05F2}{1522}
\DeclareTextGlyphY{LinLibertine_R}{uni05F3}{1523}
\DeclareTextGlyphY{LinLibertine_R}{uni05F4}{1524}
\DeclareTextGlyphY{LinLibertine_R}{uni1D15}{7445}
\DeclareTextGlyphY{LinLibertine_R}{a.superior}{7491}
\DeclareTextGlyphY{LinLibertine_R}{uni1D43}{7491}
\DeclareTextGlyphY{LinLibertine_R}{aturned.superior}{7492}
\DeclareTextGlyphY{LinLibertine_R}{uni1D44}{7492}
\DeclareTextGlyphY{LinLibertine_R}{uni1D45}{7493}
\DeclareTextGlyphY{LinLibertine_R}{uni1D46}{7494}
\DeclareTextGlyphY{LinLibertine_R}{b.superior}{7495}
\DeclareTextGlyphY{LinLibertine_R}{uni1D47}{7495}
\DeclareTextGlyphY{LinLibertine_R}{d.superior}{7496}
\DeclareTextGlyphY{LinLibertine_R}{uni1D48}{7496}
\DeclareTextGlyphY{LinLibertine_R}{e.superior}{7497}
\DeclareTextGlyphY{LinLibertine_R}{uni1D49}{7497}
\DeclareTextGlyphY{LinLibertine_R}{eturned.superior}{7498}
\DeclareTextGlyphY{LinLibertine_R}{uni1D4A}{7498}
\DeclareTextGlyphY{LinLibertine_R}{uni1D4B}{7499}
\DeclareTextGlyphY{LinLibertine_R}{uni1D4C}{7500}
\DeclareTextGlyphY{LinLibertine_R}{g.superior}{7501}
\DeclareTextGlyphY{LinLibertine_R}{uni1D4D}{7501}
\DeclareTextGlyphY{LinLibertine_R}{iturned.superior}{7502}
\DeclareTextGlyphY{LinLibertine_R}{uni1D4E}{7502}
\DeclareTextGlyphY{LinLibertine_R}{k.superior}{7503}
\DeclareTextGlyphY{LinLibertine_R}{uni1D4F}{7503}
\DeclareTextGlyphY{LinLibertine_R}{m.superior}{7504}
\DeclareTextGlyphY{LinLibertine_R}{uni1D50}{7504}
\DeclareTextGlyphY{LinLibertine_R}{eng.superior}{7505}
\DeclareTextGlyphY{LinLibertine_R}{uni1D51}{7505}
\DeclareTextGlyphY{LinLibertine_R}{o.superior}{7506}
\DeclareTextGlyphY{LinLibertine_R}{uni1D52}{7506}
\DeclareTextGlyphY{LinLibertine_R}{cturned.superior}{7507}
\DeclareTextGlyphY{LinLibertine_R}{uni1D53}{7507}
\DeclareTextGlyphY{LinLibertine_R}{uni1D54}{7508}
\DeclareTextGlyphY{LinLibertine_R}{uni1D55}{7509}
\DeclareTextGlyphY{LinLibertine_R}{p.superior}{7510}
\DeclareTextGlyphY{LinLibertine_R}{uni1D56}{7510}
\DeclareTextGlyphY{LinLibertine_R}{t.superior}{7511}
\DeclareTextGlyphY{LinLibertine_R}{uni1D57}{7511}
\DeclareTextGlyphY{LinLibertine_R}{u.superior}{7512}
\DeclareTextGlyphY{LinLibertine_R}{uni1D58}{7512}
\DeclareTextGlyphY{LinLibertine_R}{uni1D59}{7513}
\DeclareTextGlyphY{LinLibertine_R}{mturned.superior}{7514}
\DeclareTextGlyphY{LinLibertine_R}{uni1D5A}{7514}
\DeclareTextGlyphY{LinLibertine_R}{v.superior}{7515}
\DeclareTextGlyphY{LinLibertine_R}{uni1D5B}{7515}
\DeclareTextGlyphY{LinLibertine_R}{uni1D5C}{7516}
\DeclareTextGlyphY{LinLibertine_R}{uni1D5D}{7517}
\DeclareTextGlyphY{LinLibertine_R}{uni1D5E}{7518}
\DeclareTextGlyphY{LinLibertine_R}{uni1D5F}{7519}
\DeclareTextGlyphY{LinLibertine_R}{uni1D62}{7522}
\DeclareTextGlyphY{LinLibertine_R}{uni1D63}{7523}
\DeclareTextGlyphY{LinLibertine_R}{uni1D64}{7524}
\DeclareTextGlyphY{LinLibertine_R}{uni1D65}{7525}
\DeclareTextGlyphY{LinLibertine_R}{uni1D66}{7526}
\DeclareTextGlyphY{LinLibertine_R}{uni1D67}{7527}
\DeclareTextGlyphY{LinLibertine_R}{c.superior}{7580}
\DeclareTextGlyphY{LinLibertine_R}{uni1D9C}{7580}
\DeclareTextGlyphY{LinLibertine_R}{f.superior}{7584}
\DeclareTextGlyphY{LinLibertine_R}{uni1DA0}{7584}
\DeclareTextGlyphY{LinLibertine_R}{z.superior}{7611}
\DeclareTextGlyphY{LinLibertine_R}{uni1DBB}{7611}
\DeclareTextGlyphY{LinLibertine_R}{uni1E00}{7680}
\DeclareTextGlyphY{LinLibertine_R}{uni1E01}{7681}
\DeclareTextGlyphY{LinLibertine_R}{uni1E02}{7682}
\DeclareTextGlyphY{LinLibertine_R}{uni1E03}{7683}
\DeclareTextGlyphY{LinLibertine_R}{uni1E04}{7684}
\DeclareTextGlyphY{LinLibertine_R}{uni1E05}{7685}
\DeclareTextGlyphY{LinLibertine_R}{uni1E06}{7686}
\DeclareTextGlyphY{LinLibertine_R}{uni1E07}{7687}
\DeclareTextGlyphY{LinLibertine_R}{uni1E08}{7688}
\DeclareTextGlyphY{LinLibertine_R}{uni1E09}{7689}
\DeclareTextGlyphY{LinLibertine_R}{uni1E0A}{7690}
\DeclareTextGlyphY{LinLibertine_R}{uni1E0B}{7691}
\DeclareTextGlyphY{LinLibertine_R}{uni1E0C}{7692}
\DeclareTextGlyphY{LinLibertine_R}{uni1E0D}{7693}
\DeclareTextGlyphY{LinLibertine_R}{uni1E0E}{7694}
\DeclareTextGlyphY{LinLibertine_R}{uni1E0F}{7695}
\DeclareTextGlyphY{LinLibertine_R}{uni1E10}{7696}
\DeclareTextGlyphY{LinLibertine_R}{uni1E11}{7697}
\DeclareTextGlyphY{LinLibertine_R}{uni1E12}{7698}
\DeclareTextGlyphY{LinLibertine_R}{uni1E13}{7699}
\DeclareTextGlyphY{LinLibertine_R}{uni1E14}{7700}
\DeclareTextGlyphY{LinLibertine_R}{uni1E15}{7701}
\DeclareTextGlyphY{LinLibertine_R}{uni1E16}{7702}
\DeclareTextGlyphY{LinLibertine_R}{uni1E17}{7703}
\DeclareTextGlyphY{LinLibertine_R}{uni1E18}{7704}
\DeclareTextGlyphY{LinLibertine_R}{uni1E19}{7705}
\DeclareTextGlyphY{LinLibertine_R}{uni1E1A}{7706}
\DeclareTextGlyphY{LinLibertine_R}{uni1E1B}{7707}
\DeclareTextGlyphY{LinLibertine_R}{uni1E1C}{7708}
\DeclareTextGlyphY{LinLibertine_R}{uni1E1D}{7709}
\DeclareTextGlyphY{LinLibertine_R}{uni1E1E}{7710}
\DeclareTextGlyphY{LinLibertine_R}{uni1E1F}{7711}
\DeclareTextGlyphY{LinLibertine_R}{uni1E20}{7712}
\DeclareTextGlyphY{LinLibertine_R}{uni1E21}{7713}
\DeclareTextGlyphY{LinLibertine_R}{uni1E22}{7714}
\DeclareTextGlyphY{LinLibertine_R}{uni1E23}{7715}
\DeclareTextGlyphY{LinLibertine_R}{uni1E24}{7716}
\DeclareTextGlyphY{LinLibertine_R}{uni1E25}{7717}
\DeclareTextGlyphY{LinLibertine_R}{uni1E26}{7718}
\DeclareTextGlyphY{LinLibertine_R}{uni1E27}{7719}
\DeclareTextGlyphY{LinLibertine_R}{uni1E28}{7720}
\DeclareTextGlyphY{LinLibertine_R}{uni1E29}{7721}
\DeclareTextGlyphY{LinLibertine_R}{uni1E2A}{7722}
\DeclareTextGlyphY{LinLibertine_R}{uni1E2B}{7723}
\DeclareTextGlyphY{LinLibertine_R}{uni1E2C}{7724}
\DeclareTextGlyphY{LinLibertine_R}{uni1E2D}{7725}
\DeclareTextGlyphY{LinLibertine_R}{uni1E2E}{7726}
\DeclareTextGlyphY{LinLibertine_R}{uni1E2F}{7727}
\DeclareTextGlyphY{LinLibertine_R}{uni1E30}{7728}
\DeclareTextGlyphY{LinLibertine_R}{uni1E31}{7729}
\DeclareTextGlyphY{LinLibertine_R}{uni1E32}{7730}
\DeclareTextGlyphY{LinLibertine_R}{uni1E33}{7731}
\DeclareTextGlyphY{LinLibertine_R}{uni1E34}{7732}
\DeclareTextGlyphY{LinLibertine_R}{uni1E35}{7733}
\DeclareTextGlyphY{LinLibertine_R}{uni1E36}{7734}
\DeclareTextGlyphY{LinLibertine_R}{uni1E37}{7735}
\DeclareTextGlyphY{LinLibertine_R}{uni1E38}{7736}
\DeclareTextGlyphY{LinLibertine_R}{uni1E39}{7737}
\DeclareTextGlyphY{LinLibertine_R}{uni1E3A}{7738}
\DeclareTextGlyphY{LinLibertine_R}{uni1E3B}{7739}
\DeclareTextGlyphY{LinLibertine_R}{uni1E3C}{7740}
\DeclareTextGlyphY{LinLibertine_R}{uni1E3D}{7741}
\DeclareTextGlyphY{LinLibertine_R}{uni1E3E}{7742}
\DeclareTextGlyphY{LinLibertine_R}{uni1E3F}{7743}
\DeclareTextGlyphY{LinLibertine_R}{uni1E40}{7744}
\DeclareTextGlyphY{LinLibertine_R}{uni1E41}{7745}
\DeclareTextGlyphY{LinLibertine_R}{uni1E42}{7746}
\DeclareTextGlyphY{LinLibertine_R}{uni1E43}{7747}
\DeclareTextGlyphY{LinLibertine_R}{uni1E44}{7748}
\DeclareTextGlyphY{LinLibertine_R}{uni1E45}{7749}
\DeclareTextGlyphY{LinLibertine_R}{uni1E46}{7750}
\DeclareTextGlyphY{LinLibertine_R}{uni1E47}{7751}
\DeclareTextGlyphY{LinLibertine_R}{uni1E48}{7752}
\DeclareTextGlyphY{LinLibertine_R}{uni1E49}{7753}
\DeclareTextGlyphY{LinLibertine_R}{uni1E4A}{7754}
\DeclareTextGlyphY{LinLibertine_R}{uni1E4B}{7755}
\DeclareTextGlyphY{LinLibertine_R}{uni1E4C}{7756}
\DeclareTextGlyphY{LinLibertine_R}{uni1E4D}{7757}
\DeclareTextGlyphY{LinLibertine_R}{uni1E4E}{7758}
\DeclareTextGlyphY{LinLibertine_R}{uni1E4F}{7759}
\DeclareTextGlyphY{LinLibertine_R}{uni1E50}{7760}
\DeclareTextGlyphY{LinLibertine_R}{uni1E51}{7761}
\DeclareTextGlyphY{LinLibertine_R}{uni1E52}{7762}
\DeclareTextGlyphY{LinLibertine_R}{uni1E53}{7763}
\DeclareTextGlyphY{LinLibertine_R}{uni1E54}{7764}
\DeclareTextGlyphY{LinLibertine_R}{uni1E55}{7765}
\DeclareTextGlyphY{LinLibertine_R}{uni1E56}{7766}
\DeclareTextGlyphY{LinLibertine_R}{uni1E57}{7767}
\DeclareTextGlyphY{LinLibertine_R}{uni1E58}{7768}
\DeclareTextGlyphY{LinLibertine_R}{uni1E59}{7769}
\DeclareTextGlyphY{LinLibertine_R}{uni1E5A}{7770}
\DeclareTextGlyphY{LinLibertine_R}{uni1E5B}{7771}
\DeclareTextGlyphY{LinLibertine_R}{uni1E5C}{7772}
\DeclareTextGlyphY{LinLibertine_R}{uni1E5D}{7773}
\DeclareTextGlyphY{LinLibertine_R}{uni1E5E}{7774}
\DeclareTextGlyphY{LinLibertine_R}{uni1E5F}{7775}
\DeclareTextGlyphY{LinLibertine_R}{uni1E60}{7776}
\DeclareTextGlyphY{LinLibertine_R}{uni1E61}{7777}
\DeclareTextGlyphY{LinLibertine_R}{uni1E62}{7778}
\DeclareTextGlyphY{LinLibertine_R}{uni1E63}{7779}
\DeclareTextGlyphY{LinLibertine_R}{uni1E64}{7780}
\DeclareTextGlyphY{LinLibertine_R}{uni1E65}{7781}
\DeclareTextGlyphY{LinLibertine_R}{uni1E66}{7782}
\DeclareTextGlyphY{LinLibertine_R}{uni1E67}{7783}
\DeclareTextGlyphY{LinLibertine_R}{uni1E68}{7784}
\DeclareTextGlyphY{LinLibertine_R}{uni1E69}{7785}
\DeclareTextGlyphY{LinLibertine_R}{uni1E6A}{7786}
\DeclareTextGlyphY{LinLibertine_R}{uni1E6B}{7787}
\DeclareTextGlyphY{LinLibertine_R}{uni1E6C}{7788}
\DeclareTextGlyphY{LinLibertine_R}{uni1E6D}{7789}
\DeclareTextGlyphY{LinLibertine_R}{uni1E6E}{7790}
\DeclareTextGlyphY{LinLibertine_R}{uni1E6F}{7791}
\DeclareTextGlyphY{LinLibertine_R}{uni1E70}{7792}
\DeclareTextGlyphY{LinLibertine_R}{uni1E71}{7793}
\DeclareTextGlyphY{LinLibertine_R}{uni1E72}{7794}
\DeclareTextGlyphY{LinLibertine_R}{uni1E73}{7795}
\DeclareTextGlyphY{LinLibertine_R}{uni1E74}{7796}
\DeclareTextGlyphY{LinLibertine_R}{uni1E75}{7797}
\DeclareTextGlyphY{LinLibertine_R}{uni1E76}{7798}
\DeclareTextGlyphY{LinLibertine_R}{uni1E77}{7799}
\DeclareTextGlyphY{LinLibertine_R}{uni1E78}{7800}
\DeclareTextGlyphY{LinLibertine_R}{uni1E79}{7801}
\DeclareTextGlyphY{LinLibertine_R}{uni1E7A}{7802}
\DeclareTextGlyphY{LinLibertine_R}{uni1E7B}{7803}
\DeclareTextGlyphY{LinLibertine_R}{uni1E7C}{7804}
\DeclareTextGlyphY{LinLibertine_R}{uni1E7D}{7805}
\DeclareTextGlyphY{LinLibertine_R}{uni1E7E}{7806}
\DeclareTextGlyphY{LinLibertine_R}{uni1E7F}{7807}
\DeclareTextGlyphY{LinLibertine_R}{Wgrave}{7808}
\DeclareTextGlyphY{LinLibertine_R}{uni1E80}{7808}
\DeclareTextGlyphY{LinLibertine_R}{wgrave}{7809}
\DeclareTextGlyphY{LinLibertine_R}{uni1E81}{7809}
\DeclareTextGlyphY{LinLibertine_R}{Wacute}{7810}
\DeclareTextGlyphY{LinLibertine_R}{uni1E82}{7810}
\DeclareTextGlyphY{LinLibertine_R}{wacute}{7811}
\DeclareTextGlyphY{LinLibertine_R}{uni1E83}{7811}
\DeclareTextGlyphY{LinLibertine_R}{Wdieresis}{7812}
\DeclareTextGlyphY{LinLibertine_R}{uni1E84}{7812}
\DeclareTextGlyphY{LinLibertine_R}{wdieresis}{7813}
\DeclareTextGlyphY{LinLibertine_R}{uni1E85}{7813}
\DeclareTextGlyphY{LinLibertine_R}{uni1E86}{7814}
\DeclareTextGlyphY{LinLibertine_R}{uni1E87}{7815}
\DeclareTextGlyphY{LinLibertine_R}{uni1E88}{7816}
\DeclareTextGlyphY{LinLibertine_R}{uni1E89}{7817}
\DeclareTextGlyphY{LinLibertine_R}{uni1E8A}{7818}
\DeclareTextGlyphY{LinLibertine_R}{uni1E8B}{7819}
\DeclareTextGlyphY{LinLibertine_R}{uni1E8C}{7820}
\DeclareTextGlyphY{LinLibertine_R}{uni1E8D}{7821}
\DeclareTextGlyphY{LinLibertine_R}{uni1E8E}{7822}
\DeclareTextGlyphY{LinLibertine_R}{uni1E8F}{7823}
\DeclareTextGlyphY{LinLibertine_R}{uni1E90}{7824}
\DeclareTextGlyphY{LinLibertine_R}{uni1E91}{7825}
\DeclareTextGlyphY{LinLibertine_R}{uni1E92}{7826}
\DeclareTextGlyphY{LinLibertine_R}{uni1E93}{7827}
\DeclareTextGlyphY{LinLibertine_R}{uni1E94}{7828}
\DeclareTextGlyphY{LinLibertine_R}{uni1E95}{7829}
\DeclareTextGlyphY{LinLibertine_R}{uni1E96}{7830}
\DeclareTextGlyphY{LinLibertine_R}{uni1E97}{7831}
\DeclareTextGlyphY{LinLibertine_R}{uni1E98}{7832}
\DeclareTextGlyphY{LinLibertine_R}{uni1E99}{7833}
\DeclareTextGlyphY{LinLibertine_R}{uni1E9A}{7834}
\DeclareTextGlyphY{LinLibertine_R}{uni1E9B}{7835}
\DeclareTextGlyphY{LinLibertine_R}{uni1E9C}{7836}
\DeclareTextGlyphY{LinLibertine_R}{uni1E9D}{7837}
\DeclareTextGlyphY{LinLibertine_R}{Germandbls}{7838}
\DeclareTextGlyphY{LinLibertine_R}{uni1E9E}{7838}
\DeclareTextGlyphY{LinLibertine_R}{uni1E9F}{7839}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA0}{7840}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA1}{7841}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA2}{7842}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA3}{7843}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA4}{7844}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA5}{7845}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA6}{7846}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA7}{7847}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA8}{7848}
\DeclareTextGlyphY{LinLibertine_R}{uni1EA9}{7849}
\DeclareTextGlyphY{LinLibertine_R}{uni1EAA}{7850}
\DeclareTextGlyphY{LinLibertine_R}{uni1EAB}{7851}
\DeclareTextGlyphY{LinLibertine_R}{uni1EAC}{7852}
\DeclareTextGlyphY{LinLibertine_R}{uni1EAD}{7853}
\DeclareTextGlyphY{LinLibertine_R}{uni1EAE}{7854}
\DeclareTextGlyphY{LinLibertine_R}{uni1EAF}{7855}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB0}{7856}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB1}{7857}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB2}{7858}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB3}{7859}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB4}{7860}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB5}{7861}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB6}{7862}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB7}{7863}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB8}{7864}
\DeclareTextGlyphY{LinLibertine_R}{uni1EB9}{7865}
\DeclareTextGlyphY{LinLibertine_R}{uni1EBA}{7866}
\DeclareTextGlyphY{LinLibertine_R}{uni1EBB}{7867}
\DeclareTextGlyphY{LinLibertine_R}{uni1EBC}{7868}
\DeclareTextGlyphY{LinLibertine_R}{uni1EBD}{7869}
\DeclareTextGlyphY{LinLibertine_R}{uni1EBE}{7870}
\DeclareTextGlyphY{LinLibertine_R}{uni1EBF}{7871}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC0}{7872}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC1}{7873}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC2}{7874}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC3}{7875}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC4}{7876}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC5}{7877}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC6}{7878}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC7}{7879}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC8}{7880}
\DeclareTextGlyphY{LinLibertine_R}{uni1EC9}{7881}
\DeclareTextGlyphY{LinLibertine_R}{uni1ECA}{7882}
\DeclareTextGlyphY{LinLibertine_R}{uni1ECB}{7883}
\DeclareTextGlyphY{LinLibertine_R}{uni1ECC}{7884}
\DeclareTextGlyphY{LinLibertine_R}{uni1ECD}{7885}
\DeclareTextGlyphY{LinLibertine_R}{uni1ECE}{7886}
\DeclareTextGlyphY{LinLibertine_R}{uni1ECF}{7887}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED0}{7888}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED1}{7889}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED2}{7890}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED3}{7891}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED4}{7892}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED5}{7893}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED6}{7894}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED7}{7895}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED8}{7896}
\DeclareTextGlyphY{LinLibertine_R}{uni1ED9}{7897}
\DeclareTextGlyphY{LinLibertine_R}{uni1EDA}{7898}
\DeclareTextGlyphY{LinLibertine_R}{uni1EDB}{7899}
\DeclareTextGlyphY{LinLibertine_R}{uni1EDC}{7900}
\DeclareTextGlyphY{LinLibertine_R}{uni1EDD}{7901}
\DeclareTextGlyphY{LinLibertine_R}{uni1EDE}{7902}
\DeclareTextGlyphY{LinLibertine_R}{uni1EDF}{7903}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE0}{7904}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE1}{7905}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE2}{7906}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE3}{7907}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE4}{7908}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE5}{7909}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE6}{7910}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE7}{7911}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE8}{7912}
\DeclareTextGlyphY{LinLibertine_R}{uni1EE9}{7913}
\DeclareTextGlyphY{LinLibertine_R}{uni1EEA}{7914}
\DeclareTextGlyphY{LinLibertine_R}{uni1EEB}{7915}
\DeclareTextGlyphY{LinLibertine_R}{uni1EEC}{7916}
\DeclareTextGlyphY{LinLibertine_R}{uni1EED}{7917}
\DeclareTextGlyphY{LinLibertine_R}{uni1EEE}{7918}
\DeclareTextGlyphY{LinLibertine_R}{uni1EEF}{7919}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF0}{7920}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF1}{7921}
\DeclareTextGlyphY{LinLibertine_R}{Ygrave}{7922}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF2}{7922}
\DeclareTextGlyphY{LinLibertine_R}{ygrave}{7923}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF3}{7923}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF4}{7924}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF5}{7925}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF6}{7926}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF7}{7927}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF8}{7928}
\DeclareTextGlyphY{LinLibertine_R}{uni1EF9}{7929}
\DeclareTextGlyphY{LinLibertine_R}{uni1EFA}{7930}
\DeclareTextGlyphY{LinLibertine_R}{uni1EFB}{7931}
\DeclareTextGlyphY{LinLibertine_R}{uni1EFC}{7932}
\DeclareTextGlyphY{LinLibertine_R}{uni1EFD}{7933}
\DeclareTextGlyphY{LinLibertine_R}{uni1EFE}{7934}
\DeclareTextGlyphY{LinLibertine_R}{uni1EFF}{7935}
\DeclareTextGlyphY{LinLibertine_R}{uni1F00}{7936}
\DeclareTextGlyphY{LinLibertine_R}{uni1F01}{7937}
\DeclareTextGlyphY{LinLibertine_R}{uni1F02}{7938}
\DeclareTextGlyphY{LinLibertine_R}{uni1F03}{7939}
\DeclareTextGlyphY{LinLibertine_R}{uni1F04}{7940}
\DeclareTextGlyphY{LinLibertine_R}{uni1F05}{7941}
\DeclareTextGlyphY{LinLibertine_R}{uni1F06}{7942}
\DeclareTextGlyphY{LinLibertine_R}{uni1F07}{7943}
\DeclareTextGlyphY{LinLibertine_R}{uni1F08}{7944}
\DeclareTextGlyphY{LinLibertine_R}{uni1F09}{7945}
\DeclareTextGlyphY{LinLibertine_R}{uni1F0A}{7946}
\DeclareTextGlyphY{LinLibertine_R}{uni1F0B}{7947}
\DeclareTextGlyphY{LinLibertine_R}{uni1F0C}{7948}
\DeclareTextGlyphY{LinLibertine_R}{uni1F0D}{7949}
\DeclareTextGlyphY{LinLibertine_R}{uni1F0E}{7950}
\DeclareTextGlyphY{LinLibertine_R}{uni1F0F}{7951}
\DeclareTextGlyphY{LinLibertine_R}{uni1F10}{7952}
\DeclareTextGlyphY{LinLibertine_R}{uni1F11}{7953}
\DeclareTextGlyphY{LinLibertine_R}{uni1F12}{7954}
\DeclareTextGlyphY{LinLibertine_R}{uni1F13}{7955}
\DeclareTextGlyphY{LinLibertine_R}{uni1F14}{7956}
\DeclareTextGlyphY{LinLibertine_R}{uni1F15}{7957}
\DeclareTextGlyphY{LinLibertine_R}{uni1F18}{7960}
\DeclareTextGlyphY{LinLibertine_R}{uni1F19}{7961}
\DeclareTextGlyphY{LinLibertine_R}{uni1F1A}{7962}
\DeclareTextGlyphY{LinLibertine_R}{uni1F1B}{7963}
\DeclareTextGlyphY{LinLibertine_R}{uni1F1C}{7964}
\DeclareTextGlyphY{LinLibertine_R}{uni1F1D}{7965}
\DeclareTextGlyphY{LinLibertine_R}{uni1F20}{7968}
\DeclareTextGlyphY{LinLibertine_R}{uni1F21}{7969}
\DeclareTextGlyphY{LinLibertine_R}{uni1F22}{7970}
\DeclareTextGlyphY{LinLibertine_R}{uni1F23}{7971}
\DeclareTextGlyphY{LinLibertine_R}{uni1F24}{7972}
\DeclareTextGlyphY{LinLibertine_R}{uni1F25}{7973}
\DeclareTextGlyphY{LinLibertine_R}{uni1F26}{7974}
\DeclareTextGlyphY{LinLibertine_R}{uni1F27}{7975}
\DeclareTextGlyphY{LinLibertine_R}{uni1F28}{7976}
\DeclareTextGlyphY{LinLibertine_R}{uni1F29}{7977}
\DeclareTextGlyphY{LinLibertine_R}{uni1F2A}{7978}
\DeclareTextGlyphY{LinLibertine_R}{uni1F2B}{7979}
\DeclareTextGlyphY{LinLibertine_R}{uni1F2C}{7980}
\DeclareTextGlyphY{LinLibertine_R}{uni1F2D}{7981}
\DeclareTextGlyphY{LinLibertine_R}{uni1F2E}{7982}
\DeclareTextGlyphY{LinLibertine_R}{uni1F2F}{7983}
\DeclareTextGlyphY{LinLibertine_R}{uni1F30}{7984}
\DeclareTextGlyphY{LinLibertine_R}{uni1F31}{7985}
\DeclareTextGlyphY{LinLibertine_R}{uni1F32}{7986}
\DeclareTextGlyphY{LinLibertine_R}{uni1F33}{7987}
\DeclareTextGlyphY{LinLibertine_R}{uni1F34}{7988}
\DeclareTextGlyphY{LinLibertine_R}{uni1F35}{7989}
\DeclareTextGlyphY{LinLibertine_R}{uni1F36}{7990}
\DeclareTextGlyphY{LinLibertine_R}{uni1F37}{7991}
\DeclareTextGlyphY{LinLibertine_R}{uni1F38}{7992}
\DeclareTextGlyphY{LinLibertine_R}{uni1F39}{7993}
\DeclareTextGlyphY{LinLibertine_R}{uni1F3A}{7994}
\DeclareTextGlyphY{LinLibertine_R}{uni1F3B}{7995}
\DeclareTextGlyphY{LinLibertine_R}{uni1F3C}{7996}
\DeclareTextGlyphY{LinLibertine_R}{uni1F3D}{7997}
\DeclareTextGlyphY{LinLibertine_R}{uni1F3E}{7998}
\DeclareTextGlyphY{LinLibertine_R}{uni1F3F}{7999}
\DeclareTextGlyphY{LinLibertine_R}{uni1F40}{8000}
\DeclareTextGlyphY{LinLibertine_R}{uni1F41}{8001}
\DeclareTextGlyphY{LinLibertine_R}{uni1F42}{8002}
\DeclareTextGlyphY{LinLibertine_R}{uni1F43}{8003}
\DeclareTextGlyphY{LinLibertine_R}{uni1F44}{8004}
\DeclareTextGlyphY{LinLibertine_R}{uni1F45}{8005}
\DeclareTextGlyphY{LinLibertine_R}{uni1F48}{8008}
\DeclareTextGlyphY{LinLibertine_R}{uni1F49}{8009}
\DeclareTextGlyphY{LinLibertine_R}{uni1F4A}{8010}
\DeclareTextGlyphY{LinLibertine_R}{uni1F4B}{8011}
\DeclareTextGlyphY{LinLibertine_R}{uni1F4C}{8012}
\DeclareTextGlyphY{LinLibertine_R}{uni1F4D}{8013}
\DeclareTextGlyphY{LinLibertine_R}{uni1F50}{8016}
\DeclareTextGlyphY{LinLibertine_R}{uni1F51}{8017}
\DeclareTextGlyphY{LinLibertine_R}{uni1F52}{8018}
\DeclareTextGlyphY{LinLibertine_R}{uni1F53}{8019}
\DeclareTextGlyphY{LinLibertine_R}{uni1F54}{8020}
\DeclareTextGlyphY{LinLibertine_R}{uni1F55}{8021}
\DeclareTextGlyphY{LinLibertine_R}{uni1F56}{8022}
\DeclareTextGlyphY{LinLibertine_R}{uni1F57}{8023}
\DeclareTextGlyphY{LinLibertine_R}{uni1F59}{8025}
\DeclareTextGlyphY{LinLibertine_R}{uni1F5B}{8027}
\DeclareTextGlyphY{LinLibertine_R}{uni1F5D}{8029}
\DeclareTextGlyphY{LinLibertine_R}{uni1F5F}{8031}
\DeclareTextGlyphY{LinLibertine_R}{uni1F60}{8032}
\DeclareTextGlyphY{LinLibertine_R}{uni1F61}{8033}
\DeclareTextGlyphY{LinLibertine_R}{uni1F62}{8034}
\DeclareTextGlyphY{LinLibertine_R}{uni1F63}{8035}
\DeclareTextGlyphY{LinLibertine_R}{uni1F64}{8036}
\DeclareTextGlyphY{LinLibertine_R}{uni1F65}{8037}
\DeclareTextGlyphY{LinLibertine_R}{uni1F66}{8038}
\DeclareTextGlyphY{LinLibertine_R}{uni1F67}{8039}
\DeclareTextGlyphY{LinLibertine_R}{uni1F68}{8040}
\DeclareTextGlyphY{LinLibertine_R}{uni1F69}{8041}
\DeclareTextGlyphY{LinLibertine_R}{uni1F6A}{8042}
\DeclareTextGlyphY{LinLibertine_R}{uni1F6B}{8043}
\DeclareTextGlyphY{LinLibertine_R}{uni1F6C}{8044}
\DeclareTextGlyphY{LinLibertine_R}{uni1F6D}{8045}
\DeclareTextGlyphY{LinLibertine_R}{uni1F6E}{8046}
\DeclareTextGlyphY{LinLibertine_R}{uni1F6F}{8047}
\DeclareTextGlyphY{LinLibertine_R}{uni1F70}{8048}
\DeclareTextGlyphY{LinLibertine_R}{uni1F71}{8049}
\DeclareTextGlyphY{LinLibertine_R}{uni1F72}{8050}
\DeclareTextGlyphY{LinLibertine_R}{uni1F73}{8051}
\DeclareTextGlyphY{LinLibertine_R}{uni1F74}{8052}
\DeclareTextGlyphY{LinLibertine_R}{uni1F75}{8053}
\DeclareTextGlyphY{LinLibertine_R}{uni1F76}{8054}
\DeclareTextGlyphY{LinLibertine_R}{uni1F77}{8055}
\DeclareTextGlyphY{LinLibertine_R}{uni1F78}{8056}
\DeclareTextGlyphY{LinLibertine_R}{uni1F79}{8057}
\DeclareTextGlyphY{LinLibertine_R}{uni1F7A}{8058}
\DeclareTextGlyphY{LinLibertine_R}{uni1F7B}{8059}
\DeclareTextGlyphY{LinLibertine_R}{uni1F7C}{8060}
\DeclareTextGlyphY{LinLibertine_R}{uni1F7D}{8061}
\DeclareTextGlyphY{LinLibertine_R}{uni1F80}{8064}
\DeclareTextGlyphY{LinLibertine_R}{uni1F81}{8065}
\DeclareTextGlyphY{LinLibertine_R}{uni1F82}{8066}
\DeclareTextGlyphY{LinLibertine_R}{uni1F83}{8067}
\DeclareTextGlyphY{LinLibertine_R}{uni1F84}{8068}
\DeclareTextGlyphY{LinLibertine_R}{uni1F85}{8069}
\DeclareTextGlyphY{LinLibertine_R}{uni1F86}{8070}
\DeclareTextGlyphY{LinLibertine_R}{uni1F87}{8071}
\DeclareTextGlyphY{LinLibertine_R}{uni1F88}{8072}
\DeclareTextGlyphY{LinLibertine_R}{uni1F89}{8073}
\DeclareTextGlyphY{LinLibertine_R}{uni1F8A}{8074}
\DeclareTextGlyphY{LinLibertine_R}{uni1F8B}{8075}
\DeclareTextGlyphY{LinLibertine_R}{uni1F8C}{8076}
\DeclareTextGlyphY{LinLibertine_R}{uni1F8D}{8077}
\DeclareTextGlyphY{LinLibertine_R}{uni1F8E}{8078}
\DeclareTextGlyphY{LinLibertine_R}{uni1F8F}{8079}
\DeclareTextGlyphY{LinLibertine_R}{uni1F90}{8080}
\DeclareTextGlyphY{LinLibertine_R}{uni1F91}{8081}
\DeclareTextGlyphY{LinLibertine_R}{uni1F92}{8082}
\DeclareTextGlyphY{LinLibertine_R}{uni1F93}{8083}
\DeclareTextGlyphY{LinLibertine_R}{uni1F94}{8084}
\DeclareTextGlyphY{LinLibertine_R}{uni1F95}{8085}
\DeclareTextGlyphY{LinLibertine_R}{uni1F96}{8086}
\DeclareTextGlyphY{LinLibertine_R}{uni1F97}{8087}
\DeclareTextGlyphY{LinLibertine_R}{uni1F98}{8088}
\DeclareTextGlyphY{LinLibertine_R}{uni1F99}{8089}
\DeclareTextGlyphY{LinLibertine_R}{uni1F9A}{8090}
\DeclareTextGlyphY{LinLibertine_R}{uni1F9B}{8091}
\DeclareTextGlyphY{LinLibertine_R}{uni1F9C}{8092}
\DeclareTextGlyphY{LinLibertine_R}{uni1F9D}{8093}
\DeclareTextGlyphY{LinLibertine_R}{uni1F9E}{8094}
\DeclareTextGlyphY{LinLibertine_R}{uni1F9F}{8095}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA0}{8096}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA1}{8097}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA2}{8098}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA3}{8099}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA4}{8100}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA5}{8101}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA6}{8102}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA7}{8103}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA8}{8104}
\DeclareTextGlyphY{LinLibertine_R}{uni1FA9}{8105}
\DeclareTextGlyphY{LinLibertine_R}{uni1FAA}{8106}
\DeclareTextGlyphY{LinLibertine_R}{uni1FAB}{8107}
\DeclareTextGlyphY{LinLibertine_R}{uni1FAC}{8108}
\DeclareTextGlyphY{LinLibertine_R}{uni1FAD}{8109}
\DeclareTextGlyphY{LinLibertine_R}{uni1FAE}{8110}
\DeclareTextGlyphY{LinLibertine_R}{uni1FAF}{8111}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB0}{8112}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB1}{8113}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB2}{8114}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB3}{8115}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB4}{8116}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB6}{8118}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB7}{8119}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB8}{8120}
\DeclareTextGlyphY{LinLibertine_R}{uni1FB9}{8121}
\DeclareTextGlyphY{LinLibertine_R}{uni1FBA}{8122}
\DeclareTextGlyphY{LinLibertine_R}{uni1FBB}{8123}
\DeclareTextGlyphY{LinLibertine_R}{uni1FBC}{8124}
\DeclareTextGlyphY{LinLibertine_R}{uni1FBD}{8125}
\DeclareTextGlyphY{LinLibertine_R}{uni1FBE}{8126}
\DeclareTextGlyphY{LinLibertine_R}{uni1FBF}{8127}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC0}{8128}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC1}{8129}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC2}{8130}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC3}{8131}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC4}{8132}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC6}{8134}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC7}{8135}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC8}{8136}
\DeclareTextGlyphY{LinLibertine_R}{uni1FC9}{8137}
\DeclareTextGlyphY{LinLibertine_R}{uni1FCA}{8138}
\DeclareTextGlyphY{LinLibertine_R}{uni1FCB}{8139}
\DeclareTextGlyphY{LinLibertine_R}{uni1FCC}{8140}
\DeclareTextGlyphY{LinLibertine_R}{uni1FCD}{8141}
\DeclareTextGlyphY{LinLibertine_R}{uni1FCE}{8142}
\DeclareTextGlyphY{LinLibertine_R}{uni1FCF}{8143}
\DeclareTextGlyphY{LinLibertine_R}{uni1FD0}{8144}
\DeclareTextGlyphY{LinLibertine_R}{uni1FD1}{8145}
\DeclareTextGlyphY{LinLibertine_R}{uni1FD2}{8146}
\DeclareTextGlyphY{LinLibertine_R}{uni1FD3}{8147}
\DeclareTextGlyphY{LinLibertine_R}{uni1FD6}{8150}
\DeclareTextGlyphY{LinLibertine_R}{uni1FD7}{8151}
\DeclareTextGlyphY{LinLibertine_R}{uni1FD8}{8152}
\DeclareTextGlyphY{LinLibertine_R}{uni1FD9}{8153}
\DeclareTextGlyphY{LinLibertine_R}{uni1FDA}{8154}
\DeclareTextGlyphY{LinLibertine_R}{uni1FDB}{8155}
\DeclareTextGlyphY{LinLibertine_R}{uni1FDD}{8157}
\DeclareTextGlyphY{LinLibertine_R}{uni1FDE}{8158}
\DeclareTextGlyphY{LinLibertine_R}{uni1FDF}{8159}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE0}{8160}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE1}{8161}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE2}{8162}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE3}{8163}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE4}{8164}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE5}{8165}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE6}{8166}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE7}{8167}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE8}{8168}
\DeclareTextGlyphY{LinLibertine_R}{uni1FE9}{8169}
\DeclareTextGlyphY{LinLibertine_R}{uni1FEA}{8170}
\DeclareTextGlyphY{LinLibertine_R}{uni1FEB}{8171}
\DeclareTextGlyphY{LinLibertine_R}{uni1FEC}{8172}
\DeclareTextGlyphY{LinLibertine_R}{uni1FED}{8173}
\DeclareTextGlyphY{LinLibertine_R}{uni1FEE}{8174}
\DeclareTextGlyphY{LinLibertine_R}{uni1FEF}{8175}
\DeclareTextGlyphY{LinLibertine_R}{uni1FF2}{8178}
\DeclareTextGlyphY{LinLibertine_R}{uni1FF3}{8179}
\DeclareTextGlyphY{LinLibertine_R}{uni1FF4}{8180}
\DeclareTextGlyphY{LinLibertine_R}{uni1FF6}{8182}
\DeclareTextGlyphY{LinLibertine_R}{uni1FF7}{8183}
\DeclareTextGlyphY{LinLibertine_R}{uni1FF8}{8184}
\DeclareTextGlyphY{LinLibertine_R}{uni1FF9}{8185}
\DeclareTextGlyphY{LinLibertine_R}{uni1FFA}{8186}
\DeclareTextGlyphY{LinLibertine_R}{uni1FFB}{8187}
\DeclareTextGlyphY{LinLibertine_R}{uni1FFC}{8188}
\DeclareTextGlyphY{LinLibertine_R}{uni1FFD}{8189}
\DeclareTextGlyphY{LinLibertine_R}{uni1FFE}{8190}
\DeclareTextGlyphY{LinLibertine_R}{enquad}{8192}
\DeclareTextGlyphY{LinLibertine_R}{uni2000}{8192}
\DeclareTextGlyphY{LinLibertine_R}{emquad}{8193}
\DeclareTextGlyphY{LinLibertine_R}{uni2001}{8193}
\DeclareTextGlyphY{LinLibertine_R}{enspace}{8194}
\DeclareTextGlyphY{LinLibertine_R}{uni2002}{8194}
\DeclareTextGlyphY{LinLibertine_R}{emspace}{8195}
\DeclareTextGlyphY{LinLibertine_R}{uni2003}{8195}
\DeclareTextGlyphY{LinLibertine_R}{threeperemspace}{8196}
\DeclareTextGlyphY{LinLibertine_R}{uni2004}{8196}
\DeclareTextGlyphY{LinLibertine_R}{fourperemspace}{8197}
\DeclareTextGlyphY{LinLibertine_R}{uni2005}{8197}
\DeclareTextGlyphY{LinLibertine_R}{sixperemspace}{8198}
\DeclareTextGlyphY{LinLibertine_R}{uni2006}{8198}
\DeclareTextGlyphY{LinLibertine_R}{figurespace}{8199}
\DeclareTextGlyphY{LinLibertine_R}{uni2007}{8199}
\DeclareTextGlyphY{LinLibertine_R}{punctuationspace}{8200}
\DeclareTextGlyphY{LinLibertine_R}{uni2008}{8200}
\DeclareTextGlyphY{LinLibertine_R}{thinspace}{8201}
\DeclareTextGlyphY{LinLibertine_R}{uni2009}{8201}
\DeclareTextGlyphY{LinLibertine_R}{hairspace}{8202}
\DeclareTextGlyphY{LinLibertine_R}{uni200A}{8202}
\DeclareTextGlyphY{LinLibertine_R}{zerowidthspace}{8203}
\DeclareTextGlyphY{LinLibertine_R}{uni200B}{8203}
\DeclareTextGlyphY{LinLibertine_R}{hyphentwo}{8208}
\DeclareTextGlyphY{LinLibertine_R}{uni2010}{8208}
\DeclareTextGlyphY{LinLibertine_R}{hyphennobreak}{8209}
\DeclareTextGlyphY{LinLibertine_R}{uni2011}{8209}
\DeclareTextGlyphY{LinLibertine_R}{figuredash}{8210}
\DeclareTextGlyphY{LinLibertine_R}{uni2012}{8210}
\DeclareTextGlyphY{LinLibertine_R}{endash}{8211}
\DeclareTextGlyphY{LinLibertine_R}{uni2013}{8211}
\DeclareTextGlyphY{LinLibertine_R}{emdash}{8212}
\DeclareTextGlyphY{LinLibertine_R}{uni2014}{8212}
\DeclareTextGlyphY{LinLibertine_R}{horizontalbar}{8213}
\DeclareTextGlyphY{LinLibertine_R}{uni2015}{8213}
\DeclareTextGlyphY{LinLibertine_R}{uni2016}{8214}
\DeclareTextGlyphY{LinLibertine_R}{underscoredbl}{8215}
\DeclareTextGlyphY{LinLibertine_R}{uni2017}{8215}
\DeclareTextGlyphY{LinLibertine_R}{quoteleft}{8216}
\DeclareTextGlyphY{LinLibertine_R}{uni2018}{8216}
\DeclareTextGlyphY{LinLibertine_R}{quoteright}{8217}
\DeclareTextGlyphY{LinLibertine_R}{uni2019}{8217}
\DeclareTextGlyphY{LinLibertine_R}{quotesinglbase}{8218}
\DeclareTextGlyphY{LinLibertine_R}{uni201A}{8218}
\DeclareTextGlyphY{LinLibertine_R}{quotereversed}{8219}
\DeclareTextGlyphY{LinLibertine_R}{uni201B}{8219}
\DeclareTextGlyphY{LinLibertine_R}{quotedblleft}{8220}
\DeclareTextGlyphY{LinLibertine_R}{uni201C}{8220}
\DeclareTextGlyphY{LinLibertine_R}{quotedblright}{8221}
\DeclareTextGlyphY{LinLibertine_R}{uni201D}{8221}
\DeclareTextGlyphY{LinLibertine_R}{quotedblbase}{8222}
\DeclareTextGlyphY{LinLibertine_R}{uni201E}{8222}
\DeclareTextGlyphY{LinLibertine_R}{quotedblrev}{8223}
\DeclareTextGlyphY{LinLibertine_R}{uni201F}{8223}
\DeclareTextGlyphY{LinLibertine_R}{dagger}{8224}
\DeclareTextGlyphY{LinLibertine_R}{uni2020}{8224}
\DeclareTextGlyphY{LinLibertine_R}{daggerdbl}{8225}
\DeclareTextGlyphY{LinLibertine_R}{uni2021}{8225}
\DeclareTextGlyphY{LinLibertine_R}{bullet}{8226}
\DeclareTextGlyphY{LinLibertine_R}{uni2022}{8226}
\DeclareTextGlyphY{LinLibertine_R}{trianglebullet}{8227}
\DeclareTextGlyphY{LinLibertine_R}{uni2023}{8227}
\DeclareTextGlyphY{LinLibertine_R}{onedotenleader}{8228}
\DeclareTextGlyphY{LinLibertine_R}{uni2024}{8228}
\DeclareTextGlyphY{LinLibertine_R}{twodotenleader}{8229}
\DeclareTextGlyphY{LinLibertine_R}{uni2025}{8229}
\DeclareTextGlyphY{LinLibertine_R}{ellipsis}{8230}
\DeclareTextGlyphY{LinLibertine_R}{uni2026}{8230}
\DeclareTextGlyphY{LinLibertine_R}{hyphendot}{8231}
\DeclareTextGlyphY{LinLibertine_R}{uni2027}{8231}
\DeclareTextGlyphY{LinLibertine_R}{uni202F}{8239}
\DeclareTextGlyphY{LinLibertine_R}{perthousand}{8240}
\DeclareTextGlyphY{LinLibertine_R}{uni2030}{8240}
\DeclareTextGlyphY{LinLibertine_R}{pertenthousand}{8241}
\DeclareTextGlyphY{LinLibertine_R}{uni2031}{8241}
\DeclareTextGlyphY{LinLibertine_R}{minute}{8242}
\DeclareTextGlyphY{LinLibertine_R}{uni2032}{8242}
\DeclareTextGlyphY{LinLibertine_R}{second}{8243}
\DeclareTextGlyphY{LinLibertine_R}{uni2033}{8243}
\DeclareTextGlyphY{LinLibertine_R}{primetriple}{8244}
\DeclareTextGlyphY{LinLibertine_R}{uni2034}{8244}
\DeclareTextGlyphY{LinLibertine_R}{primereversed}{8245}
\DeclareTextGlyphY{LinLibertine_R}{uni2035}{8245}
\DeclareTextGlyphY{LinLibertine_R}{uni2036}{8246}
\DeclareTextGlyphY{LinLibertine_R}{uni2037}{8247}
\DeclareTextGlyphY{LinLibertine_R}{guilsinglleft}{8249}
\DeclareTextGlyphY{LinLibertine_R}{uni2039}{8249}
\DeclareTextGlyphY{LinLibertine_R}{guilsinglright}{8250}
\DeclareTextGlyphY{LinLibertine_R}{uni203A}{8250}
\DeclareTextGlyphY{LinLibertine_R}{uni203B}{8251}
\DeclareTextGlyphY{LinLibertine_R}{exclamdbl}{8252}
\DeclareTextGlyphY{LinLibertine_R}{uni203C}{8252}
\DeclareTextGlyphY{LinLibertine_R}{interrobang}{8253}
\DeclareTextGlyphY{LinLibertine_R}{uni203D}{8253}
\DeclareTextGlyphY{LinLibertine_R}{uni203E}{8254}
\DeclareTextGlyphY{LinLibertine_R}{uni2042}{8258}
\DeclareTextGlyphY{LinLibertine_R}{fraction}{8260}
\DeclareTextGlyphY{LinLibertine_R}{uni2044}{8260}
\DeclareTextGlyphY{LinLibertine_R}{question_question}{8263}
\DeclareTextGlyphY{LinLibertine_R}{uni2047}{8263}
\DeclareTextGlyphY{LinLibertine_R}{question_exclam}{8264}
\DeclareTextGlyphY{LinLibertine_R}{uni2048}{8264}
\DeclareTextGlyphY{LinLibertine_R}{exclam_question}{8265}
\DeclareTextGlyphY{LinLibertine_R}{uni2049}{8265}
\DeclareTextGlyphY{LinLibertine_R}{uni204A}{8266}
\DeclareTextGlyphY{LinLibertine_R}{uni204B}{8267}
\DeclareTextGlyphY{LinLibertine_R}{uni204F}{8271}
\DeclareTextGlyphY{LinLibertine_R}{zero.superior}{8304}
\DeclareTextGlyphY{LinLibertine_R}{uni2070}{8304}
\DeclareTextGlyphY{LinLibertine_R}{i.superior}{8305}
\DeclareTextGlyphY{LinLibertine_R}{uni2071}{8305}
\DeclareTextGlyphY{LinLibertine_R}{four.superior}{8308}
\DeclareTextGlyphY{LinLibertine_R}{uni2074}{8308}
\DeclareTextGlyphY{LinLibertine_R}{five.superior}{8309}
\DeclareTextGlyphY{LinLibertine_R}{uni2075}{8309}
\DeclareTextGlyphY{LinLibertine_R}{six.superior}{8310}
\DeclareTextGlyphY{LinLibertine_R}{uni2076}{8310}
\DeclareTextGlyphY{LinLibertine_R}{seven.superior}{8311}
\DeclareTextGlyphY{LinLibertine_R}{uni2077}{8311}
\DeclareTextGlyphY{LinLibertine_R}{eight.superior}{8312}
\DeclareTextGlyphY{LinLibertine_R}{uni2078}{8312}
\DeclareTextGlyphY{LinLibertine_R}{nine.superior}{8313}
\DeclareTextGlyphY{LinLibertine_R}{uni2079}{8313}
\DeclareTextGlyphY{LinLibertine_R}{plus.superior}{8314}
\DeclareTextGlyphY{LinLibertine_R}{uni207A}{8314}
\DeclareTextGlyphY{LinLibertine_R}{minus.superior}{8315}
\DeclareTextGlyphY{LinLibertine_R}{uni207B}{8315}
\DeclareTextGlyphY{LinLibertine_R}{equal.superior}{8316}
\DeclareTextGlyphY{LinLibertine_R}{uni207C}{8316}
\DeclareTextGlyphY{LinLibertine_R}{parenleft.superior}{8317}
\DeclareTextGlyphY{LinLibertine_R}{uni207D}{8317}
\DeclareTextGlyphY{LinLibertine_R}{parenright.superior}{8318}
\DeclareTextGlyphY{LinLibertine_R}{uni207E}{8318}
\DeclareTextGlyphY{LinLibertine_R}{n.superior}{8319}
\DeclareTextGlyphY{LinLibertine_R}{uni207F}{8319}
\DeclareTextGlyphY{LinLibertine_R}{zero.inferior}{8320}
\DeclareTextGlyphY{LinLibertine_R}{uni2080}{8320}
\DeclareTextGlyphY{LinLibertine_R}{one.inferior}{8321}
\DeclareTextGlyphY{LinLibertine_R}{uni2081}{8321}
\DeclareTextGlyphY{LinLibertine_R}{two.inferior}{8322}
\DeclareTextGlyphY{LinLibertine_R}{uni2082}{8322}
\DeclareTextGlyphY{LinLibertine_R}{three.inferior}{8323}
\DeclareTextGlyphY{LinLibertine_R}{uni2083}{8323}
\DeclareTextGlyphY{LinLibertine_R}{four.inferior}{8324}
\DeclareTextGlyphY{LinLibertine_R}{uni2084}{8324}
\DeclareTextGlyphY{LinLibertine_R}{five.inferior}{8325}
\DeclareTextGlyphY{LinLibertine_R}{uni2085}{8325}
\DeclareTextGlyphY{LinLibertine_R}{six.inferior}{8326}
\DeclareTextGlyphY{LinLibertine_R}{uni2086}{8326}
\DeclareTextGlyphY{LinLibertine_R}{seven.inferior}{8327}
\DeclareTextGlyphY{LinLibertine_R}{uni2087}{8327}
\DeclareTextGlyphY{LinLibertine_R}{eight.inferior}{8328}
\DeclareTextGlyphY{LinLibertine_R}{uni2088}{8328}
\DeclareTextGlyphY{LinLibertine_R}{nine.inferior}{8329}
\DeclareTextGlyphY{LinLibertine_R}{uni2089}{8329}
\DeclareTextGlyphY{LinLibertine_R}{plus.inferior}{8330}
\DeclareTextGlyphY{LinLibertine_R}{uni208A}{8330}
\DeclareTextGlyphY{LinLibertine_R}{minus.inferior}{8331}
\DeclareTextGlyphY{LinLibertine_R}{uni208B}{8331}
\DeclareTextGlyphY{LinLibertine_R}{equal.inferior}{8332}
\DeclareTextGlyphY{LinLibertine_R}{uni208C}{8332}
\DeclareTextGlyphY{LinLibertine_R}{parenleft.inferior}{8333}
\DeclareTextGlyphY{LinLibertine_R}{uni208D}{8333}
\DeclareTextGlyphY{LinLibertine_R}{parenright.inferior}{8334}
\DeclareTextGlyphY{LinLibertine_R}{uni208E}{8334}
\DeclareTextGlyphY{LinLibertine_R}{a.inferior}{8336}
\DeclareTextGlyphY{LinLibertine_R}{uni2090}{8336}
\DeclareTextGlyphY{LinLibertine_R}{e.inferior}{8337}
\DeclareTextGlyphY{LinLibertine_R}{uni2091}{8337}
\DeclareTextGlyphY{LinLibertine_R}{o.inferior}{8338}
\DeclareTextGlyphY{LinLibertine_R}{uni2092}{8338}
\DeclareTextGlyphY{LinLibertine_R}{x.inferior}{8339}
\DeclareTextGlyphY{LinLibertine_R}{uni2093}{8339}
\DeclareTextGlyphY{LinLibertine_R}{uni2094}{8340}
\DeclareTextGlyphY{LinLibertine_R}{uni2095}{8341}
\DeclareTextGlyphY{LinLibertine_R}{uni2096}{8342}
\DeclareTextGlyphY{LinLibertine_R}{uni2097}{8343}
\DeclareTextGlyphY{LinLibertine_R}{uni2098}{8344}
\DeclareTextGlyphY{LinLibertine_R}{uni2099}{8345}
\DeclareTextGlyphY{LinLibertine_R}{uni209A}{8346}
\DeclareTextGlyphY{LinLibertine_R}{uni209B}{8347}
\DeclareTextGlyphY{LinLibertine_R}{uni209C}{8348}
\DeclareTextGlyphY{LinLibertine_R}{uni20A2}{8354}
\DeclareTextGlyphY{LinLibertine_R}{franc}{8355}
\DeclareTextGlyphY{LinLibertine_R}{uni20A3}{8355}
\DeclareTextGlyphY{LinLibertine_R}{lira}{8356}
\DeclareTextGlyphY{LinLibertine_R}{uni20A4}{8356}
\DeclareTextGlyphY{LinLibertine_R}{peseta}{8359}
\DeclareTextGlyphY{LinLibertine_R}{uni20A7}{8359}
\DeclareTextGlyphY{LinLibertine_R}{uni20A8}{8360}
\DeclareTextGlyphY{LinLibertine_R}{dong}{8363}
\DeclareTextGlyphY{LinLibertine_R}{uni20AB}{8363}
\DeclareTextGlyphY{LinLibertine_R}{Euro}{8364}
\DeclareTextGlyphY{LinLibertine_R}{uni20AC}{8364}
\DeclareTextGlyphY{LinLibertine_R}{uni20AF}{8367}
\DeclareTextGlyphY{LinLibertine_R}{peso}{8369}
\DeclareTextGlyphY{LinLibertine_R}{uni20B1}{8369}
\DeclareTextGlyphY{LinLibertine_R}{uni2100}{8448}
\DeclareTextGlyphY{LinLibertine_R}{uni2101}{8449}
\DeclareTextGlyphY{LinLibertine_R}{uni2102}{8450}
\DeclareTextGlyphY{LinLibertine_R}{centigrade}{8451}
\DeclareTextGlyphY{LinLibertine_R}{uni2103}{8451}
\DeclareTextGlyphY{LinLibertine_R}{afii61248}{8453}
\DeclareTextGlyphY{LinLibertine_R}{uni2105}{8453}
\DeclareTextGlyphY{LinLibertine_R}{uni2106}{8454}
\DeclareTextGlyphY{LinLibertine_R}{fahrenheit}{8457}
\DeclareTextGlyphY{LinLibertine_R}{uni2109}{8457}
\DeclareTextGlyphY{LinLibertine_R}{uni210C}{8460}
\DeclareTextGlyphY{LinLibertine_R}{uni210D}{8461}
\DeclareTextGlyphY{LinLibertine_R}{uni210E}{8462}
\DeclareTextGlyphY{LinLibertine_R}{uni210F}{8463}
\DeclareTextGlyphY{LinLibertine_R}{Ifraktur}{8465}
\DeclareTextGlyphY{LinLibertine_R}{uni2111}{8465}
\DeclareTextGlyphY{LinLibertine_R}{afii61289}{8467}
\DeclareTextGlyphY{LinLibertine_R}{uni2113}{8467}
\DeclareTextGlyphY{LinLibertine_R}{uni2115}{8469}
\DeclareTextGlyphY{LinLibertine_R}{numero}{8470}
\DeclareTextGlyphY{LinLibertine_R}{uni2116}{8470}
\DeclareTextGlyphY{LinLibertine_R}{uni2119}{8473}
\DeclareTextGlyphY{LinLibertine_R}{uni211A}{8474}
\DeclareTextGlyphY{LinLibertine_R}{Rfraktur}{8476}
\DeclareTextGlyphY{LinLibertine_R}{uni211C}{8476}
\DeclareTextGlyphY{LinLibertine_R}{uni211D}{8477}
\DeclareTextGlyphY{LinLibertine_R}{uni2120}{8480}
\DeclareTextGlyphY{LinLibertine_R}{trademark}{8482}
\DeclareTextGlyphY{LinLibertine_R}{uni2122}{8482}
\DeclareTextGlyphY{LinLibertine_R}{uni2124}{8484}
\DeclareTextGlyphY{LinLibertine_R}{uni2126}{8486}
\DeclareTextGlyphY{LinLibertine_R}{Omegainv}{8487}
\DeclareTextGlyphY{LinLibertine_R}{uni2127}{8487}
\DeclareTextGlyphY{LinLibertine_R}{estimated}{8494}
\DeclareTextGlyphY{LinLibertine_R}{uni212E}{8494}
\DeclareTextGlyphY{LinLibertine_R}{aleph}{8501}
\DeclareTextGlyphY{LinLibertine_R}{uni2135}{8501}
\DeclareTextGlyphY{LinLibertine_R}{uni2136}{8502}
\DeclareTextGlyphY{LinLibertine_R}{uni2137}{8503}
\DeclareTextGlyphY{LinLibertine_R}{uni2138}{8504}
\DeclareTextGlyphY{LinLibertine_R}{uni2139}{8505}
\DeclareTextGlyphY{LinLibertine_R}{uni214F}{8527}
\DeclareTextGlyphY{LinLibertine_R}{onethird}{8531}
\DeclareTextGlyphY{LinLibertine_R}{uni2153}{8531}
\DeclareTextGlyphY{LinLibertine_R}{twothirds}{8532}
\DeclareTextGlyphY{LinLibertine_R}{uni2154}{8532}
\DeclareTextGlyphY{LinLibertine_R}{onefifth}{8533}
\DeclareTextGlyphY{LinLibertine_R}{uni2155}{8533}
\DeclareTextGlyphY{LinLibertine_R}{twofifths}{8534}
\DeclareTextGlyphY{LinLibertine_R}{uni2156}{8534}
\DeclareTextGlyphY{LinLibertine_R}{threefifths}{8535}
\DeclareTextGlyphY{LinLibertine_R}{uni2157}{8535}
\DeclareTextGlyphY{LinLibertine_R}{fourfifths}{8536}
\DeclareTextGlyphY{LinLibertine_R}{uni2158}{8536}
\DeclareTextGlyphY{LinLibertine_R}{onesixth}{8537}
\DeclareTextGlyphY{LinLibertine_R}{uni2159}{8537}
\DeclareTextGlyphY{LinLibertine_R}{fivesixths}{8538}
\DeclareTextGlyphY{LinLibertine_R}{uni215A}{8538}
\DeclareTextGlyphY{LinLibertine_R}{oneeighth}{8539}
\DeclareTextGlyphY{LinLibertine_R}{uni215B}{8539}
\DeclareTextGlyphY{LinLibertine_R}{threeeighths}{8540}
\DeclareTextGlyphY{LinLibertine_R}{uni215C}{8540}
\DeclareTextGlyphY{LinLibertine_R}{fiveeighths}{8541}
\DeclareTextGlyphY{LinLibertine_R}{uni215D}{8541}
\DeclareTextGlyphY{LinLibertine_R}{seveneighths}{8542}
\DeclareTextGlyphY{LinLibertine_R}{uni215E}{8542}
\DeclareTextGlyphY{LinLibertine_R}{onenumerator}{8543}
\DeclareTextGlyphY{LinLibertine_R}{uni215F}{8543}
\DeclareTextGlyphY{LinLibertine_R}{Oneroman}{8544}
\DeclareTextGlyphY{LinLibertine_R}{uni2160}{8544}
\DeclareTextGlyphY{LinLibertine_R}{Tworoman}{8545}
\DeclareTextGlyphY{LinLibertine_R}{uni2161}{8545}
\DeclareTextGlyphY{LinLibertine_R}{Threeroman}{8546}
\DeclareTextGlyphY{LinLibertine_R}{uni2162}{8546}
\DeclareTextGlyphY{LinLibertine_R}{Fourroman}{8547}
\DeclareTextGlyphY{LinLibertine_R}{uni2163}{8547}
\DeclareTextGlyphY{LinLibertine_R}{Fiveroman}{8548}
\DeclareTextGlyphY{LinLibertine_R}{uni2164}{8548}
\DeclareTextGlyphY{LinLibertine_R}{Sixroman}{8549}
\DeclareTextGlyphY{LinLibertine_R}{uni2165}{8549}
\DeclareTextGlyphY{LinLibertine_R}{Sevenroman}{8550}
\DeclareTextGlyphY{LinLibertine_R}{uni2166}{8550}
\DeclareTextGlyphY{LinLibertine_R}{Eightroman}{8551}
\DeclareTextGlyphY{LinLibertine_R}{uni2167}{8551}
\DeclareTextGlyphY{LinLibertine_R}{Nineroman}{8552}
\DeclareTextGlyphY{LinLibertine_R}{uni2168}{8552}
\DeclareTextGlyphY{LinLibertine_R}{Tenroman}{8553}
\DeclareTextGlyphY{LinLibertine_R}{uni2169}{8553}
\DeclareTextGlyphY{LinLibertine_R}{Elevenroman}{8554}
\DeclareTextGlyphY{LinLibertine_R}{uni216A}{8554}
\DeclareTextGlyphY{LinLibertine_R}{Twelveroman}{8555}
\DeclareTextGlyphY{LinLibertine_R}{uni216B}{8555}
\DeclareTextGlyphY{LinLibertine_R}{uni216C}{8556}
\DeclareTextGlyphY{LinLibertine_R}{uni216D}{8557}
\DeclareTextGlyphY{LinLibertine_R}{uni216E}{8558}
\DeclareTextGlyphY{LinLibertine_R}{uni216F}{8559}
\DeclareTextGlyphY{LinLibertine_R}{oneroman}{8560}
\DeclareTextGlyphY{LinLibertine_R}{uni2170}{8560}
\DeclareTextGlyphY{LinLibertine_R}{tworoman}{8561}
\DeclareTextGlyphY{LinLibertine_R}{uni2171}{8561}
\DeclareTextGlyphY{LinLibertine_R}{threeroman}{8562}
\DeclareTextGlyphY{LinLibertine_R}{uni2172}{8562}
\DeclareTextGlyphY{LinLibertine_R}{fourroman}{8563}
\DeclareTextGlyphY{LinLibertine_R}{uni2173}{8563}
\DeclareTextGlyphY{LinLibertine_R}{fiveroman}{8564}
\DeclareTextGlyphY{LinLibertine_R}{uni2174}{8564}
\DeclareTextGlyphY{LinLibertine_R}{sixroman}{8565}
\DeclareTextGlyphY{LinLibertine_R}{uni2175}{8565}
\DeclareTextGlyphY{LinLibertine_R}{sevenroman}{8566}
\DeclareTextGlyphY{LinLibertine_R}{uni2176}{8566}
\DeclareTextGlyphY{LinLibertine_R}{eightroman}{8567}
\DeclareTextGlyphY{LinLibertine_R}{uni2177}{8567}
\DeclareTextGlyphY{LinLibertine_R}{nineroman}{8568}
\DeclareTextGlyphY{LinLibertine_R}{uni2178}{8568}
\DeclareTextGlyphY{LinLibertine_R}{tenroman}{8569}
\DeclareTextGlyphY{LinLibertine_R}{uni2179}{8569}
\DeclareTextGlyphY{LinLibertine_R}{elevenroman}{8570}
\DeclareTextGlyphY{LinLibertine_R}{uni217A}{8570}
\DeclareTextGlyphY{LinLibertine_R}{twelveroman}{8571}
\DeclareTextGlyphY{LinLibertine_R}{uni217B}{8571}
\DeclareTextGlyphY{LinLibertine_R}{uni217C}{8572}
\DeclareTextGlyphY{LinLibertine_R}{uni217D}{8573}
\DeclareTextGlyphY{LinLibertine_R}{uni217E}{8574}
\DeclareTextGlyphY{LinLibertine_R}{uni217F}{8575}
\DeclareTextGlyphY{LinLibertine_R}{uni2180}{8576}
\DeclareTextGlyphY{LinLibertine_R}{uni2181}{8577}
\DeclareTextGlyphY{LinLibertine_R}{uni2182}{8578}
\DeclareTextGlyphY{LinLibertine_R}{uni2183}{8579}
\DeclareTextGlyphY{LinLibertine_R}{uni2184}{8580}
\DeclareTextGlyphY{LinLibertine_R}{arrowleft}{8592}
\DeclareTextGlyphY{LinLibertine_R}{uni2190}{8592}
\DeclareTextGlyphY{LinLibertine_R}{arrowup}{8593}
\DeclareTextGlyphY{LinLibertine_R}{uni2191}{8593}
\DeclareTextGlyphY{LinLibertine_R}{arrowright}{8594}
\DeclareTextGlyphY{LinLibertine_R}{uni2192}{8594}
\DeclareTextGlyphY{LinLibertine_R}{arrowdown}{8595}
\DeclareTextGlyphY{LinLibertine_R}{uni2193}{8595}
\DeclareTextGlyphY{LinLibertine_R}{arrowboth}{8596}
\DeclareTextGlyphY{LinLibertine_R}{uni2194}{8596}
\DeclareTextGlyphY{LinLibertine_R}{arrowupdn}{8597}
\DeclareTextGlyphY{LinLibertine_R}{uni2195}{8597}
\DeclareTextGlyphY{LinLibertine_R}{uni2196}{8598}
\DeclareTextGlyphY{LinLibertine_R}{uni2197}{8599}
\DeclareTextGlyphY{LinLibertine_R}{uni2198}{8600}
\DeclareTextGlyphY{LinLibertine_R}{uni2199}{8601}
\DeclareTextGlyphY{LinLibertine_R}{uni219A}{8602}
\DeclareTextGlyphY{LinLibertine_R}{uni219B}{8603}
\DeclareTextGlyphY{LinLibertine_R}{uni21A6}{8614}
\DeclareTextGlyphY{LinLibertine_R}{arrowupdnbse}{8616}
\DeclareTextGlyphY{LinLibertine_R}{uni21A8}{8616}
\DeclareTextGlyphY{LinLibertine_R}{uni21AE}{8622}
\DeclareTextGlyphY{LinLibertine_R}{uni21BC}{8636}
\DeclareTextGlyphY{LinLibertine_R}{uni21BD}{8637}
\DeclareTextGlyphY{LinLibertine_R}{uni21C0}{8640}
\DeclareTextGlyphY{LinLibertine_R}{uni21C1}{8641}
\DeclareTextGlyphY{LinLibertine_R}{uni21CB}{8651}
\DeclareTextGlyphY{LinLibertine_R}{uni21CC}{8652}
\DeclareTextGlyphY{LinLibertine_R}{uni21CD}{8653}
\DeclareTextGlyphY{LinLibertine_R}{uni21CE}{8654}
\DeclareTextGlyphY{LinLibertine_R}{uni21CF}{8655}
\DeclareTextGlyphY{LinLibertine_R}{arrowdblleft}{8656}
\DeclareTextGlyphY{LinLibertine_R}{uni21D0}{8656}
\DeclareTextGlyphY{LinLibertine_R}{arrowdblup}{8657}
\DeclareTextGlyphY{LinLibertine_R}{uni21D1}{8657}
\DeclareTextGlyphY{LinLibertine_R}{arrowdblright}{8658}
\DeclareTextGlyphY{LinLibertine_R}{uni21D2}{8658}
\DeclareTextGlyphY{LinLibertine_R}{arrowdbldown}{8659}
\DeclareTextGlyphY{LinLibertine_R}{uni21D3}{8659}
\DeclareTextGlyphY{LinLibertine_R}{arrowdblboth}{8660}
\DeclareTextGlyphY{LinLibertine_R}{uni21D4}{8660}
\DeclareTextGlyphY{LinLibertine_R}{uni21D5}{8661}
\DeclareTextGlyphY{LinLibertine_R}{Nwarrow}{8662}
\DeclareTextGlyphY{LinLibertine_R}{uni21D6}{8662}
\DeclareTextGlyphY{LinLibertine_R}{Nearrow}{8663}
\DeclareTextGlyphY{LinLibertine_R}{uni21D7}{8663}
\DeclareTextGlyphY{LinLibertine_R}{Searrow}{8664}
\DeclareTextGlyphY{LinLibertine_R}{uni21D8}{8664}
\DeclareTextGlyphY{LinLibertine_R}{Swarrow}{8665}
\DeclareTextGlyphY{LinLibertine_R}{uni21D9}{8665}
\DeclareTextGlyphY{LinLibertine_R}{uni2200}{8704}
\DeclareTextGlyphY{LinLibertine_R}{uni2201}{8705}
\DeclareTextGlyphY{LinLibertine_R}{partialdiff}{8706}
\DeclareTextGlyphY{LinLibertine_R}{uni2202}{8706}
\DeclareTextGlyphY{LinLibertine_R}{existential}{8707}
\DeclareTextGlyphY{LinLibertine_R}{uni2203}{8707}
\DeclareTextGlyphY{LinLibertine_R}{uni2204}{8708}
\DeclareTextGlyphY{LinLibertine_R}{emptyset}{8709}
\DeclareTextGlyphY{LinLibertine_R}{uni2205}{8709}
\DeclareTextGlyphY{LinLibertine_R}{uni2206}{8710}
\DeclareTextGlyphY{LinLibertine_R}{gradient}{8711}
\DeclareTextGlyphY{LinLibertine_R}{uni2207}{8711}
\DeclareTextGlyphY{LinLibertine_R}{element}{8712}
\DeclareTextGlyphY{LinLibertine_R}{uni2208}{8712}
\DeclareTextGlyphY{LinLibertine_R}{notelement}{8713}
\DeclareTextGlyphY{LinLibertine_R}{uni2209}{8713}
\DeclareTextGlyphY{LinLibertine_R}{uni220A}{8714}
\DeclareTextGlyphY{LinLibertine_R}{suchthat}{8715}
\DeclareTextGlyphY{LinLibertine_R}{uni220B}{8715}
\DeclareTextGlyphY{LinLibertine_R}{uni220C}{8716}
\DeclareTextGlyphY{LinLibertine_R}{uni220D}{8717}
\DeclareTextGlyphY{LinLibertine_R}{product}{8719}
\DeclareTextGlyphY{LinLibertine_R}{uni220F}{8719}
\DeclareTextGlyphY{LinLibertine_R}{uni2210}{8720}
\DeclareTextGlyphY{LinLibertine_R}{summation}{8721}
\DeclareTextGlyphY{LinLibertine_R}{uni2211}{8721}
\DeclareTextGlyphY{LinLibertine_R}{minus}{8722}
\DeclareTextGlyphY{LinLibertine_R}{uni2212}{8722}
\DeclareTextGlyphY{LinLibertine_R}{uni2213}{8723}
\DeclareTextGlyphY{LinLibertine_R}{uni2214}{8724}
\DeclareTextGlyphY{LinLibertine_R}{uni2215}{8725}
\DeclareTextGlyphY{LinLibertine_R}{uni2216}{8726}
\DeclareTextGlyphY{LinLibertine_R}{asteriskmath}{8727}
\DeclareTextGlyphY{LinLibertine_R}{uni2217}{8727}
\DeclareTextGlyphY{LinLibertine_R}{uni2218}{8728}
\DeclareTextGlyphY{LinLibertine_R}{uni2219}{8729}
\DeclareTextGlyphY{LinLibertine_R}{radical}{8730}
\DeclareTextGlyphY{LinLibertine_R}{uni221A}{8730}
\DeclareTextGlyphY{LinLibertine_R}{uni221B}{8731}
\DeclareTextGlyphY{LinLibertine_R}{uni221C}{8732}
\DeclareTextGlyphY{LinLibertine_R}{proportional}{8733}
\DeclareTextGlyphY{LinLibertine_R}{uni221D}{8733}
\DeclareTextGlyphY{LinLibertine_R}{infinity}{8734}
\DeclareTextGlyphY{LinLibertine_R}{uni221E}{8734}
\DeclareTextGlyphY{LinLibertine_R}{uni221F}{8735}
\DeclareTextGlyphY{LinLibertine_R}{angle}{8736}
\DeclareTextGlyphY{LinLibertine_R}{uni2220}{8736}
\DeclareTextGlyphY{LinLibertine_R}{uni2221}{8737}
\DeclareTextGlyphY{LinLibertine_R}{uni2222}{8738}
\DeclareTextGlyphY{LinLibertine_R}{uni2223}{8739}
\DeclareTextGlyphY{LinLibertine_R}{uni2224}{8740}
\DeclareTextGlyphY{LinLibertine_R}{uni2225}{8741}
\DeclareTextGlyphY{LinLibertine_R}{uni2226}{8742}
\DeclareTextGlyphY{LinLibertine_R}{logicaland}{8743}
\DeclareTextGlyphY{LinLibertine_R}{uni2227}{8743}
\DeclareTextGlyphY{LinLibertine_R}{logicalor}{8744}
\DeclareTextGlyphY{LinLibertine_R}{uni2228}{8744}
\DeclareTextGlyphY{LinLibertine_R}{intersection}{8745}
\DeclareTextGlyphY{LinLibertine_R}{uni2229}{8745}
\DeclareTextGlyphY{LinLibertine_R}{uni222A}{8746}
\DeclareTextGlyphY{LinLibertine_R}{integral}{8747}
\DeclareTextGlyphY{LinLibertine_R}{uni222B}{8747}
\DeclareTextGlyphY{LinLibertine_R}{uni222C}{8748}
\DeclareTextGlyphY{LinLibertine_R}{uni222D}{8749}
\DeclareTextGlyphY{LinLibertine_R}{uni222E}{8750}
\DeclareTextGlyphY{LinLibertine_R}{uni2236}{8758}
\DeclareTextGlyphY{LinLibertine_R}{similar}{8764}
\DeclareTextGlyphY{LinLibertine_R}{uni223C}{8764}
\DeclareTextGlyphY{LinLibertine_R}{uni2241}{8769}
\DeclareTextGlyphY{LinLibertine_R}{congruent}{8773}
\DeclareTextGlyphY{LinLibertine_R}{uni2245}{8773}
\DeclareTextGlyphY{LinLibertine_R}{approxequal}{8776}
\DeclareTextGlyphY{LinLibertine_R}{uni2248}{8776}
\DeclareTextGlyphY{LinLibertine_R}{uni2249}{8777}
\DeclareTextGlyphY{LinLibertine_R}{uni2259}{8793}
\DeclareTextGlyphY{LinLibertine_R}{notequal}{8800}
\DeclareTextGlyphY{LinLibertine_R}{uni2260}{8800}
\DeclareTextGlyphY{LinLibertine_R}{equivalence}{8801}
\DeclareTextGlyphY{LinLibertine_R}{uni2261}{8801}
\DeclareTextGlyphY{LinLibertine_R}{uni2262}{8802}
\DeclareTextGlyphY{LinLibertine_R}{lessequal}{8804}
\DeclareTextGlyphY{LinLibertine_R}{uni2264}{8804}
\DeclareTextGlyphY{LinLibertine_R}{greaterequal}{8805}
\DeclareTextGlyphY{LinLibertine_R}{uni2265}{8805}
\DeclareTextGlyphY{LinLibertine_R}{uni226A}{8810}
\DeclareTextGlyphY{LinLibertine_R}{uni226B}{8811}
\DeclareTextGlyphY{LinLibertine_R}{uni226E}{8814}
\DeclareTextGlyphY{LinLibertine_R}{uni226F}{8815}
\DeclareTextGlyphY{LinLibertine_R}{uni2270}{8816}
\DeclareTextGlyphY{LinLibertine_R}{uni2271}{8817}
\DeclareTextGlyphY{LinLibertine_R}{propersubset}{8834}
\DeclareTextGlyphY{LinLibertine_R}{uni2282}{8834}
\DeclareTextGlyphY{LinLibertine_R}{propersuperset}{8835}
\DeclareTextGlyphY{LinLibertine_R}{uni2283}{8835}
\DeclareTextGlyphY{LinLibertine_R}{notsubset}{8836}
\DeclareTextGlyphY{LinLibertine_R}{uni2284}{8836}
\DeclareTextGlyphY{LinLibertine_R}{uni2285}{8837}
\DeclareTextGlyphY{LinLibertine_R}{circleplus}{8853}
\DeclareTextGlyphY{LinLibertine_R}{uni2295}{8853}
\DeclareTextGlyphY{LinLibertine_R}{uni2296}{8854}
\DeclareTextGlyphY{LinLibertine_R}{circlemultiply}{8855}
\DeclareTextGlyphY{LinLibertine_R}{uni2297}{8855}
\DeclareTextGlyphY{LinLibertine_R}{uni2298}{8856}
\DeclareTextGlyphY{LinLibertine_R}{uni22A2}{8866}
\DeclareTextGlyphY{LinLibertine_R}{uni22A3}{8867}
\DeclareTextGlyphY{LinLibertine_R}{uni22A4}{8868}
\DeclareTextGlyphY{LinLibertine_R}{perpendicular}{8869}
\DeclareTextGlyphY{LinLibertine_R}{uni22A5}{8869}
\DeclareTextGlyphY{LinLibertine_R}{uni22A6}{8870}
\DeclareTextGlyphY{LinLibertine_R}{uni22B6}{8886}
\DeclareTextGlyphY{LinLibertine_R}{uni22B7}{8887}
\DeclareTextGlyphY{LinLibertine_R}{dotmath}{8901}
\DeclareTextGlyphY{LinLibertine_R}{uni22C5}{8901}
\DeclareTextGlyphY{LinLibertine_R}{uni22EE}{8942}
\DeclareTextGlyphY{LinLibertine_R}{uni22EF}{8943}
\DeclareTextGlyphY{LinLibertine_R}{uni2300}{8960}
\DeclareTextGlyphY{LinLibertine_R}{uni2302}{8962}
\DeclareTextGlyphY{LinLibertine_R}{uni2303}{8963}
\DeclareTextGlyphY{LinLibertine_R}{uni2310}{8976}
\DeclareTextGlyphY{LinLibertine_R}{integraltop}{8992}
\DeclareTextGlyphY{LinLibertine_R}{uni2320}{8992}
\DeclareTextGlyphY{LinLibertine_R}{integralbottom}{8993}
\DeclareTextGlyphY{LinLibertine_R}{uni2321}{8993}
\DeclareTextGlyphY{LinLibertine_R}{uni2326}{8998}
\DeclareTextGlyphY{LinLibertine_R}{uni2327}{8999}
\DeclareTextGlyphY{LinLibertine_R}{uni2329}{9001}
\DeclareTextGlyphY{LinLibertine_R}{uni232A}{9002}
\DeclareTextGlyphY{LinLibertine_R}{uni232B}{9003}
\DeclareTextGlyphY{LinLibertine_R}{uni237D}{9085}
\DeclareTextGlyphY{LinLibertine_R}{uni2380}{9088}
\DeclareTextGlyphY{LinLibertine_R}{uni239B}{9115}
\DeclareTextGlyphY{LinLibertine_R}{uni239C}{9116}
\DeclareTextGlyphY{LinLibertine_R}{uni239D}{9117}
\DeclareTextGlyphY{LinLibertine_R}{uni239E}{9118}
\DeclareTextGlyphY{LinLibertine_R}{uni239F}{9119}
\DeclareTextGlyphY{LinLibertine_R}{uni23A0}{9120}
\DeclareTextGlyphY{LinLibertine_R}{uni23A1}{9121}
\DeclareTextGlyphY{LinLibertine_R}{uni23A2}{9122}
\DeclareTextGlyphY{LinLibertine_R}{uni23A3}{9123}
\DeclareTextGlyphY{LinLibertine_R}{uni23A4}{9124}
\DeclareTextGlyphY{LinLibertine_R}{uni23A5}{9125}
\DeclareTextGlyphY{LinLibertine_R}{uni23A6}{9126}
\DeclareTextGlyphY{LinLibertine_R}{uni23A7}{9127}
\DeclareTextGlyphY{LinLibertine_R}{uni23A8}{9128}
\DeclareTextGlyphY{LinLibertine_R}{uni23A9}{9129}
\DeclareTextGlyphY{LinLibertine_R}{uni23AA}{9130}
\DeclareTextGlyphY{LinLibertine_R}{uni23AB}{9131}
\DeclareTextGlyphY{LinLibertine_R}{uni23AC}{9132}
\DeclareTextGlyphY{LinLibertine_R}{uni23AD}{9133}
\DeclareTextGlyphY{LinLibertine_R}{integralextension}{9134}
\DeclareTextGlyphY{LinLibertine_R}{uni23AE}{9134}
\DeclareTextGlyphY{LinLibertine_R}{uni23D3}{9171}
\DeclareTextGlyphY{LinLibertine_R}{uni2423}{9251}
\DeclareTextGlyphY{LinLibertine_R}{uni2460}{9312}
\DeclareTextGlyphY{LinLibertine_R}{uni2461}{9313}
\DeclareTextGlyphY{LinLibertine_R}{uni2462}{9314}
\DeclareTextGlyphY{LinLibertine_R}{uni2463}{9315}
\DeclareTextGlyphY{LinLibertine_R}{uni2464}{9316}
\DeclareTextGlyphY{LinLibertine_R}{uni2465}{9317}
\DeclareTextGlyphY{LinLibertine_R}{uni2466}{9318}
\DeclareTextGlyphY{LinLibertine_R}{uni2467}{9319}
\DeclareTextGlyphY{LinLibertine_R}{uni2468}{9320}
\DeclareTextGlyphY{LinLibertine_R}{uni2469}{9321}
\DeclareTextGlyphY{LinLibertine_R}{uni246A}{9322}
\DeclareTextGlyphY{LinLibertine_R}{uni246B}{9323}
\DeclareTextGlyphY{LinLibertine_R}{uni246C}{9324}
\DeclareTextGlyphY{LinLibertine_R}{uni246D}{9325}
\DeclareTextGlyphY{LinLibertine_R}{uni246E}{9326}
\DeclareTextGlyphY{LinLibertine_R}{uni246F}{9327}
\DeclareTextGlyphY{LinLibertine_R}{uni2470}{9328}
\DeclareTextGlyphY{LinLibertine_R}{uni2471}{9329}
\DeclareTextGlyphY{LinLibertine_R}{uni2472}{9330}
\DeclareTextGlyphY{LinLibertine_R}{uni2473}{9331}
\DeclareTextGlyphY{LinLibertine_R}{uni2474}{9332}
\DeclareTextGlyphY{LinLibertine_R}{uni2475}{9333}
\DeclareTextGlyphY{LinLibertine_R}{uni2476}{9334}
\DeclareTextGlyphY{LinLibertine_R}{uni2477}{9335}
\DeclareTextGlyphY{LinLibertine_R}{uni2478}{9336}
\DeclareTextGlyphY{LinLibertine_R}{uni2479}{9337}
\DeclareTextGlyphY{LinLibertine_R}{uni247A}{9338}
\DeclareTextGlyphY{LinLibertine_R}{uni247B}{9339}
\DeclareTextGlyphY{LinLibertine_R}{uni247C}{9340}
\DeclareTextGlyphY{LinLibertine_R}{uni247D}{9341}
\DeclareTextGlyphY{LinLibertine_R}{uni247E}{9342}
\DeclareTextGlyphY{LinLibertine_R}{uni247F}{9343}
\DeclareTextGlyphY{LinLibertine_R}{uni2480}{9344}
\DeclareTextGlyphY{LinLibertine_R}{uni2481}{9345}
\DeclareTextGlyphY{LinLibertine_R}{uni2482}{9346}
\DeclareTextGlyphY{LinLibertine_R}{uni2483}{9347}
\DeclareTextGlyphY{LinLibertine_R}{uni2484}{9348}
\DeclareTextGlyphY{LinLibertine_R}{uni2485}{9349}
\DeclareTextGlyphY{LinLibertine_R}{uni2486}{9350}
\DeclareTextGlyphY{LinLibertine_R}{uni2487}{9351}
\DeclareTextGlyphY{LinLibertine_R}{uni24B6}{9398}
\DeclareTextGlyphY{LinLibertine_R}{uni24B7}{9399}
\DeclareTextGlyphY{LinLibertine_R}{uni24B8}{9400}
\DeclareTextGlyphY{LinLibertine_R}{uni24B9}{9401}
\DeclareTextGlyphY{LinLibertine_R}{uni24BA}{9402}
\DeclareTextGlyphY{LinLibertine_R}{uni24BB}{9403}
\DeclareTextGlyphY{LinLibertine_R}{uni24BC}{9404}
\DeclareTextGlyphY{LinLibertine_R}{uni24BD}{9405}
\DeclareTextGlyphY{LinLibertine_R}{uni24BE}{9406}
\DeclareTextGlyphY{LinLibertine_R}{uni24BF}{9407}
\DeclareTextGlyphY{LinLibertine_R}{uni24C0}{9408}
\DeclareTextGlyphY{LinLibertine_R}{uni24C1}{9409}
\DeclareTextGlyphY{LinLibertine_R}{uni24C2}{9410}
\DeclareTextGlyphY{LinLibertine_R}{uni24C3}{9411}
\DeclareTextGlyphY{LinLibertine_R}{uni24C4}{9412}
\DeclareTextGlyphY{LinLibertine_R}{uni24C5}{9413}
\DeclareTextGlyphY{LinLibertine_R}{uni24C6}{9414}
\DeclareTextGlyphY{LinLibertine_R}{uni24C7}{9415}
\DeclareTextGlyphY{LinLibertine_R}{uni24C8}{9416}
\DeclareTextGlyphY{LinLibertine_R}{uni24C9}{9417}
\DeclareTextGlyphY{LinLibertine_R}{uni24CA}{9418}
\DeclareTextGlyphY{LinLibertine_R}{uni24CB}{9419}
\DeclareTextGlyphY{LinLibertine_R}{uni24CC}{9420}
\DeclareTextGlyphY{LinLibertine_R}{uni24CD}{9421}
\DeclareTextGlyphY{LinLibertine_R}{uni24CE}{9422}
\DeclareTextGlyphY{LinLibertine_R}{uni24CF}{9423}
\DeclareTextGlyphY{LinLibertine_R}{uni24D0}{9424}
\DeclareTextGlyphY{LinLibertine_R}{uni24D1}{9425}
\DeclareTextGlyphY{LinLibertine_R}{uni24D2}{9426}
\DeclareTextGlyphY{LinLibertine_R}{uni24D3}{9427}
\DeclareTextGlyphY{LinLibertine_R}{uni24D4}{9428}
\DeclareTextGlyphY{LinLibertine_R}{uni24D5}{9429}
\DeclareTextGlyphY{LinLibertine_R}{uni24D6}{9430}
\DeclareTextGlyphY{LinLibertine_R}{uni24D7}{9431}
\DeclareTextGlyphY{LinLibertine_R}{uni24D8}{9432}
\DeclareTextGlyphY{LinLibertine_R}{uni24D9}{9433}
\DeclareTextGlyphY{LinLibertine_R}{uni24DA}{9434}
\DeclareTextGlyphY{LinLibertine_R}{uni24DB}{9435}
\DeclareTextGlyphY{LinLibertine_R}{uni24DC}{9436}
\DeclareTextGlyphY{LinLibertine_R}{uni24DD}{9437}
\DeclareTextGlyphY{LinLibertine_R}{uni24DE}{9438}
\DeclareTextGlyphY{LinLibertine_R}{uni24DF}{9439}
\DeclareTextGlyphY{LinLibertine_R}{uni24E0}{9440}
\DeclareTextGlyphY{LinLibertine_R}{uni24E1}{9441}
\DeclareTextGlyphY{LinLibertine_R}{uni24E2}{9442}
\DeclareTextGlyphY{LinLibertine_R}{uni24E3}{9443}
\DeclareTextGlyphY{LinLibertine_R}{uni24E4}{9444}
\DeclareTextGlyphY{LinLibertine_R}{uni24E5}{9445}
\DeclareTextGlyphY{LinLibertine_R}{uni24E6}{9446}
\DeclareTextGlyphY{LinLibertine_R}{uni24E7}{9447}
\DeclareTextGlyphY{LinLibertine_R}{uni24E8}{9448}
\DeclareTextGlyphY{LinLibertine_R}{uni24E9}{9449}
\DeclareTextGlyphY{LinLibertine_R}{uni24EA}{9450}
\DeclareTextGlyphY{LinLibertine_R}{uni24EB}{9451}
\DeclareTextGlyphY{LinLibertine_R}{uni24EC}{9452}
\DeclareTextGlyphY{LinLibertine_R}{uni24ED}{9453}
\DeclareTextGlyphY{LinLibertine_R}{uni24EE}{9454}
\DeclareTextGlyphY{LinLibertine_R}{uni24EF}{9455}
\DeclareTextGlyphY{LinLibertine_R}{uni24F0}{9456}
\DeclareTextGlyphY{LinLibertine_R}{uni24F1}{9457}
\DeclareTextGlyphY{LinLibertine_R}{uni24F2}{9458}
\DeclareTextGlyphY{LinLibertine_R}{uni24F3}{9459}
\DeclareTextGlyphY{LinLibertine_R}{uni24F4}{9460}
\DeclareTextGlyphY{LinLibertine_R}{uni24F5}{9461}
\DeclareTextGlyphY{LinLibertine_R}{uni24F6}{9462}
\DeclareTextGlyphY{LinLibertine_R}{uni24F7}{9463}
\DeclareTextGlyphY{LinLibertine_R}{uni24F8}{9464}
\DeclareTextGlyphY{LinLibertine_R}{uni24F9}{9465}
\DeclareTextGlyphY{LinLibertine_R}{uni24FA}{9466}
\DeclareTextGlyphY{LinLibertine_R}{uni24FB}{9467}
\DeclareTextGlyphY{LinLibertine_R}{uni24FC}{9468}
\DeclareTextGlyphY{LinLibertine_R}{uni24FD}{9469}
\DeclareTextGlyphY{LinLibertine_R}{uni24FE}{9470}
\DeclareTextGlyphY{LinLibertine_R}{uni24FF}{9471}
\DeclareTextGlyphY{LinLibertine_R}{filledbox}{9632}
\DeclareTextGlyphY{LinLibertine_R}{uni25A0}{9632}
\DeclareTextGlyphY{LinLibertine_R}{H22073}{9633}
\DeclareTextGlyphY{LinLibertine_R}{uni25A1}{9633}
\DeclareTextGlyphY{LinLibertine_R}{triagup}{9650}
\DeclareTextGlyphY{LinLibertine_R}{uni25B2}{9650}
\DeclareTextGlyphY{LinLibertine_R}{uni25B3}{9651}
\DeclareTextGlyphY{LinLibertine_R}{uni25B6}{9654}
\DeclareTextGlyphY{LinLibertine_R}{uni25B7}{9655}
\DeclareTextGlyphY{LinLibertine_R}{triagdn}{9660}
\DeclareTextGlyphY{LinLibertine_R}{uni25BC}{9660}
\DeclareTextGlyphY{LinLibertine_R}{uni25BD}{9661}
\DeclareTextGlyphY{LinLibertine_R}{uni25C0}{9664}
\DeclareTextGlyphY{LinLibertine_R}{uni25C1}{9665}
\DeclareTextGlyphY{LinLibertine_R}{uni25C6}{9670}
\DeclareTextGlyphY{LinLibertine_R}{uni25C7}{9671}
\DeclareTextGlyphY{LinLibertine_R}{uni25C9}{9673}
\DeclareTextGlyphY{LinLibertine_R}{lozenge}{9674}
\DeclareTextGlyphY{LinLibertine_R}{uni25CA}{9674}
\DeclareTextGlyphY{LinLibertine_R}{bigcircle}{9675}
\DeclareTextGlyphY{LinLibertine_R}{uni25CB}{9675}
\DeclareTextGlyphY{LinLibertine_R}{uni25CE}{9678}
\DeclareTextGlyphY{LinLibertine_R}{H18533}{9679}
\DeclareTextGlyphY{LinLibertine_R}{uni25CF}{9679}
\DeclareTextGlyphY{LinLibertine_R}{uni25D0}{9680}
\DeclareTextGlyphY{LinLibertine_R}{uni25D1}{9681}
\DeclareTextGlyphY{LinLibertine_R}{uni25D2}{9682}
\DeclareTextGlyphY{LinLibertine_R}{uni25D3}{9683}
\DeclareTextGlyphY{LinLibertine_R}{uni25D4}{9684}
\DeclareTextGlyphY{LinLibertine_R}{uni25D5}{9685}
\DeclareTextGlyphY{LinLibertine_R}{uni25D6}{9686}
\DeclareTextGlyphY{LinLibertine_R}{uni25D7}{9687}
\DeclareTextGlyphY{LinLibertine_R}{openbullet}{9702}
\DeclareTextGlyphY{LinLibertine_R}{uni25E6}{9702}
\DeclareTextGlyphY{LinLibertine_R}{uni2605}{9733}
\DeclareTextGlyphY{LinLibertine_R}{uni2609}{9737}
\DeclareTextGlyphY{LinLibertine_R}{uni2619}{9753}
\DeclareTextGlyphY{LinLibertine_R}{uni261B}{9755}
\DeclareTextGlyphY{LinLibertine_R}{uni261E}{9758}
\DeclareTextGlyphY{LinLibertine_R}{uni2627}{9767}
\DeclareTextGlyphY{LinLibertine_R}{uni262F}{9775}
\DeclareTextGlyphY{LinLibertine_R}{uni2639}{9785}
\DeclareTextGlyphY{LinLibertine_R}{uni263A}{9786}
\DeclareTextGlyphY{LinLibertine_R}{uni263B}{9787}
\DeclareTextGlyphY{LinLibertine_R}{uni263C}{9788}
\DeclareTextGlyphY{LinLibertine_R}{uni263D}{9789}
\DeclareTextGlyphY{LinLibertine_R}{uni263E}{9790}
\DeclareTextGlyphY{LinLibertine_R}{uni263F}{9791}
\DeclareTextGlyphY{LinLibertine_R}{female}{9792}
\DeclareTextGlyphY{LinLibertine_R}{uni2640}{9792}
\DeclareTextGlyphY{LinLibertine_R}{uni2641}{9793}
\DeclareTextGlyphY{LinLibertine_R}{male}{9794}
\DeclareTextGlyphY{LinLibertine_R}{uni2642}{9794}
\DeclareTextGlyphY{LinLibertine_R}{uni2643}{9795}
\DeclareTextGlyphY{LinLibertine_R}{uni2644}{9796}
\DeclareTextGlyphY{LinLibertine_R}{uni2645}{9797}
\DeclareTextGlyphY{LinLibertine_R}{uni2646}{9798}
\DeclareTextGlyphY{LinLibertine_R}{uni2647}{9799}
\DeclareTextGlyphY{LinLibertine_R}{uni2648}{9800}
\DeclareTextGlyphY{LinLibertine_R}{uni2649}{9801}
\DeclareTextGlyphY{LinLibertine_R}{uni264A}{9802}
\DeclareTextGlyphY{LinLibertine_R}{uni264B}{9803}
\DeclareTextGlyphY{LinLibertine_R}{uni264C}{9804}
\DeclareTextGlyphY{LinLibertine_R}{uni264D}{9805}
\DeclareTextGlyphY{LinLibertine_R}{uni264E}{9806}
\DeclareTextGlyphY{LinLibertine_R}{uni264F}{9807}
\DeclareTextGlyphY{LinLibertine_R}{uni2650}{9808}
\DeclareTextGlyphY{LinLibertine_R}{uni2651}{9809}
\DeclareTextGlyphY{LinLibertine_R}{uni2652}{9810}
\DeclareTextGlyphY{LinLibertine_R}{uni2653}{9811}
\DeclareTextGlyphY{LinLibertine_R}{uni2660}{9824}
\DeclareTextGlyphY{LinLibertine_R}{uni2663}{9827}
\DeclareTextGlyphY{LinLibertine_R}{uni2665}{9829}
\DeclareTextGlyphY{LinLibertine_R}{uni2666}{9830}
\DeclareTextGlyphY{LinLibertine_R}{uni2669}{9833}
\DeclareTextGlyphY{LinLibertine_R}{musicalnote}{9834}
\DeclareTextGlyphY{LinLibertine_R}{uni266A}{9834}
\DeclareTextGlyphY{LinLibertine_R}{musicalnotedbl}{9835}
\DeclareTextGlyphY{LinLibertine_R}{uni266B}{9835}
\DeclareTextGlyphY{LinLibertine_R}{uni266C}{9836}
\DeclareTextGlyphY{LinLibertine_R}{uni266D}{9837}
\DeclareTextGlyphY{LinLibertine_R}{uni266E}{9838}
\DeclareTextGlyphY{LinLibertine_R}{uni266F}{9839}
\DeclareTextGlyphY{LinLibertine_R}{uni2695}{9877}
\DeclareTextGlyphY{LinLibertine_R}{uni2698}{9880}
\DeclareTextGlyphY{LinLibertine_R}{uni26A2}{9890}
\DeclareTextGlyphY{LinLibertine_R}{uni26A3}{9891}
\DeclareTextGlyphY{LinLibertine_R}{uni26A4}{9892}
\DeclareTextGlyphY{LinLibertine_R}{uni26A5}{9893}
\DeclareTextGlyphY{LinLibertine_R}{uni26A6}{9894}
\DeclareTextGlyphY{LinLibertine_R}{uni26A7}{9895}
\DeclareTextGlyphY{LinLibertine_R}{uni26AC}{9900}
\DeclareTextGlyphY{LinLibertine_R}{married}{9901}
\DeclareTextGlyphY{LinLibertine_R}{uni26AD}{9901}
\DeclareTextGlyphY{LinLibertine_R}{divorced}{9902}
\DeclareTextGlyphY{LinLibertine_R}{uni26AE}{9902}
\DeclareTextGlyphY{LinLibertine_R}{uni26AF}{9903}
\DeclareTextGlyphY{LinLibertine_R}{uni2714}{10004}
\DeclareTextGlyphY{LinLibertine_R}{uni2718}{10008}
\DeclareTextGlyphY{LinLibertine_R}{died}{10013}
\DeclareTextGlyphY{LinLibertine_R}{uni271D}{10013}
\DeclareTextGlyphY{LinLibertine_R}{uni2767}{10087}
\DeclareTextGlyphY{LinLibertine_R}{uni2776}{10102}
\DeclareTextGlyphY{LinLibertine_R}{uni2777}{10103}
\DeclareTextGlyphY{LinLibertine_R}{uni2778}{10104}
\DeclareTextGlyphY{LinLibertine_R}{uni2779}{10105}
\DeclareTextGlyphY{LinLibertine_R}{uni277A}{10106}
\DeclareTextGlyphY{LinLibertine_R}{uni277B}{10107}
\DeclareTextGlyphY{LinLibertine_R}{uni277C}{10108}
\DeclareTextGlyphY{LinLibertine_R}{uni277D}{10109}
\DeclareTextGlyphY{LinLibertine_R}{uni277E}{10110}
\DeclareTextGlyphY{LinLibertine_R}{uni277F}{10111}
\DeclareTextGlyphY{LinLibertine_R}{uni27C2}{10178}
\DeclareTextGlyphY{LinLibertine_R}{uni27E6}{10214}
\DeclareTextGlyphY{LinLibertine_R}{uni27E7}{10215}
\DeclareTextGlyphY{LinLibertine_R}{uni27E8}{10216}
\DeclareTextGlyphY{LinLibertine_R}{uni27E9}{10217}
\DeclareTextGlyphY{LinLibertine_R}{uni2C60}{11360}
\DeclareTextGlyphY{LinLibertine_R}{uni2C61}{11361}
\DeclareTextGlyphY{LinLibertine_R}{uni2C62}{11362}
\DeclareTextGlyphY{LinLibertine_R}{uni2C63}{11363}
\DeclareTextGlyphY{LinLibertine_R}{uni2C64}{11364}
\DeclareTextGlyphY{LinLibertine_R}{uni2C65}{11365}
\DeclareTextGlyphY{LinLibertine_R}{uni2C66}{11366}
\DeclareTextGlyphY{LinLibertine_R}{uni2C67}{11367}
\DeclareTextGlyphY{LinLibertine_R}{uni2C68}{11368}
\DeclareTextGlyphY{LinLibertine_R}{uni2C69}{11369}
\DeclareTextGlyphY{LinLibertine_R}{uni2C6A}{11370}
\DeclareTextGlyphY{LinLibertine_R}{uni2C6B}{11371}
\DeclareTextGlyphY{LinLibertine_R}{uni2C6C}{11372}
\DeclareTextGlyphY{LinLibertine_R}{uni2C6E}{11374}
\DeclareTextGlyphY{LinLibertine_R}{uni2C6F}{11375}
\DeclareTextGlyphY{LinLibertine_R}{uni2C74}{11380}
\DeclareTextGlyphY{LinLibertine_R}{uni2C75}{11381}
\DeclareTextGlyphY{LinLibertine_R}{uni2C76}{11382}
\DeclareTextGlyphY{LinLibertine_R}{uni2C77}{11383}
\DeclareTextGlyphY{LinLibertine_R}{uni2E02}{11778}
\DeclareTextGlyphY{LinLibertine_R}{uni2E03}{11779}
\DeclareTextGlyphY{LinLibertine_R}{uni2E04}{11780}
\DeclareTextGlyphY{LinLibertine_R}{uni2E05}{11781}
\DeclareTextGlyphY{LinLibertine_R}{uni2E08}{11784}
\DeclareTextGlyphY{LinLibertine_R}{uni2E09}{11785}
\DeclareTextGlyphY{LinLibertine_R}{uni2E0A}{11786}
\DeclareTextGlyphY{LinLibertine_R}{uni2E17}{11799}
\DeclareTextGlyphY{LinLibertine_R}{uni2E18}{11800}
\DeclareTextGlyphY{LinLibertine_R}{uniA656}{42582}
\DeclareTextGlyphY{LinLibertine_R}{uniA657}{42583}
\DeclareTextGlyphY{LinLibertine_R}{uniA71D}{42781}
\DeclareTextGlyphY{LinLibertine_R}{uniA720}{42784}
\DeclareTextGlyphY{LinLibertine_R}{uniA721}{42785}
\DeclareTextGlyphY{LinLibertine_R}{uniA765}{42853}
\DeclareTextGlyphY{LinLibertine_R}{Tux}{57344}
\DeclareTextGlyphY{LinLibertine_R}{uniE000}{57344}
\DeclareTextGlyphY{LinLibertine_R}{uniE001}{57345}
\DeclareTextGlyphY{LinLibertine_R}{uniE002}{57346}
\DeclareTextGlyphY{LinLibertine_R}{uniE003}{57347}
\DeclareTextGlyphY{LinLibertine_R}{uniE004}{57348}
\DeclareTextGlyphY{LinLibertine_R}{uniE005}{57349}
\DeclareTextGlyphY{LinLibertine_R}{uniE006}{57350}
\DeclareTextGlyphY{LinLibertine_R}{uniE007}{57351}
\DeclareTextGlyphY{LinLibertine_R}{uniE008}{57352}
\DeclareTextGlyphY{LinLibertine_R}{uniE009}{57353}
\DeclareTextGlyphY{LinLibertine_R}{uniE00A}{57354}
\DeclareTextGlyphY{LinLibertine_R}{uniE00B}{57355}
\DeclareTextGlyphY{LinLibertine_R}{copyleft}{57356}
\DeclareTextGlyphY{LinLibertine_R}{uniE00C}{57356}
\DeclareTextGlyphY{LinLibertine_R}{publicdomain}{57357}
\DeclareTextGlyphY{LinLibertine_R}{uniE00D}{57357}
\DeclareTextGlyphY{LinLibertine_R}{creativecommons}{57358}
\DeclareTextGlyphY{LinLibertine_R}{uniE00E}{57358}
\DeclareTextGlyphY{LinLibertine_R}{zero.slashfitted}{57359}
\DeclareTextGlyphY{LinLibertine_R}{uniE00F}{57359}
\DeclareTextGlyphY{LinLibertine_R}{zero.fitted}{57360}
\DeclareTextGlyphY{LinLibertine_R}{uniE010}{57360}
\DeclareTextGlyphY{LinLibertine_R}{one.fitted}{57361}
\DeclareTextGlyphY{LinLibertine_R}{uniE011}{57361}
\DeclareTextGlyphY{LinLibertine_R}{two.fitted}{57362}
\DeclareTextGlyphY{LinLibertine_R}{uniE012}{57362}
\DeclareTextGlyphY{LinLibertine_R}{three.fitted}{57363}
\DeclareTextGlyphY{LinLibertine_R}{uniE013}{57363}
\DeclareTextGlyphY{LinLibertine_R}{four.fitted}{57364}
\DeclareTextGlyphY{LinLibertine_R}{uniE014}{57364}
\DeclareTextGlyphY{LinLibertine_R}{five.fitted}{57365}
\DeclareTextGlyphY{LinLibertine_R}{uniE015}{57365}
\DeclareTextGlyphY{LinLibertine_R}{six.fitted}{57366}
\DeclareTextGlyphY{LinLibertine_R}{uniE016}{57366}
\DeclareTextGlyphY{LinLibertine_R}{seven.fitted}{57367}
\DeclareTextGlyphY{LinLibertine_R}{uniE017}{57367}
\DeclareTextGlyphY{LinLibertine_R}{eight.fitted}{57368}
\DeclareTextGlyphY{LinLibertine_R}{uniE018}{57368}
\DeclareTextGlyphY{LinLibertine_R}{nine.fitted}{57369}
\DeclareTextGlyphY{LinLibertine_R}{uniE019}{57369}
\DeclareTextGlyphY{LinLibertine_R}{Euro.fitted}{57370}
\DeclareTextGlyphY{LinLibertine_R}{uniE01A}{57370}
\DeclareTextGlyphY{LinLibertine_R}{Yen.fitted}{57371}
\DeclareTextGlyphY{LinLibertine_R}{uniE01B}{57371}
\DeclareTextGlyphY{LinLibertine_R}{uniE01C}{57372}
\DeclareTextGlyphY{LinLibertine_R}{a.alt}{57373}
\DeclareTextGlyphY{LinLibertine_R}{uniE01D}{57373}
\DeclareTextGlyphY{LinLibertine_R}{uniE01E}{57374}
\DeclareTextGlyphY{LinLibertine_R}{perthousandzero}{57375}
\DeclareTextGlyphY{LinLibertine_R}{uniE01F}{57375}
\DeclareTextGlyphY{LinLibertine_R}{zero.oldstyle}{57376}
\DeclareTextGlyphY{LinLibertine_R}{uniE020}{57376}
\DeclareTextGlyphY{LinLibertine_R}{one.oldstyle}{57377}
\DeclareTextGlyphY{LinLibertine_R}{uniE021}{57377}
\DeclareTextGlyphY{LinLibertine_R}{two.oldstyle}{57378}
\DeclareTextGlyphY{LinLibertine_R}{uniE022}{57378}
\DeclareTextGlyphY{LinLibertine_R}{three.oldstyle}{57379}
\DeclareTextGlyphY{LinLibertine_R}{uniE023}{57379}
\DeclareTextGlyphY{LinLibertine_R}{four.oldstyle}{57380}
\DeclareTextGlyphY{LinLibertine_R}{uniE024}{57380}
\DeclareTextGlyphY{LinLibertine_R}{five.oldstyle}{57381}
\DeclareTextGlyphY{LinLibertine_R}{uniE025}{57381}
\DeclareTextGlyphY{LinLibertine_R}{six.oldstyle}{57382}
\DeclareTextGlyphY{LinLibertine_R}{uniE026}{57382}
\DeclareTextGlyphY{LinLibertine_R}{seven.oldstyle}{57383}
\DeclareTextGlyphY{LinLibertine_R}{uniE027}{57383}
\DeclareTextGlyphY{LinLibertine_R}{eight.oldstyle}{57384}
\DeclareTextGlyphY{LinLibertine_R}{uniE028}{57384}
\DeclareTextGlyphY{LinLibertine_R}{nine.oldstyle}{57385}
\DeclareTextGlyphY{LinLibertine_R}{uniE029}{57385}
\DeclareTextGlyphY{LinLibertine_R}{uniE02A}{57386}
\DeclareTextGlyphY{LinLibertine_R}{Adieresis.alt}{57388}
\DeclareTextGlyphY{LinLibertine_R}{uniE02C}{57388}
\DeclareTextGlyphY{LinLibertine_R}{Odieresis.alt}{57389}
\DeclareTextGlyphY{LinLibertine_R}{uniE02D}{57389}
\DeclareTextGlyphY{LinLibertine_R}{Udieresis.alt}{57390}
\DeclareTextGlyphY{LinLibertine_R}{uniE02E}{57390}
\DeclareTextGlyphY{LinLibertine_R}{W.alt}{57391}
\DeclareTextGlyphY{LinLibertine_R}{uniE02F}{57391}
\DeclareTextGlyphY{LinLibertine_R}{f_b}{57392}
\DeclareTextGlyphY{LinLibertine_R}{uniE030}{57392}
\DeclareTextGlyphY{LinLibertine_R}{f_f_h}{57394}
\DeclareTextGlyphY{LinLibertine_R}{uniE032}{57394}
\DeclareTextGlyphY{LinLibertine_R}{f_f_j}{57395}
\DeclareTextGlyphY{LinLibertine_R}{uniE033}{57395}
\DeclareTextGlyphY{LinLibertine_R}{f_f_k}{57396}
\DeclareTextGlyphY{LinLibertine_R}{uniE034}{57396}
\DeclareTextGlyphY{LinLibertine_R}{f_f_t}{57397}
\DeclareTextGlyphY{LinLibertine_R}{uniE035}{57397}
\DeclareTextGlyphY{LinLibertine_R}{f_h}{57398}
\DeclareTextGlyphY{LinLibertine_R}{uniE036}{57398}
\DeclareTextGlyphY{LinLibertine_R}{f_j}{57399}
\DeclareTextGlyphY{LinLibertine_R}{uniE037}{57399}
\DeclareTextGlyphY{LinLibertine_R}{f_k}{57400}
\DeclareTextGlyphY{LinLibertine_R}{uniE038}{57400}
\DeclareTextGlyphY{LinLibertine_R}{f_t}{57401}
\DeclareTextGlyphY{LinLibertine_R}{uniE039}{57401}
\DeclareTextGlyphY{LinLibertine_R}{c_k}{57402}
\DeclareTextGlyphY{LinLibertine_R}{uniE03A}{57402}
\DeclareTextGlyphY{LinLibertine_R}{c_h}{57403}
\DeclareTextGlyphY{LinLibertine_R}{uniE03B}{57403}
\DeclareTextGlyphY{LinLibertine_R}{t_t}{57404}
\DeclareTextGlyphY{LinLibertine_R}{uniE03C}{57404}
\DeclareTextGlyphY{LinLibertine_R}{c_t}{57405}
\DeclareTextGlyphY{LinLibertine_R}{uniE03D}{57405}
\DeclareTextGlyphY{LinLibertine_R}{longs_i}{57406}
\DeclareTextGlyphY{LinLibertine_R}{uniE03E}{57406}
\DeclareTextGlyphY{LinLibertine_R}{longs_longs}{57407}
\DeclareTextGlyphY{LinLibertine_R}{uniE03F}{57407}
\DeclareTextGlyphY{LinLibertine_R}{uniE040}{57408}
\DeclareTextGlyphY{LinLibertine_R}{uniE041}{57409}
\DeclareTextGlyphY{LinLibertine_R}{uniE042}{57410}
\DeclareTextGlyphY{LinLibertine_R}{longs_l}{57411}
\DeclareTextGlyphY{LinLibertine_R}{uniE043}{57411}
\DeclareTextGlyphY{LinLibertine_R}{longs_longs_i}{57412}
\DeclareTextGlyphY{LinLibertine_R}{uniE044}{57412}
\DeclareTextGlyphY{LinLibertine_R}{longs_s}{57413}
\DeclareTextGlyphY{LinLibertine_R}{uniE045}{57413}
\DeclareTextGlyphY{LinLibertine_R}{ae.alt}{57414}
\DeclareTextGlyphY{LinLibertine_R}{uniE046}{57414}
\DeclareTextGlyphY{LinLibertine_R}{longs_h}{57415}
\DeclareTextGlyphY{LinLibertine_R}{uniE047}{57415}
\DeclareTextGlyphY{LinLibertine_R}{Q_u}{57416}
\DeclareTextGlyphY{LinLibertine_R}{uniE048}{57416}
\DeclareTextGlyphY{LinLibertine_R}{T_h}{57417}
\DeclareTextGlyphY{LinLibertine_R}{uniE049}{57417}
\DeclareTextGlyphY{LinLibertine_R}{t_z}{57418}
\DeclareTextGlyphY{LinLibertine_R}{uniE04A}{57418}
\DeclareTextGlyphY{LinLibertine_R}{h.alt}{57419}
\DeclareTextGlyphY{LinLibertine_R}{uniE04B}{57419}
\DeclareTextGlyphY{LinLibertine_R}{germandbls.alt}{57420}
\DeclareTextGlyphY{LinLibertine_R}{uniE04C}{57420}
\DeclareTextGlyphY{LinLibertine_R}{germandbls.ss03}{57421}
\DeclareTextGlyphY{LinLibertine_R}{uniE04D}{57421}
\DeclareTextGlyphY{LinLibertine_R}{Germandbls.alt}{57422}
\DeclareTextGlyphY{LinLibertine_R}{uniE04E}{57422}
\DeclareTextGlyphY{LinLibertine_R}{uniE04F}{57423}
\DeclareTextGlyphY{LinLibertine_R}{ampersand.alt}{57424}
\DeclareTextGlyphY{LinLibertine_R}{uniE050}{57424}
\DeclareTextGlyphY{LinLibertine_R}{a.sc}{57425}
\DeclareTextGlyphY{LinLibertine_R}{uniE051}{57425}
\DeclareTextGlyphY{LinLibertine_R}{b.sc}{57426}
\DeclareTextGlyphY{LinLibertine_R}{uniE052}{57426}
\DeclareTextGlyphY{LinLibertine_R}{c.sc}{57427}
\DeclareTextGlyphY{LinLibertine_R}{uniE053}{57427}
\DeclareTextGlyphY{LinLibertine_R}{d.sc}{57428}
\DeclareTextGlyphY{LinLibertine_R}{uniE054}{57428}
\DeclareTextGlyphY{LinLibertine_R}{e.sc}{57429}
\DeclareTextGlyphY{LinLibertine_R}{uniE055}{57429}
\DeclareTextGlyphY{LinLibertine_R}{f.sc}{57430}
\DeclareTextGlyphY{LinLibertine_R}{uniE056}{57430}
\DeclareTextGlyphY{LinLibertine_R}{g.sc}{57431}
\DeclareTextGlyphY{LinLibertine_R}{uniE057}{57431}
\DeclareTextGlyphY{LinLibertine_R}{h.sc}{57432}
\DeclareTextGlyphY{LinLibertine_R}{uniE058}{57432}
\DeclareTextGlyphY{LinLibertine_R}{i.sc}{57433}
\DeclareTextGlyphY{LinLibertine_R}{uniE059}{57433}
\DeclareTextGlyphY{LinLibertine_R}{j.sc}{57434}
\DeclareTextGlyphY{LinLibertine_R}{uniE05A}{57434}
\DeclareTextGlyphY{LinLibertine_R}{k.sc}{57435}
\DeclareTextGlyphY{LinLibertine_R}{uniE05B}{57435}
\DeclareTextGlyphY{LinLibertine_R}{l.sc}{57436}
\DeclareTextGlyphY{LinLibertine_R}{uniE05C}{57436}
\DeclareTextGlyphY{LinLibertine_R}{m.sc}{57437}
\DeclareTextGlyphY{LinLibertine_R}{uniE05D}{57437}
\DeclareTextGlyphY{LinLibertine_R}{n.sc}{57438}
\DeclareTextGlyphY{LinLibertine_R}{uniE05E}{57438}
\DeclareTextGlyphY{LinLibertine_R}{o.sc}{57439}
\DeclareTextGlyphY{LinLibertine_R}{uniE05F}{57439}
\DeclareTextGlyphY{LinLibertine_R}{p.sc}{57440}
\DeclareTextGlyphY{LinLibertine_R}{uniE060}{57440}
\DeclareTextGlyphY{LinLibertine_R}{q.sc}{57441}
\DeclareTextGlyphY{LinLibertine_R}{uniE061}{57441}
\DeclareTextGlyphY{LinLibertine_R}{r.sc}{57442}
\DeclareTextGlyphY{LinLibertine_R}{uniE062}{57442}
\DeclareTextGlyphY{LinLibertine_R}{s.sc}{57443}
\DeclareTextGlyphY{LinLibertine_R}{uniE063}{57443}
\DeclareTextGlyphY{LinLibertine_R}{t.sc}{57444}
\DeclareTextGlyphY{LinLibertine_R}{uniE064}{57444}
\DeclareTextGlyphY{LinLibertine_R}{u.sc}{57445}
\DeclareTextGlyphY{LinLibertine_R}{uniE065}{57445}
\DeclareTextGlyphY{LinLibertine_R}{v.sc}{57446}
\DeclareTextGlyphY{LinLibertine_R}{uniE066}{57446}
\DeclareTextGlyphY{LinLibertine_R}{w.sc}{57447}
\DeclareTextGlyphY{LinLibertine_R}{uniE067}{57447}
\DeclareTextGlyphY{LinLibertine_R}{x.sc}{57448}
\DeclareTextGlyphY{LinLibertine_R}{uniE068}{57448}
\DeclareTextGlyphY{LinLibertine_R}{y.sc}{57449}
\DeclareTextGlyphY{LinLibertine_R}{uniE069}{57449}
\DeclareTextGlyphY{LinLibertine_R}{z.sc}{57450}
\DeclareTextGlyphY{LinLibertine_R}{uniE06A}{57450}
\DeclareTextGlyphY{LinLibertine_R}{uniE06B}{57451}
\DeclareTextGlyphY{LinLibertine_R}{hyphen.sc}{57453}
\DeclareTextGlyphY{LinLibertine_R}{uniE06D}{57453}
\DeclareTextGlyphY{LinLibertine_R}{agrave.sc}{57456}
\DeclareTextGlyphY{LinLibertine_R}{uniE070}{57456}
\DeclareTextGlyphY{LinLibertine_R}{aacute.sc}{57457}
\DeclareTextGlyphY{LinLibertine_R}{uniE071}{57457}
\DeclareTextGlyphY{LinLibertine_R}{acircumflex.sc}{57458}
\DeclareTextGlyphY{LinLibertine_R}{uniE072}{57458}
\DeclareTextGlyphY{LinLibertine_R}{atilde.sc}{57459}
\DeclareTextGlyphY{LinLibertine_R}{uniE073}{57459}
\DeclareTextGlyphY{LinLibertine_R}{adieresis.sc}{57460}
\DeclareTextGlyphY{LinLibertine_R}{uniE074}{57460}
\DeclareTextGlyphY{LinLibertine_R}{aring.sc}{57461}
\DeclareTextGlyphY{LinLibertine_R}{uniE075}{57461}
\DeclareTextGlyphY{LinLibertine_R}{ae.sc}{57462}
\DeclareTextGlyphY{LinLibertine_R}{uniE076}{57462}
\DeclareTextGlyphY{LinLibertine_R}{ccedilla.sc}{57463}
\DeclareTextGlyphY{LinLibertine_R}{uniE077}{57463}
\DeclareTextGlyphY{LinLibertine_R}{egrave.sc}{57464}
\DeclareTextGlyphY{LinLibertine_R}{uniE078}{57464}
\DeclareTextGlyphY{LinLibertine_R}{eacute.sc}{57465}
\DeclareTextGlyphY{LinLibertine_R}{uniE079}{57465}
\DeclareTextGlyphY{LinLibertine_R}{ecircumflex.sc}{57466}
\DeclareTextGlyphY{LinLibertine_R}{uniE07A}{57466}
\DeclareTextGlyphY{LinLibertine_R}{edieresis.sc}{57467}
\DeclareTextGlyphY{LinLibertine_R}{uniE07B}{57467}
\DeclareTextGlyphY{LinLibertine_R}{igrave.sc}{57468}
\DeclareTextGlyphY{LinLibertine_R}{uniE07C}{57468}
\DeclareTextGlyphY{LinLibertine_R}{iacute.sc}{57469}
\DeclareTextGlyphY{LinLibertine_R}{uniE07D}{57469}
\DeclareTextGlyphY{LinLibertine_R}{icircumflex.sc}{57470}
\DeclareTextGlyphY{LinLibertine_R}{uniE07E}{57470}
\DeclareTextGlyphY{LinLibertine_R}{idieresis.sc}{57471}
\DeclareTextGlyphY{LinLibertine_R}{uniE07F}{57471}
\DeclareTextGlyphY{LinLibertine_R}{eth.sc}{57472}
\DeclareTextGlyphY{LinLibertine_R}{uniE080}{57472}
\DeclareTextGlyphY{LinLibertine_R}{ntilde.sc}{57473}
\DeclareTextGlyphY{LinLibertine_R}{uniE081}{57473}
\DeclareTextGlyphY{LinLibertine_R}{ograve.sc}{57474}
\DeclareTextGlyphY{LinLibertine_R}{uniE082}{57474}
\DeclareTextGlyphY{LinLibertine_R}{oacute.sc}{57475}
\DeclareTextGlyphY{LinLibertine_R}{uniE083}{57475}
\DeclareTextGlyphY{LinLibertine_R}{ocircumflex.sc}{57476}
\DeclareTextGlyphY{LinLibertine_R}{uniE084}{57476}
\DeclareTextGlyphY{LinLibertine_R}{otilde.sc}{57477}
\DeclareTextGlyphY{LinLibertine_R}{uniE085}{57477}
\DeclareTextGlyphY{LinLibertine_R}{odieresis.sc}{57478}
\DeclareTextGlyphY{LinLibertine_R}{uniE086}{57478}
\DeclareTextGlyphY{LinLibertine_R}{oe.sc}{57479}
\DeclareTextGlyphY{LinLibertine_R}{uniE087}{57479}
\DeclareTextGlyphY{LinLibertine_R}{oslash.sc}{57480}
\DeclareTextGlyphY{LinLibertine_R}{uniE088}{57480}
\DeclareTextGlyphY{LinLibertine_R}{ugrave.sc}{57481}
\DeclareTextGlyphY{LinLibertine_R}{uniE089}{57481}
\DeclareTextGlyphY{LinLibertine_R}{uacute.sc}{57482}
\DeclareTextGlyphY{LinLibertine_R}{uniE08A}{57482}
\DeclareTextGlyphY{LinLibertine_R}{ucircumflex.sc}{57483}
\DeclareTextGlyphY{LinLibertine_R}{uniE08B}{57483}
\DeclareTextGlyphY{LinLibertine_R}{udieresis.sc}{57484}
\DeclareTextGlyphY{LinLibertine_R}{uniE08C}{57484}
\DeclareTextGlyphY{LinLibertine_R}{yacute.sc}{57485}
\DeclareTextGlyphY{LinLibertine_R}{uniE08D}{57485}
\DeclareTextGlyphY{LinLibertine_R}{thorn.sc}{57486}
\DeclareTextGlyphY{LinLibertine_R}{uniE08E}{57486}
\DeclareTextGlyphY{LinLibertine_R}{ydieresis.sc}{57487}
\DeclareTextGlyphY{LinLibertine_R}{uniE08F}{57487}
\DeclareTextGlyphY{LinLibertine_R}{ij.sc}{57488}
\DeclareTextGlyphY{LinLibertine_R}{uniE090}{57488}
\DeclareTextGlyphY{LinLibertine_R}{germandbls.scalt}{57489}
\DeclareTextGlyphY{LinLibertine_R}{uniE091}{57489}
\DeclareTextGlyphY{LinLibertine_R}{germandbls.sc}{57490}
\DeclareTextGlyphY{LinLibertine_R}{uniE092}{57490}
\DeclareTextGlyphY{LinLibertine_R}{Q_u.sc}{57491}
\DeclareTextGlyphY{LinLibertine_R}{uniE093}{57491}
\DeclareTextGlyphY{LinLibertine_R}{q.sc_u.sc}{57492}
\DeclareTextGlyphY{LinLibertine_R}{uniE094}{57492}
\DeclareTextGlyphY{LinLibertine_R}{dcroat.sc}{57495}
\DeclareTextGlyphY{LinLibertine_R}{uniE097}{57495}
\DeclareTextGlyphY{LinLibertine_R}{abreve.sc}{57496}
\DeclareTextGlyphY{LinLibertine_R}{uniE098}{57496}
\DeclareTextGlyphY{LinLibertine_R}{aogonek.sc}{57497}
\DeclareTextGlyphY{LinLibertine_R}{uniE099}{57497}
\DeclareTextGlyphY{LinLibertine_R}{cacute.sc}{57498}
\DeclareTextGlyphY{LinLibertine_R}{uniE09A}{57498}
\DeclareTextGlyphY{LinLibertine_R}{ccaron.sc}{57499}
\DeclareTextGlyphY{LinLibertine_R}{uniE09B}{57499}
\DeclareTextGlyphY{LinLibertine_R}{dcaron.sc}{57500}
\DeclareTextGlyphY{LinLibertine_R}{uniE09C}{57500}
\DeclareTextGlyphY{LinLibertine_R}{eogonek.sc}{57501}
\DeclareTextGlyphY{LinLibertine_R}{uniE09D}{57501}
\DeclareTextGlyphY{LinLibertine_R}{ecaron.sc}{57502}
\DeclareTextGlyphY{LinLibertine_R}{uniE09E}{57502}
\DeclareTextGlyphY{LinLibertine_R}{gbreve.sc}{57503}
\DeclareTextGlyphY{LinLibertine_R}{uniE09F}{57503}
\DeclareTextGlyphY{LinLibertine_R}{lacute.sc}{57504}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A0}{57504}
\DeclareTextGlyphY{LinLibertine_R}{lslash.sc}{57505}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A1}{57505}
\DeclareTextGlyphY{LinLibertine_R}{nacute.sc}{57506}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A2}{57506}
\DeclareTextGlyphY{LinLibertine_R}{ncaron.sc}{57507}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A3}{57507}
\DeclareTextGlyphY{LinLibertine_R}{eng.sc}{57508}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A4}{57508}
\DeclareTextGlyphY{LinLibertine_R}{ohungarumlaut.sc}{57509}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A5}{57509}
\DeclareTextGlyphY{LinLibertine_R}{racute.sc}{57510}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A6}{57510}
\DeclareTextGlyphY{LinLibertine_R}{rcaron.sc}{57511}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A7}{57511}
\DeclareTextGlyphY{LinLibertine_R}{sacute.sc}{57512}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A8}{57512}
\DeclareTextGlyphY{LinLibertine_R}{scedilla.sc}{57513}
\DeclareTextGlyphY{LinLibertine_R}{uniE0A9}{57513}
\DeclareTextGlyphY{LinLibertine_R}{scaron.sc}{57514}
\DeclareTextGlyphY{LinLibertine_R}{uniE0AA}{57514}
\DeclareTextGlyphY{LinLibertine_R}{tcedilla.sc}{57515}
\DeclareTextGlyphY{LinLibertine_R}{uniE0AB}{57515}
\DeclareTextGlyphY{LinLibertine_R}{tbar.sc}{57516}
\DeclareTextGlyphY{LinLibertine_R}{uniE0AC}{57516}
\DeclareTextGlyphY{LinLibertine_R}{uring.sc}{57517}
\DeclareTextGlyphY{LinLibertine_R}{uniE0AD}{57517}
\DeclareTextGlyphY{LinLibertine_R}{uhungarumlaut.sc}{57518}
\DeclareTextGlyphY{LinLibertine_R}{uniE0AE}{57518}
\DeclareTextGlyphY{LinLibertine_R}{zacute.sc}{57519}
\DeclareTextGlyphY{LinLibertine_R}{uniE0AF}{57519}
\DeclareTextGlyphY{LinLibertine_R}{zdotaccent.sc}{57520}
\DeclareTextGlyphY{LinLibertine_R}{uniE0B0}{57520}
\DeclareTextGlyphY{LinLibertine_R}{zcaron.sc}{57521}
\DeclareTextGlyphY{LinLibertine_R}{uniE0B1}{57521}
\DeclareTextGlyphY{LinLibertine_R}{lcaron.sc}{57522}
\DeclareTextGlyphY{LinLibertine_R}{uniE0B2}{57522}
\DeclareTextGlyphY{LinLibertine_R}{tcaron.sc}{57523}
\DeclareTextGlyphY{LinLibertine_R}{uniE0B3}{57523}
\DeclareTextGlyphY{LinLibertine_R}{tcommaaccent.sc}{57524}
\DeclareTextGlyphY{LinLibertine_R}{uniE0B4}{57524}
\DeclareTextGlyphY{LinLibertine_R}{scommaaccent.sc}{57525}
\DeclareTextGlyphY{LinLibertine_R}{uniE0B5}{57525}
\DeclareTextGlyphY{LinLibertine_R}{idotaccent.sc}{57526}
\DeclareTextGlyphY{LinLibertine_R}{uniE0B6}{57526}
\DeclareTextGlyphY{LinLibertine_R}{ampersand.sc}{57533}
\DeclareTextGlyphY{LinLibertine_R}{uniE0BD}{57533}
\DeclareTextGlyphY{LinLibertine_R}{a.scalt}{57534}
\DeclareTextGlyphY{LinLibertine_R}{uniE0BE}{57534}
\DeclareTextGlyphY{LinLibertine_R}{q.superior}{57552}
\DeclareTextGlyphY{LinLibertine_R}{uniE0D0}{57552}
\DeclareTextGlyphY{LinLibertine_R}{gravecomb.sups}{57563}
\DeclareTextGlyphY{LinLibertine_R}{uniE0DB}{57563}
\DeclareTextGlyphY{LinLibertine_R}{acutecomb.sups}{57564}
\DeclareTextGlyphY{LinLibertine_R}{uniE0DC}{57564}
\DeclareTextGlyphY{LinLibertine_R}{circumflexcomb.sups}{57565}
\DeclareTextGlyphY{LinLibertine_R}{uniE0DD}{57565}
\DeclareTextGlyphY{LinLibertine_R}{tildecomb.sups}{57566}
\DeclareTextGlyphY{LinLibertine_R}{uniE0DE}{57566}
\DeclareTextGlyphY{LinLibertine_R}{macroncomb.sups}{57567}
\DeclareTextGlyphY{LinLibertine_R}{uniE0DF}{57567}
\DeclareTextGlyphY{LinLibertine_R}{f.short}{57568}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E0}{57568}
\DeclareTextGlyphY{LinLibertine_R}{f_f.short}{57569}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E1}{57569}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E2}{57570}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E3}{57571}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E4}{57572}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E5}{57573}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E6}{57574}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E7}{57575}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E8}{57576}
\DeclareTextGlyphY{LinLibertine_R}{uniE0E9}{57577}
\DeclareTextGlyphY{LinLibertine_R}{uniE0EA}{57578}
\DeclareTextGlyphY{LinLibertine_R}{K.alt}{57579}
\DeclareTextGlyphY{LinLibertine_R}{uniE0EB}{57579}
\DeclareTextGlyphY{LinLibertine_R}{R.alt}{57580}
\DeclareTextGlyphY{LinLibertine_R}{uniE0EC}{57580}
\DeclareTextGlyphY{LinLibertine_R}{J.alt}{57581}
\DeclareTextGlyphY{LinLibertine_R}{uniE0ED}{57581}
\DeclareTextGlyphY{LinLibertine_R}{uniE0EE}{57582}
\DeclareTextGlyphY{LinLibertine_R}{uniE0EF}{57583}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F0}{57584}
\DeclareTextGlyphY{LinLibertine_R}{w.alt}{57585}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F1}{57585}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F2}{57586}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F3}{57587}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F4}{57588}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F5}{57589}
\DeclareTextGlyphY{LinLibertine_R}{y.alt}{57590}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F6}{57590}
\DeclareTextGlyphY{LinLibertine_R}{A.alt}{57591}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F7}{57591}
\DeclareTextGlyphY{LinLibertine_R}{uniE0F9}{57593}
\DeclareTextGlyphY{LinLibertine_R}{uniE0FB}{57595}
\DeclareTextGlyphY{LinLibertine_R}{kreis}{57600}
\DeclareTextGlyphY{LinLibertine_R}{uniE100}{57600}
\DeclareTextGlyphY{LinLibertine_R}{uniE101}{57601}
\DeclareTextGlyphY{LinLibertine_R}{uniE104}{57604}
\DeclareTextGlyphY{LinLibertine_R}{uniE105}{57605}
\DeclareTextGlyphY{LinLibertine_R}{uniE106}{57606}
\DeclareTextGlyphY{LinLibertine_R}{uniE107}{57607}
\DeclareTextGlyphY{LinLibertine_R}{zero.cap}{57608}
\DeclareTextGlyphY{LinLibertine_R}{uniE108}{57608}
\DeclareTextGlyphY{LinLibertine_R}{one.cap}{57609}
\DeclareTextGlyphY{LinLibertine_R}{uniE109}{57609}
\DeclareTextGlyphY{LinLibertine_R}{two.cap}{57610}
\DeclareTextGlyphY{LinLibertine_R}{uniE10A}{57610}
\DeclareTextGlyphY{LinLibertine_R}{three.cap}{57611}
\DeclareTextGlyphY{LinLibertine_R}{uniE10B}{57611}
\DeclareTextGlyphY{LinLibertine_R}{four.cap}{57612}
\DeclareTextGlyphY{LinLibertine_R}{uniE10C}{57612}
\DeclareTextGlyphY{LinLibertine_R}{five.cap}{57613}
\DeclareTextGlyphY{LinLibertine_R}{uniE10D}{57613}
\DeclareTextGlyphY{LinLibertine_R}{six.cap}{57614}
\DeclareTextGlyphY{LinLibertine_R}{uniE10E}{57614}
\DeclareTextGlyphY{LinLibertine_R}{seven.cap}{57615}
\DeclareTextGlyphY{LinLibertine_R}{uniE10F}{57615}
\DeclareTextGlyphY{LinLibertine_R}{eight.cap}{57616}
\DeclareTextGlyphY{LinLibertine_R}{uniE110}{57616}
\DeclareTextGlyphY{LinLibertine_R}{nine.cap}{57617}
\DeclareTextGlyphY{LinLibertine_R}{uniE111}{57617}
\DeclareTextGlyphY{LinLibertine_R}{zero.taboldstyle}{57624}
\DeclareTextGlyphY{LinLibertine_R}{uniE118}{57624}
\DeclareTextGlyphY{LinLibertine_R}{one.taboldstyle}{57625}
\DeclareTextGlyphY{LinLibertine_R}{uniE119}{57625}
\DeclareTextGlyphY{LinLibertine_R}{two.taboldstyle}{57626}
\DeclareTextGlyphY{LinLibertine_R}{uniE11A}{57626}
\DeclareTextGlyphY{LinLibertine_R}{three.taboldstyle}{57627}
\DeclareTextGlyphY{LinLibertine_R}{uniE11B}{57627}
\DeclareTextGlyphY{LinLibertine_R}{four.taboldstyle}{57628}
\DeclareTextGlyphY{LinLibertine_R}{uniE11C}{57628}
\DeclareTextGlyphY{LinLibertine_R}{five.taboldstyle}{57629}
\DeclareTextGlyphY{LinLibertine_R}{uniE11D}{57629}
\DeclareTextGlyphY{LinLibertine_R}{six.taboldstyle}{57630}
\DeclareTextGlyphY{LinLibertine_R}{uniE11E}{57630}
\DeclareTextGlyphY{LinLibertine_R}{seven.taboldstyle}{57631}
\DeclareTextGlyphY{LinLibertine_R}{uniE11F}{57631}
\DeclareTextGlyphY{LinLibertine_R}{eight.taboldstyle}{57632}
\DeclareTextGlyphY{LinLibertine_R}{uniE120}{57632}
\DeclareTextGlyphY{LinLibertine_R}{nine.taboldstyle}{57633}
\DeclareTextGlyphY{LinLibertine_R}{uniE121}{57633}
\DeclareTextGlyphY{LinLibertine_R}{uniE128}{57640}
\DeclareTextGlyphY{LinLibertine_R}{uniE129}{57641}
\DeclareTextGlyphY{LinLibertine_R}{uniE12A}{57642}
\DeclareTextGlyphY{LinLibertine_R}{uniE130}{57648}
\DeclareTextGlyphY{LinLibertine_R}{leaf}{57656}
\DeclareTextGlyphY{LinLibertine_R}{uniE138}{57656}
\DeclareTextGlyphY{LinLibertine_R}{uniE13B}{57659}
\DeclareTextGlyphY{LinLibertine_R}{uniE13C}{57660}
\DeclareTextGlyphY{LinLibertine_R}{uniE13D}{57661}
\DeclareTextGlyphY{LinLibertine_R}{b.inferior}{57673}
\DeclareTextGlyphY{LinLibertine_R}{uniE149}{57673}
\DeclareTextGlyphY{LinLibertine_R}{c.inferior}{57674}
\DeclareTextGlyphY{LinLibertine_R}{uniE14A}{57674}
\DeclareTextGlyphY{LinLibertine_R}{d.inferior}{57675}
\DeclareTextGlyphY{LinLibertine_R}{uniE14B}{57675}
\DeclareTextGlyphY{LinLibertine_R}{f.inferior}{57677}
\DeclareTextGlyphY{LinLibertine_R}{uniE14D}{57677}
\DeclareTextGlyphY{LinLibertine_R}{g.inferior}{57678}
\DeclareTextGlyphY{LinLibertine_R}{uniE14E}{57678}
\DeclareTextGlyphY{LinLibertine_R}{h.inferior}{57679}
\DeclareTextGlyphY{LinLibertine_R}{uniE14F}{57679}
\DeclareTextGlyphY{LinLibertine_R}{i.inferior}{57680}
\DeclareTextGlyphY{LinLibertine_R}{uniE150}{57680}
\DeclareTextGlyphY{LinLibertine_R}{j.inferior}{57681}
\DeclareTextGlyphY{LinLibertine_R}{uniE151}{57681}
\DeclareTextGlyphY{LinLibertine_R}{k.inferior}{57682}
\DeclareTextGlyphY{LinLibertine_R}{uniE152}{57682}
\DeclareTextGlyphY{LinLibertine_R}{l.inferior}{57683}
\DeclareTextGlyphY{LinLibertine_R}{uniE153}{57683}
\DeclareTextGlyphY{LinLibertine_R}{m.inferior}{57684}
\DeclareTextGlyphY{LinLibertine_R}{uniE154}{57684}
\DeclareTextGlyphY{LinLibertine_R}{n.inferior}{57685}
\DeclareTextGlyphY{LinLibertine_R}{uniE155}{57685}
\DeclareTextGlyphY{LinLibertine_R}{p.inferior}{57687}
\DeclareTextGlyphY{LinLibertine_R}{uniE157}{57687}
\DeclareTextGlyphY{LinLibertine_R}{q.inferior}{57688}
\DeclareTextGlyphY{LinLibertine_R}{uniE158}{57688}
\DeclareTextGlyphY{LinLibertine_R}{r.inferior}{57689}
\DeclareTextGlyphY{LinLibertine_R}{uniE159}{57689}
\DeclareTextGlyphY{LinLibertine_R}{s.inferior}{57690}
\DeclareTextGlyphY{LinLibertine_R}{uniE15A}{57690}
\DeclareTextGlyphY{LinLibertine_R}{t.inferior}{57691}
\DeclareTextGlyphY{LinLibertine_R}{uniE15B}{57691}
\DeclareTextGlyphY{LinLibertine_R}{u.inferior}{57692}
\DeclareTextGlyphY{LinLibertine_R}{uniE15C}{57692}
\DeclareTextGlyphY{LinLibertine_R}{v.inferior}{57693}
\DeclareTextGlyphY{LinLibertine_R}{uniE15D}{57693}
\DeclareTextGlyphY{LinLibertine_R}{w.inferior}{57694}
\DeclareTextGlyphY{LinLibertine_R}{uniE15E}{57694}
\DeclareTextGlyphY{LinLibertine_R}{y.inferior}{57696}
\DeclareTextGlyphY{LinLibertine_R}{uniE160}{57696}
\DeclareTextGlyphY{LinLibertine_R}{z.inferior}{57697}
\DeclareTextGlyphY{LinLibertine_R}{uniE161}{57697}
\DeclareTextGlyphY{LinLibertine_R}{uniE188}{57736}
\DeclareTextGlyphY{LinLibertine_R}{uniE189}{57737}
\DeclareTextGlyphY{LinLibertine_R}{afii10086.alt}{57756}
\DeclareTextGlyphY{LinLibertine_R}{uniE19C}{57756}
\DeclareTextGlyphY{LinLibertine_R}{uniE19D}{57757}
\DeclareTextGlyphY{LinLibertine_R}{grave.cap}{58200}
\DeclareTextGlyphY{LinLibertine_R}{uniE358}{58200}
\DeclareTextGlyphY{LinLibertine_R}{acute.cap}{58201}
\DeclareTextGlyphY{LinLibertine_R}{uniE359}{58201}
\DeclareTextGlyphY{LinLibertine_R}{circumflex.cap}{58202}
\DeclareTextGlyphY{LinLibertine_R}{uniE35A}{58202}
\DeclareTextGlyphY{LinLibertine_R}{caron.cap}{58203}
\DeclareTextGlyphY{LinLibertine_R}{uniE35B}{58203}
\DeclareTextGlyphY{LinLibertine_R}{breve.cap}{58204}
\DeclareTextGlyphY{LinLibertine_R}{uniE35C}{58204}
\DeclareTextGlyphY{LinLibertine_R}{hungarumlaut.cap}{58205}
\DeclareTextGlyphY{LinLibertine_R}{uniE35D}{58205}
\DeclareTextGlyphY{LinLibertine_R}{space_uni030F.cap}{58206}
\DeclareTextGlyphY{LinLibertine_R}{uniE35E}{58206}
\DeclareTextGlyphY{LinLibertine_R}{breveinvertedcmb.cap}{58207}
\DeclareTextGlyphY{LinLibertine_R}{uniE35F}{58207}
\DeclareTextGlyphY{LinLibertine_R}{breve.cyrcap}{58208}
\DeclareTextGlyphY{LinLibertine_R}{uniE360}{58208}
\DeclareTextGlyphY{LinLibertine_R}{breve.cyr}{58209}
\DeclareTextGlyphY{LinLibertine_R}{uniE361}{58209}
\DeclareTextGlyphY{LinLibertine_R}{dieresis.cap}{58210}
\DeclareTextGlyphY{LinLibertine_R}{uniE362}{58210}
\DeclareTextGlyphY{LinLibertine_R}{hookabovecomb.cap}{58211}
\DeclareTextGlyphY{LinLibertine_R}{uniE363}{58211}
\DeclareTextGlyphY{LinLibertine_R}{dotaccent.cap}{58212}
\DeclareTextGlyphY{LinLibertine_R}{uniE364}{58212}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E0}{58336}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E1}{58337}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E2}{58338}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E3}{58339}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E4}{58340}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E5}{58341}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E6}{58342}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E7}{58343}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E8}{58344}
\DeclareTextGlyphY{LinLibertine_R}{uniE3E9}{58345}
\DeclareTextGlyphY{LinLibertine_R}{uniE3EA}{58346}
\DeclareTextGlyphY{LinLibertine_R}{uniE3EB}{58347}
\DeclareTextGlyphY{LinLibertine_R}{uniE3EC}{58348}
\DeclareTextGlyphY{LinLibertine_R}{uniE3ED}{58349}
\DeclareTextGlyphY{LinLibertine_R}{uniE3F0}{58352}
\DeclareTextGlyphY{LinLibertine_R}{uniE3F1}{58353}
\DeclareTextGlyphY{LinLibertine_R}{uniE3F2}{58354}
\DeclareTextGlyphY{LinLibertine_R}{uniE3F3}{58355}
\DeclareTextGlyphY{LinLibertine_R}{metric}{58400}
\DeclareTextGlyphY{LinLibertine_R}{uniE420}{58400}
\DeclareTextGlyphY{LinLibertine_R}{zero.slash}{63032}
\DeclareTextGlyphY{LinLibertine_R}{uniF638}{63032}
\DeclareTextGlyphY{LinLibertine_R}{parenleft.sc}{63150}
\DeclareTextGlyphY{LinLibertine_R}{uniF6AE}{63150}
\DeclareTextGlyphY{LinLibertine_R}{parenright.sc}{63151}
\DeclareTextGlyphY{LinLibertine_R}{uniF6AF}{63151}
\DeclareTextGlyphY{LinLibertine_R}{bracketleft.sc}{63152}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B0}{63152}
\DeclareTextGlyphY{LinLibertine_R}{bracketright.sc}{63153}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B1}{63153}
\DeclareTextGlyphY{LinLibertine_R}{braceleft.sc}{63154}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B2}{63154}
\DeclareTextGlyphY{LinLibertine_R}{braceright.sc}{63155}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B3}{63155}
\DeclareTextGlyphY{LinLibertine_R}{exclamdown.sc}{63156}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B4}{63156}
\DeclareTextGlyphY{LinLibertine_R}{questiondown.sc}{63157}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B5}{63157}
\DeclareTextGlyphY{LinLibertine_R}{guillemotleft.sc}{63158}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B6}{63158}
\DeclareTextGlyphY{LinLibertine_R}{guillemotright.sc}{63159}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B7}{63159}
\DeclareTextGlyphY{LinLibertine_R}{guilsinglleft.sc}{63160}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B8}{63160}
\DeclareTextGlyphY{LinLibertine_R}{guilsinglright.sc}{63161}
\DeclareTextGlyphY{LinLibertine_R}{uniF6B9}{63161}
\DeclareTextGlyphY{LinLibertine_R}{hyphen.cap}{63162}
\DeclareTextGlyphY{LinLibertine_R}{uniF6BA}{63162}
\DeclareTextGlyphY{LinLibertine_R}{uniF6BE}{63166}
\DeclareTextGlyphY{LinLibertine_R}{afii10066.ital}{63173}
\DeclareTextGlyphY{LinLibertine_R}{uniF6C5}{63173}
\DeclareTextGlyphY{LinLibertine_R}{f_f}{64256}
\DeclareTextGlyphY{LinLibertine_R}{uniFB00}{64256}
\DeclareTextGlyphY{LinLibertine_R}{f_i}{64257}
\DeclareTextGlyphY{LinLibertine_R}{uniFB01}{64257}
\DeclareTextGlyphY{LinLibertine_R}{f_l}{64258}
\DeclareTextGlyphY{LinLibertine_R}{uniFB02}{64258}
\DeclareTextGlyphY{LinLibertine_R}{f_f_i}{64259}
\DeclareTextGlyphY{LinLibertine_R}{uniFB03}{64259}
\DeclareTextGlyphY{LinLibertine_R}{f_f_l}{64260}
\DeclareTextGlyphY{LinLibertine_R}{uniFB04}{64260}
\DeclareTextGlyphY{LinLibertine_R}{longs_t}{64261}
\DeclareTextGlyphY{LinLibertine_R}{uniFB05}{64261}
\DeclareTextGlyphY{LinLibertine_R}{s_t}{64262}
\DeclareTextGlyphY{LinLibertine_R}{uniFB06}{64262}
\DeclareTextGlyphY{LinLibertine_R}{uniFFFD}{65533}
\DeclareTextGlyphY{LinLibertine_R}{u1D538}{120120}
\DeclareTextGlyphY{LinLibertine_R}{uni1D538}{120120}
\DeclareTextGlyphY{LinLibertine_R}{u1D539}{120121}
\DeclareTextGlyphY{LinLibertine_R}{uni1D539}{120121}
\DeclareTextGlyphY{LinLibertine_R}{u1D53B}{120123}
\DeclareTextGlyphY{LinLibertine_R}{uni1D53B}{120123}
\DeclareTextGlyphY{LinLibertine_R}{u1D53C}{120124}
\DeclareTextGlyphY{LinLibertine_R}{uni1D53C}{120124}
\DeclareTextGlyphY{LinLibertine_R}{u1D53D}{120125}
\DeclareTextGlyphY{LinLibertine_R}{uni1D53D}{120125}
\DeclareTextGlyphY{LinLibertine_R}{u1D53E}{120126}
\DeclareTextGlyphY{LinLibertine_R}{uni1D53E}{120126}
\DeclareTextGlyphY{LinLibertine_R}{u1D540}{120128}
\DeclareTextGlyphY{LinLibertine_R}{uni1D540}{120128}
\DeclareTextGlyphY{LinLibertine_R}{u1D541}{120129}
\DeclareTextGlyphY{LinLibertine_R}{uni1D541}{120129}
\DeclareTextGlyphY{LinLibertine_R}{u1D542}{120130}
\DeclareTextGlyphY{LinLibertine_R}{uni1D542}{120130}
\DeclareTextGlyphY{LinLibertine_R}{u1D543}{120131}
\DeclareTextGlyphY{LinLibertine_R}{uni1D543}{120131}
\DeclareTextGlyphY{LinLibertine_R}{u1D544}{120132}
\DeclareTextGlyphY{LinLibertine_R}{uni1D544}{120132}
\DeclareTextGlyphY{LinLibertine_R}{u1D546}{120134}
\DeclareTextGlyphY{LinLibertine_R}{uni1D546}{120134}
\DeclareTextGlyphY{LinLibertine_R}{u1D547}{120135}
\DeclareTextGlyphY{LinLibertine_R}{uni1D547}{120135}
\DeclareTextGlyphY{LinLibertine_R}{u1D54A}{120138}
\DeclareTextGlyphY{LinLibertine_R}{uni1D54A}{120138}
\DeclareTextGlyphY{LinLibertine_R}{u1D54B}{120139}
\DeclareTextGlyphY{LinLibertine_R}{uni1D54B}{120139}
\DeclareTextGlyphY{LinLibertine_R}{u1D54C}{120140}
\DeclareTextGlyphY{LinLibertine_R}{uni1D54C}{120140}
\DeclareTextGlyphY{LinLibertine_R}{u1D54D}{120141}
\DeclareTextGlyphY{LinLibertine_R}{uni1D54D}{120141}
\DeclareTextGlyphY{LinLibertine_R}{u1D54E}{120142}
\DeclareTextGlyphY{LinLibertine_R}{uni1D54E}{120142}
\DeclareTextGlyphY{LinLibertine_R}{u1D54F}{120143}
\DeclareTextGlyphY{LinLibertine_R}{uni1D54F}{120143}
\DeclareTextGlyphY{LinLibertine_R}{u1D550}{120144}
\DeclareTextGlyphY{LinLibertine_R}{uni1D550}{120144}

